Spectral Asymptotics for Magnetic Schroedinger Operator

In this article we obtain eigenvalue asymptotics for 2D and 3D-Schroedinger, Schroedinger-Pauli and Dirac operators in the situations in which the role of the magnetic field is important. These operators are essentially different and there is a significant difference between 2D and 3D-operators.

==> Ch11/book11.tex <==
% !TEX root = ../book_new.tex

\part{Asymptotics of Spectra\label{part-4}}
\setcounter{secnumdepth}{2}

\chapter{Weyl Asymptotics of Spectra}
\label{sect-11}
\minitoc

This chapter is devoted to applications of the results of Parts~\ref{part-2} and~\ref{part-3} to the eigenvalue asymptotics. Now we consider operator $A$ depending on parameters; then all the functions $\rho, \tilde{\rho}, \varrho,$ and $\gamma$ with different indices and zones $X_\reg$ and $X_\sing$ depend on these parameters as well. Further, the main part of the asymptotics $\N^\W$ (given by Weyl formula but may be with corrections) and the remainder $R$ depend on this parameter as well; both of them tend to infinity but under appropriate assumptions $R\ll \N^\W$. Further, as parameters tend to their limits $X_\sing$ shrinks.

In Section~\ref{sect-11-1} we treat semiclassical asymptotics. In this case we consider operator $A_h= A(x,hD,h)$ and select $\rho_h = h^{-1}\rho $, $\gamma_h=\gamma$ and $h_\eff= (\rho_h\gamma_h)^{-1}= h\rho^{-1}\gamma^{-1}$; then $X_{\reg,h}=\{\rho_h \gamma_h \ge 1\}=\{x:\rho \gamma \ge h\}$ and
$X_\sing=\{\rho \gamma \le 2h\}$.

In Sections~\ref{sect-11-2}--\ref{sect-11-6} we consider asymptotics with respect to the spectral parameter $\tau$; in this case $A_\tau =A-\tau$ and usually $\rho_\tau = |\tau|^{1/m} +\rho$, $\gamma_\tau =\gamma$ as we assume that $A$ satisfies some conditions with functions $\rho$, $\gamma$ and $\varrho=\rho^m$. Then $h_\eff= (|\tau|^{1/m} +\rho)^{-1}\gamma^{-1}$ and
$X_{\reg,\tau}=\{ (|\tau|^{1/m} +\rho) \gamma \ge 1\}$ and
$X_{\sing,\tau}=\{ (|\tau|^{1/m} +\rho) \gamma \le 2\}$.

More precisely, in Sections~\ref{sect-11-2}--\ref{sect-11-5} we consider asymptotics of the eigenvalues tending to infinity, then $\tau \to +\infty$ but there are different scenarios:

\begin{itemize}[label=-, labelindent=0pt]
\item in Section~\ref{sect-11-2} domain $X$ is ``essentially'' bounded (i.e., exits to infinity are thin enough) and the coefficients are weakly singular;

\item
 in Section~\ref{sect-11-4} the coefficients are strongly singular and the coercivity condition is fulfilled but the domain is still ``essentially'' bounded;

\item
in Section~\ref{sect-11-5} the domain is ``very unbounded'' and the spectrum is discrete only because the lower order terms are coercive. In particular, we treat the Schr\"{o}dinger operator with potential $V$ tending to $+\infty $ at infinity and with the spectral parameter $\tau $ tending to $+\infty $, usually like $|x|^{2\mu}$ with $\mu>0$ and the growths of both $\N^\W_\tau$ and $R_\tau$ depend on $\mu$.
\end{itemize}

Further, in Section~\ref{sect-11-6} we treat asymptotics of the eigenvalues tending to the boundary of the essential spectrum. In particular, we treat the Schr\"{o}dinger and Dirac operators with potentials tending to $0$ at infinity, usually like $|x|^{2\mu}$ with $\mu\in (-1,0)$ and the spectral parameter
$\tau $ tending to $-0$ and $M-0$ or $-M+0$ respectively (where $M$ is the mass in the case of the Dirac operator). Then the rates of the growth of both $\N^\W_\tau$ and $R_\tau$ depend on $\mu$.

Section~\ref{sect-11-7} is devoted to the multiparameter asymptotics; for example, there is the semiclassical parameter $h\to+0$ and the spectral parameter $\tau $ tending either to $+\infty $ or $-\infty $ (for the Schr\"{o}dinger and Dirac operators in bounded domains or for the Schr\"{o}dinger operator in unbounded domains), or to $-0$, $M-0$ or $-M+0$ (for the Schr\"{o}dinger and Dirac operators in unbounded domains), or to
$\inf V+0$, $\inf V+M+0$, $\sup V-M-0$ (for the Schr\"{o}dinger
and Dirac operators) where for the Schr\"{o}dinger operator $\inf V$
is not necessarily finite. Moreover, the case of a vector
semiclassical parameter $\boldsymbol{h}=(h_1,\dots ,h_d)$ is treated as well.

For semi-bounded operators, Riesz means are also treated.

Finally, in Section~\ref{sect-11-8} we consider asymptotics of the spectrum of the negative order pseudodifferential operators tending to $0$. While these operators are not exactly covered by the general theory and require special analysis, some special cases (like $\Delta ^{-m}V$) are and the general results are the same.

For simplicity we assume the sufficient smoothness but the reader can generalize easily these results applying results for rough and irregular operators.

\section{Semiclassical eigenvalue asymptotics}
\label{sect-11-1}
In this section the operator is fixed and only the semiclassical parameter
$h\to +0$ varies.

\subsection{General analysis}
\label{sect-11-1-1}

\subsubsection{Standard remainder estimates}
\label{sect-11-1-1-1}
Let us consider first operators which are semi-bounded from below and apply the results of Chapter~\ref{sect-9} derived on the basis of the results of Part~\ref{part-2}. This means that $\tau_1=-\infty$ and without any loss of the generality one can assume that $\tau_2=0$.

Let us consider operator
\begin{gather}
A_h=\sum_{|\alpha |,|\beta |\le m}(hD)^\alpha a_{\alpha ,\beta } (hD)^\beta
\label{11-1-1}
\intertext{with coefficients satisfying}
a_{\alpha ,\beta }=a_{\beta ,\alpha }^\dag ,
\label{11-1-2}
\end{gather}
\begin{multline}
\1D^\sigma a_{\alpha ,\beta }\1\le
c\varrho \rho ^{-|\alpha |-|\beta |}\gamma ^{-|\sigma |}\\
\forall \alpha ,\beta :|\alpha |\le m,|\beta |\le m\;\forall
\sigma :|\sigma |\le K
\label{11-1-3}
\end{multline}
and
\begin{multline}
\sum_{|\alpha |=|\beta |=m}
\blangle a_{\alpha ,\beta } v_\alpha ,v_\beta \brangle \ge
\epsilon_0\varrho \rho ^{-2m}\sum_{|\alpha |=m}\1v_\alpha \1^2\\
\forall v=(v_\alpha )_{|\alpha |=m}\quad
\forall x:\rho \gamma \le h_0
\label{11-1-4}
\end{multline}
where scaling function $\gamma $ satisfies \ref{9-1-6-1} on $X$ and \begin{equation}
\mes (\cX_\sing)=0\qquad \text{where\ \ }\cX_\sing=\{x,\gamma (x)=0\},
\label{11-1-5}
\end{equation}
functions $\rho $, $\varrho $ satisfying \ref{9-1-6-2} and \ref{9-1-6-3} are defined in $\cX_\reg=X\setminus \cX_\sing$, and $h_0=\const>0$.

The sets $\cX_\reg$ and $\cX_\sing$ are called \emph{regular}%
\index{regular!set}%
\index{set!regular}
and \emph{singular sets}%
\index{singular!set}%
\index{set!singular}
respectively. These sets do not coincide with but are obviously related to the
\emph{regular}%
\index{regular!zone}%
\index{zone!regular}
$X_{\reg,h}=\{x,\rho \gamma \ge h\}$ and
\emph{singular zones}%
\index{singular!zone}%
\index{zone!singular}
$X_{\sing,h}=\{x,\rho \gamma \le 2h\}$ and respectively:
$X_{\reg,h}\subset \cX_\reg$ and expands to it, $X_{\sing,h}\supset \cX_\sing$ and shrinks to it as $h\to +0$.

In particular, for the Schr\"{o}dinger operator
\begin{equation}
A= \sum_{1\le j,k\le d}(hD_j-V_j)g^{jk}(hD_k-V_k)+V
\label{11-1-6}
\end{equation}
with real-valued functions $g^{jk}=g^{kj}$, $V_j$ and $V$ we always take $\varrho =\rho ^2$ and conditions (\ref{11-1-3})--(\ref{11-1-4}) become
\begin{gather}
|D ^\alpha g^{jk}|\le c\gamma ^{-|\alpha |},\quad
|D ^\alpha V_j|\le c\rho \gamma ^{-|\alpha |},\quad
|D ^\alpha V|\le c\rho ^2\gamma ^{-|\alpha |}
\label{11-1-7}
\shortintertext{and}
\epsilon_0|\xi |^2\le \sum_{j,k}g^{jk}\xi_j\xi_k\le c|\xi |^2
\qquad \forall \xi \in\bR^d.
\label{11-1-8}
\end{gather}

Moreover, we assume that conditions (\ref{9-1-15}) (the boundary regularity
condition) are fulfilled in $\cX_\reg$. For the sake of simplicity we assume that the Dirichlet boundary conditions are given in which case the ellipticity condition for the boundary value problem is fulfilled automatically. However later we discuss Neumann-like problems as well.

Then one can apply Theorem~\ref{thm-9-1-7} with
$X_\reg=X_{\reg,h}=\{x\in X,\rho \gamma >h\}$ and
$X_\sing=X_{\sing,h}= \{x\in X, \rho \gamma \le 2h\}$ provided $h\le h_0$. Here
conditions (\ref{11-1-2})--(\ref{11-1-4}) yield the following estimate on $X_\sing$:
\begin{multline}
(A_hu,u)\ge \\
\epsilon_0\int \varrho \Bigl( h^{2m}\rho ^{-2m}
\sum_{|\alpha |=m}|D ^\alpha u|^2-C_0\sum_{|\alpha |\le m-1}
h^{2|\alpha |}\rho^{-2|\alpha |}|D ^\alpha u|^2 \Bigr)\,dx
\label{11-1-9}
\end{multline}
for all compactly supported functions $u\in \sC^{2m}(\bar{X}_\sing,\bH )$
satisfying the Dirichlet boundary condition. Therefore Rozenblioum estimate (\ref{9-A-11}) yields that the contribution of the zone $X_\sing$ to the upper estimate of $\N^-_h$ in Theorem~\ref{thm-9-1-7} does not exceed $CR_0h^{-d}$ with
\begin{multline}
R_0=\\
C\Bigl(\int_{X_\sing}\varrho ^{-p}\rho ^{2mp}\,dx\Bigr)^{\frac{d}{2mp}}
\Bigl(\int_{X_\sing}\varrho ^q\,dx\Bigr)^{\frac{d}{2mq}}
\Bigl(\mes(X_\sing)\Bigr)^{1-\frac{d}{2m}(\frac{1}{p} + \frac{1}{q})}
\label{11-1-10}
\end{multline}
where $p,q$ are arbitrarily chosen numbers such that
\begin{equation}
\frac{1}{p} + \frac{1}{q} \le \frac{2m}{d} ,\qquad p\ge 1,q\ge 1
\label{11-1-11}
\end{equation}
and
\begin{align}
& \text{either\ } \quad \frac{1}{p}+\frac{1}{q}<\frac{2m}{d},
\label{11-1-12}\\
& \text{or\ } \quad
\frac{1}{p}+\frac{1}{q}=\frac{2m}{d},d\ge m \text{\ \ and\ \ } d>m \implies q>1\notag\\
&{\hskip100pt}\text{and\ \ } p>1\implies 2m<{\frac{d}{p}}(p+1).\notag
\end{align}
Recall that $X_\sing$ does not contribute to the lower estimate of $N^-_h$.

At the same time the contribution of the zone $X_\reg$ to both lower and upper estimates does not exceed $Ch^{1-d}R_1+Ch^{s-d}R_2$ where
\begin{align}
R_1&=\int_{X_{\reg,h}\setminus X_{\reg,\elli,h}}\rho ^{d-1}\gamma ^{-1}\,dx, \label{11-1-13}\\
R_2&=\int_{X_{\reg,h}}\rho ^{d-s}\gamma ^{-s}\,dx
\label{11-1-14}
\end{align}
with arbitrarily chosen $s$ and we assume that in every ball
$\cB\bigl(y,\gamma (y),X\bigr)$ with $y\in X_\reg$ one of the conditions of Part~\ref{part-2} providing remainder estimate $O(h^{1-d}_\eff)$\,\footnote{\label{foot-11-1} To be discussed in Remarks~\ref{rem-11-1-3} and \ref{rem-11-1-4}.} is fulfilled; here
$h_\eff = h (\rho\gamma)^{-1}$.

Further, the principal term of the upper and lower estimates is $\N^\W_h=h^{-d}\N^\W $ with the \emph{cut Weyl expression\/}\index{Weyl expression!cut}
\begin{equation}
\N^\W =(2\pi )^{-d}\int_{T^*X_{\reg,h}}\boldsymbol{n}(x,\xi ,-\infty ,0)\,dx d\xi
\label{11-1-15}
\end{equation}
where $\boldsymbol{n}(x,\xi ,.,.)$ is the eigenvalue counting function for
the symbol
\begin{equation}
a(x,\xi )=\sum_{\alpha ,\beta }a_{\alpha ,\beta }\xi ^{\alpha +\beta };
\label{11-1-16}
\end{equation}
recall that both $X_\reg$ and $X_\sing$ and thus $\N^\W $ depend on $h$.

So the following statement is proven:

\begin{theorem}\label{thm-11-1-1}
Let $A$ be a self-adjoint operator (with the Dirichlet boundary conditions) of the form \textup{(\ref{11-1-1})} in $\sL^2(X,\bH)$ and let conditions
\textup{(\ref{11-1-2})}--\textup{(\ref{11-1-5})} be fulfilled.
Moreover, let us assume that, in every ball
$\sB\bigl(y,\gamma (y),X\bigr)$ with $y\in \cX_\reg$, one of the conditions of Part~\ref{part-2} providing remainder estimate $O(h^{1-d}_\eff)$\,\footref{foot-11-1} is fulfilled. Then the estimates
\begin{multline}
h^{-d}\N^\W -Ch^{1-d}R_1\le \N^-(A_h)\le \\[2pt]
h^{-d}\N^\W +Ch^{1-d}R_1+Ch^{s-d}R_2+CR_0h^{-d}
\label{11-1-17}
\end{multline}
hold with $\N^\W $, $R_1$, $R_2$ and $R''$ given by \textup{(\ref{11-1-15})}, \textup{(\ref{11-1-13})}, \textup{(\ref{11-1-14})} and \textup{(\ref{11-1-10})} respectively.
\end{theorem}

\begin{corollary}\label{cor-11-1-2}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{cor-11-1-2-i}
For $\N^\W $ in formula \textup{(\ref{11-1-15})} let us replace
the domain $X_{\reg,h}$ by the domain $\cX_\reg$ (or $X$); then the error
does not exceed $C\int_{X_{\sing,h}}\rho ^d\,dx\le CR_0$ due to H\"{o}lder
inequality. Therefore
\begin{equation}
|\N^-(A_h)-\N^\W h^{-d}|\le Ch^{1-d}R_1+Ch^{s-d}R_2+ Ch^{-d}R_0
\label{11-1-18}
\end{equation}
where $\N^\W $ is now given by (uncut) Weyl expression and no longer depends on $h$.

\item\label{cor-11-1-2-ii}
This estimate yields that if
\begin{gather}
\rho ^{d-s}\gamma ^{-s}\in \sL^1(\{X,\ \rho \gamma \ge h_0\} ),
\label{11-1-19}\\[3pt]
\rho ^{d-1}\gamma ^{-1}\in
\sL^1( X \setminus X_{\reg,\elli,h_0})
\label{11-1-20}
\shortintertext{and}
R_0=O(h)\qquad \text{as\ }\;h\to+0,
\label{11-1-21}\\
\shortintertext{then}
\N^-(A_h)=h^{-d}\N^\W +O(h^{1-d}).
\label{11-1-22}
\end{gather}
These asymptotics will be improved and generalized below, where other asymptotics due to the results of Chapter~\ref{sect-9} will be derived.

\item\label{cor-11-1-2-iii}
Let us assume that
\begin{equation}
\varrho \asymp \rho ^k\quad \text{in\ \ } \cX_\reg
\label{11-1-23}
\end{equation}
and that one of the following conditions are fulfilled:
\begin{phantomequation}\label{11-1-24}\end{phantomequation}
\begin{align}
&d>2m,&&k\in [0,2m];
\tag*{$\textup{(\ref*{11-1-24})}_1$}\label{11-1-24-1}\\
&m<d\le 2m,&&k\in [2m-d,d); \tag*{$\textup{(\ref*{11-1-24})}_2$}\label{11-1-24-2}\\
&d=m,&&k=d.
\tag*{$\textup{(\ref*{11-1-24})}_3$}\label{11-1-24-3}
\end{align}
Then one can choose $p,q$ satisfying condition \textup{(\ref{11-1-11})} with
equality and condition \textup{(\ref{11-1-12})} and such that
\begin{equation*}
R_0\asymp \int_{X_{\sing,h}}\rho ^d\, dx\le
2h\int_{X_{\sing,h}}\rho ^{d-1} \gamma ^{-1}\, dx.
\end{equation*}
This inequality and \textup{(\ref{11-1-20})} yield that $R_0=o(h)$ and therefore
condition \textup{(\ref{11-1-21})} is fulfilled. In particular, for $d>2m$ one can take $k=2m$.
\end{enumerate}
\end{corollary}

\begin{remark}\label{rem-11-1-3}
Let us list some cases when according to Part~\ref{part-2} contribution of $\cB(y,\gamma (y),X)$ to the remainder is $O(h^{1-d}\rho^{d-1}\gamma^{d-1})$; these conditions are uniform with respect to $y$ (after rescaling):

\begin{claim}\label{11-1-25}
Assumptions (\ref{11-1-3}), (\ref{11-1-4}) and (\ref{9-1-15}) are fulfilled with $K=K(d)$ and operator $A$ is microhyperbolic on the energy level $0$;
\end{claim}
\vglue-10pt
\begin{claim}\label{11-1-26}
$A$ is Schr\"odinger operator, $d\ge2$, assumptions (\ref{11-1-7}), (\ref{11-1-8}) and (\ref{9-1-15}) are fulfilled with $K=K(d)$;
\end{claim}
\vglue-10pt
\begin{claim}\label{11-1-27}
$A$ is ``rough'' operator described in Section~\ref{sect-4-6} as $B(y,\gamma(y))\subset X_\reg$ and in Section~\ref{sect-7-5} otherwise.
\end{claim}

Through bracketing $A^- \le A\le A^+$ between two rough operators such that contributions to $\N^\W$ of $\cB(y,\gamma(y),X)$ for $A^-$ and $A^+$ differ by $O(h_\eff^{1-d})$ we cover also

\begin{claim}\label{11-1-28}
Assumptions (\ref{11-1-3}), (\ref{11-1-4}) are fulfilled with $K=1$,
$\nabla a_{\alpha,\beta}$ are continuous with continuity modulus
$C\varrho \rho^{-|\alpha|-|\beta|}\gamma^{-1} |\log (|x-y|\gamma^{-1})|^{-1}$ and either $B(y,\gamma(y))\subset X_\reg$ or extra conditions of Theorem~\ref{thm-7-5-15} to the boundary are fulfilled, operator $A$ is $\xi$-microhyperbolic on the energy level $0$;
\end{claim}
\vglue-10pt
\begin{claim}\label{11-1-29}
$A$ is Schr\"odinger operator, assumptions (\ref{11-1-7}), (\ref{11-1-8}) are fulfilled with $K=1$, $\nabla g^{kl}$, $\nabla V_k$ and $\nabla V$ are continuous with continuity moduli
$C\rho^p\gamma^{-1} |\log (|x-y|\gamma^{-1})|^{-1}$, $p=0,1,2$ respectively
and either $B(y,\gamma(y))\subset X_\reg$ or extra conditions of Theorem~\ref{thm-7-5-15} to the boundary are fulfilled, $d\ge 3$ or
$|V|+\gamma |\nabla V|\ge \epsilon \rho^2$;
\end{claim}
\vglue-10pt
\begin{claim}\label{11-1-30}
$A$ is Schr\"odinger operator, $d=2$, assumptions (\ref{11-1-7}), (\ref{11-1-8}) are fulfilled with $K=2$, $\nabla^2 g^{kl}$, $\nabla^2 V_k$ and $\nabla^2 V$ are continuous with continuity moduli
$C\rho^p\gamma^{-2} |\log (|x-y|\gamma^{-1})|^{-2}$, $p=0,1,2$ respectively
and either $B(y,\gamma(y))\subset X_\reg$ or extra conditions of Theorem~\ref{thm-7-5-15} to the boundary are fulfilled.
\end{claim}
\end{remark}

\begin{remark}\label{rem-11-1-4}
Actually we can weaken assumptions (\ref{11-1-28})--(\ref{11-1-30}) because we can bracket symbol $a(x,\xi)$ between $a (x,\xi) \pm b_\varepsilon (x)$ where
\begin{gather}
b_\varepsilon (x) = C_0 \max_{\alpha,\beta}\osc (\nabla a_{\alpha,\beta},
x,\varepsilon) *\phi_\varepsilon
\label{11-1-31}\\
\shortintertext{where}
\osc (a,x, \varepsilon)=
\max_{y:|x-y|\le \varepsilon}a -\min_{y:|x-y|\le \varepsilon}a
\label{11-1-32}
\end{gather}
$\phi_\varepsilon $ is a standard mollification function. An easy proof is left to the reader.

Then for $\xi$-microhyperbolic operator contributions of $\cB(y,\gamma(y),X)$ to $\N^\W$ for $A^-$ and $A^+$ differ by no more than
\begin{gather}
Ch_\eff^{-d}\max_{\alpha,\beta} \int \osc (\nabla a_{\alpha,\beta},
x,\varepsilon) \, dx
\label{11-1-33}
\intertext{with an integral taken over $\cB(y,\gamma(y),X)$ rescaled and in the end of the day results in an additional error}
R_3=Ch_\eff^{1-d}\max_{\alpha,\beta}
\int_{X_\reg\setminus X_{\reg,\elli}}
\rho^d\osc \bigl(\nabla a_{\alpha,\beta},x,\rho^{-1}\log (\rho\gamma)\bigr)\,dx.
\label{11-1-34}
\end{gather}
So, to estimate (\ref{11-1-33}) by $O(h_\eff^{1-d})$ we actually need to impose estimate $O(|\log \varepsilon |^{-1})$ to $\sL^1$-norm rather than $\sL^\infty$-norm of $\osc (\nabla a_{\alpha,\beta}, x,\varepsilon)$.
\end{remark}

We leave to the reader the following easy problem:

\begin{problem}\label{problem-11-1-5}
Apply rescaling to modified expressions (\ref{11-1-33}) and (\ref{11-1-34}) for Schr\"odinger operator ($d\ge 3$) without condition $|V|\ge\epsilon\rho^2$.
\end{problem}

\begin{remark}\label{rem-11-1-6}
Some of the conditions of Theorem~\ref{thm-11-1-1} and Corollary~\ref{cor-11-1-2} are too restrictive but we can weaken them.

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-1-6-i}
First of all, one can assume that $X=\cX_\reg\cup \cX_\sing \cup \cY$ where
the domains $(\cX_\reg\cup \cX_\sing)$ and $\cY$ are properly overlapping (with
respect to the scaling function $\gamma $), and that in
$(\cX_\reg\cup \cX_\sing)$ all the previous conditions are fulfilled and we assume that in $\cY$ the inequality
\begin{equation}
\sum_{\alpha ,\beta }
\blangle a_{\alpha ,\beta }v_\alpha ,v_\beta \brangle \ge
\epsilon_0\sum_{|\alpha |=m}\varrho_1\1v_\alpha \1^2-
c\sum_{|\alpha |\le m-1} \varrho_1\rho_1^{2|\alpha |}\1v_\alpha \1^2
\label{11-1-35}
\end{equation}
holds with appropriate measurable functions $\varrho_1$ and $\rho_1$. Then one can
take $X_\reg=\{x\in \cX_\reg, \rho \gamma \ge h\}$ and
$X_\sing=\{x\in \cX_\reg, \rho \gamma \le 2h\}\cup X_\sing\cup \cY$ in which case $R_0$ is given by the formula
\begin{multline}
R_0=
C\Bigl(\int_{\cX_\reg\cap\{\rho \gamma \le 2h\}}\rho ^{-p}\rho^{2mp}\,dx +\int_\cY\varrho_1^{-p}dx\Bigr)^{\frac{d}{2mp}}\times \\
\Bigl(\int_{\cX_\reg\cap\{\rho \gamma \le 2h\}}\varrho ^q\,dx+
\int_\cY\varrho_1 ^q\rho_1 ^{2mq}\,dx \Bigr)^{\frac{d}{2mq}}\times \\
\bigl(\mes ({\cX_\reg\cap\{\rho \gamma \le 2h\}}\cup \cY)\bigr)
^{1-\frac{d}{2m}(\frac{1}{p}+\frac{1}{q})}.
\label{11-1-36}
\end{multline}


\item\label{rem-11-1-6-ii}
Further, one can assume that the Dirichlet boundary condition
is given only on $\partial X\cap (\bar{\cX}_\reg\cap \{\rho\gamma\le h_0\}\cup \bar{\cY})$; on other part of $\partial X$ it could be different (but still appropriate boundary condition).

Furthermore, assume that even in $\partial X_{\sing,h}$ Dirichlet boundary condition is assumed only on $Y_\D$ while on $Y_\N= \partial X_{\sing,h}\setminus Y_\D$ another boundary condition is given, not necessary Neumann one but satisfying
\begin{multline}
(Au,u)_{ X_{\sing,h}} \ge \\
\epsilon \sum_{\alpha:|\alpha |=m} h ^{2m} \| D^\alpha u\|^2-
C \sum_{\alpha:|\alpha |\le m-1}
h^{2|\alpha|}\| \rho_1 ^{m-|\alpha|} D^\alpha u\|^2 \\
\forall u\in \fD(A):\ u=0\qquad \text{on\ \ } X\setminus X_{\sing,h}
\label{11-1-37}
\end{multline}
Finally, let us assume that conditions (\ref{9-A-23})--(\ref{9-A-26}) are fulfilled for $X$ replaced by $X_{\sing,h}$; recall that the inner boundary
$\partial X_{\sing,h} \cap \overset{\circ}{X}$ is considered as part of $Y_\D$.

Then the previous estimate remain true with $\varrho_1 = 1$ and with $\rho_1$ replaced by
\begin{equation}
\rho_2 = \rho_1 +\sum_j h_j^{-1}\chi_j
\label{11-1-38}
\end{equation}
in the estimates from above where $\chi_j$ is a characteristic function of $X_j$. In some examples specific arguments will improve even this estimate.

\item\label{rem-11-1-6-iii}
All these results remain true if we replace $hD_j$ by $hD_j-V_j$ in the operator $A$ where $V_j$ are real-valued functions supported in $X_{\reg,h}$ such that
\begin{equation}
|D ^\alpha (D_jV_k-D_kV_j)|\le c\rho \gamma ^{-|\alpha |-1}\qquad
\forall \alpha :|\alpha |\le K.
\label{11-1-39}
\end{equation}
In fact, after an appropriate gradient transform in every ball $\cB(x,\epsilon \gamma (x),X)$ lying in $X_{\reg,h}$ condition
\begin{equation}
|D ^\alpha V_j|\le c\rho \gamma ^{-|\alpha |}\qquad
\forall \alpha :|\alpha |\le K
\label{11-1-40}
\end{equation}
is fulfilled.

\item\label{rem-11-1-6-iv}
If the operator $(A-\tau )$ satisfies all the conditions of Theorem~\ref{thm-11-1-1} uniformly with respect to $\tau \in [\tau_1,0]$ with
$\tau_1<0$ then all the estimates and asymptotics of Theorem~\ref{thm-11-1-1} and Corollary~\ref{cor-11-1-2} remain true for this operator uniformly with respect to $\tau \in [\tau_1,0]$. In particular, for the Schr\"{o}dinger operator with $d\ge 2$ the condition of this statement is fulfilled automatically for $\tau_1=-\infty $.
\end{enumerate}
\end{remark}

\begin{remark}\label{rem-11-1-7}
Let us consider the Riesz means
\begin{equation}
\N^-_{(\vartheta)} (A) =\int \tau_- ^{\vartheta -1}\N^-(A-\tau )\,d\tau
\label{11-1-41}
\end{equation}
of order $\vartheta >0$ (i.e., we calculate them for the spectral parameter $\tau =0$). Let us include in $\N^\W_{(\vartheta)}$ (depending on $h$ for $A=A_h$) a sufficient number of terms. So, in principle $\N^\W_{(0)}$ does not necessarily coincide with $\N^\W$ (in more sharp asymptotics it may contain one extra term).

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-1-7-i}
Then the remainder estimates in the local semiclassical spectral asymptotics zone $X_{\reg,h}$ yield that terms $h^{1-d}R_1$ and $h^s R_2$ should be replaced by $h^{1+\vartheta -d}R_{1(\vartheta)}$ and $h^s R_{2(\vartheta)}$ with
\begin{gather}
R_{1(\vartheta)} = \int_{X_{\reg,h}\setminus X_{\reg,\elli,h} }
\varrho ^\vartheta \rho ^{d-\vartheta -1}\gamma ^{-\vartheta -1}\,dx,
\label{11-1-42}\\
R_{2 (\vartheta)} =
\int_{X_\reg} \varrho ^\vartheta \rho ^{d-s}\gamma ^{-s}\,dx.
\label{11-1-43}
\end{gather}
To do this we need $O(h_\eff^{1+\vartheta-d})$ remainder estimate which requires a stronger regularity:
$K=1+\lfloor \vartheta\rfloor$ and the $K$-th derivatives should be continuous with the continuity modulus $O(|x-y|^{\vartheta-\lfloor \vartheta\rfloor}|\log |x-y||^{-1})$ and the boundary should be a bit smoother.

\item\label{rem-11-1-7-ii}
Further, in virtue of SubSection~\ref{sect-9-2-4} and Appendix~\ref{sect-9-A-2} term $h^{-d}R_0$ with $R_0$ defined by (\ref{11-1-10}) should be replaced by $h^{-d}R_{0(\vartheta)}$ with $R_{0(\vartheta)}$ defined by the same formula but with the second factor in the right-hand expression should be given in the form
\begin{equation}
\int_0^\infty \tau ^{\vartheta -1}
\Bigl( \int_{X_{\sing,h}}(\varrho_1-\tau )_+^q\,dx\Bigr)^{\frac{d}{2mq}}\,d\tau.
\label{11-1-44}
\end{equation}
In particular, if one can take $q=\frac{d}{2m}$ and $p=\infty$ then
\begin{equation}
R_{0(\vartheta)} =C\int_{X_{\sing,h}}\varrho ^{{\frac{d}{2m}}+\vartheta }\,dx
\times \sup_{X_{\sing,h}} (\varrho ^{-{\frac{d}{2m}}}\rho ^d).
\label{11-1-45}
\end{equation}
Furthermore, in virtue of Appendix~\ref{sect-9-A-2} we can use this formula even if $d=2m$ but $\vartheta>0$ which is the case for the Schr\"{o}dinger operator with $d=2$.

\item\label{rem-11-1-7-iii}
In particular, replacing conditions (\ref{11-1-19})--(\ref{11-1-21}) by conditions
\begin{gather}
\varrho_1 ^\vartheta\rho ^{d-s}\gamma ^{-s}\in
\sL^1(\{X,\ \rho \gamma \ge h_0\} ),
\label{11-1-46}\\[3pt]
\varrho_1^\vartheta \rho ^{d-1-\vartheta }\gamma ^{-1-\vartheta }\in
\sL^1( X \setminus X_{\reg,\elli,h_0} )
\label{11-1-47}
\shortintertext{and}
R_{0(\vartheta)}=O(h^{1+\vartheta})\qquad \text{as\ }\;h\to+0,
\label{11-1-48}
\end{gather}
we obtain t asymptotics
\begin{equation}
\N^-_{(\vartheta)} (A_h)=h ^{-d}\N^\W_{(\vartheta)}+O(h^{1+\vartheta -d}).
\label{11-1-49}
\end{equation}

In particular, in the framework of (\ref{11-1-23})--(\ref{11-1-24}) (upgraded to $d\ge 2m, k\in [0,2m]$ as $\vartheta>0$) conditions (\ref{11-1-48}) and (\ref{11-1-50}) below follow from (\ref{11-1-47}).
\end{enumerate}
\end{remark}

\subsubsection{Non-standard remainder estimates}
\label{sect-11-1-1-2}

So far we assumed that the remainder estimate in the local spectral asymptotics is $O(h_\eff^{1-d+\vartheta})$ as $\vartheta\ge 0$; $\vartheta=0$ refers to the most interesting case of the asymptotics without averaging.

\paragraph{Sharp and sharper asymptotics}
\label{sect-11-1-1-2-1}

However the remainder estimate in the local spectral asymptotics could be better than this: it could be $o(h_\eff^{1+\vartheta-d})$ or even
$O(h_\eff^{\kappa +\vartheta-d})$ with $\kappa>1$. In the former case conditions
(\ref{11-1-46})--(\ref{11-1-47}) imply that the contribution of $X_{\reg,h}$ to the remainder is $o(h^{1-d})$. Adding assumption
\begin{equation}
R_{0(\vartheta)}=o(h^{1+\vartheta})\qquad \text{as\ }\;h\to+0,
\label{11-1-50}
\end{equation}
we arrive to asymptotics
\begin{equation}
\N^-_{(\vartheta)} (A)=h ^{-d}\N^\W_{(\vartheta)}+o(h^{1+\vartheta -d}).
\label{11-1-51}%
\end{equation}

In the latter case conditions (\ref{11-1-47})--(\ref{11-1-48}) should be upgraded to
\begin{gather}
\varrho_1^\vartheta \rho ^{d-\kappa-\vartheta }\gamma ^{-\kappa-\vartheta }\in
\sL^1( X \setminus X_{\reg,\elli,h_0} )
\label{11-1-52}
\shortintertext{and}
R_{0(\vartheta)}=O(h^{\kappa+\vartheta})\qquad \text{as\ }\;h\to+0
\label{11-1-53}
\end{gather}
respectively. Note that in the framework of (\ref{11-1-23})--(\ref{11-1-24}) (upgraded to $d\ge 2m, k\in [0,2m]$ as $\vartheta>0$) condition (\ref{11-1-53}) follows from (\ref{11-1-52}).

Then we arrive to
\begin{equation}
\N^-_{(\vartheta)} (A)=h ^{-d}\N^\W_{(\vartheta)}+O(h^{\kappa+\vartheta -d}).
\label{11-1-54}
\end{equation}

\begin{remark}\label{rem-11-1-8}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-1-8-i}
Let us recall that sharp local asymptotics are due to corresponding non-periodicity condition:
\begin{equation}
\upmu_0 \bigl((\Pi_+ \cup \Lambda_+)\cap (\Pi_- \cup \Lambda_-) )=0
\label{11-1-55}
\end{equation}
where $\upmu_0$ is a measure introduced on $\Sigma_0$ and
\begin{equation}
\Pi_\pm =\{z: \exists t:\pm t>0: \Psi_{t}(z)\ni z\}
\label{11-1-56}
\end{equation}
is the set of points ``periodic'' with respect to Hamiltonian flow $\Psi_t$ with reflections, possibly branching and $\Lambda_\pm$ is the set of dead-end trajectories.

\item\label{rem-11-1-8-ii}
Recall, that we need also a bit more smoothness: for example, as $\vartheta=0$ the first derivatives of the coefficients should be continuous with the continuity modulus $o(|\log |x-y||^{-1})$ rather than $O(|\log |x-y||^{-1})$ (after rescaling) and condition to the smoothness of the boundary should be also a bit stronger.

As $\vartheta>0$ smoothness conditions grow stronger: $K=1+\lfloor \vartheta\rfloor$ and the $K$-th derivatives should be continuous with the continuity modulus $o(|x-y|^{\vartheta-\lfloor \vartheta\rfloor}|\log |x-y||^{-1})$.

We refer to these assumptions as \emph{improved regularity conditions\/}.\index{regularity conditions!improved}


\item\label{rem-11-1-8-iii}
Also a bit less degeneration is allowed:
as we consider Schr\"odinger operator with $d=2$ and $\vartheta=0$ we need to assume that
\begin{equation}
\mes (\{x, V(x)=0, F =|D_1V_2-D_2V_1|\ne 0\})=0.
\label{11-1-57}
\end{equation}
We refer to these assumptions as \emph{improved non-degeneracy condition}
\index{non-degeneracy condition!improved}
\end{enumerate}
\end{remark}

\begin{remark}\label{rem-11-1-9}
Recall that for sharper remainder estimates these improved conditions are required in the stronger form but since non-periodicity condition is so difficult to check we will consider only some special cases.
\end{remark}

\paragraph{Less sharp asymptotics}
\label{sect-11-1-1-2-2}
However, either due to irregularity (as in Theorem~\ref{thm-4-6-21} and similar) or to degeneration or both the local asymptotics may have remainder estimate not as good as $O(h_\eff^{1-d +\vartheta})$; for example it could be $O(h_\eff^{\kappa-d +\vartheta})$ with $\kappa<1$. Then again under assumptions (\ref{11-1-46}), (\ref{11-1-52}), (\ref{11-1-53}) we arrive to asymptotics (\ref{11-1-54}), this time with $\kappa<1$.

While estimates from above relied upon taking $T\asymp 1$ in $X_\reg\cap X_\sing$ which is not necessary the case now, it does not matter as $\rho\gamma \asymp h$ in $X_\reg\cap X_\sing$.

\subsection{Examples}
\label{sect-11-1-2}
Let us consider a series of examples.

%\renewcommand{\thetheorem}{10.1.5}
\begin{example}\label{ex-11-1-10}
Let $d\ge 2$ and let $X$ be a compact domain (or manifold) with the boundary. Let assumptions of Theorem~\ref{thm-11-1-1} be fulfilled with $\rho\asymp 1$ and $\gamma \asymp 1$. Then asymptotics \textup{(\ref{11-1-22})} holds.

Further, under appropriate smoothness condition (see Remark~\ref{rem-11-1-8}(i)) asymptotics \textup{(\ref{11-1-49})} holds.

Furthermore, under non-periodicity condition (\ref{11-1-55})--(\ref{11-1-56}), improved smoothness and non-degeneracy conditions of Remark~\ref{rem-11-1-8} asymptotics (\ref{11-1-54}) holds. Here $\Lambda_\pm=\emptyset$.

Finally, under corresponding stronger non-periodicity conditions sharper asymptotics hold.
\end{example}

The conditions of our theorems are local and all our analysis is local (until the end of the subsection). So we assume that outside of the singularities indicated below everything is well (in the sense of Example~\ref{ex-11-1-10}).


\begin{example}[Conical vertex]\label{ex-11-1-11}%
\index{conical singularity!semiclassical asymptotics of}%
\index{singularity!conical!semiclassical asymptotics of}%
\index{semiclassical asymptotics!conical singularity}%
\index{asymptotics!semiclassical!conical singularity}
Let $d\ge 2$ and in a neighborhood of $0$ let the domain $X$ coincide with the cone $X^0=\{(r,\theta )\in \bR^+\times U\}$ where $(r,\theta )$ are spherical coordinates, $U$ is a domain on the sphere $\bS^{d-1}$ with the boundary $\partial U$.

Moreover, let the conditions of Theorem~\ref{thm-11-1-1} be fulfilled with $\varrho =\rho ^{2m}$, $\rho =r ^\mu $, $\gamma =\epsilon r$ where here and below $\epsilon >0$ is a small constant.


\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-1-11-i}
Then $\rho ^d$ and (or) $\rho ^{d-1}\gamma ^{-1}$ belong to $\sL^1(X)$ if and only if $\mu >-1$. Let us assume that
\begin{equation}
\mu >\max(-1,-\frac{d}{2m}).
\label{11-1-58}
\end{equation}
Then asymptotics (\ref{11-1-22}) holds.

\item\label{ex-11-1-11-ii}
Further, under non-periodicity condition and improved regularity and non-degeneracy condition asymptotics \textup{(\ref{11-1-54})} holds. Here $\Lambda_\pm$ are sets of points such that $\Psi_t(z)$ ``falls'' to $0$ in the finite time. For example, if problem is spherically symmetric then $\Lambda_\pm $ consists of points with $\xi \parallel x$ (i.e. with angular momentum equal $0$).

\item\label{ex-11-1-11-iii}
On the other hand,
$\varrho ^\vartheta \rho ^{d-1-\vartheta }\gamma ^{-1-\vartheta }
\in \sL^1(X)$ if and only if
\begin{equation}
(\mu +1-2\mu m)\vartheta <(d-1)(\mu +1)
\label{11-1-59}
\end{equation}
and if this condition is fulfilled and if also $\mu >-{\frac{d}{2m}}$ then
asymptotics (\ref{11-1-49}) holds for given $\vartheta $.

Moreover, under non-periodicity condition (\ref{11-1-55})--(\ref{11-1-56}), improved smoothness and non-degeneracy conditions of Remark~\ref{rem-11-1-8} asymptotics (\ref{11-1-54}) holds.

\item\label{ex-11-1-11-iv}
Furthermore, in the case
\begin{equation}
(\mu +1-2\mu m)\vartheta =(d-1)(\mu +1)
\label{11-1-60}
\end{equation}
we obtain asymptotics
\begin{equation}
\N^-_{(\vartheta)} (A)=h^{-d}\N^\W_{(\vartheta)}
+O(h^{1-d+\vartheta }\log h);
\label{11-1-61}
\end{equation}
here we use Theorem~\ref{thm-11-1-1} instead of Corollary~\ref{cor-11-1-2}\,\footnote{\label{foot-11-2} Here and below
$\N^\W_{(\vartheta)} $ is given by the Weyl formula but in general we only integrate over the domain
$X_{\reg,h}=\{x\in X, |x|\ge \epsilon h^{1/(\mu +1)}\}$ so we have cut Weyl expression. Moreover, one can skip all the terms with $n-d>p$ in the local semiclassical spectral asymptotics and in the terms with $n-d<p$ integrate over $X$; $p=1-d+\vartheta $ under condition (\ref{11-1-60}).}.

\item\label{ex-11-1-11-v}
Finally, in the case
\begin{equation}
(\mu +1-2\mu m)\vartheta >(d-1)(\mu +1),\quad
2\mu m\vartheta +d(\mu +1)>0
\label{11-1-62}
\end{equation}
we obtain asymptotics
\begin{gather}
\N^-_{(\vartheta)} (A)=h^{-d}\N^\W_{(\vartheta)}+O(h^p)
\label{11-1-63}
\shortintertext{with}
p=\frac{2\mu}{\mu +1} m\vartheta \in (-d,\ 1+\vartheta -d)
\label{11-1-64}
\end{gather}
where only terms with the degree of $h$ less than $p+d$ are included in
$\N^\W_{(\vartheta)}$.
\end{enumerate}
\end{example}

\begin{remark}\label{rem-11-1-12}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-1-12-i}
We assumed that $\mu > -d/2m$ only to guarantee that
\begin{equation}
a_{\alpha\beta}\in \sL^1(X\cap \{|x|\le\epsilon\})
\label{11-1-65}
\end{equation}
and one can replace it by the latter, while also taking care that Rozenblioum estimate works; we leave details to the reader.

\item\label{rem-11-1-12-ii}
On the other hand, as $\mu \le -1$ it may happen that the corresponding quadratic form is not semi-bounded from below and thus operator $A$ is not defined; even if we define it, its essential spectrum may occupy the whole $\bR$.
\end{enumerate}
\end{remark}


\begin{remark}\label{rem-11-1-13}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-1-13-i}
One can easily see that in the domain
$X_{\sing,h}=\{x\in X, r\le \epsilon h^{\frac{1}{\mu +1}}\}$ inequality
\begin{multline}
(A_hu,u)\ge \epsilon_0\sum_{|\alpha |=m}h^{2m}\|D ^\alpha u\|^2 \\
\forall u\in \sC^m(\bar{X}):
\supp u\subset B(0,\epsilon h^{\frac{1}{\mu +1}})
\label{11-1-66}
\end{multline}
holds. This inequality follows from the inequalities
\begin{equation}
h^k\sum_{|\alpha |=k}\|D ^\alpha u\|\ge \epsilon_0
\varepsilon^{-\delta }\|r^{\mu k}u\|\qquad \forall k=1,\dots ,m
\label{11-1-67}
\end{equation}
for the same $u$ as in (\ref{11-1-66}). Here $\delta >0$ is a small enough exponent and $\epsilon_0$ does not depend on $\varepsilon$.

In fact, for $h=\epsilon =1$ estimate (\ref{11-1-67}) follows easily from condition (\ref{11-1-58}), and the estimate in the general case follows from the estimate in this special case by means of rescaling.

Therefore one can take $\rho =0$, $\varrho =r^{2\mu m}$ in $X_{\sing,h}$
and this simplifies the estimate of $R_0$. Further, we obtain that for
\begin{equation}
m\vartheta +d(\mu +1)=0
\label{11-1-68}
\end{equation}
asymptotics (\ref{11-1-63}) holds with $p=-d$ and with $\N^\W_{(\vartheta)} $ given only by the integration of the $n=0$ term over the domain $X_{\reg,h}$. Here $\N^\W_{(\vartheta)} =O(\log h)$; moreover, if
\begin{equation}
\inf_{v:\1v\1=1,\xi \in \bR^d}\blangle a(x,\xi )v,v\brangle \le
-\epsilon_0\rho ^{2m} \qquad\forall x\in \Gamma \cap\{|x|\le \epsilon \}
\label{11-1-69}
\end{equation}
for some non-empty cone $\Gamma \subset \bR^+\times U$ with vertex in $0$ then $\N^\W_{(\vartheta)} \asymp \log h$.

\item\label{rem-11-1-13-ii}
Further, let us note that under condition (\ref{11-1-60}) the main contribution to the remainder estimate in (\ref{11-1-63}) is delivered by the
zone
\begin{equation}
X_{h,\varepsilon}\coloneqq   \{X, ch^{\frac{1}{\mu +1}}\le |x|\le \varepsilon_h\}
\label{11-1-70}
\end{equation}
with $\varepsilon_h=o(1)$ for $h\to +0$ (the contribution of the other zones is ``$o$'' with respect to the contribution of this zone). In order to improve the remainder estimate let us assume that the operator $A$ stabilizes at $0$ to the quasi-homogeneous operator $A^0$, i.e., that
\begin{equation}
D^\alpha (a_\beta -a^0_\beta )=o(|x| ^{\mu |\beta |-|\alpha |})\qquad
\forall \beta :|\beta |\le 2m\quad \forall \alpha :|\alpha |\le K
\label{11-1-71}
\end{equation}
for $|x|\to 0$ where $a^0_\beta $ are positively homogeneous of degrees
$\mu |\beta |$. Further, let us
assume that the symbol
\begin{equation}
a^0(x,\xi )=\sum_\beta a^0_\beta (x)\xi ^\beta
\label{11-1-72}
\end{equation}
satisfies non-periodicity condition (\ref{11-1-55})--(\ref{11-1-56}) to Hamiltonian flow. Here and below $\Sigma ^0_\tau $, $\upmu^0_\tau$, $\Pi^0_\pm$, $\Lambda^0_\pm$ are constructed for $a^0$.

Then asymptotics
\begin{equation}
\N^-_{(\vartheta)} (A)=h^{-d}\N^\W_{(\vartheta)}
+o(h^{1-d+\vartheta }\log h)
\label{11-1-73}
\end{equation}
holds. Here in the term with $n=-d+1+\vartheta$ we integrate over the domain $X_{\reg,h}$ and this term is $O(h^{1+\vartheta}\log h)$; in all the other terms we can integrate over $X$.
\end{enumerate}
\end{remark}

\begin{example}\label{ex-11-1-14}
We can treat the case when the singularity is more complicated. Namely, for the Schr\"{o}dinger operator we can consider positively homogeneous $g^{jk}$, $V_j$, $V$ and also $\partial U$ which are not necessarily as regular as required by Theorem~\ref{thm-11-1-1} on $\bS^{d-1}$.

Let us assume that on $\bS^{d-1}$ all the conditions are fulfilled with $\hat{\rho}$ and $\hat{\gamma}$ instead of $\rho $ and $\gamma $. Then we can take $\rho =\hat{\rho}(\theta)r^\mu$ and
$\gamma =\epsilon \hat{\gamma}(\theta )r$ with a small enough constant
$\epsilon >0$.

Let us note that $\rho ^{2\vartheta +d}\in \sL ^1$ if and only if
$\hat{\rho}^{2\vartheta +d}\in \sL^1(U)$ and $(2\vartheta +d)\mu +d>0$; moreover, let us note that
$\rho ^{\vartheta +d-1}\gamma ^{-\vartheta -1}\in \sL ^1$ if and only if
$\hat{\rho}^{\vartheta d-1}\hat{\gamma} ^{-\vartheta -1}\in \sL^1(U)$
and $(\mu -1)\vartheta +(\mu +1)(d-1)>0$.

Therefore a more complicated structure is possible: one can treat a hierarchy
of singularities: ``vertices of singularities,'' ``edges of singularities,'' ``faces of singularities,'' etc.
\end{example}

We leave to the reader

\begin{problem}\label{problem-11-1-15}
Analyze the case in which
\begin{equation}
\gamma =\epsilon \min (|x_{(1)}|,\dots ,|x_{(l)}|),\quad
\rho =\prod_{S\subset \{1,\dots ,l\}}\zeta_S^{\mu_S},\quad
\zeta_S=\sum_{j\in S}|x_{(j)}|
\label{11-1-74}
\end{equation}
where
$x=(x_{(1)},\dots ,x_{(l)})\in \bR^{d_1}\times \ldots \times
\bR^{d_l}$ is an appropriate partition.
\end{problem}

\begin{example}[Conical edge]\label{ex-11-1-16}
Let us consider a more general case. Let $X$ be a bounded domain locally coinciding with $\bR^{d'}\times \bR^+\times U$ where spherical coordinates $(r,\theta)$ are introduced in $\bR^{d''}$ ($d''=d-d'$), and where
$U\subset \bS^{d''-1}$, $0\le d'\le d-1$. Let conditions of Theorem~\ref{thm-11-1-1} be fulfilled with $\varrho =\rho ^{2m}$,
$\rho =r^\mu $, $\gamma =\epsilon r$ and let
\begin{equation}
\mu >\max (-1,-{\frac{d''}{2m}}).
\label{11-1-75}
\end{equation}
Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-1-16-i}
For
\begin{equation}
(\mu +1-2\mu m)\vartheta <(\mu +1)(d-1)-d'
\label{11-1-76}
\end{equation}
asymptotics (\ref{11-1-49}) holds. Further, under non-periodicity condition and improved regularity and non-degeneracy condition asymptotics \textup{(\ref{11-1-54})} holds. Here $\Lambda_\pm$ are sets of points such that $\Psi_t(z)$ ``falls'' to $\bR^{d'}\times 0$ in the finite time.

\item\label{ex-11-1-16-ii}
On the other hand, for
\begin{equation}
(\mu +1-2\mu m)\vartheta =(\mu +1)(d-1)-d'
\label{11-1-77}
\end{equation}
asymptotics (\ref{11-1-61}) holds and for
\begin{equation}
(\mu +1-2\mu m)\vartheta >(\mu +1)(d-1)-d',\quad 2\mu m\vartheta +d\mu +d''\ge 0
\label{11-1-78}
\end{equation}
asymptotics (\ref{11-1-63}) holds with
\begin{gather}
p=\frac{2\mu}{\mu+1}( m\vartheta -d')
\label{11-1-79}\\
\shortintertext{where for}
2\mu m\vartheta +d\mu +d''= 0
\label{11-1-80}
\end{gather}
only one term in $\N^\W_{(\vartheta)} $ remains and integration is taken over $X_{\reg,h}$. In this case $\N^\W_{(\vartheta)} =O(\log h)$ and
$\N^\W_{(\vartheta)} \asymp \log h$ under condition (\ref{11-1-69}) fulfilled in $V\times \Gamma \cap \{x, |x''|\le \epsilon \}$ where $V$ is a neighborhood of $0$ in $\bR^{d'}$ and $\Gamma $ is a non-empty cone in $\bR^+\times U$ with vertex at $0$.

Let us note that in this example (in contrast to Example~\ref{ex-11-1-11})
the variants are possible even for $\vartheta =0$.

\item\label{ex-11-1-16-iii}
Let $\vartheta =0$. Then asymptotics (\ref{11-1-22}) and (\ref{11-1-61})
are replaced by asymptotics (\ref{11-1-63}) with $p=-d+1-\delta $ with
arbitrarily small exponent $\delta >0$ while asymptotics (\ref{11-1-63}) with $p<-d+1$ remains true.
\end{enumerate}
\end{example}

Consider conical singularity with the critical exponents:

\begin{example}\label{ex-11-1-17}
Let $0\in \bar{X}$ and all the conditions be fulfilled with
$\gamma =\epsilon r$, $\rho =r ^\mu |\log r|^{-\nu}$, $r=|x|$ where we assume that
\begin{multline}
\mu >-{\frac{2m}{d}},\;\mu \ge -1,\;\vartheta \ge 0,\;\nu >0,\\
2m\mu \vartheta +(d-\vartheta -1)(\mu +1)=0.
\label{11-1-81}
\end{multline}
Then repeating the arguments of the previous examples with
\begin{align}
&X_{\sing,h}=\{x\in X, |x| \le \epsilon h^{\frac{1}{\mu +1}}
|\log h| ^{\frac{\nu }{\mu +1}}\} &&\text{for\ \ }\mu >-1
\label{11-1-82}
\shortintertext{and}
&X_{\sing,h}=\{x\in X, \log |x|\le -Ch^{-\frac{1}{\nu }}\}
&&\text{for\ \ }\mu =-1
\label{11-1-83}
\end{align}
and with corresponding $X_{\reg,h}$ we conclude that

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-1-17-i}
Under condition
\begin{equation}
(2m\vartheta +d-\vartheta -1)\nu >1
\label{11-1-84}
\end{equation}
asymptotics (\ref{11-1-49}) holds; moreover, under standard non-periodicity condition and improved regularity and non-degeneracy conditions asymptotics (\ref{11-1-51}) holds.

\item\label{ex-11-1-17-ii}
On the other hand, under condition
\begin{equation}
(2m\vartheta +d-\vartheta -1)\nu =1
\label{11-1-85}
\end{equation}
asymptotics (\ref{11-1-61}) holds.

\item\label{ex-11-1-17-iii}
Finally, if
\begin{gather}
(2m\vartheta +d-\vartheta -1)\nu <1
\label{11-1-86}
\shortintertext{and if either}
\mu >-1
\tag*{$\textup{(\ref*{11-1-87})}_1$}\label{11-1-87-1}
\shortintertext{or}
\mu =-1(\implies \vartheta =0),\; \nu \ge {\frac{1}{d}}
\tag*{$\textup{(\ref*{11-1-87})}_2$}\label{11-1-87-2}
\end{gather}
\begin{phantomequation}\label{11-1-87}\end{phantomequation}
then asymptotics (\ref{11-1-63}) holds with
\begin{equation}
p=2m\vartheta -\vartheta -\frac{1}{\nu}.
\label{11-1-88}
\end{equation}
For $\mu =-1$, $\vartheta =0$, $\nu =\frac{1}{d}$ we see that $\N^\W =O(\log h)$ and $\N^\W \asymp\log h$ provided condition (\ref{11-1-69}) is fulfilled in some non-empty cone with vertex at $0$ (for $|x|\le\epsilon $).

\item\label{ex-11-1-17-iv}
 Moreover, in the first critical case (\ref{11-1-85}) one can improve asymptotics (\ref{11-1-61}). We do not do a careful analysis of the Hamiltonian trajectories here but refer to the arguments of the proofs of Example~\ref{ex-11-5-21} (see below). Let us assume that the coefficients $a_\beta $ of $A$ stabilize to functions
$a^0_\beta \big|\log |x|\big|^{-\nu |\beta |}$ in the sense that
\begin{multline}
D^\sigma
(a_\beta \bigl|\log |x|\bigr|^{\nu |\beta |}-a^0_\beta )=
o(|x| ^{\mu |\beta |-|\sigma |})\\
\forall \beta :|\beta |\le 2m \;\forall \sigma :|\sigma |\le 1
\label{11-1-89}
\end{multline}
where $a ^0_\beta $ are positively homogeneous of degree $\mu |\beta |$.
Moreover, let us assume that the quasi-homogeneous symbol (\ref{11-1-72})
satisfies the standard non-periodicity condition.

Then one can easily prove that asymptotics (\ref{11-1-73}) holds with all
the explanations made in Remark~\ref{rem-11-1-13}.

\item\label{ex-11-1-17-v}
For $\nu >0$ satisfying the critical condition (\ref{11-1-85}) one
can treat the case in which
$\rho =r^\mu |\log r| ^{-\nu }\bigl|\log|\log r|\bigr|^{-\nu '}$ and
analyze all the possible cases. In this case the conditions on $\nu $ are
replaced by similar conditions on $\nu '$. One can continue this
process of complication.

\item\label{ex-11-1-17-vi}
On the other hand, one can treat the case in which
$\rho =r^\mu |\log r| ^{-\nu }$ even if equality in (\ref{11-1-81}) is violated, i.e., $\mu $ is not the critical value. In this case for
$2m\mu \vartheta +(d-\vartheta -1)(\mu +1)>0$ asymptotics (\ref{11-1-49}) (and even (\ref{11-1-51}) under the standard non-periodicity condition to the Hamiltonian flow) holds and for
$2m\mu \vartheta +(d-\vartheta -1)(\mu +1)<0$ asymptotics (\ref{11-1-63}) holds with the remainder estimate $O(h^p|\log h|^q)$ instead of $O(h^p)$. The
calculation of $q$ is left to the reader.

\item\label{ex-11-1-17-vii}
In all the above statements the condition $\nu >0$ is not necessary
if $\mu >-1$.

\item\label{ex-11-1-17-viii}
Statement \ref{ex-11-1-16-ii} of Example~\ref{ex-11-1-16} remains true (with obvious modifications).

Different combinations of Statements~\ref{ex-11-1-17-v} and~\ref{ex-11-1-17-vi} are possible.
\end{enumerate}
\end{example}

\begin{example}[Quasi-conical singularity]\label{ex-11-1-18}%
\index{quasi-conical singularity!semiclassical asymptotics of}%
\index{singularity!quasi-conical!semiclassical asymptotics of}%
\index{semiclassical asymptotics!quasi-conical singularity}%
\index{asymptotics!semiclassical!quasi-conical singularity}%
Let $0\in\bar{X}$ and let us consider operator with coefficients $a_{\alpha\beta}$ which are \emph{$L$-quasi-homogeneous
of degrees\/} $(2m-|\alpha|-|\beta|)\mu $ respectively, smooth away from $0$.
In a neighborhood of zero let $X$ be an \emph{$L$-quasi-conical\/} domain and let $\partial X$ be smooth away from $0$. Here $L=(L_1,\dots ,L_d)$ is an exponent vector with $L_j>0$ $\forall j$ and $\max_jL_j=1$.

Let us assume that either a Dirichlet or some other appropriate boundary condition is given and in the second case let us assume that the
domain $X$ satisfies the standard cone condition.

In this case $\gamma (x) =\epsilon [x]_L$, $\rho (x)=\gamma ^{\mu }$,
$\varrho (x)=\gamma ^{2m\mu }$ with \emph{$L$-quasi-homogeneous norm\/} $[x]_L=\sum_j |x_j|^{\frac{1}{L_j}}$. Then repeating the arguments of Example~\ref{ex-11-1-11} and assuming that
\begin{equation}
\mu >\max \bigl(-1,-{\frac{L^*}{2m}}\bigr),\qquad
L^*=L_1+\dots +L_d
\label{11-1-90}
\end{equation}
we conclude that

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-1-18-i}
For
\begin{equation}
(\mu +1-2\mu m)\vartheta <(d-1)\mu +L^*
\label{11-1-91}
\end{equation}
asymptotics (\ref{11-1-49}) holds.

Moreover, under non-periodicity condition and improved regularity and non-degeneracy conditions asymptotics (\ref{11-1-51}) holds.

\label{ex-11-1-18-ii}
On the other hand, for
\begin{equation}
(\mu +1-2\mu m)\vartheta =(d-1)\mu +L^*
\label{11-1-92}
\end{equation}
asymptotics (\ref{11-1-61}) holds and for
\begin{equation}
(\mu +1-2\mu m)\vartheta >(d-1)\mu +L^*,
\quad 2m\mu \vartheta +d\mu +L^*>0
\label{11-1-93}
\end{equation}
asymptotics (\ref{11-1-63}) holds with
$p=(2m\mu \vartheta +L^*-d)(\mu +1) ^{-1}$.
\end{enumerate}
\end{example}

However the author have failed to solve
\begin{Problem}\label{Problem-11-1-19}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{Problem-11-1-19-i}
Apply more advanced arguments of Remark~\ref{rem-11-1-13}.

\item\label{Problem-11-1-19-ii}
Investigate the second critical case
$2m\mu \vartheta +d\mu +L^*= 0$.
\end{enumerate}
\end{Problem}

We leave to the reader to

\begin{problem}\label{problem-11-1-20}
Investigate the case $\rho =r ^\mu $, $\gamma =\epsilon r^{1+\nu }$ with
$\nu >0$ arising in the analysis of the Schr\"{o}dinger operator with potential
$V=\rho ^{2\mu }\sin r^{-\nu }$ and other examples of this type.
\end{problem}

Let us treat exits to infinity. We assume that

\begin{claim}\label{11-1-94}
Either $X_{\sing,h}=\emptyset$ or a Dirichlet boundary condition is
given on $\partial X\cap \{|x|\ge c\}$.\footnote{\label{foot-11-3} In the next sections we discuss how to weaken this assumption (albeit it is impossible to get rid off it).}
\end{claim}

\begin{example}[Exit to infinity]\label{ex-11-1-21}%
\index{exit to infinity!semiclassical asymptotics of}%
\index{semiclassical asymptotics!exit to infinity}%
\index{asymptotics!semiclassical!exit to infinity}
\begin{enumerate}[label=(\alph*), wide, labelindent=0pt]
\item\label{ex-11-1-21-a}
In a neighborhood of infinity let $X$ coincide with
$\{x, x_1>0,x'=F(x_1)\Omega \}$ where $\Omega \subset \bR^{d-1}$ is a
bounded domain satisfying assumptions of Theorem~\ref{thm-11-1-1} with $\gamma(x')\asymp 1$, $x'=(x_2,\dots ,x_d)$, $t\Omega =\{tx', x'\in \Omega \}$ and
\begin{gather}
F(x_1)\asymp x_1 ^\beta ,\qquad \beta \le 1,
\label{11-1-95}\\[2pt]
|D ^\alpha F|\le cF^{1-|\alpha |}\qquad \forall \alpha :|\alpha |\le 2.
\label{11-1-96}
\end{gather}
For $\beta =1$ we have a conical exit, for $\beta \in (0,1)$ we
have a slowly expanding quasi-conical exit, for $\beta =0$ we have
a cylindrical exit and for $\beta <0$ we have a constricting exit
and these exits could be corrugated along the $x_1$ axis.

\item\label{ex-11-1-21-b}
 Similarly, let us consider the case in which $X$ coincides with
$\{x, x'=F(|x''|)\Omega \}$ in a neighborhood of infinity where
$x=(x'',x')\in \bR^{d''}\times \bR^{d'}$, $0<d'<d=d'+d''$
and the function $F$ satisfies conditions (\ref{11-1-95})--(\ref{11-1-96}).
\end{enumerate}

Then geometry yields that (at least for $|x''|\ge c$)
\begin{claim}\label{11-1-97}
$X$ satisfies conditions of Theorem~\ref{thm-11-1-1} with
$\gamma \asymp F(|x''|)$.
\end{claim}
Actually all we need is (\ref{11-1-96}) with $K=1$ and (\ref{11-1-97}).
Moreover, let us assume that the other conditions are fulfilled with
$\gamma =\epsilon F(|x''|)$ and $\rho =|x''|^\mu $. Then


\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-1-21-i}
If $\mu +\beta \ge 0$ one can take $X_{\reg,h}=X$ and $X_{\sing,h}=\emptyset$. Then under the condition
\begin{equation}
2m\mu \vartheta +d\mu +d'\beta +d''<0
\label{11-1-98}
\end{equation}
(which provides that $\N^\W_{(\vartheta)} $ converges)
asymptotics (\ref{11-1-49}) holds. Note that $\mu+\beta\ge 0$ and (\ref{11-1-98}) imply that $\mu <0$, $\vartheta>0$.

Moreover, under the standard non-periodicity condition and improved regularity and non-degeneracy conditions asymptotics (\ref{11-1-51}) holds.

\item\label{ex-11-1-21-ii}
Let $\mu +\beta <0$. Then one can take
$X_{\reg,h}=X\cap \{r\le Ch^{1/( \mu +\beta )}\}$ and
$X_{\sing,h}=X\cap \{r\ge \frac{1}{2}Ch^{1/(\mu +\beta )}\}$ where
$r=|x''|$. Let us assume that a Dirichlet condition is given on
$\partial X\cap \{|x''|\ge C\}$\,\footref{foot-11-3}. Then inequality
\begin{equation}
h^m\sum_{\alpha :|\alpha |=m}\|{D'} ^\alpha u\|_{(x'')}\ge
\epsilon_0 F(r)^{-m}\|u\|_{(x'')}
\label{11-1-99}
\end{equation}
(where $\|.\|_{(x'')}$ means the $\sL ^2$-norm over sections of $X$ at
points $x''$) yields that under condition
\begin{equation}
(2m\mu -\beta -\mu )\vartheta +(d-1)\mu -\beta +d'\beta +d''<0
\label{11-1-100}
\end{equation}
asymptotics (\ref{11-1-49}) holds.

Moreover, under standard non-periodicity condition and improved regularity and non-degeneracy conditions asymptotics (\ref{11-1-51}) holds.

\item\label{ex-11-1-21-iii}
On the other hand, for
\begin{equation}
(2m\mu -\beta -\mu )\vartheta +(d-1)\mu -\beta +d'\beta +d''=0
\label{11-1-101}
\end{equation}
asymptotics (\ref{11-1-61}) holds and for
\begin{multline}
(2m\mu -\beta -\mu )\vartheta +(d-1)\mu -\beta +d'\beta +d''>0,\\
2m\mu \vartheta +d\mu +d'\beta +d''\le 0
\label{11-1-102}
\end{multline}
asymptotics (\ref{11-1-63}) holds with
$p=(2m\mu \vartheta +d''-d''\beta )(\mu +\beta ) ^{-1}$; here in the case of equality in the last condition the integral in $\N^\W_{(\vartheta)} $ is calculated over the domain $X_{\reg,h}$ and $\N^\W_{(\vartheta)} =O(\log h)$.

Moreover, let condition (\ref{11-1-69}) be fulfilled for $|x''|\ge c,x''\in \Gamma $ and $x'\in F(|x''|)\Omega'$ where $\Gamma \subset \bR^{d''}$ is a non-empty cone and $\Omega '\subset\Omega $ is a non-empty domain. Then
$\N^\W_{(\vartheta)} \asymp \log h$.
\end{enumerate}
\end{example}

We leave to the reader to analyze the case of more general dependence of $F$ on $x''$.

\begin{example}[Conical exit to infinity]\label{ex-11-1-22}%
\index{conical exit to infinity!semiclassical asymptotics of}%
\index{exit to infinity!conical!semiclassical asymptotics of}%
\index{semiclassical asymptotics!conical exit to infinity}%
\index{asymptotics!semiclassical!conical exit to infinity}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-1-22-i}
In a neighborhood of infinity let the domain $X$ coincide
with the cone $X^0=\{(r,\theta )\in \bR^+\times U\}$ and let the conditions be fulfilled with $\gamma =\epsilon r$, $\rho =r ^\mu $. Then if
\begin{equation}
\mu \ge -1,\qquad 2m\mu \vartheta +(\mu +1)d<0
\label{11-1-103}
\end{equation}
then
asymptotics (\ref{11-1-49}) holds.

Moreover, under standard non-periodicity condition and improved regularity and non-degeneracy conditions asymptotics (\ref{11-1-51}) holds.

\item\label{ex-11-1-22-ii}
 Let us treat the case
\begin{equation}
\mu <\min (-1,-\frac{2m}{d});
\label{11-1-104}
\end{equation}
then estimates
(\ref{11-1-66}) and (\ref{11-1-67}) hold for functions $u$ supported in
$\bR^d\setminus B(0,\epsilon^{-1} h^{1/(\mu+1)})$ and therefore
under condition $\textup{(\ref{11-1-59})}^\#$ asymptotics (\ref{11-1-49}) holds.

Moreover, under standard non-periodicity condition and improved regularity and non-degeneracy conditions asymptotics (\ref{11-1-51}) holds.

Here the superscript ``$\#$'' means that the condition is replaced by its opposite (i.e., ``$>$'' by ``$<$'' and v.v., and ``$=$'' remains), $|x|\to 0$ is replaced by $|x|\to \infty$ and $|x|\le \epsilon$ is replaced by $|x|\ge C$.


\item\label{ex-11-1-22-iii}
Further, under condition $\textup{(\ref{11-1-60})}^\#$ we obtain asymptotics (\ref{11-1-61}) and under condition $\textup{(\ref{11-1-62})}^\#$ we obtain asymptotics (\ref{11-1-63})
with $p$ given by the same formula as before.

Finally, under condition $\textup{(\ref{11-1-68})}^\#$ asymptotics (\ref{11-1-63}) remains true with the same clarifications as before.

Moreover, under conditions $\textup{(\ref{11-1-60})}^\#$, $\textup{(\ref{11-1-71})}^\#$ and the standard non-periodicity condition and improved regularity and non-degeneracy conditions we obtain asymptotics
(\ref{11-1-73}).
\end{enumerate}
\end{example}

\begin{example}[Conical exit to infinity. II]\label{ex-11-1-23}
Let $\gamma =\epsilon r$, $\rho =r^\mu \log^{-\nu }r$ where
\begin{equation}
\mu \le -1.\qquad \mu <-{\frac{2m}{d}}
\label{11-1-105}
\end{equation}
satisfies (\ref{11-1-59}).

Then all the results of Example~\ref{ex-11-1-17} remain true and the inequalities on $\nu $ do not change and in the stabilization conditions and in (\ref{11-1-69}) $|x|\to 0$ is replaced by $|x|\to \infty $ and $|x|\le \epsilon $ is replaced by $|x|\ge C$. Again we need to change all inequalities to their opposites.
\end{example}

\begin{example}[Quasi-conical exit to infinity]\label{ex-11-1-24}%
\index{quasi-conical exit to infinity!semiclassical asymptotics of}%
\index{exit to infinity!quasi-conical!semiclassical asymptotics of}%
\index{semiclassical asymptotics!quasi-conical exit to infinity}%
\index{asymptotics!semiclassical!quasi-conical exit to infinity}
In a neighborhood of infinity let $X$ be an $L$-quasi-conical domain and $\partial X\in \sC^2$. Then in a neighborhood of infinity one can take
$\gamma =\epsilon [x]_{\delta L} ^\delta$ where we assume that $L=(L_1,\dots ,L_d)$, $L_j\ge 1$ \ $\forall j$ and $\delta \le \min_j L_j^{-1}$. Let us assume that $\rho =\gamma ^\mu $ and $\varrho =\gamma ^{2\mu m}$.

In this case all the statements of Example~\ref{ex-11-1-18} remain true with
the inequalities on $\mu $ replaced by their opposites.
\end{example}

We leave to the reader the following rather easy problem:

\begin{problem}\label{problem-11-1-25}
Investigate the case in which $X=\bR^{d'}\times \bT^{d''}$
in a neighborhood of infinity and $\gamma =1$.
\end{problem}


\subsection{Non-semi-bounded operators}
\label{sect-11-1-3}

Let us now consider operators which are non-semi-bounded. In this case we assume that $\vartheta =0$ unless otherwise indicated. Since the order of operator is not necessarily even anymore, denote it by $m$ rather than by $2m$.

Theorem~\ref{thm-11-1-1} and Corollary~\ref{cor-11-1-2}, as well as Example~\ref{ex-11-1-10}, remain true in this case with obvious modifications. Moreover, one can treat the Dirac operator in $X=\bR^d$ assuming that for $|x|\ge c$
\begin{gather}
V+M-\tau_2\ge \epsilon_0\rho ^2,
\qquad M-V+\tau_1\ge \epsilon_0\rho ^2
\label{11-1-106}
\shortintertext{and}
\rho \gamma \ge \epsilon_0,\label{11-1-107}\\
\int \rho ^{d-s} \gamma ^{-s}dx<\infty
\label{11-1-108}
\end{gather}
because these conditions ensure that $\{|x|\ge c\}\subset X_{\reg,\elli}$. Recall that $M$ is the mass.

We leave to the reader

\begin{problem}\label{problem-11-1-26}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-1-26-i}
Include a neighborhood of infinity in $X_{\sing,h}$ and skip condition (\ref{11-1-108});
\item\label{problem-11-1-26-ii}
Treat the case $X=\bR^{d'}\times \bT^{d''}$ with $d'>0,d''>0$.
\end{enumerate}
\end{problem}

Furthermore, one can treat the \emph{generalized Dirac}%
\index{generalized Dirac operator}%
\index{Dirac operator!generalized}%
\index{operator!Dirac!generalized}
operator
\begin{equation}
A=\begin{pmatrix} V_1 &{\cL}\\ {\cL}^* &V_2\end{pmatrix}
\label{11-1-109}
\end{equation}
where $V_k$ are matrix-valued functions, ${\cL}$ is a uniformly elliptic operator of order $m$ and for $|x|\ge c$
\begin{equation}
V_2-\tau_2\ge \epsilon_0\rho ^{2m},\qquad
V_1-\tau_1\le -\epsilon_0(\rho +1)^{2m},
\qquad \rho \gamma \ge \epsilon_0.
\label{11-1-110}
\end{equation}
Moreover, we assume that the coefficients of ${\cL}$ satisfy conditions
\begin{gather}
\1D ^\alpha b_\beta \1\le c\rho ^{m-|\beta |}\gamma ^{-|\alpha |}
\qquad \forall \beta:|\beta |\le m
\label{11-1-111}\\
\shortintertext{and}
\1D ^\alpha V_2\1\le c\rho ^{2m}\gamma ^{-|\alpha |},\qquad
\1D ^\alpha V_1\1\le c(\rho +1)^{2m} \gamma ^{-|\alpha |}\label{11-1-112}\\[2pt]
\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad
\forall \alpha :1\le |\alpha |\le K\notag
\end{gather}
We can assume instead that the corresponding roughness conditions are fulfilled.

Then
\begin{claim}\label{11-1-113}
All examples with singularities at $0$\,\footnote{\label{foot-11-4} I.e. Examples~\ref{ex-11-1-10},~\ref{ex-11-1-11} and \ref{ex-11-1-14}--\ref{ex-11-1-18}.} remain true for $X=\bR^d$ if in the inequalities for exponents we replace $2m$ by $m$; however, we do not modify the inequalities (\ref{11-1-58}) and (\ref{11-1-75}) to reflect that $m$ rather than $2m$ is an order of the operator.
\end{claim}

Further,
\begin{claim}\label{11-1-114}
All examples with singularities at infinity\footnote{\label{foot-11-5} I.e. Examples~\ref{ex-11-1-21}--\ref{ex-11-1-24}.} remain true
without modification in the inequalities on exponents provided in a
neighborhood of infinity
\begin{equation}
V_1-\tau_1\le -\epsilon_0,\qquad
V_2-\tau_2\le -\epsilon_0\rho ^{2m}.
\label{11-1-115}
\end{equation}
Recall that in these examples $\rho \le c$.
\end{claim}

Finally, let us note that under conditions (in $X$)
\begin{equation}
V_1-\tau_1\le -\epsilon_0,\qquad
V_2-\tau_1\ge \epsilon_0, \qquad \rho \le c
\label{11-1-116}
\end{equation}
one can treat
\begin{equation}
\N^-_{(\vartheta)} (A)=
\int_{\tau_1}^{\tau_2}(\tau_2-\tau )_+^{\vartheta -1}d\tau
\label{11-1-117}
\end{equation}
with $\vartheta >0$. Then Example~\ref{ex-11-1-10} and all the examples with
singularities at infinity\footref{foot-11-5} remain true.

We leave to the reader
\begin{problem}\label{problem-11-1-27}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-1-27-i}
Justify these claims (\ref{11-1-113}) and (\ref{11-1-114}) basing on the results of Chapter~\ref{sect-10}.

\item\label{problem-11-1-27-ii}
Based on Remark~\ref{rem-10-2-23} pass from operators with rough coefficients to operators with irregular coefficients. In particular, using the fact that eigenvalues are monotone with respect to $V_1,V_2$ consider the case when only $V_1$ and $V_2$ are irregular and either $\tau_1$ or $\tau_2$ belong to spectral gap.
\end{enumerate}
\end{problem}


\section[Large eigenvalues for weakly singular potentials]{Large eigenvalues for operators with weakly singular potentials}
\label{sect-11-2}

This section is devoted to the General scheme and main theorems.

\subsection{General scheme}
\label{sect-11-2-1}

In this and the following two sections we consider the asymptotics of the eigenvalues of operator $A$, tending to $+\infty$. In fact, one can treat more general problem
\begin{equation}
(A-\lambda J)u=0\qquad u\in \fD (A)
\label{11-2-1}
\end{equation}
where $A$ and $J$ are operators of orders $2m$ and $n<2m$ respectively
($m\in {\frac{1}{2}}\bZ$). Recall that in this problem one should assume that
\begin{claim}\label{11-2-2}
$A$ is a self-adjoint operator, $J$ is a symmetric operator and $J$ is $A$-compact\footnote{\label{foot-11-6} This condition will be fulfilled automatically in the frameworks of the theorems below.} and at least one of operators $A$ and $J$ is positive definite.
\end{claim}
Surely, the case $J=I$ is the most natural and interesting from the point of view of miscellaneous, in particular physical applications; in the next sections that case will be treated but in this section we consider the more general case (\ref{11-2-1}) as well.

In this section we assume that $A$ is semi-bounded from below; at the end of the section $J=I$ and $A$ is not necessarily semi-bounded. Note that Birman-Schwinger principle yields that

\begin{claim}\label{11-2-3}
If the operator $J$ is positive definite then the the number of eigenvalues of the problem (\ref{11-2-1}) less than $\tau $ is equal to $\N^-(\tau) $ which is
the number of negative eigenvalues of the operator $(A-\tau J)$
\end{claim}
and
\begin{claim}\label{11-2-4}
If the operator $A$ is positive definite then the number of eigenvalues
$\lambda \in (0,\tau )$ of the problem (\ref{11-2-1}) (with $\tau >0$) is equal to $\N^-(\tau) -\N^-(+0)$ where $\N^-(\tau)$ is again the number of negative eigenvalues of the operator $(A-\tau J)$ and
$\N^-(+0)=\lim_{\tau \to +0}\N^-(\tau )$.
\end{claim}

There is no contradiction since as both $A$ and $J$ are positive definite problem (\ref{11-2-1}) has only positive eigenvalues.

Therefore in the both cases we should consider the asymptotics of
$\N^-(\tau )$ as $\tau \to +\infty $.

Let us assume that $A$ is given by (\ref{11-1-1}) with $h=1$, $m\in\bZ$, that conditions (\ref{11-1-2}) and (\ref{11-1-3}) are fulfilled and
\begin{gather}
J=\sum_{|\alpha |,|\beta |\le m, |\alpha |+|\beta |\le n}
D ^\alpha j_{\alpha ,\beta }D ^\beta ,
\label{11-2-5}\\
\intertext{with the coefficients satisfying}
|D ^\sigma a_{\alpha ,\beta }|\le
c\varrho \rho ^{-|\alpha |-|\beta |}\gamma ^{-|\sigma |},
\label{11-2-6}\\[3pt]
|D ^\sigma j_{\alpha ,\beta }|\le c\varrho_0\rho ^{-|\alpha |-|\beta |}
\gamma ^{-|\sigma |} \qquad \forall \sigma :|\sigma |\le K\label{11-2-7}
\end{gather}
or corresponding ``rough'' conditions.

Further, let us assume that the boundary $\partial X$ is smooth enough after rescaling of $\cB(y,\gamma(y),X)$ and that the coefficients of the boundary operator $B=(B_1,\dots ,B_l)$ satisfy condition \ref{9-2-3-2}. Furthermore, let us assume that the operator $\varrho ^{-1}\rho ^{2m}A$ is uniformly elliptic and that the boundary value problem
$(\varrho^{-1}\rho ^{2m}A, \varrho_{(1)}^{-1}B_1,\dots,\varrho_{(l)}^{-1}B_l)$ is uniformly elliptic as well.

One can easily see that in the zone $\{x\in X, \rho_\tau \gamma_\tau \ge 1\}$ operator $(A-\tau J)$ satisfies all the conditions of Section~\ref{sect-9-1}\footnote{\label{foot-11-7} With the possible exception of the microhyperbolicity, or $\xi$-microhyperbolicity, or some other non-degeneracy condition.} with functions
\begin{multline}
\gamma_\tau=\gamma, \quad
\rho_\tau=
\rho\bigl(1+\frac{\tau\varrho_0}{\varrho} \bigr)^{\frac{1}{2m-n}},\quad
\varrho_\tau=
\varrho \bigl(1 + \frac{\tau \varrho_0}{\varrho } \bigr)^{\frac{2m}{2m-n}}, \\
\varrho _{\tau(j)}=
\varrho_{(j)}\bigl({\frac{\tilde{\rho}}{\rho}}\bigr)^{-m_j}
\label{11-2-8}
\end{multline}
instead of $\gamma$, $\rho$, $\varrho$ and $\varrho_{(j)}$
respectively\footnote{\label{foot-11-8} We use the notation $\varrho_{(k)}$ instead of the $\varrho_k$ of Section~\ref{sect-9-1} in order to avoid misunderstanding.}.

Let us treat the microhyperbolicity or non-degeneracy condition in the zone
\begin{gather}
X'_\reg= \bigl\{x\in X, \tau \varrho_0\ge
C\varrho \bigl(1+(\rho \gamma )^{n-2m}\bigr) \bigr\}\label{11-2-9}\\
\shortintertext{in which}
\rho_\tau\gamma \ge C'\quad\text{and}\quad \rho_\tau \ge C'\rho \label{11-2-10}
\end{gather}
provided $C=C(C')$. We easily see that for large enough $C'$ in this zone one can replace the complete symbols of the operators $A$, $B$ and $J$ by their senior symbols\footnote{\label{foot-11-9} I.e., the higher degree homogeneous symbols.} in the verification of such condition and after rescaling with respect to $x$ and $\xi $\,\footnote{\label{foot-11-10} I.e., rescaling with respect to $x$ and multiplication of the operators by appropriate factors.} we easily see that
\begin{claim}\label{11-2-11}
One needs to check this non-degeneracy condition with $\gamma \partial_x$ instead of $\partial_x$ and with $\partial_\xi $ preserved for the symbol
$\bigl(\tilde{a}(x,\xi )-\tilde{\jmath}(x,\xi ),\tilde{b}(x,\xi )\bigr)$
\end{claim}
where tilde means that one needs to multiply $a$, $j$ and $b_k$ by
$\varrho ^{-1}$, $\varrho_0^{-1}$ and $\varrho_{(k)}^{-1}$
respectively at point $x$; these factors are ``well-differentiable'' (in the corresponding scale) with respect to $x$.

Let us first check the conditions which are not associated with the symbol $\tilde{b}$ of the boundary operator. Note that for $|\xi |\ge \epsilon$ with an arbitrarily small constant $\epsilon >0$ the ellipticity of $\tilde{a}(x,\xi )$, the homogeneity of $\tilde{a}(x,\xi)$ and $\tilde{\jmath} (x,\xi )$ of degrees $2m$ and $n$ with respect to $\xi $ and the Euler identity yield that
$\xi$-microhyperbolicity condition is fulfilled. Therefore
\emph{the remaining check should be done for $\xi =0$ only}.

For general matrix operators one needs to check $\xi$-microhyperbolicity or microhyperbolicity condition and since $\tilde{a}$ with its first order derivatives vanishes at $\xi =0$ this condition should be checked for $\tilde{\jmath} (x,\xi )$.

The three following cases are possible:

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{sect-11-2-1-i}
$n=0$; then microhyperbolicity condition means exactly that
\begin{claim}\label{11-2-12}
$n=0$ and for every $x\in X_\reg$ there exists $\ell \in T_x X$ such that $|\ell|=1$ and\vglue-20pt
\begin{equation}
\gamma \blangle \ell j(x)v,v\brangle \ge
\epsilon_0 \varrho_0\1v\1^2- c\varrho_0 ^{-1}\1j(x)v\1 ^2
\qquad \forall v\in \bH
\label{11-2-13}
\end{equation}
\end{claim}\vglue-20pt\noindent
where $j(x)=J(x)$ and we returned to $j$ from $\tilde{\jmath} $. In
particular, this condition is fulfilled automatically if
\begin{claim}\label{11-2-14}
$n=0$ and \quad
$\1j(x)v\1\ge\epsilon\varrho_0\1v\1\qquad\forall x\in X'\quad\forall v\in\bH$;
\end{claim}

\item\label{sect-11-2-1-ii}
$n=1$; in this case $\tilde{\jmath} (x,0)=0$ and one should differentiate with respect to $\xi $ only; then microhyperbolicity condition means exactly that
\begin{claim}\label{11-2-15}
$n=1$ and for every $x\in X_\reg$ there exists $\xi \in T^*_xX$ such that
$|\xi |=1$ and
\begin{equation*}
\blangle j(x,\xi )v,v\brangle \ge
\epsilon_0\varrho_0\rho ^{-1}\1v\1 ^2\qquad \forall v\in \bH
\end{equation*}
\end{claim}
\vglue-15pt\noindent
where $j(x,\xi )$ is the senior symbol of $J(x,D_x)$.

\item\label{sect-11-2-1-iii}
$n\ge 2$; in this case $\tilde{\jmath} $ and its first order derivatives
vanish at $\xi =0$ and the microhyperbolicity condition is surely
violated.

Note that $\xi$-microhyperbolicity condition is fulfilled in the cases (\ref{11-2-14}) and (\ref{11-2-15}) only; in this case remainder estimate $O(h_\eff^{1-d})$ is ensured under regularity conditions marginally stronger than $K=1$ (see Sections~\ref{sect-4-6} and \ref{sect-7-5}); we refer to them as \emph{minimal regularity assumptions\/}.

For scalar symbols $a$ and $j$\,\footnote{\label{foot-11-11} It is sufficient to assume that either the eigenvalues of $a(x,\xi )-j(x,\xi )$ close to $0$ are simple in a neighborhood of $\{\xi =0\}$ or these eigenvalues are of constant multiplicity there and $\rho \gamma \le C$ in the latter case. For $n\ge 1$ that automatically yields that $(a-j)$ is a scalar symbol and the homogeneity of $a$ and $j$ yield that $a$ and $j$ are scalar symbols.

For $n=0$ this conjecture is not necessary. In this case in the appropriate local coordinates $j=\begin{pmatrix} j''&0\\0&j'I\end{pmatrix} $,
$a=\begin{pmatrix} *&*\\ *&a'I\end{pmatrix} $ where $j''$ is a
non-degenerate matrix and $j'$ and $a'$ are scalar symbols and
under the above condition all the following conditions should be checked
for symbols $a'$ and $j'$.}
the following additional possibilities arise:

\item\label{sect-11-2-1-iv}
$m=1$, $d\ge 2$; then $(A-\lambda J)$ after all rescaling is the Schr\"odinger operator and no microhyperbolicity is needed; so we assume that
\begin{claim}\label{11-2-16}
$m=1$, $n=0,1$, $a$ and $j$ are scalar symbols and $d\ge 2$; further, as \underline{either} $d\ge 3$ \underline{or} $d=2$ or (\ref{11-2-12}) holds we recover local remainder estimate $O(h_\eff^{1-d})$ under minimal regularity assumptions;
\end{claim}

\item\label{sect-11-2-1-v}
$m=1$, $d=1$, $n=0$; we recover local remainder estimate $O(h_\eff^{1-d})$ as $K=K(p)$ provided

\begin{claim}\label{11-2-17}
$m=1$, $d=1$, $n=0$ and for every $x\in X_\reg$
\begin{equation}
\sum_{\alpha :|\alpha |\le p}\gamma ^{|\alpha |}|D ^\alpha j|\ge
\epsilon_0\varrho_0;
\label{11-2-18}
\end{equation}
as $p=1$ we recover local remainder estimate $O(\log(h_\eff))$ under minimal regularity assumptions\footnote{\label{foot-11-12} As $p\ge 2$ we need to assume that $A$ and $J$ are scalar operators.};
\end{claim}

\item\label{sect-11-2-1-vi}
$m=1$, $d=1$, $n=1$; then
\begin{equation}
J= \frac{1}{2} (\langle D_x,j(x)\rangle +\langle j(x),D_x\rangle )+j'(x)
\label{11-2-19}
\end{equation}
and different variants of non-degeneracy condition are possible:
\begin{claim}\label{11-2-20}
$m=1$, $d=1$, $n=1$ and $|j(x)|\ge \epsilon_0\varrho_0\rho ^{-1}$ for every $x\in X_\reg$ ensures local remainder estimate $O(\log(h_\eff))$ under under minimal regularity assumptions;
\end{claim}
\vglue-10pt\noindent
while\vglue-10pt
\begin{claim}\label{11-2-21}
$m=1$, $d=1$, $n=1$ and (\ref{11-2-18}) ensures local remainder estimate $O(1)$ as $K=K(p)$\,\footref{foot-11-12}.
\end{claim}

\item\label{sect-11-2-1-vii}
If $m\ge 2$ then the first and the second order derivatives of
$a$ vanish at $\xi =0$ and we obtain the following cases ensuring local remainder estimate $O(h_\eff^{1-d})$ under smoothness assumptions:
\begin{claim}\label{11-2-22}
$m\ge 2$, $d\ge 2$, $n=0$ and for every $x\in X_\reg$ inequality
\begin{equation}
|j(x)|+\gamma |\nabla j(x)|\le \epsilon_0\varrho_0
\label{11-2-23}
\end{equation}
yields that $\Hess j(x)$ has two eigenvalues with absolute values
greater than $\epsilon_0\varrho_0\gamma ^{-2}$;
\end{claim}
\vglue-10pt
\begin{claim}\label{11-2-24}
$m\ge 2$, $d\ge 2$, $n=0$ and for every $x\in X_\reg$
(\ref{11-2-18}) holds with $p=1$ or $p=2$\,\footref{foot-11-12};
\end{claim}
\vglue-10pt
\begin{claim}\label{11-2-25}
$m\ge 2$, $n=1$ and for every $x\in X_\reg$ inequality
\begin{equation}
|j(x)|+\gamma |(Dj )(x)|\ge \epsilon_0\varrho_0\rho ^{-1}
\label{11-2-26}
\end{equation}
holds where here $J$ is defined by (\ref{11-2-19}), $j=j(x)$ is a vector field and $(Dj)$ is the matrix of its derivatives, $j'=j'(x)$.
\end{claim}
\item\label{sect-11-2-1-viii}
Finally, as $m\ge 2$ we can consider $n=2$ and arrive to
\begin{claim}\label{11-2-27}
$m\ge 2$, $d\ge 2$, $n=2$ and
\begin{equation}
\sum_{\alpha :|\alpha|=2}|j_\alpha|\ge \epsilon_0\varrho_0\rho ^{-2}
\label{11-2-28}
\end{equation}
for every $x\in X_\reg$ where $j_\alpha$ are the coefficients of the senior
symbol of $J$.
\end{claim}
\end{enumerate}

\begin{remark}\label{rem-11-2-1}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-2-1-i}
For $\vartheta>0$ we recover a local remainder estimate \newline $O(h_\eff^{1-d+\vartheta}\tau^\vartheta)$ under corresponding regularity assumptions.

\item\label{rem-11-2-1-ii}
Let both $A$ and $J$ be scalar operators. Then in the smooth case we do not need any non-degeneracy assumptions to recover a local remainder estimate
$O(h_\eff^{1-d+\vartheta}\tau^\vartheta)$ as $\vartheta>0$ and $O(h_\eff^{1-d-\delta})$ with arbitrarily small $\delta>0$ as $\vartheta=0$; ``smooth'' means ``with $K=K(d,\vartheta)$ or $K=K(d,\delta)$ respectively''.
\end{enumerate}
\end{remark}

\begin{remark}\label{rem-11-2-2}
To avoid $\N^\W =0$ we need to assume that
\begin{claim}\label{11-2-29}
$j(x,\xi )$ (the principal symbol of $J$) is not a non-positive definite matrix
(as long as we assume that $a(x,\xi)$ is a positive definite matrix).\end{claim}
\end{remark}

We leave to the the following

\begin{problem}\label{problem-11-2-3}
Investigate the opposite case when according to Chapter~\ref{sect-7} the local remainder estimate may be $O(h_\eff^{2-d})$ and $\N^\W\asymp h_\eff^{1-d}$.
\end{problem}

Let us discuss conditions associated with the boundary value problem. Recall that this condition for $1$-dimensional operator
$f= \tilde{a}-\tilde{\jmath}$ is of the form
\begin{multline}
\Re \blangle \ell f v,v\brangle_+
+\Re\blangle \ell \tilde{b}v,\upbeta v\brangle_0\ge
\epsilon_0\1v\1_+^2\\[2pt]
\forall v\in \sS'(\bR^+,\bH):f v=0\;\text{and\ \ } bv|_{x_1=0}=0
\label{11-2-30}
\end{multline}
where we use the notation of Chapter~\ref{sect-7} and make a rescaling; here
$f =f (z,D_1)$, $b=b(z,D_1)$ and $\upbeta=\upbeta (z,D_1)$ is defined by equality
\begin{multline}
\blangle f u,v\brangle_+ +\blangle \tilde{b}u,\upbeta v\brangle_0=
\blangle u,f v\brangle_+ +\blangle \upbeta u,\tilde{b}v\brangle_0\\
\forall u,v\in \sS (\bR^+,\bH)
\label{11-2-31}
\end{multline}
where $z=(x',\xi ')$.

Let us note that
\begin{claim}\label{11-2-32}
Condition (\ref{11-2-30}) survives substitution $D_1\mapsto \theta (z)D_1$ with
$\theta \asymp 1$.
\end{claim}
In fact, it is obvious for $\theta =\const$ and therefore we need check this statement only for $\theta $ equal to $1$ at the point in question. In this case additional term
\begin{equation}
(\ell\theta )(z)\times \Re\bigl(\blangle f'v,v\brangle_+
+\blangle \tilde{b}'v,\upbeta v\brangle_0\bigr)
\label{11-2-33}
\end{equation}
in the left-hand expression of (\ref{11-2-30}) appears where the prime means
derivative with respect to $\theta $. Let us introduce
$v_\theta (x_1)=v(\theta ^{-1}x_1)$; then $f_\theta v_\theta =0$ and $\tilde{b}_\theta v_\theta |_{x_1=0}=0$. Therefore treating $\theta $ as an independent variable, differentiating and taking $\theta =1$ we obtain that
\begin{equation}
f'v+f v'=0,\qquad \tilde{b}'v+\tilde{b}v'=0
\label{11-2-34}
\end{equation}
where the prime on $v$ means derivative on $\theta $ also and therefore
$v'=-x_1\partial_1v$. Then (\ref{11-2-34}), (\ref{11-2-31}) and the equalities
$f v=0$, $\tilde{b}v|_{x_1=0}=0$ obviously yield that the second factor in (\ref{11-2-30}) vanishes; (\ref{11-2-32}) has been proven.

Let us consider first $|\xi '|\ge \epsilon_0$ and let us introduce
$\ell=\langle \xi ',\partial_{x'}\rangle $, $\theta =|\xi '|$. Then
$1$-dimensional operators $\tilde{a}(x',\xi ',\theta D_1)$ and
$\tilde{\jmath} (x',\xi ',\theta D_1)$ are positive homogeneous of degrees $2m$ and $n$ on $\xi '$ respectively. Moreover, operators
$\tilde{b}_k(x',\xi ',\theta D_1)$ are positive homogeneous of degrees $m_k$ on $\xi '$ and $b_kv=0$. Therefore the Euler identity yields that the left-hand expression of (\ref{11-2-30}) is equal to
\begin{equation*}
2m\blangle \tilde{a}v,v\brangle_+-n\blangle \tilde{\jmath} v,v\brangle_+.
\end{equation*}
Since $(\tilde{a}-\tilde{\jmath} )v=0$ we obtain that this expression is equal to
\begin{equation*}
(2m-n)\blangle \tilde{a}v,v\brangle_+=
(2m-n)\blangle \tilde{\jmath} v,v\brangle_+.
\end{equation*}

Therefore we arrive to

\begin{proposition}\label{prop-11-2-4}
As $|\x'|\ge \epsilon_0$ condition \textup{(\ref{11-2-30})} is fulfilled provided either
\begin{gather}
\blangle \tilde{a}v,v\brangle_+\ge \epsilon_0\1v\1_+^2\qquad
\forall v\in \sS(\bR^+,\bH):\; \tilde{b}v=0\;\text{at\ \ }x_1=0
\label{11-2-35}
\intertext{or the same condition is fulfilled for $\tilde{\jmath} $:}
\blangle \tilde{\jmath}v,v\brangle_+\ge \epsilon_0\1v\1_+^2\qquad
\forall v\in \sS(\bR^+,\bH):\; \tilde{b}v=0\;\text{at\ \ }x_1=0
\label{11-2-36}
\end{gather}
\end{proposition}

If $A$ is a semi-bounded operator (under the boundary condition $Bv=0$) then the ellipticity of the boundary value problem $(A,B)$ yields that condition (\ref{11-2-35}) is fulfilled. \emph{In what follows when we consider non-semi-bounded operators $A$ we assume that $J=I$\/} and then condition (\ref{11-2-36}) is fulfilled automatically.

Let us consider the case $\xi '=0$. Let us prove that
\begin{claim}\label{11-2-37}
As $|\xi'|=0$ the kernel of the problem
\begin{equation}
f v=0,\qquad \tilde{b}v=0\quad \text{at\ \ }x_1=0,
\qquad\quad v\in \sS (\bR^+,\bH)
\label{11-2-38}
\end{equation}
is trivial.
\end{claim}
Then condition (\ref{11-2-30}) will be automatically fulfilled.

Let us note that if $\xi'=0$ then $\tilde{a}=a_0D_1 ^{2m}$,
$\tilde{\jmath} =j_0D_1 ^n$, $\tilde{b}_k=b_{0k}D_1^{m_k}$ where
$a_0$, $j_0$, $b_{0k}$ are matrices (depending on $z$). Let us replace $D_1$ by $\theta D_1$ and let us introduce $v_\theta (x_1)=v(\theta ^{-1}x_1)$ with an arbitrary parameter $\theta $. The above arguments yield the following equality
\begin{equation*}
\blangle f'v,v\brangle_+
+\blangle \tilde{b}'v,\upbeta v\brangle_0=0
\end{equation*}
for any solution of the problem (\ref{11-2-38}). Let us note that in our
case $\tilde{b}'v=0$ at $x_1=0$. Then equalities $f v=0$,
$f=\tilde{a}-\tilde{\jmath}$ and $f'=2m\tilde{a}-n\tilde{\jmath}$ obviously yield that
\begin{equation*}
\blangle \tilde{a}v,v\brangle_+=0,\qquad
\blangle \tilde{\jmath} v,v\brangle_+=0.
\end{equation*}
The first equality is impossible for $v\ne 0$ if $A$ is a semi-bounded elliptic operator and the second equality is impossible for $v\ne 0$ if $J=I$. So, (\ref{11-2-37}) and thus (\ref{11-2-30}) are established.

Thus we arrive to the following

\begin{proposition}\label{prop-11-2-5}
Let one of the following assumptions be fulfilled:

\begin{enumerate}[label=(\alph*), wide, labelindent=0pt]
\item\label{prop-11-2--5-a}
\underline{Either} $A$ and $J$ are matrix matrix operators satisfying one of the conditions \textup{(\ref{11-2-12})}--\textup{(\ref{11-2-15})} \underline{or} $A$ and $J$ are operators with scalar senior symbols satisfying condition \textup{(\ref{11-2-20})};

\item\label{prop-11-2--5-b}
 $B\bigl(x,\gamma (x)\bigr)\cap \partial X=\emptyset$ and $A$ and $J$ are operators with with scalar senior symbols satisfying one of the conditions
\textup{(\ref{11-2-16})}, \textup{(\ref{11-2-17})}, \textup{(\ref{11-2-21})}--\textup{(\ref{11-2-15})};

\item\label{prop-11-2--5-c}
 $d\ge 2$ and $A$ is the Schr\"{o}dinger operator with a Dirichlet or Neumann boundary condition\footnote{\label{foot-11-13} Or a Robin boundary condition with appropriate restrictions on lower order coefficients.} on $\partial X\cap B\bigl(x,\gamma (x)\bigr)$.
\end{enumerate}

Then the contribution of $\cB\bigl(x,\gamma (x), X\bigr)\subset X'_\reg$ to the principal part of the asymptotics for $\N^\W_{(\vartheta)}(\tau)$ is $O(h_\eff^{-d}\tau^\vartheta)$\,\footnote{\label{foot-11-14} Recall that under assumption \textup{(\ref{11-2-29})} it is $\asymp h_\eff^{-d}\tau^\vartheta$.} and its contribution to the remainder is
$O(h_\eff^{1-d+\vartheta }\tau^\vartheta)$ with
\begin{equation}
h_\eff = \bigl(\frac{\tau\varrho_0}{\varrho}\bigr)^{-\frac{1}{2m-n}}\rho^{-1}\gamma^{-1}
\label{11-2-39}
\end{equation}
and therefore the total contribution of $X'_\reg$ defined by \textup{(\ref{11-2-9})} to the remainder does not exceed
\begin{equation}
R_{1(\vartheta)}(\tau)=\tau ^{\frac{d-1-\vartheta}{2m-n}+\vartheta}
\int_{X'_\reg}
\bigl(\frac{\varrho_0}{\varrho}\bigr)^{\frac{d-1-\vartheta}{2m-n}}\rho^{d-1-\vartheta}\gamma^{-1-\vartheta}\,dx.
\label{11-2-40}
\end{equation}
\end{proposition}

\subsection{Weak singularity}
\label{sect-11-2-2}

Now consider the contribution of
\begin{equation}
X''_\reg =
X_\reg\setminus X'_\reg=\{ \rho\gamma \ge 1, \ \tau\varrho_0 \le C_0\varrho\};
\label{11-2-41}
\end{equation}
we estimate the contribution of $\cB\bigl(x,\gamma (x), X\bigr)\subset X''_\reg$ to both the main part and remainder estimate by
$O(h_\eff^{-d}\varrho ^\vartheta\varrho_0^{-\vartheta})$ with $h_\eff =\rho^{-1}\gamma^{-1}$ and the total contribution of $X''_\reg$ does not exceed
\begin{gather}
R_{2(\vartheta)}(\tau)=\int_{X''_\reg}
\rho^d \varrho^\vartheta \varrho_0^{-\vartheta}\,dx\label{11-2-42} \\
\intertext{provided}
\vartheta >0 \implies J=I\quad\text{i.e.\ \ }n=0,\ \varrho_0=1.
\label{11-2-43}
\end{gather}
As $A$ and $J$ are scalar operators we can use Remark~\ref{rem-11-2-1} and vastly improve the estimate of the contribution of $X''_\reg$ to the remainder.

As we use such crude estimate in $X''_\reg$ and hope to recover a reasonable result we will need to assume that singularity is weak.

Further, we need to estimate the contribution of $X_\sing$. If we can apply Rozenblioum estimate we arrive to the following

\begin{proposition}\label{prop-11-2-6}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{prop-11-2--6-i}
As $\vartheta=0$ the contribution of $X_\sing$ to asymptotics does not exceed
\begin{equation}
CR_0+CR'_0
\label{11-2-44}
\end{equation}
where $R_0$ is given by \textup{(\ref{11-1-10})} with exponents satisfying \textup{(\ref{11-1-11})} and \textup{(\ref{11-1-12})} and
\begin{multline}
R'_0=
\tau ^{\frac{d}{2m-n}}\Bigl(\int_{X_\sing} \varrho ^{-p'}\rho ^{2mp'} \,dx\Bigr)^{\frac{d}{(2m-n)p'}}
\times \\
\Bigl(\int_{X_\sing}\varrho_0^{q'}\rho ^{-nq'}\,dx\Bigr)^{\frac{d}{{(2m-n)q}'}} \times
\bigl(\mes(X_\sing)\bigr) ^{1-{\frac{d}{2mq'}}({\frac{1}{p'}}+ {\frac{1}{q'}})}
\label{11-2-45}
\end{multline}
with exponents $p'$ and $q'$ satisfying conditions $\textup{(\ref{11-1-11})}^\#$ and $\textup{(\ref{11-1-12})}^\#$ where the $^\#$ means that we replace $2m$, $p$ and $q$ by $2m-n$, $p'$ and $q'$ respectively.

We assume that a Dirichlet boundary condition is given on
$\partial X\cap \bar{X}_\sing$. Otherwise we should assume that a cone condition is fulfilled (with constant angle and height of the cone),
$\varrho \asymp \rho ^{2m}$ and $\mes (X_\sing)< \infty $.

\item\label{prop-11-2--6-ii}
As $\vartheta>0$ and $J=I$ the contribution of the zone $X_\sing$ to the asymptotics does not exceed
\begin{equation}
CR_{0(\vartheta)} +CR'_{0(\vartheta)}
\label{11-2-46}
\end{equation}
where
\begin{multline}
R_{0(\vartheta)} =\int_0 ^\infty t^{\vartheta -1}
\Bigl(\int_{X_\sing}(\varrho -t)_+^q\,dx\Bigr)^{\frac{d}{2mq}}dt\times \\
\Bigl(\int_{X_sing}\varrho ^{-p}\rho ^{2mp}\,dx\Bigr)^{\frac{d}{2mp}}
\times \bigl(\mes(X_\sing)\bigr)^{1-\frac{d}{2m} ( \frac{1}{p} + \frac{1}{q} )},
\label{11-2-47}
\end{multline}
\begin{equation}
R'_{0(\vartheta)} =
\tau ^{\vartheta +{\frac{d}{2m}}}\Bigl(\int_{X_\sing}\varrho ^{-p}\rho ^{2mp}\,dx\Bigr)^{\frac{d}{2mp}}\times
\bigl(\mes(X_\sing)\bigr)^{1-\frac{d}{2mp}}
\label{11-2-48}
\end{equation}
and exponents $p$ and $q$ satisfy conditions \textup{(\ref{11-1-11})}--\textup{(\ref{11-1-12})}.
\end{enumerate}
\end{proposition}

\subsection{Main theorems}
\label{sect-11-2-3}

Let us start from the standard asymptotics. Then we improve the remainder estimate under conditions on the Hamiltonian trajectories in $X'_\reg$. Resulting from this analysis we obtain the following statements:

\begin{theorem}\label{thm-11-2-7}
Let $X=\cX_\reg\cup \cX_\sing$, $\mes(\cX_\sing)=0$. Let us assume that in $\cX_\reg$ all the conditions \textup{(\ref{9-1-5})}--\textup{(\ref{9-1-13})}, \textup{(\ref{9-1-15})} (excluding restriction $\rho \gamma \ge 1$) are fulfilled.

Further, let us assume that $\varrho^{-1}\rho^{2m}a^0(x,\xi)$ is uniformly classically elliptic and the corresponding boundary value problem for it is also uniformly classically elliptic at the boundary points.

Furthermore, let us assume that in each ball
$\cB(x,\gamma (x),X)\subset\cX_\reg$ one of the assumptions \ref{prop-11-2--5-a}, \ref{prop-11-2--5-b} or \ref{prop-11-2--5-c} of Proposition \ref{prop-11-2-5} is fulfilled. Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-2--7-i}
The following lower estimate holds:
\begin{equation}
\N(0,\tau) \ge \N^\W (0,\tau) - CR_{1(0)}(\tau)
\label{11-2-49}
\end{equation}
where $\N^\W (0,\tau)$ is defined by cut Weyl formula (with integration over $X'_\reg$):
\begin{gather}
\N^\W (0,\tau )=\varkappa_0(\tau)\tau ^{\frac{d}{2m-n}},\label{11-2-50}\\
\varkappa_0(\tau) =
(2\pi )^{-d}\int_{X'_\reg(\tau)} \boldsymbol{n}(x,\xi ;0,1)\,dxd\xi ,
\label{11-2-51}
\end{gather}
$\boldsymbol{n}(x,\xi ;0,1 )$ is the eigenvalue counting function for the symbol $j^{-1}(x,\xi )a(x,\xi )$ on the interval $(0,1)$, $R_{1(0)}(\tau)$ is defined by \textup{(\ref{11-2-40})} with $\vartheta=0$; $X'_\reg(\tau)$ is defined by \textup{(\ref{11-2-10})}.

\item\label{thm-11-2--7-ii}
Further, let us assume that in
\begin{equation}
X_\sing(\tau)=X\setminus \bigl(X'_\reg(\tau) \cup X''_\reg(\tau)\bigr)
\label{11-2-52}
\end{equation}
we can apply Rozenblioum estimate. Then the upper estimate holds
\begin{equation}
\N (0,\tau )\le \N^\W (0,\tau)+
CR_{1(0)}(\tau) + CR_{2(0)}(\tau) + CR_0(\tau) + CR'_{0}(\tau)
\label{11-2-53}
\end{equation}
where $R_{2(0)}(\tau)$, $R_0(\tau)$, $R'_0(\tau)$ are defined by
\textup{(\ref{11-2-42})}, \textup{(\ref{11-1-10})}, \textup{(\ref{11-2-45})} respectively with $X''_\reg(\tau)$ and $X_\sing(\tau)$ defined by \textup{(\ref{11-2-42})} and \textup{(\ref{11-2-52})}.
\end{enumerate}
\end{theorem}

Similarly, as $\vartheta>0$ we arrive to

\begin{theorem}\label{thm-11-2-8}
Let assumptions of Theorem~\ref{thm-11-2-7} be fulfilled. Moreover, let us assume that $J=I$ and $A$ is semi-bounded from below. Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-2--8-i}
The following lower estimate holds:
\begin{equation}
\N^-_{(\vartheta)} (\tau) \ge \N^\W_{(\vartheta)} (\tau) - CR_{1(\vartheta)}(\tau)
\label{11-2-54}
\end{equation}
where $\N^\W_{(\vartheta)} (\tau)$ is defined by cut Weyl formula (with integration over $X'_\reg$), $R_{1(\vartheta)}(\tau)$ is defined by \textup{(\ref{11-2-40})}.

item\label{thm-11-2--8-ii}
Further, let us assume that in $X_\sing(\tau)$ defined by \textup{(\ref{11-2-52})} we can apply Rozenblioum estimate. Then the upper estimate holds
\begin{multline}
\N^-_{(\vartheta)} (\tau )\ge \N^\W_{(\vartheta)} (\tau)+\\
CR_{1(\vartheta)}(\tau) + CR_{2(\vartheta)}(\tau) + CR_{0(\vartheta)}(\tau) + CR'_{0(\vartheta)}(\tau)
\label{11-2-55}
\end{multline}
where $R_{2(\vartheta)}(\tau)$, $R_{0(\vartheta)}(\tau)$, $R'_{0(\vartheta)}(\tau)$ are defined by \textup{(\ref{11-2-42})}, \textup{(\ref{11-2-46})}, \textup{(\ref{11-2-45})} respectively with $X''_\reg(\tau)$ defined by \textup{(\ref{11-2-42})}.
\end{enumerate}
\end{theorem}

Obviously, if $X$ is a compact domain with the smooth boundary and $J(x)=I$ we conclude that
\begin{gather}
\N^-_{(\vartheta)}(\tau)= \N^\W_{(\vartheta)}(\tau) + O\bigl(\tau^{\frac{d-1-\vartheta}{2m} + \vartheta}\bigr)
\qquad\text{as\ \ }\tau\to +\infty
\label{11-2-56}\\
\shortintertext{with}
\N^\W_{(\vartheta)}(\tau)\asymp \tau^{\frac{d}{2m} + \vartheta}.
\label{11-2-57}
\end{gather}

Our goal now is to consider the \emph{weakly singular\/} case when this conclusion holds. Since $X'_\reg$ extends to $\cX_\reg $ as $\tau\to +\infty$, we need to assume that
\begin{gather}
\bigl(\frac{\varrho_0}{\varrho}\rho^{2m-n}\bigr)^{\frac{d}{2m-n}}
\in \sL^1(X)\label{11-2-58}\\
\shortintertext{and}
\bigl(\frac{\varrho_0}{\varrho}\rho^{2m-n}\bigr)^{\frac{d-1-\vartheta}{2m-n}}
\gamma^{-1-\vartheta}\in \sL^1(X).
\label{11-2-59}
\end{gather}

\begin{corollary}\label{cor-11-2-9}
Assume that conditions of Theorem~\ref{thm-11-2-7} as $\vartheta=0$ or Theorem~\ref{thm-11-2-8} as $\vartheta>0$ are fulfilled. Further, let
conditions \textup{(\ref{11-2-58})}--\textup{(\ref{11-2-59})} be fulfilled. Then
\begin{gather}
R_{2(\vartheta)}(\tau)=o\bigl(\tau^{\frac{d-1-\vartheta}{2m-n}+\vartheta}\bigr)
\qquad\text{as\ \ }\tau\to +\infty
\label{11-2-60}\\
\intertext{and assuming that}
R_{0(\vartheta)}(\tau)+ R'_{0(\vartheta)}(\tau)
=O\bigl(\tau^{\frac{d-1-\vartheta}{2m-n}+\vartheta}\bigr)
\qquad\text{as\ \ }\tau\to +\infty
\label{11-2-61}
\end{gather}
we conclude that \textup{(\ref{11-2-56})}--\textup{(\ref{11-2-57})} hold.
\end{corollary}

\begin{remark}\label{rem-11-2-10}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-2--10-i}
One can easily see that extending integration in $\N^\W (\tau)$ from $X_\reg$ to $X$ causes an error not exceeding (\ref{11-2-44}). So we can replace cut Weyl expression by the full Weyl expression.

\item\label{rem-11-2--10-ii}
Also skipping lower degree terms in $\N^\W$ leads to an error not exceeding $CR_{1(0)}(\tau)$; this leads to (\ref{11-2-50})--(\ref{11-2-51}).

\item\label{rem-11-2--10-iii}
Combining Statements \ref{rem-11-2--10-i} and \ref{rem-11-2--10-ii} we arrive to (\ref{11-2-51}) with integration over $X$ (then $\varkappa_0$ does not depend on $\tau$).

\item\label{rem-11-2--10-iv}
Some of these conclusions remain true for $\vartheta>0$, at least with some modifications: for example, (\ref{11-2-50})--(\ref{11-2-51}) becomes
\begin{equation}
\N^\W_{(\vartheta)} (0,\tau) =\sum_{0\le n<1+ \vartheta} \varkappa_n (\tau) \tau^{\frac{d-n}{2m-n}+\vartheta}
\label{11-2-62}
\end{equation}
but extension of integration in $\varkappa_n(\tau)$ terms is justified only under assumption (\ref{11-2-59}) with $\vartheta$ replaced by $n$ (and some other assumptions may be required as well).


\item\label{rem-11-2--10-v}
Theorems~\ref{thm-11-2-7} and~\ref{thm-11-2-8} and Corollary~\ref{cor-11-2-9} remain true for compact $\sC^K$ manifolds.
\end{enumerate}
\end{remark}

\begin{remark}\label{rem-11-2-11}
In the case $\varrho =\rho ^{2m}$ and $2m-n<d$ one can set $q'=\frac{d}{2m-n}$ and then (\ref{11-2-59}) yields (\ref{11-2-61}).
\end{remark}

We can slightly improve the results of above theorems under assumptions to Hamiltonian trajectories:

\begin{theorem}\label{thm-11-2-12}
Assume that conditions of Theorem~\ref{thm-11-2-7} as $\vartheta=0$ or Theorem~\ref{thm-11-2-8} as $\vartheta>0$ are fulfilled.

Further, let us assume that non-periodicity condition \textup{(\ref{11-1-55})}--\textup{(\ref{11-1-56})} and improved smoothness and non-degeneracy conditions of Remark~\ref{rem-11-1-8} hold for symbol $a^0(x,\xi)-j^0(x,\xi)$ on the energy level $0$. Then sharp versions of asymptotics \textup{(\ref{11-2-54})}, \textup{(\ref{11-2-55})} hold where ``sharp version'' means that
$R_{1(\vartheta)}(\tau)$ is replaced by
\begin{equation}
R'_{1(\vartheta)}(\tau)=
o(1)R_{1(\vartheta)}(\tau)+ R_{1(\vartheta-\delta)}(\tau)
\label{11-2-63}
\end{equation}
where $\delta>0$ is sufficiently small exponent and formula \textup{(\ref{11-1-39})} defining $R_{1(\vartheta)}$ is extended to $\vartheta<0$ if needed; also in $\N^\W_{(\vartheta)}$ one extra term should be included if needed.
\end{theorem}

Sharper asymptotics under more restrictive conditions on the Hamiltonian flow will be treated later.

\subsection{Examples}
\label{sect-11-2-4}

Consider some examples. Let us start with examples in which $J=I$,
$\varrho =\rho =1$. Then conditions (\ref{11-2-58}), (\ref{11-2-59}) mean respectively that
\begin{gather}
1\in \sL^1(X) \qquad\text{i.e.\ \ }\mes (X)<\infty,\label{11-2-64}\\[2pt]
\gamma ^{-1-\vartheta }\in \sL^1(X)\label{11-2-65}.
\end{gather}
\emph{In the first examples the coefficients of $A$ are regular and $\gamma $ is
completely defined by the geometry of the domain $X$}.

\begin{example}[Quasi-polygonal and quasi-polyhedral domains]\label{ex-11-2-13}%
\index{quasi-polygonal domain!large eigenvalue asymptotics of}%
\index{domain!quasi-polygonal!large eigenvalue asymptotics of}%
\index{large eigenvalue asymptotics!quasi-polygonal domain}%
\index{asymptotics!large eigenvalue!quasi-polygonal domain}
\index{quasi-polyhedral domain!large eigenvalue asymptotics of}%
\index{domain!quasi-polyhedral!large eigenvalue asymptotics of}%
\index{large eigenvalue asymptotics!quasi-polyhedral domain}%
\index{asymptotics!large eigenvalue!quasi-polyhedral domain}
Let $X$ be a bounded domain with $\partial X$ contained in the union of a finite number of $\sC^K$ hypersurfaces\footnote{\label{foot-11-15} Actually we need only regularity required to produce local remainder estimate $O(h_\eff^{1-d+\vartheta})$ or $o(h_\eff^{1-d+\vartheta})$ in case we are interested in the sharp asymptotics.} $\tilde{S}_l$ (with $l=1,\ldots ,L$).

Let $S_l=\tilde{S}_l\cap \partial X$ and $\updelta S_l$ be the relative boundary of $S_l$ in $\tilde{S}_l$. Introduce the \emph{singular set\/} of $\partial X$
\begin{equation}
{\cK}=\bigcup_{l\ne k}(S_l\cap S_k) \cup \bigcup_l\updelta S_k
\label{11-2-66}
\end{equation}
\vglue-5pt
Obviously, we can take
\begin{gather}
\gamma (x)\asymp\min \Bigl(\min_{l\ne k}\gamma_{lk}(x),\dist (x,{\cK})\Bigr),\label{11-2-67}\\
\shortintertext{with}
\gamma_{lk}(x)=\max \bigl(\gamma_l(x),\gamma_k(x)\bigr)
\label{11-2-68}
\end{gather}
where $\gamma_l(x)=\dist (x,S_l)$.

Then condition (\ref{11-2-65}) needs to be verified for $\gamma_{lk}$ for all $l\ne k$ and for $\gamma '(x)=\dist (x,{\cK})$ separately.

First of all,
\begin{claim}\label{11-2-69}
If the hypersurfaces $\tilde{S}_l$ and $\tilde{S}_k$ are transversal at
$S_k\cap S_l$ then condition (\ref{11-2-65}) is fulfilled for
$\gamma =\gamma_{kl}$ and $\vartheta <\vartheta ^*(=1)$.
\end{claim}
Moreover,
\begin{claim}\label{11-2-70}
If ${\cK}$ is contained in the union of a finite number of $\sC^K$ manifolds of codimension 2 then condition (\ref{11-2-65}) is fulfilled for $\gamma =\gamma '$ for $\vartheta <\vartheta ^*=1$ as well.
\end{claim}
One can see easily that the above assumptions yield the cone condition. Therefore


\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{sect-11-2-4-i}
For appropriate boundary conditions\footnote{\label{foot-11-16} Such as
Dirichlet, Neumann and Robin boundary conditions, or boundary conditions which are smooth, elliptic, regular (see condition (\ref{7-1-14})) on
$S_l\setminus {\cK}$ and such that $A$ is self-adjoint and
$(Au,u)\ge \epsilon_0\|u\|_m^2-c\|u\|_0^2$.} asymptotics (\ref{11-2-56}) holds for $\vartheta <\vartheta ^*$.

Moreover, under standard non-periodicity condition (\ref{11-1-55})--(\ref{11-1-56}) to the Hamiltonian flow of the symbol $a^0(x,\xi )$ on the energy level  $1$ asymptotics
\begin{equation}
\N^-_{(\vartheta)}(\tau)= \N^\W_{(\vartheta)}(\tau) + o\bigl(\tau^{\frac{d-1-\vartheta}{2m} + \vartheta}\bigr)
\qquad\text{as\ \ }\tau\to +\infty
\tag*{$\textup{(\ref*{11-2-56})}^*$}\label{11-2-56-*}
\end{equation}
holds.

\item\label{sect-11-2-4-ii}
Further, our analysis yields that for $\vartheta =\vartheta ^*$ asymptotics
\begin{gather}
\N^-_{(\vartheta)} (\tau )=\N^\W_{(\vartheta)} (\tau )+
O\bigl(\tau ^{{\frac{1}{2m}}(d-\vartheta -1)+\vartheta }\log \tau
\bigr)
\label{11-2-71}\\
\intertext{holds as $\tau \to+\infty $ and for $\vartheta >\vartheta ^*$
asymptotics}
\quad \,\N^-_{(\vartheta)} (\tau )=\N^\W_{(\vartheta)} (\tau )+
O\bigl(\tau ^{{\frac{1}{2m}}(d-\vartheta^* -1)+\vartheta}\bigr)
\label{11-2-72}
\end{gather}
holds as $\tau \to+\infty $.
\end{enumerate}

Later we will show that under appropriate assumptions sharper asymptotics than
(\ref{11-2-71})--(\ref{11-2-72}) holds and in the latter case some extra non-Weyl term(s) associated with the singularities at $\cK$ come into play.
\end{example}
\begin{figure}[h]
\centering
\subfloat[]{\label{fig-11-1-a}%
\begin{tikzpicture}[scale=.9]
\draw[ultra thick] (0,0) ..controls (1,0.5).. (2,2)..controls (3,2.5).. (4,2)--(5,1)--(5.5,2.5)..controls (7,0).. (6,-3)--(3,0)--(0,0);
\draw[ultra thick] (2,2) ..controls (2.5,1) .. (3,1);
\draw[ultra thick] (4,0) ..controls (5.5,0.5) .. (6,0);
\draw[ultra thick] (5,0.3) -- (5,-1);
\end{tikzpicture}}
%\qquad
\subfloat[]{\label{fig-11-1-b}%
\begin{tikzpicture}[scale=.9]
\draw[ultra thick] (0,0) ..controls (-2,0) and (-4,0.2) .. (-2,2) .. controls (1, 3).. (4,2) ..controls (3,0).. (2,0);
\draw[ultra thick] (0,0) ..controls (-2,0) and (-4,-0.2) .. (-2,-2) .. controls (1,-1).. (4,-2) ..controls (3,0).. (2,0)--(1,0);
\end{tikzpicture}}
\caption{\label{fig-11-1} Conclusions of Example~\ref{ex-11-2-13} holds despite on \protect\subref{fig-11-1-b} transversally condition violated}
\end{figure}

\begin{example}[Spikes and conjugations]\label{ex-11-2-14}
Let us drop transversally condition (\ref{11-2-69}) thus allowing \emph{spikes\/}. Consider first spikes directed inward as on Figure \ref{fig-11-1-b}.


\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-2--14-i}
Assume first that locally only two surfaces $S_k$ and $S_l$ are involved and in appropriate coordinates
\begin{equation}
S_j = \{x_d = f_j(x'), \ x'\in X'\},\qquad (f_j-f_i)|_{\partial X'}=0
\label{11-2-73}
\end{equation}
where $X'\subset \bR^{d-1}$, $x'=(x_1,\dots, x_{d-1}$,
$|\nabla f_j|\le \epsilon$. Then assuming that locally $\complement X$ is between surfaces
\begin{multline}
\complement X = \{f_k(x')\le x_d \le f_l(x'), \ x'\in X'\}\cup\\
\{f_l(x')\le x_d \le f_k(x'), \ x'\in X'\}
\label{11-2-74}
\end{multline}
we conclude that $\gamma (x)\asymp \gamma (x')=\dist (x,\cK)$ with
\begin{equation}
\cK= \{x: x'=\cK' , x_d =f_j(x')\},\quad \cK'=\partial X' \cup \{x',f_j(x')=f_k(x')\}.
\label{11-2-75}
\end{equation}
Then condition (\ref{11-2-65}) is fulfilled for $\vartheta <\vartheta ^*=1$ provided condition (\ref{11-2-70}) is fulfilled. Moreover, cone condition is fulfilled as well and then all conclusions of Example~\ref{ex-11-2-13} remain valid.

\item\label{ex-11-2--14-ii}
Further, the same conclusions obviously remain true as locally there is \emph{conjugation\/} instead of spike
\begin{equation}
S_j = \{x_d = f_j(x'), \ x'\in X'_j\},\qquad (f_j-f_k)|_{\partial X'_j\cap \partial X'_k}=0 \quad\text{for\ \ } k\ne j
\label{11-2-76}
\end{equation}
as $X'_j$ form locally a partition of the vicinity of $0$ in $\bR^{d-1}$.

\item\label{ex-11-2--14-iii}
Furthermore, we can consider inward spike or conjugation and add extra surfaces to $\partial X$ assuming that each new surface is either transversal to existing surfaces or further limits $\complement X$. For example, we can consider multidimensional inward spike:
\begin{equation}
\complement X= \{x_1>0, x'\in f(x_1)X'\}
\label{11-2-77}
\end{equation}
with $f >0, f'_j>0$ as $x_1>0$, $f(0)=f'(0)=0$ and $X'$ bounded convex quasipolygon of Example~\ref{ex-11-2-14}.
\end{enumerate}
\end{example}

\begin{figure}[h]
\centering
\begin{tikzpicture}[scale=.9]
\draw[ultra thick] (0,0) ..controls (-2,0) and (-4,0.2) .. (-5,2);
\draw[ultra thick] (0,0) ..controls (-2,0) and (-4,-0.2) .. (-5,-2);
\draw[ultra thick] (-5,2) ..controls (-6,0) .. (-5,-2);
\end{tikzpicture}
\caption{\label{fig-11-2} Outward spike}
\end{figure}

\begin{example}[Spikes. II]\label{ex-11-2-15} Outward spike are completely different matter. Assume first that locally only two surfaces $S_k$ and $S_l$ are involved and in appropriate coordinates (\ref{11-2-73}) and (\ref{11-2-74}) are fulfilled with $\complement X$ replaced by $X$
\begin{multline}
X = \{f_k(x')< x_d < f_l(x'), \ x'\in X'\}\cup\\
\{f_l(x')< x_d < f_k(x'), \ x'\in X'\}
\label{11-2-78}
\end{multline}
as on Figure~\ref{fig-11-2}. Obviously, without any loss of the generality one can assume that $f_k=f$, $f_l=-f$ and then
$\gamma_{kl} \asymp |f|$. Therefore condition (\ref{11-2-65}) becomes
\begin{equation}
|f|^{-\vartheta}\in \sL^1 (X')
\label{11-2-79}
\end{equation}
which obviously is fulfilled for $\vartheta=0$, violated for $\vartheta \ge 1$ and may be fulfilled or not for any particular $\vartheta\in (0,1)$; f.e. as $f=f(x_1)\asymp x_1^r$ for $x_1>0$ ($r>1$) this condition holds for $\vartheta <\vartheta^*=r^{-1}$ while for $f=O(x_1^\infty)$ at $0$ this condition holds only for $\vartheta=0$.

So, if (\ref{11-2-79}) is fulfilled then asymptotics (\ref{11-2-56}) holds for appropriate boundary conditions. Moreover, under the standard non-periodicity condition (\ref{11-1-55})--(\ref{11-1-56}) to the Hamiltonian flow of the symbol $a^0(x,\xi )$ on the energy level  $1$ asymptotics \ref{11-2-56-*} holds.
\end{example}

\begin{problem}\label{problem-11-2-16}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-2--16-i}
Derive asymptotics similar to (\ref{11-1-69}) or (\ref{11-1-70}) for particular functions $f$ as condition (\ref{11-2-79}) is violated.

\item\label{problem-11-2--16-ii}
Consider multidimensional outward spikes like one similar to (\ref{11-2-77}):
\begin{equation}
X= \{x_1>0, x'\in f(x_1)X'\}
\label{11-2-80}
\end{equation}
with $f >0, f'_j>0$ as $x_1>0$, $f(0)=f'(0)=0$ and $X'$ bounded convex quasipolygon of Example~\ref{ex-11-2-14}.


\item\label{problem-11-2--16-iii}
Consider the mixture of inward-outward spikes like (\ref{11-2-80}) but without any convexity assumptions.
\end{enumerate}
\end{problem}

\begin{remark}\label{rem-11-2-17}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-2--17-i}
n the case of ``outward spike'' the cone condition now is not ensured, so ``appropriate boundary conditions'' in \ref{problem-11-2-16}\ref{problem-11-2--16-i}, \ref{problem-11-2--16-ii} includes cone condition. In particular cone condition is fulfilled if at least on one side of the spike we have a Dirichlet boundary condition. There is not much known about more general conditions. Still for $2$-dimensional Laplace operator with Neumann boundary condition Yu.~Netrusov and Yu.~Safarov~\cite{netrusov:safarov, netrusov:safarov:2} in pretty special case derived variational estimate which allows to allow Neumann boundary condition on the whole boundary.

\item\label{rem-11-2--17-ii}
 Later in Section~\ref{sect-12-6} we will derive spectral asymptotics for multidimensional Neumann Laplacian and those methods could be applied in some of the examples discussed here to estimate the contribution of zone $\{x: \gamma(x)\le \tau^{-1/2}\}$ to the asymptotics thus extending corresponding results (see Subsection~\ref{sect-12-6-8}). However there will be also plenty of examples when conclusions valid for Dirichlet Laplacian are wrong for Neumann Laplacian.
\end{enumerate}
\end{remark}

In the series of examples below $\gamma (x)\asymp \dist (x,{\cK})$ where ${\cK}$ is the union of a finite number of $\sC^K$ manifolds of codimension
$\delta \ge 2$. Namely, we consider domains with conical singularities of the boundary, domains the boundaries of which contain components of codimension $\delta\in [2,4m-1]$\,\footnote{\label{foot-11-17} For operators of order $2m$ a boundary operator of degree less than $2m-\frac{1}{2}\delta$ can be considered on a $\delta $-codimensional submanifold.}. Then under appropriate assumptions critical exponent is $\vartheta ^*=\delta -1$.

\begin{example}[Scheme]\label{ex-11-2-18}
Let $X'$ be a domain in $\bR^{d'}$. Assume that

\begin{claim}\label{11-2-81}
$X'$ satisfies condition (\ref{9-1-15}) with $\gamma$ replaced by
$\gamma '=\gamma '(x')$ such that $\gamma '\le c$ and
${\gamma'}^{-1-\vartheta } \in \sL^1(X')$
\end{claim}
Let
$X=\{x=(x',x''),x''\in\bR^{d''},x'\in f(x'')X'\}$\,\footnote{\label{foot-11-18} For $d''=1$ one can take only one semiaxis, i.e., replace $\bR$ by $\bR^\pm$.}
where the function $f$ satisfies condition
\begin{equation}
|D^\alpha f|\le cf^{1-|\alpha |}\qquad \forall \alpha: |\alpha |\le K.
\label{11-2-82}
\end{equation}
Then for the domain $X$ the function
\begin{equation}
\gamma(x)=\epsilon\gamma'(x'f^{-1}(x''))f(x'')
\label{11-2-83}
\end{equation}
is admissible and in this case condition (\ref{11-2-65}) is equivalent to
\begin{equation}
f^{d'-\vartheta -1}\in \sL^1;
\label{11-2-84}
\end{equation}
in particular, this condition as $\vartheta=0$ is equivalent to the condition
\begin{claim}\label{11-2-85}
the $(d-1)$-dimensional measure of $\partial X$ is finite.
\end{claim}
\end{example}

\begin{example}[Cusps]\label{ex-11-2-19}%
\index{cusp!large eigenvalue asymptotics of}%
\index{large eigenvalue asymptotics!cusp}%
\index{asymptotics!large eigenvalue!cusp}%
This scheme described in Example~\ref{ex-11-2-18} includes cusps (exits to infinity): if $f\asymp |x''| ^\nu $ with $\nu <0$ for $|x''|\ge 1$ then the following cases are possible:

\begin{enumerate}[label=(\alph*), wide, labelindent=0pt]
\item\label{ex-11-2-19-a}
Let $\vartheta<\vartheta^*$ with
\begin{equation}
\vartheta^*=d'-1-d'' \nu^{-1} \iff (d'-1-\vartheta )\nu +d''=0.
\label{11-2-86}
\end{equation}
Then asymptotics (\ref{11-2-56}) holds.

Moreover, under standard non-periodicity condition (\ref{11-1-55})--(\ref{11-1-56}) to the Hamiltonian flow of the symbol $a^0(x,\xi )$ on the energy level  $1$ asymptotics \ref{11-2-56-*} holds.

\item\label{ex-11-2-19-b}
For $\vartheta=\vartheta^*$ asymptotics with the remainder estimate $O\bigl(\tau^{\frac{1}{2m}(d-1-\vartheta)+\vartheta}\log\tau\bigr)$
holds.

\item\label{ex-11-2-19-c}
For $\vartheta>\vartheta^*$, $d'\nu +d''<0$, asymptotics with
the remainder estimate $O\bigl(\tau^{\frac{1}{2m}(d-1-\vartheta^*)+\vartheta}\bigr)$
holds.

Moreover, if $\vartheta ^*\in\bZ^+$ then the last term of these asymptotics is of the form $\varkappa_{\vartheta,\vartheta^*+1}(\tau)
\tau^{\frac{1}{2m}(d-1-\vartheta^*)+\vartheta}$
with $\varkappa_{\vartheta ,\vartheta ^*+1}(\tau )= O(\log \tau )$ while all other terms in this case and all terms in the other cases are of the form
$\varkappa_{\vartheta ,n}\tau ^{{\frac{1}{2m}}(d-n)+\vartheta }$.

\item\label{ex-11-2-19-d}
If $d'\nu +d''=0$ then the previous statement remains true with
only the term $\varkappa_{\vartheta ,0}(\tau )\tau ^{{\frac{d}{2m}}+\vartheta }$ in the principal part with $\varkappa_{\vartheta ,0}(\tau )\asymp\log\tau $.
\end{enumerate}
\end{example}

\begin{figure}[h]
\centering
\subfloat[$d'=d''=1$]{\label{fig-11-3-a}%
\begin{tikzpicture}
\begin{scope}
\clip (-6,-2) rectangle (-2,2);
\draw[ultra thick] (-5,-2) .. controls (-4,-0.2) and (-2,0) ..(0,0) ..controls (-2,0) and (-4,0.2) .. (-5,2);
\clip (-5,-2) .. controls (-4,-0.2) and (-2,0) ..(0,0) ..controls (-2,0) and (-4,0.2) .. (-5,2);
\end{scope}
\end{tikzpicture}}
\qquad
\subfloat[$d'=2$, $d''=1$] {\label{fig-11-3-b}%
\begin{tikzpicture}
\begin{scope}
\clip (-6,-2) rectangle (-2,2);
\draw[ultra thick] (-5,-2) .. controls (-4,-0.2) and (-2,0) ..(0,0) ..controls (-2,0) and (-4,0.2) .. (-5,2);
\clip (-5,-2) .. controls (-4,-0.2) and (-2,0) ..(0,0) ..controls (-2,0) and (-4,0.2) .. (-5,2);
\draw[thick, dashed](-5,0) ellipse (15pt and 56pt);
\end{scope}
\clip (-6,-2) rectangle (-5,2);
\draw[thick](-5,0) ellipse (15pt and 56pt);
\end{tikzpicture}}
\quad
\subfloat[$d'=1$, $d''=2$] {\label{fig-11-3-c}%
\begin{tikzpicture}
\begin{scope}
\draw[thick](0,0.2) ellipse (145pt and 10pt);
\filldraw[ultra thick,fill=white]plot function {8/(x*x+4)};
\draw[thick,dashed](0,0.2) ellipse (145pt and 10pt);
\end{scope}
\end{tikzpicture}}
\caption{\label{fig-11-3} Cusps; in \protect\subref{fig-11-3-c} $X$ bounded by a drawn ``infinitely wide hat'' and horizontal plane}
\end{figure}

\begin{remark}\label{rem-11-2-20}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-2--20-i}
As $d''\ge 2$ we can consider more general cusp bases than $X''=\bR^{d''}$, most notably we can consider smooth consider a cone $X''\subset \bR^{d''}$ with a smooth boundary; rounding near $\partial X''$ here is obvious.

\item\label{rem-11-2--20-ii}
 We treat Example~\ref{ex-11-2-19} in Section~\ref{sect-12-1} again and obtain non-Weyl asymptotics with a more precise remainder estimate in cases \ref{ex-11-2-19-b}--\ref{ex-11-2-19-d} and and also in the case
 $d'\nu +d''>0$. We will consider also a generalization mention above.

\item\label{rem-11-2--20-iii}
In Example~\ref{ex-11-2-19} we need to assume that a Dirichlet boundary condition is given on a significant part of $\partial X$ so the cone condition if fulfilled. For example, we can assume that the Dirichlet boundary condition is given as $x'\in Y_\D\subset \partial X'$ and the following infinite cone condition is fulfilled:
\begin{claim}\label{11-2-87}
there exist an infinite cone $\Gamma \subset \bR^{d'}$ with a vertex at $0$ such that for each $x'\in X'$ connected component of $(x'+\Gamma)\cap X'$ is disjoint from $\partial X'\setminus Y_\D$.
\end{claim}

\item\label{rem-11-2--20-iv}
 Without the assumption of \ref{rem-11-2--20-iii} (f.e. for Neumann  Laplacian in domain with cusps we need to assume that the cusp is very thin: $|\log f |\asymp |x''|^\kappa$ with $\kappa>0$. Otherwise massive essential spectrum appears. We treat the Neumann Laplacian in domain with ``piggy-tail'' cusps in Section~\ref{sect-12-6} and derive possibly non-Weyl asymptotics.
\end{enumerate}
\end{remark}

\begin{figure}[h]%[9]{l}[0pt]{6truecm}
\centering
\begin{tikzpicture}
\clip (-2.5,-1.2) rectangle (2.5,2.5);
\draw[ultra thick] (-2,1).. controls (-3,-1) and (3,-1)..(2,1);
\draw[ultra thick, dotted] (-2,1).. controls (-1,2) and (1,2) ..(2,1);
\draw [brown, pattern=dots, pattern color=brown] (-2.25,-.5)--(-2,1)--(-1.75,-.5);
\draw [brown, pattern=dots, pattern color=brown] (2.25,-.5)--(2,1)--(1.75,-.5);
\node at (0,-.8) {$Y_\D$};
\node at (0,2) {$\partial X\setminus Y_\D$};
\end{tikzpicture}
\caption{\label{fig-11-4} Infinite cone condition}
\end{figure}

\begin{example}[Conical and sharp quasi-conical singularities]\label{ex-11-2-21}%
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-2--21-i}
The \newline
scheme described in Example~\ref{ex-11-2-18} covers conical
singularities as well as sharp quasi-conical singularities%
\index{sharp quasi-conical singularity}%
\index{quasi-conical singularity!sharp}%
\index{singularity!quasi-conical!sharp}
directed outward. Namely let
\begin{equation}
X=\{x=(x',x''), \ x'\in |x''| ^\nu\cdot X',\ |x''|\le 1 \}
\label{11-2-88}
\end{equation}
with $\nu \ge 1$; for $d''=1$ one can take only half of this singularity (lying in $\{x,x_1>0\}$ where here $x''=(x_1)$ for $d''=1$)). Then we have conical and quasi-conical singularities as $\nu=1$ and $\nu>1$ respectively. Here we use $X'$, $\gamma'$ and $\gamma$ described in Example~\ref{ex-11-2-19}.

The classification coincides with that in Example~\ref{ex-11-2-19} but in all the inequalities on the exponents ``$<$'' should be replaced by ``$>$'' and v.v., and case \ref{ex-11-2-19-d} is impossible.

\item\label{ex-11-2--21-ii}
If the domain $X$ described in \ref{ex-11-2--21-i} is contained in the ball $B(0,R)$ then
$\gamma (x)= \max \bigl(\gamma_\old (x)),\dist (x,\partial X)\bigr)$ works for the domain $\complement X$ where $\gamma_\old$ is defined as $\gamma$ in \ref{ex-11-2--21-i}. One can easily see that the classification given in \ref{ex-11-2--21-i} remains true. It allows us to cover sharp quasi-conical singularities directed inward.
\end{enumerate}
\end{example}

\begin{figure}[h]
\centering
\subfloat[acute]{\label{fig-11-5-a}%
\begin{tikzpicture}[scale=.8]
\begin{scope}
\clip (-6,-2) rectangle (-1,2);
\draw[ultra thick] (-5,-2) .. controls (-4,-0.2) and (-2,0) ..(0,0) ..controls (-2,0) and (-4,0.2) .. (-5,2);
\clip (-5,-2) .. controls (-4,-0.2) and (-2,0) ..(0,0) ..controls (-2,0) and (-4,0.2) .. (-5,2);
\draw[thick, dashed](-5,0) ellipse (15pt and 56pt);
\end{scope}
\clip (-6,-2) rectangle (-5,2);
\draw[thick](-5,0) ellipse (15pt and 56pt);
\end{tikzpicture}}
%\quad
\subfloat[cone]{\label{fig-11-5-b}%
\begin{tikzpicture}[scale=.8]
\begin{scope}
\draw[ultra thick] (-5,-2) -- (0,0) -- (-5,2);
\clip (-5,-2) -- (0,0) -- (-5,2);
\draw[thick, dashed](-5,0) ellipse (15pt and 56pt);
\end{scope}
\clip (-6,-2) rectangle (-5,2);
\draw[thick](-5,0) ellipse (15pt and 56pt);
\end{tikzpicture}}
%\quad
\subfloat[blunt]{%
\begin{tikzpicture}[scale=.8]
\begin{scope}
\draw[ultra thick] (-5,-2) .. controls (-4,-2) and (-2,-2) ..(0,0) ..controls (-2,2) and (-4,2) .. (-5,2);
\clip (-5,-2) (-5,-2) .. controls (-4,-2) and (-2,-2) ..(0,0) ..controls (-2,2) and (-4,2) .. (-5,2);
\draw[thick, dashed](-5,0) ellipse (15pt and 56pt);
\end{scope}
\clip (-6,-2) rectangle (-5,2);
\draw[thick](-5,0) ellipse (15pt and 56pt);
\end{tikzpicture}}
\caption{\label{fig-11-5} Conical and quasi-conical singularities, could be directed inward and outward}
\end{figure}


\begin{example}[Blunt quasi-conical singularity]\label{ex-11-2-22}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-2-22-i}
Let $X'$ and $\gamma '$ be as in Example~\ref{ex-11-2-19} again, let $0\in X'$ and let $X=\{x=(x',x''), x''\in B(0,R), x'\in f(|x''|)X'\}$ where $f(0)=0$ and $f$ is a monotone decreasing function such that the
inverse function $f$ satisfies condition (\ref{11-2-82}) in dimension $1$.
Then for $x''\in B(0,{\frac{1}{2}}R)$ one can take
$\gamma (x)=\epsilon |x|\gamma '(x'f^{-1}(|x''|))$. Then condition
(\ref{11-2-65}) fulfilled if and only if
\begin{equation}
f^{d '}(r)r^{-\vartheta -1+d''-1}\in \sL^1([0,1]).
\label{11-2-89}
\end{equation}
This example covers various blunt quasi-conical singularities%
\index{blunt quasi-conical singularity}%
\index{quasi-conical singularity!blunt}%
\index{singularity!quasi-conical!blunt}
directed outward of the type $X=\{x=(x',x''),|x'|\le |x''| ^\nu \}$
with $\nu \in (0,1]$.

\item\label{ex-11-2--22-ii}
One can replace $X$ by $B(0,R)\setminus X$ with the $\gamma$
defined above. Again condition (\ref{11-2-89}) is crucial. This example
covers various blunt quasi-conical singularities directed inward.
\end{enumerate}
\end{example}

\begin{remark}\label{rem-11-2-23}
In Examples~\ref{ex-11-2-21} and \ref{ex-11-2-22} cone condition poses restrictions, especially as $\nu>1$ in their parts~(i). And again under certain assumptions we will be able to allow Neumann Laplacian (see Section~\ref{sect-12-6}).
\end{remark}

\begin{example}[Clews]\label{ex-11-2-24}
We can consider domain containing ``disk with an infinite cut'' $r=r(\theta)$ with $\theta_0\le \theta <\infty$ with $r(\theta)=\theta^{-\alpha}$ as
$\theta \to \infty$ (we use polar coordinates here). As $\alpha \le 1$ the length of the cut is infinite.

On this cut Dirichlet boundary condition should be imposed. We leave details to the reader.
\end{example}


\begin{example}[Combs]\label{ex-11-2-25}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-2-25-i}
Let
\begin{equation}
X=\{x=(x_1,x_2,x''), 0<x_1<1,\;-1<x_2<f(x_1),|x''|<1\}
\label{11-2-90}
\end{equation}
where $f(x_1)$ is the jump function given by $f(x_1)=h_i=\const\ge 0$ for $x_1\in I_i$ and $f(x_1)=0$ for $x_1\in I_{\infty}$ where
$I_i\cap I_j=\emptyset$ for $i\ne j$, $I_i$ with $i<\infty $ are open intervals of lengths $l_i$, $I_{\infty }=[0,1]\setminus \cup_{i<\infty }I_i$ and
$\mes(I_{\infty })=0$.

Then the subdomain $X\cap \{x_2>0\}$ consists of separate ``boxes'' in each of which one should take $\gamma $ according to scheme described in Example~\ref{ex-11-2-18}. Then for $\vartheta \in [0,1)$ the contribution of the $i$-th box to $\int \gamma ^{-1-\vartheta }dx$ is of the order
$h_il_i^{-\vartheta }+l_i^{1-\vartheta }$.

On the other hand, on $X\cap \{x_2\le 0\}$ one can take
$\gamma (x)={\frac{1}{2}}(-x_2+\delta (x_1))$ where
$\delta (x_1)=\dist (x_1,I_{\infty })$. Then the contribution of this subdomain is of the order
\begin{align*}
\int |\log \updelta (x_1)|dx_1\asymp \sum_i -l_i\log l_i\qquad
&\text{for\ }\vartheta =0,\\
\int \updelta (x_1)^{-\vartheta }dx_1\asymp
\sum_i l_i^{1-\vartheta}\qquad &\text{for\ }\vartheta >0.
\end{align*}
Therefore condition (\ref{11-2-65}) with $\vartheta =0$ means that
\begin{equation}
\sum_i h_i<\infty ,\quad \sum_i -l_i\log l_i<\infty
\label{11-2-91}
\end{equation}
and condition (\ref{11-2-65}) with $\vartheta>0$ means that
\begin{equation}
\sum_i h_il_i^{-\vartheta }<\infty ,\qquad \sum_i l_i^{1-\vartheta }<\infty.
\label{11-2-92}
\end{equation}

\item\label{ex-11-2-25-ii}
Recall that under the cone condition, a Dirichlet boundary value problem can be replaced by an arbitrary regular boundary value problem. Recall that this condition does not mean that the cone $\Gamma$ lies completely in $X$; we assume that the intersection of $\Gamma$ with $X$ is connected and a Dirichlet condition is given on $\Gamma \cap \partial X$.
\end{enumerate}
\end{example}

\begin{example}[Trees]\label{ex-11-2-26}
One can consider example when $X$ is a \emph{tree}: for example it consists of cylindrical pipes $P_{i,j}$ of the lengths $l_{i,j}$ and radii $r_i$ ($d''=1$, $d'=d-1$) where $i=1,\dots, \infty$, $j= 1,\dots, J(i)$ and each pipe $P_{i,*}$
has no more than $c$ pipes $P_{i+1,j}$ on its end. Let us assume that $l_i\ge r_i$ and $r_{i+1}\le r_i\le c r_{i+1}$ for all $i$.

Assume that the cross-section of pipes and conjugations are regular enough so we can select $\epsilon_0 r_i$ as $\gamma$ around $P_{i,*}$. Then the total volume is finite if and only if
\begin{gather}
\sum_i r_i^{d-1}L_i<\infty,
\label{11-2-93}\\
\intertext{and condition (\ref{11-2-65}) holds if and only if}
\sum_i r_i^{d-2-\vartheta}L_i<\infty,
\label{11-2-94}
\end{gather}
where $L_i=\sum_{1\le j\le J(i)}l_{i,j}$.

These pipes are not necessarily cylindrical: we can take any bounded domain with $\sC^K$ boundary and make $P_{i,j}$ by scaling it $l_i$ times along $x''=(x_1)$ and $r_i$ times along $x'$. These trees could be bounded as $\sum_i l^*_i<\infty $ or extended to infinity as $\sum_i l^*_i=\infty$,
$l^*_i=\max_{1\le j\le J(i)}l_{i,j}$.
\end{example}

\begin{figure}[h]
\centering
\subfloat[Comb]{\label{fig-11-6-a}%
\begin{tikzpicture}
\clip (1.9,-0.4) rectangle (6,5.2);
\filldraw [teal!50] (2,-0.3) rectangle (5,0.3);
\filldraw [teal!50] (4.5,-0.3) rectangle (5,5);
\filldraw [teal!50] (3.6,-0.3) rectangle (4,4);
\filldraw [teal!50] (2.9,-0.3) rectangle (3.2,4);
\filldraw [teal!50] (2.4,-0.3) rectangle (2.6,4);
\filldraw [teal!50] (2.1,-0.3) rectangle (2.2,4);
\fill[white] plot function {x*x/4-0.5};
\end{tikzpicture}}
\qquad
\subfloat[Tree]{\label{fig-11-6-b}%
\begin{tikzpicture}[scale=.9]
\filldraw [teal!50] (0,-0.3) rectangle (2.2,0.3);
\filldraw [xshift=60,yshift=0,teal!50,rotate=30] (0,-0) rectangle (2.2,0.4);
\filldraw [xshift=60,yshift=0,teal!50,rotate=-30] (0,-0) rectangle (2.2,-0.4);
\filldraw [xshift=110,yshift=33,teal!50,rotate=75] (0,-0) rectangle (2.2,0.2);
\filldraw [xshift=110,yshift=33,teal!50,rotate=-15] (0,-0) rectangle (2.2,-0.2);
\filldraw [xshift=110,yshift=-33,teal!50,rotate=-75] (0,-0) rectangle (2.2,-0.2);
\filldraw [xshift=110,yshift=-33,teal!50,rotate=15] (0,-0) rectangle (2.2,0.2);
\end{tikzpicture}}
\caption{\label{fig-11-6} Comb (Example~\ref{ex-11-2-25}) and tree (Example~\ref{ex-11-2-26}) with infinite numbers of teeth and branches}
\end{figure}

Let us discuss mixed boundary value problems assuming the cone condition is fulfilled in the indicated form.

Let the geometry of the domain (and the singularities of the coefficients of the operator $A$) are compatible with the scaling function
$\gamma (x)=\gamma_0(x)$. Then in order to take into account the
singularities of the boundary value problem we should replace
$\gamma_0 (x)$ by $\min (\gamma_0 (x),\gamma_1(x))$ where scaling function
$\gamma_1(x)$ corresponds to the singularities of the boundary value problem.

If $\gamma_0(y)\le 2\dist (y,\partial X)$ then one can take
$\gamma (x)\asymp \gamma_0 (x)$ in $\bigl(y,{\frac{1}{3}}\gamma(y)\bigr)$. Otherwise one can straighten $\partial X$ in
$\cB\bigl(y, \frac{2}{3} \gamma(y),X\bigr)$ by means of a map which is uniformly smooth in the $\gamma_0$-scale with Jacobian disjoint from $0$. Therefore
without any loss of generality one can assume that
\begin{equation}
X\cap \cB\bigl(y,\gamma(y),X\bigr)= \{x_1>0\}\cap B\bigl(y, \gamma (y)\bigr).
\label{11-2-95}
\end{equation}
Then $\gamma_1(x)\asymp x_1+\gamma_1(x')$ in
$X\cap \cB\bigl(y, \frac{1}{2} \gamma(y),X\bigr)$ where here
$\gamma_1(x)$ is defined only on $\partial X$ in order to take into account
the singularities of the boundary value problem. Assuming that
$\gamma_0 ^{-1-\vartheta }\in \sL^1(X)$ we conclude that
\begin{equation}
\gamma_1^{-1-\vartheta }\in \sL^1(X) \iff
\left\{\begin{aligned}
\log \gamma_1\in \sL^1(\partial \cX_\reg)\qquad&\text{for\ \ }\vartheta =0,\\
\gamma_1^{-\vartheta}\in \sL^1(\partial\cX_\reg)\qquad
&\text{for\ \ }\vartheta >0
\end{aligned}\right.
\label{11-2-96}
\end{equation}
where the standard surface measure is used on $\partial \cX_\reg$. In
particular, this condition is fulfilled for $\vartheta \in [0,\delta )$
as $\gamma_1(x)\ge \epsilon_0\dist (x,\cK)$ where $\cK$ is
a subset of $\partial X$ with the following property:
\begin{claim}\label{11-2-97}
For every $y\in \cX_\reg$\quad $\cK\cap B\bigl(y,\gamma_0(y),X\bigr)$
is contained in $\bigcup_{1\le l\le L}{\cK}_l$ where ${\cK}_l$
(depending on $y$ also) are uniformly $\sC^K$ submanifolds (in the $\gamma_0$-scale) of $\partial \cX_\reg$ of codimension $\delta$.
\end{claim}
This analysis provides us immediately with a series of examples for the Laplacian when on part of the boundary the Dirichlet condition is given and on the remaining part the Neumann boundary condition is given and
$\vartheta <1$.

\begin{example}\label{ex-11-2-27}
Let us consider a boundary value problem of variational origin with the functional
\begin{multline}
\boldPhi(u)=\boldPhi_{\inn}(u)+\boldPhi_{\bound}(u)=\\
\shoveright{\int_{X}\sum_{\alpha ,\beta :|\alpha |\le m,|\beta |\le m}
a_{\alpha ,\beta }\langle a_{\alpha ,\beta }D ^\alpha u,D ^\beta u\rangle\, dx +\qquad}\\
\int_{\partial X}\sum_{\alpha ,\beta :|\alpha |\le m-1,|\beta |\le m-1}
a_{\alpha ,\beta }\langle b_{\alpha ,\beta }D ^\alpha u,
D ^\beta u\rangle\, dS
\label{11-2-98}
\end{multline}
where $dS$ is a standard measure at $\partial X$. Let us assume that the boundary terms of this functional are regular in the sense that after the rescaling $x\mapsto (x- \bar{x})\gamma(\bar{x})^{-1}$ and multiplication by $\gamma (\bar{x})^{2m-d}$ we obtain a functional the coefficients of which (and all their derivatives of order $\le K$) are bounded in $B(0,1)$. The same should be true for the boundary conditions which define $\fD (\boldPhi )$ but the $l$-th condition has its own weight $\varrho_{(l)}$ for multiplication and is given on the set $\Xi_l\subset\partial X$ ($l=1,\dots ,L$).

Let us assume that the cone condition is fulfilled. Then $\cK$ is the union of the relative (in $\partial X$) boundaries of $\Xi_l$. However, the possibly irregular structure of ${\cK}$ prevents us from immediately applying the above
arguments. Nevertheless, for $\vartheta =0$ we avoid this difficulty by means of variational arguments. Namely, let us consider a covering of
$\partial \Xi_l$ of finite multiplicity by balls
$B\bigl(x^k,\epsilon \gamma (x ^k)\bigr)$ lying in the
$2\epsilon \gamma $-neighborhood of $\partial \Xi_l$; let
$\omega_{l,\epsilon }$ be the union of these balls. Let us replace
$\Xi_l$ by $\Xi '_l=\Xi_l\cap\omega_{l,\epsilon }$ or by
$\Xi ''_l=\Xi_l\setminus \omega_{l,\epsilon }$. We do the same with the set $\Xi_0$ where the Dirichlet boundary condition is given.

In the first case (when all the sets $\Xi_l$ expand) the domain of $\boldPhi $ shrinks and $\N^-(\tau )$ decreases, and in the second case (when all the sets $\Xi_l$ shrink) the domain of $\boldPhi $ expands and $\N^-(\tau )$ increases. Further, the cone condition remains true in both cases for small enough
$\epsilon >0$. Furthermore, in both cases the required regularity conditions
are now fulfilled (because $\partial \Xi '_l$ and $\partial \Xi ''_l$
intersected with $\partial X_r$ lie in the union of spheres
$S\bigl(x^k,\epsilon \gamma (x^k)\bigr)$ and every ball
$B\bigl(\bar{x},\gamma (\bar{x})\bigr)$ intersects no more than $C=C_\epsilon $ of these spheres. Therefore
\begin{equation}
\N^{\prime-}(\tau )\le \N^- (\tau )\le \N ^{\prime\prime-}(\tau )
\label{11-2-99}
\end{equation}
and
$\N^{\prime-}(\tau)=\varkappa_0\tau^{\frac{d}{2m}}+O(\tau^{\frac{1}{2m}(d-1)})$
and the same is true for $\N ^{\prime\prime-}(\tau)$ with the same coefficient $\varkappa_0$ (because it does not depend on the boundary conditions). Therefore \emph{the same is true for the problem in question:}
\begin{equation}
\N^- (\tau )=\varkappa_0\tau ^{\frac{d}{2m}}+
O\bigl(\tau ^{ \frac{1}{2m} (d-1)}\bigr)\qquad\text{as\ }\tau \to+\infty.
\label{11-2-100}
\end{equation}

Moreover, under the standard non-periodicity condition to Hamiltonian
trajectories\footnote{\label{foot-11-19} This condition is not associated with
$\partial \Xi '_l$ or $\partial \Xi ''_l$ because the $2d$-dimensional
measures of points lying on trajectories issuing from these
sets obviously vanish.} asymptotics
\begin{equation*}
\N '(\tau )=\varkappa_0\tau ^{\frac{d}{2m}}+
\varkappa '_1\tau ^{ \frac{1}{2m} (d-1)}+
o\bigl(\tau ^{\frac{1}{2m} (d-1)}\bigr)
\end{equation*}
holds and the same is true for $\N ''(\tau )$. Here $\varkappa '_1$ is a monotone non-increasing and $\varkappa ''_1$ is a monotone non-decreasing function of $\epsilon\in (0,\epsilon_0)$ and $\varkappa '_1\le \varkappa ''_1$. Let us recall that the coefficient
$\varkappa_1$ consists of two terms; one of them does not depend on boundary conditions and the other is an integral over $\partial X_r$ of some function of the principal coefficients of the operator and the boundary operators. Therefore, assuming that
\begin{equation}
\mes_{\partial X}(\partial \Xi_l)=0\qquad \forall l=0,\dots ,L
\label{11-2-101}
\end{equation}
we obtain that the limits of $\varkappa '_1$ and $\varkappa ''_1$ as
$\epsilon \to +\infty $ coincide and therefore the asymptotics
\begin{equation}
\N^- (\tau )=\varkappa_0\tau ^{\frac{d}{2m}}+
\varkappa_1\tau ^{\frac{1}{2m}(d-1)}+
o\bigl(\tau ^{\frac{1}{2m}(d-1)}\bigr)\qquad \text{as\ }\tau \to+\infty
\label{11-2-102}
\end{equation}
holds.
\end{example}

Let us treat the case in which the boundary is very irregular.

\begin{example}\label{ex-11-2-28}
Let us assume that the operator $A$ satisfies our conditions with
$\gamma =\const>0$. Then one can take $\gamma (x)=\dist (x,\partial X)$ in which case the remainder estimate in the asymptotics of $\N^-_{(\vartheta)} (\tau )$ is ``$O$'' of
\begin{multline}
\tau ^{{\frac{1}{2m}}(d-1-\vartheta )+\vartheta }
\int_{r\ge \tau ^{\frac{1}{2m}}}r^{-1-\vartheta }d\upmu (r)+
\tau ^{{\frac{d}{2m}}+\vartheta }\upmu (\tau ^{-{\frac{1}{2m}}})\asymp
\\
\tau ^{{\frac{1}{2m}}(d-1-\vartheta )+\vartheta}
\int_{r\ge \tau ^{\frac{1}{2m}}}r^{-2-\vartheta }\upmu (r)dr +
\tau ^{{\frac{d}{2m}}+\vartheta }\upmu (\tau ^{-{\frac{1}{2m}}})
\label{11-2-103}
\end{multline}
with $\upmu (r)=\mes (\{x\in X,\dist (x,\partial X)\le r\})$; we assume that $\mes(X)<\infty $. In particular, if $\upmu (r)=O(r ^\delta )$ as $r\to +0$ then for $\vartheta <\delta-1$\,\footref{foot-11-17} we obtain the remainder estimate
$O\bigl(\tau ^{{\frac{1}{2m}}(d-1-\vartheta )+\vartheta }\bigr)$; moreover, under standard non-periodicity condition to the Hamiltonian
trajectories we obtain the remainder estimate
$o\bigl(\tau^{\frac{1}{2m}(d-1-\vartheta)+\vartheta}\bigr)$.

On the other hand, we obtain the remainder estimate
$O\bigl(\tau^{\frac{1}{2m}(d-1-\vartheta)+\vartheta}\log\tau\bigr)$
for $\vartheta=\delta-1$ and we obtain the remainder
estimate $O\bigl(\tau ^{{\frac{1}{2m}}(d-\delta )+\vartheta }\bigr)$
for $\vartheta >\delta-1$.

For $\vartheta =0,\delta =1$ and for $\vartheta =0, \delta \in (0,1)$
we obtain the results of the papers J.~Br\"{u}ning~\cite{bruning:spectral} and J.~Fleckinger, M.~Lapidus~\cite{fleck:fractal} respectively. Finally, in these two cases under the condition $\upmu (r)=o(r ^\delta )$ as $r\to +0$ we obtain ``$o$'' in the remainder
estimates.
\end{example}

\begin{remark}\label{rem-11-2-29}
Condition $\upmu (r)=O(r ^\delta )$ as $r\to +0$ means exactly that \emph{inner Minkowski dimension of $\partial X$ does not exceed $d-\delta$}. So called \emph{Weyl-Berry conjecture} (in sanitized form: originally M.~Berry thought about Hausdorff dimension) claims the second term $\kappa_\delta \tau^{(d-\delta)/2}$ and the remainder estimate $o(\tau^{(d-\delta)/2})$ for Dirichlet (Euclidean) Laplacian.

However, as J.~Brossard and R.~Carmona \cite{brossard:fractal} had shown it is almost never the case as capacity enters the game (recall that Weyl conjecture is almost always true for sure for Euclidean domains and may be even always true).
\end{remark}

\section[Large eigenvalues for weakly singular potentials (end)]{Large eigenvalues for operators with weakly singular potentials (end)}
\label{sect-11-3}


\subsection{Operators with non-periodic flows}
\label{sect-11-3-1}

We start this subsection by discussing existence and some properties of the Hamiltonian billiard flow for second order operators.

Then we consider examples in which restrictive conditions on the Hamiltonian flow imply asymptotics with highly accurate remainder estimates (those we used to call \emph{sharper\/}). %Let us assume for the sake of simplicity that
$\vartheta =0$.
Here we do not treat smooth closed manifolds without boundary; the reader can find all those results in A.~Volovoy~\cite{volovoy:compact, volovoy:weyl} and in
the earlier papers P.~B\'{e}rard~\cite{berard:compact}, B.~Randoll~\cite{randoll:zeta}. For the Laplace-Beltrami operator these statements yield the following


\begin{example}\label{ex-11-3-1}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-3-1-i}
For the Laplace-Beltrami operator on a compact closed Riemannian $\sC^K$ manifold of non-positive sectional curvature (for $d\ge 3$) or without conjugate
points (for $d=2$) asymptotics of $\N^- (\tau )$ with remainder estimate
$O\bigl(\tau ^{\frac{1}{2}(d-1)}\log ^{-1}\tau \bigr)$ holds.

\item\label{ex-11-3-1-ii}
For a certain class of surfaces of rotation and for a certain class of graded Lie algebras asymptotics of $\N^- (\tau )$ with the remainder estimate $O\bigl(\tau ^{{\frac{1}{2}}(d-1-\delta )}\bigr)$ holds with $\delta >0$.
\end{enumerate}
\end{example}

\begin{remark}\label{rem-11-3-2}
In the context of our book the results on Hamiltonian flows obtained in these papers yield asymptotics for $\N^-_{(\vartheta)} (\tau )$ with remainder estimates $O\bigl(\tau ^{{\frac{1}{2}}(d+\vartheta -1)}
\log ^{-\vartheta -1}\tau \bigr)$ and
$O\bigl(\tau ^{{\frac{1}{2}}(d+\vartheta -1-\delta )}\bigr)$
respectively.
\end{remark}

\subsubsection{Existence of the billiard flow}
\label{sect-11-3-1-1}
Let us consider the Laplace(-Beltrami) operator in compact domains
or on compact manifolds with singularities. The following
statement is necessary:

\begin{theorem}\label{thm-11-3-3}
Let $X$ be a bounded domain in $\bR^d$ which is a Riemannian manifold with boundary with metric $g(x,\xi )$ satisfying conditions
\begin{gather}
g^{jk}=g^{kj},\qquad
\epsilon_0|\xi |^2\le g(x,\xi )=\sum_{jk}g^{jk}\xi_j\xi_k\le c|\xi|^2,
\label{11-3-1}\\
|D^\alpha g^{jk}|\le c\gamma ^{-|\alpha |}\qquad
\forall \alpha :|\alpha |\le K\quad \forall j,k
\label{11-3-2}
\end{gather}
and with scaling function $\gamma (x)$ such that $\gamma ^{-1}\in \sL^1(X)$.

Then there exist a set of measure $0$ and also of the first Baire category
$\Lambda \subset S^*\bar{X}$ and a continuous Hamiltonian flow $\Psi_t$ on
$S^*\bar{X}\setminus \Lambda $ with reflection at the boundary such that all its trajectories lie in
$S^*\bar{X}_r$, $\bar{X}_\reg=\{x\in \bar{X}, \gamma (x)>0\}$ and
are transversal to $\partial X$; as usual $\bar{X}=X\cup\partial X$.

This flow conserves the natural measure $d\upmu=dxd\xi :d\sqrt g$ on $S^*X$.
\end{theorem}

\begin{proof}
The proof coincides with the arguments of Chapter~6 in the book I.~P.~Cornfeld, S.~V.~Fomin and Y.~G.~Sinai, \cite{cornfeld:ergodic}. This proof follows the following scheme: first we establish that the flow where it is defined preserves measure $\upmu$.

Then we consider the set $\Lambda_{t_1,t_2}$ of all points such that $\Psi_t$ exists on time interval $[0,t_1]$ but breaks on $(t_1,t_2]$ (as $0<t_1<t_2$). Invariance of the measure $\upmu$ implies that
$\upmu (\Lambda_{T,T+\varepsilon})=\upmu (\Lambda_{0,\varepsilon})$ and therefore
\begin{equation}
\upmu (\Lambda_{0,T})\le \upmu (\Lambda_{0,\varepsilon}) \lceil \frac{T}{\varepsilon}\rceil.
\label{11-3-3}
\end{equation}

On the other hand, due to the bounded speed of propagation $\Lambda_{0,\varepsilon}$ is covered by
$\{(x,\xi): \gamma (x)\le C_1\varepsilon\}$ and by union of subsets
\begin{equation*}
\bigl\{(x,\xi):\ \gamma(x)\asymp \gamma \dist (x,\partial X)\le C_0\varepsilon\bigr\}
\end{equation*}
which trajectories have an angle less than $\delta$ with the boundary; here $\delta=\delta(\varepsilon\gamma^{-1})=o(1)$ as $\varepsilon \to +0$, with
$\gamma\ge C_1\varepsilon$.

Actually those points belong to $C_0\delta\varepsilon$-vicinity of $\partial X$. Obviously $\upmu$-measure of the first set does not exceed
$C\mes (\{x,\gamma (x)\le C_0\varepsilon\})$ and $\upmu$-measure of the second set does not exceed $C\delta^2\varepsilon\gamma^{-1} \mes(\{x,\gamma(x)\asymp \gamma\})$.

Note that in virtue of $\gamma^{-1}\in \sL^1$ we estimate the measure of the first set
\begin{equation}
\mes (\{x,\gamma (x)\le C_1\varepsilon\})=o(\varepsilon)
\label{11-3-4}
\end{equation}
and the measure of the second set by
\begin{equation*}
C\int_{x:\gamma(x)\ge C_1\varepsilon} \delta^2 \bigl(\frac{\varepsilon}{\gamma(x)}\bigr) \gamma^{-1}(x)\, dx = o(\varepsilon);
\end{equation*}
so $\upmu (\Lambda_{0,\varepsilon})=o(\varepsilon)$ as $\varepsilon\to +0$.

Combining with (\ref{11-3-3}) we conclude that $\upmu (\Lambda_{0,T})=o(1)$ and thus $\upmu (\Lambda_{0,T})=0$. Negative time direction is covered by the same way.
\end{proof}

\begin{remark}\label{rem-11-3-4}
Let us note that if we are interested only in trajectories of length not exceeding $T$ then in the statement of this lemma one can replace $\Lambda $ by a closed nowhere dense subset $\Lambda_T$. However,
$S^*\bar{X}\setminus \Lambda_T$ is not invariant with respect to the flow $\Psi_t$.
\end{remark}

\subsubsection{Properties of Hamiltonian billiard flows and asymptotics}
\label{sect-11-3-1-2}

Recall that to recover sharper remainder estimate we need to estimate the ``divergence'' of the billiard flow and its non-periodicity. The first notion is covered by the following

\begin{definition}\label{def-11-3-5}
Let $X$ be a compact $\gamma$-admissible Riemannian manifold with boundary
where $\gamma $ is an admissible scaling function such that
$\gamma ^{-1}\in \sL^1(X)$.

We say that


\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{def-11-3-5-i}
$\Psi_t$ is \emph{a power geodesic flow with reflections}%
\index{power geodesic flow with reflection}%
\index{geodesic flow!power!with reflection}%
\index{flow!geodesic!power with reflection}%
is given on $X$ if for every $T\ge 0$ there exists a closed set
$\Xi_T\subset\Sigma$ with $\upmu (\Xi_T)\le CT^{-1}$ such that through every point $z\in \Sigma \setminus \Xi_T$ there passes a geodesic trajectory
$\Psi_t(z)=\bigl(x(t),\xi (t)\bigr)$ with reflections from
$\partial X$ with $t\in [0,T]$ or $t\in [-T,0]$, along which
$\gamma (x(t))\ge \varepsilon (T)$, the angle with $\partial X$ is not
less than $\varepsilon (T)$ at every point where the distance from the
boundary is less than $\varepsilon (T)$, and also
$|D\Psi_t |\le \varepsilon (T)^{-1}$ where $\varepsilon (T)=T^{-L}$
with large enough $C,L$.

\item\label{def-11-3-5-ii}
\index{exponential geodesic flow with reflection}%
\index{geodesic flow!exponential!with reflection}%
\index{flow!geodesic!exponential with reflection}
Similarly, we say that $\Psi_t$ is \emph{an exponential geodesic flow with reflections} if \ref{def-11-3-5-i} holds with $\varepsilon (T)=e^{-CT}$ respectively.
\end{enumerate}
\end{definition}

We have a non-trivial \emph{non-periodicity}%
\index{non-periodicity condition}%
\index{condition!non-periodicity}
condition. In order to take it into account we introduce

\begin{definition}\label{def-11-3-6}
In the framework of Definition~\ref{def-11-3-5} we say that $\Psi_t$ is a
\emph{non-periodic power (or exponential) geodesic flow}%
\index{non-periodic!power geodesic flow}%
\index{geodesic flow!non-periodic power}%
\index{flow!geodesic!non-periodic power}%
\index{non-periodic!exponential geodesic flow}%
\index{geodesic flow!non-periodic exponential}%
\index{flow!geodesic!non-periodic exponential}
if in addition to the conditions of definition \ref{def-11-3-5}
\begin{multline}
\upmu\bigl(\bigl\{z\in \Sigma \setminus \Xi_T,\exists t\in (0,T):
|t|^{-1} \dist (z,\Psi_t(z))\le \varepsilon (T)\bigr\}\bigr)=\\
O(T ^{-1})
\label{11-3-5}
\end{multline}
where we increase $C$ and $L$ in the definition of $\varepsilon (T)$ if
necessary.
\end{definition}

We conclude immediately that

\begin{theorem}\label{thm-11-3-7}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-3-7-i}
Let $X$ be a domain with non-periodic power geodesic flow. Let $\gamma_0$ be scaling function describing singularities of domain and $\gamma\le \gamma_0$ be scaling function describing singularities of operator and boundary conditions. Then as
\begin{equation}
\gamma^{-1-\vartheta-\delta_1} \in \sL^1(X)
\label{11-3-6}
\end{equation}
with arbitrarily small exponent $\delta_1>0$, asymptotics
\begin{equation}
\N^-_{(\vartheta)}= \N^\W_{(\vartheta)}+O\bigl(\tau^{\frac{d-1-\vartheta}{2m} + \vartheta-\delta}\bigr)
\label{11-3-7}
\end{equation}
holds with $\delta>0$ as $\tau\to +\infty$.

\item\label{thm-11-3-7-ii}
Let $X$ be a domain with non-periodic exponential geodesic flow. Let $\gamma_0$ be scaling function describing singularities of domain and $\gamma\le \gamma_0$ be scaling function describing singularities of operator and boundary conditions. Then as
\begin{equation}
\gamma^{-1-\vartheta} |\log \gamma|^{1+\vartheta} \in \sL^1 (X)
\label{11-3-8}
\end{equation}
with arbitrarily small exponent $\delta_1>0$, asymptotics
\begin{equation}
\N^-_{(\vartheta)}= \N^\W_{(\vartheta)}+O\bigl(\tau^{\frac{d-1-\vartheta}{2m} + \vartheta}|\log \tau|^{-1-\vartheta}\bigr)
\label{11-3-9}
\end{equation}
holds as $\tau\to +\infty$.
\end{enumerate}
\end{theorem}

\subsubsection{Examples}
\label{sect-11-3-1-3}

\paragraph{Polygons and polyhedra}\label{sect-11-3-1-3-1}
Recall that according to Theorem~\ref{thm-7-4-11} in a compact Euclidean polyhedral domain in $\bR^d$ \ $|D\Psi_t(x,\xi )|\le C(|t|+1)$.

\begin{theorem}\label{thm-11-3-8}
Let $X$ be a polyhedral domain with cuts; assume that $X$ is $\gamma$-admissible with $\gamma ^{-1-\sigma }\in \sL^1(X)$ with $\sigma>0$. Then there is a non-periodic power geodesic flow.
\end{theorem}

\begin{proof}
Note first that
\begin{equation}
\mes\bigl(\bigl\{z=(x,\xi )\in \Sigma , \dist (x,\partial X)\le \varepsilon
\bigr\}\bigr)\le C\varepsilon.
\label{11-3-10}
\end{equation}

Let us cover set
$\bigl\{z=(x,\xi ) \in\Sigma, \dist(x,\partial X)\ge \varepsilon \bigr\}$
with no more than $C\varepsilon^{1-4d}$ balls of radius $O(\varepsilon ^2)$ and let us divide the time interval $[0,T]$ into no more than
$O(T\varepsilon ^{-2})$ intervals of length $O(\varepsilon ^2)$. Let $\varepsilon =O(T^{-L})$ with large enough exponent $L$.

Then if the distance between the $\Psi_t$-image of some ball and this ball is less than $\varepsilon ^2$ for some $t$ from the above subinterval then for all points $(x,\xi )$ of this ball and for all $t$ of this subinterval the geodesic flow is given by the formula
\begin{equation*}
\Psi_t(x,\xi )=(y+\Pi x+t\Pi \xi ,\Pi \xi )
\end{equation*}
with constant $y$ and $\Pi $ such that $\dist(\xi ,\Pi \xi)\le \varepsilon$ for all $\xi $ in question. Here $\Pi \in O(d)$ as in the proof of Theorem~\ref{thm-7-4-11}.

Taking into account that for every $x$ the $\bS^{d-1}$-measure of the
set
\begin{equation*}
\bigl\{\xi \in \bS^{d-1}, |y+\Pi x-x+t\Pi \xi |\le \varepsilon^N \quad
\mbox{for some $t$ with }|t|\ge \varepsilon \bigr\}
\end{equation*}
does not exceed $O(\varepsilon ^N )$ we obtain after summation over all
the balls and subintervals that (\ref{11-3-5}) holds.
\end{proof}

\begin{example}\label{ex-11-3-9}
Obviously in Euclidean polyhedral domains (without cuts) $\gamma_0^{-1-\vartheta}\in \sL^1(X)$ as $\vartheta<1$. So the only condition to be checked is $\gamma^{-1-\vartheta}\in \sL^1(X)$ where $\gamma=\dist(x,\cK)$ and $\cK$ is the set of the cut ends and transition points. This condition is equivalent to $\gamma^{-\vartheta}\in \sL^1(\partial X)$ as $\vartheta>0$ and
$|\log \gamma|\in \sL^1(\partial X)$ as $\vartheta=0$.
\end{example}

\paragraph{Elliptical domains}\label{sect-11-3-1-3-2}

According to Theorem~\ref{thm-7-4-12} in Euclidean elliptical domains
(or domains between two confocal ellipses) $\Psi_t$ is power growth geodesic flow with singularities (see (\ref{7-4-32})-- (\ref{7-4-34}) for more details).

\begin{theorem}\label{thm-11-3-10}
Let $X$ be a domain in $\bR^2$ bounded by one or two confocal ellipses.
Then there is a non-periodic power geodesic flow.
\end{theorem}

\begin{proof}
Obviously (\ref{11-3-5}) is equivalent to
\begin{multline}
\mes_{\Sigma '_2}\bigl(\bigl\{z'\in \Sigma '_2:\exists
k=1,\dots ,n:\dist (z',\Phi ^kz')\le \varepsilon =n^{-M}\bigr\}\bigr)=\\
O(n^{-\sigma })\quad \text{as\ }n\to +\infty
\label{11-3-11}
\end{multline}
for appropriate $M$ and $\sigma >0$. Recall that
$\Sigma '_2=\Sigma |_{Y_2}=B^*Y_2$ where $Y_2$ is an outer ellipse and we use other notations of the proof of Theorem~\ref{thm-7-4-12}.


\begin{enumerate}[label=(\alph*), wide, labelindent=0pt]
\item\label{proof-11-3-10-a}
Let us first consider the zone $\{(x,\xi ),\beta >0\}$. Let us consider the lines $\{\eta =\const\}$. These lines are analytically parameterized by a cyclic parameter $u\in\bR/2\pi \bZ$ (see the proof of theorem-\ref{thm-7-4-12})\footnote{\label{foot-11-20} More precisely, this line consists of two connected components. Billiard map $\Phi $ transforms every component into itself and the $x$-projection is an analytic diffeomorphism of this component to the ellipse $Y_2$. Every component is parameterized by $u$. Permutation of these components is equivalent to replacing $\Phi$ by
$\Phi ^{-1}$.}.

Let $w\in \bR/\bZ$ be a new cyclic coordinate:
$w=w_\eta (u)=\nu_\eta ((0,u))m_\eta ^{-1}$ for $u\in [0,2\pi ]$ and then by periodicity. Here $m_\eta =\nu_\eta ([0,2\pi ])$. One can easily see that
$m_\eta \asymp \log |\beta |$ as $\beta \to +0$ for $a_2>b_2$ and
$m_\eta \asymp \beta ^{-1}$ as $\beta \to +0$ for $a_2=b_2$.

For every fixed $\eta $ the map $\Phi_\eta $ of this line is analytic and
preserves the measure $dw_\eta =m_\eta ^{-1}d\nu_\eta $ and
the orientation\footnote{\label{foot-11-21} Moreover, it is well known
(see I.P.~Cornfeld, S.~V.~Fomin and Y.~G.~Sinai, \cite{cornfeld:ergodic}) that for generic $\eta$, $\Phi_\eta$ is an ergodic map.} and therefore
$\Phi_\eta $ is a shift $\Phi_\eta :w_\eta \to w_\eta +f(\eta )$.

Then in the proof of (\ref{11-3-11}) for $\Sigma '_2\cap\{\beta >0\}$ one needs to prove that
\begin{multline}
Cn\mes\bigl(\bigl\{\eta :\exists k,l=1,\dots ,n: |f(\eta )-{\frac{k}{l}}|\le
\varepsilon =n^{-L}\bigr\}\bigr) =O(n^{-\sigma })\\
\text{as\ }n\to +\infty
\label{11-3-12}
\end{multline}
for admissible $L$ and $\sigma >0$; here $\mes $ means Lebesgue measure.

Obviously, $f(\eta )$ is a continuous function. One can easily prove
that
\begin{equation}
\epsilon \beta ^p\le |\frac{df}{d\eta}|\le c\beta ^{-p}\qquad \text{for\ \ }
|\eta |\le a_2-\epsilon_0,
\label{11-3-13}
\end{equation}
i.e., for $\beta \in (0,\beta_0)$ with
small enough $\epsilon_0>0,\beta_0>0$. Recall that
$\beta =b_2^2-a_2^2b_2^2\eta ^2$. Therefore (\ref{11-3-12}) holds for the
$\eta $ indicated here.

On the other hand, $\Phi $ is an analytic map for $\beta \ne b_1^2$ (the case when rays are tangent to the inner ellipse $Y_1$). Therefore function $f(\eta )$ is analytic for $|\eta |<\eta_1=a_2^{-1}b_2^{-1}(b_2^2-b_1^2)^{\frac{1}{2}}$ and for $\eta_1<|\eta |\le a_2^{-1}$. Obviously, $f(\eta )$ is not constant in
each of these three intervals. One can easily see that
$f_\pm (\zeta )=f(\bar{\eta}\pm \zeta ^2)$ is an analytic function
for $|\zeta |\le \epsilon_0$ and $\bar{\eta}=+\eta_1,-\eta_1$.

However one can easily see that
\begin{gather}
\mes (\{\zeta:|f(\zeta)|\le \varepsilon\})=O(\varepsilon^\delta)\label{11-3-14}\\
\intertext{holds for every $\sC^K$ function on the closed segment provided}
\sum_{1\le j\le K-1}|f^{(j)}|\ge \epsilon_0.\label{11-3-15}
\end{gather}
Therefore (\ref{11-3-12}) holds.

\item\label{proof-11-3-10-b}
Let us treat the zone $\{(x,\xi ): 0>\beta >b_2^2-a_2^2\}$. In this
case every line $\{\eta =\const\}$ consists of two connected components and every component is equivalent to $\bS^1$ and the $x$-projection maps every component to one of two segments on the ellipse $Y_2$ describing by the inequality $x_2^2\ge -\beta b_2^2(a_2^2-b_2^2) ^{-1}$. The inverse map is
two-valued.

Let us introduce on this connected component the cyclic coordinate $u'$ which can be done in the following way: let us consider the confocal hyperbola described by the equation
$\frac{x_1^2}{a^{\prime 2}}-\frac{x_2^2}{b^{\prime 2}}$ with
$a ^{\prime 2}+b ^{\prime 2}=a_2^2-b_2^2$. This hyperbola intersects $Y_2$ in four points $(\bar{x}_1,\bar{x}_2)$ with
\begin{equation*}
\bar{x}_1^2=a_2^2(a_2^2-b_2^2+\beta )(a_2^2-b_2^2) ^{-1},\ \ \bar{x}_2^2=-b_2^2\beta (a_2^2-b_2^2) ^{-1}.
\end{equation*}
Let us introduce parameter $u'\in \bS^1$ on this hyperbola: $x_1=a'\sec u'$, $x_2=b'\tan u'$. Through every point of the hyperbola corresponding to this parameter there passes a tangent straight line hitting the corresponding segment of the ellipse. Then $(x_1,x_2)$ is an intersection point and $(\xi_1,\xi_2)$ is a unit vector along this tangent line, directed inside and outside for $\eta <0$ and $\eta >0$
respectively.

Let us introduce the parameter $w'\in \bR/\bZ$ in the same way as before. Again we take $dw'=m_\eta ^{-1}d\nu_\eta $ with $m_\eta \asymp \log |\beta |$ as $\beta \to -0$ and $m_\eta \asymp 1$ as $\beta \to b_2^2-a_2^2$. Moreover, in the latter case $m_\eta $ is an analytic function of
$\zeta '=(\beta +a_2^2-b_2^2)^{\frac{1}{2}}$. One can easily see
that if there is no inner ellipse $Y_1$ then $\Phi $ transforms one connected component of every line $\{\eta =\const\}$ to another and therefore for
$\beta <-n^{-\sigma }$ the inequality $\dist (z',\Phi ^k(z'))<\epsilon $ is impossible for odd $k$ and the measure of the set $\{|\beta |\le n^{-\sigma }\}$ is $O(n^{-\delta })$.

On the other hand, if there is an inner ellipse $Y_1$ then the map $\Phi $ preserves both connected components of $\eta =\const$ but changes their orientations, i.e., the map is of the form
$w_\eta \to {\frac{1}{2}}f(\eta )-w_\eta $ and therefore for odd $k$ the
$d\nu_\eta $-measure of points with
$\dist(z',\Phi ^kz')\le \varepsilon $ is $O(n^p\varepsilon )$.
Therefore \emph{in both cases only even $k$ should be treated}.

Furthermore, on every connected component map $\Phi ^2$ is of the form
$w_\eta \to w_\eta +f(\eta )$ where function $f$ is again continuous and
satisfies (\ref{11-3-13}), this time for
$|\eta |\ge a_2^{-1}+\epsilon_0$, i.e. $\beta \in (-\beta_0,0)$ with
small enough $\epsilon_0$ and $\beta_0$.

This function is analytic for $a_2^{-1} <|\eta |<b_2^{-1}$, i.e., for
$\beta \in (0,b_2^2-a_2^2)$, and the functions $f(\pm (b_2^{-1}-\zeta ^2))$ are analytic with respect to $\zeta $ with $|\zeta |\le \epsilon_0$. Therefore we obtain that (\ref{11-3-15}) and thus (\ref{11-3-14}) and (\ref{11-3-12}) remain true in this case.
\end{enumerate}
\end{proof}

\begin{example}\label{ex-11-3-11}
Let $X$ be an elliptical domain or domain between two confocal ellipses. Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-3-11-i}
If the boundary problem is regular then asymptotics (\ref{11-3-7}) holds for any $\vartheta\ge 0$.

\item\label{ex-11-3-11-ii}
We can allow singularities: transitions between different boundary value problems and cuts along some segments on semi-axis of the ellipses\footnote{\label{foot-11-22} One can show easily that the reflection from cuts does not violate power non-periodicity.}

Then the only condition to be checked is $\gamma^{-1-\vartheta}\in \sL^1(X)$ where $\gamma=\dist(x,\cK)$ and $\cK$ is the set of the cut ends and transition points. This condition again is equivalent to $\gamma^{-\vartheta}\in \sL^1(\partial X)$ and $|\log \gamma|\in \sL^1(\partial X)$ as $\vartheta=0$.
\end{enumerate}
\end{example}

\begin{example}\label{ex-11-3-12}
Let $X$ be a ball or domain between two concentric spheres in $\bR^d$.

Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-3-12-i}
If the boundary problem is regular then asymptotics (\ref{11-3-7}) holds for any $\vartheta\ge 0$.

\item\label{ex-11-3-12-ii}
We can allow singularities: transitions between different boundary value problems. Then the only condition to be checked is $\gamma^{-1-\vartheta}\in \sL^1(X)$ where $\gamma=\dist(x,\cK)$ and $\cK$ is the set of the cut ends and transition points. Again, this condition is equivalent to $\gamma^{-\vartheta}\in \sL^1(\partial X)$ for $\vartheta>0$ and
$|\log \gamma|\in \sL^1(\partial X)$ as $\vartheta=0$.
\end{enumerate}
\end{example}

There are many open problems:

\begin{Problem}\label{Problem-11-3-13}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{Problem-11-3-13-i}
Investigate domains bounded by one or two ellipses and one or two hyperbolas (all with the same foci).\enlargethispage{2\baselineskip}

\item\label{Problem-11-3-13-ii}
Investigate domains whose boundary consists of segments of ellipses and hyperbolas (all with the same foci); investigate if one can add cuts along some segments on semi-axis.

\item\label{Problem-11-3-13-iii}
Investigate ellipsoids of revolutions (i.e. with semi-axis $a_1=a_2=\dots=a_p=a> a_{p+1}=\ldots =a_{d}=b$) or domains between two confocal ellipsoids of revolution (with the obvious meaning).

\item\label{Problem-11-3-13-iv}
Investigate general ellipsoids.
\end{enumerate}
\end{Problem}

\paragraph{Miscellaneous remarks}\label{sect-11-3-1-3-3}

\begin{remark}\label{rem-11-3-14}
Since the billiard trajectories of the principal symbol $a^m$ coincide with those of $a$, all our discussion remains true for operators with the senior part $\Delta^m$.
\end{remark}

\begin{remark}\label{rem-11-3-15}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-3-15-i}
Billiard geodesic flow has power growth for certain Lie groups. One can easily see that in this case
\begin{equation*}
\upmu \bigl(\bigl\{z,\exists t\in [0,T]: \gamma (\Psi_t(z))\le \varepsilon \bigr\}\bigr)\le C\varepsilon ^\sigma T
\end{equation*}
and
$\upmu ({\cQ}_{T,\varepsilon})\le C\varepsilon T$ where
$\cQ_{T,\varepsilon}=\bigl\{z, \exists t\in [0,T]$ such that the distance from
$x$ to $\partial X$ and the angle between $\frac{dx}{dt}$ and
$T\partial X$ do not exceed $\epsilon \varepsilon $, and
$\gamma (\Psi_t(z))\ge \varepsilon \bigr\}$.

\item\label{rem-11-3-15-ii}
Billiard geodesic flow has power growth for manifolds with periodic geodesic flow (such manifolds can be either smooth or $\gamma$-admissible
with $\gamma ^{-1-\sigma }\in \sL^1(X)$ for arbitrarily small
$\sigma >0$). We will analyze them in the next subsection.

\item\item\label{rem-11-3-15-iii}
Recall that according to Theorem~\ref{thm-7-4-10} in Euclidean strongly convex domains with $\sC^3$-boundary geodesic billiard flow has (no more than) exponential growth. The same is true for compact Riemannian manifolds with geodesically strongly concave boundary and for compact closed Riemannian manifolds.
\end{enumerate}
\end{remark}

\begin{remark}\label{rem-11-3-16}
One can construct new manifolds of the corresponding
type by the following methods:

\begin{enumerate}[label=(\alph*), wide, labelindent=0pt]
\item\label{rem-11-3-16-a}
Taking a Cartesian product.

\item\label{rem-11-3-16-b}
 Taking a factor manifold of $X$ with respect to a finite group of
its isometries.

\item\label{rem-11-3-16-c}
Considering reflections, i.e., metric preserving diffeomorphisms
$S:\bar{X}\to \bar{X}$ such that $S^2=Id$ and $S(x)=x\implies dS(x)\ne dx$ ($X$ can have cuts so $S$ does not necessarily preserve $X$) and removing from $X$ some appropriate subset $K$ of the set of fixed points of $S$. The condition on $K$ is $\delta ^{-1-\sigma }\in \sL^1(X)$ for $\delta (x)=\dist (x,K)$.
\end{enumerate}
\end{remark}

\begin{remark}\label{rem-11-3-17}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-3-17-i}
Let us note that $\dist (z,\Psi_t(z))\asymp |t|$ for
$|t|\le \epsilon \gamma (x)$, $z=(x,\xi )$. Therefore the non-periodicity condition should be checked only for $|t|\ge \epsilon \varepsilon (T)$.

\item\label{rem-11-3-17-ii}
Let us consider the Cartesian product $X$ of two Riemannian manifolds $X'$
and $X''$ with dimensions $\ge 1$. Let us note that
$\Psi_t(x',x'',\xi ',\xi '')=
(\Psi'_{t|\xi '|}(x',\xi '),\Psi''_{t|\xi ''|}(x',\xi ''))$ for
$(x',x'',\xi ',\xi '') \in S^*X$.

Then, if inequality $\dist (z',\Psi_t(z'))\ge \varepsilon |t|$ is fulfilled for all $t\in (0,T)$ for a point $z'=(x',\xi_0')\in S^*X'$ then the same inequality with $\varepsilon^2$ instead of $\varepsilon $ is fulfilled for a point $(x',x'',\xi ',\xi '')\in S^*X$ with $\xi '=|\xi '|\xi '_0$ and
$|\xi'|\ge \varepsilon $.

Note that $\upmu\{(x,\xi):|\xi '|\le \varepsilon =O(\varepsilon)$. Therefore one should treat only points $(x',x'',\xi',\xi'')\in S^*X$ such that the non-periodicity condition is violated at both points
$z'=(x',\xi '|\xi '| ^{-1})\in S^*X'$ and
$z''=(x'',\xi ''|\xi ''| ^{-1})\in S^*X''$. Let
\begin{equation*}
T'=\min\bigl(t\ge\epsilon\varepsilon:\dist(z',\Psi'_t(z'))\le\varepsilon\bigr)
\end{equation*}
and let define $T''$ in a similar way. Recall that we can assume that $|\xi'|\ge\varepsilon$ and $|\xi''|\ge\varepsilon$. Then taking into
account condition on the Jacobi matrix we obtain that
$\dist (\Psi '_t(z'),z')\ge \varepsilon ^2$
provided $|\frac{t}{T'}-m|\ge \varepsilon $ $\forall m\in\bZ$ and
$|t|\le T$ (where $\varepsilon =\varepsilon (T)$. Therefore one needs
to estimate the measure of the set
\begin{multline*}
{\cQ}=\bigl\{\phi \in \bS^1: \exists m',m''\in \bZ:\\
|m'|\le \varepsilon ^{-\sigma }, |m''|\le \varepsilon ^{-\sigma },
|m'T'\cos \phi +m''T''\sin \phi| \le \varepsilon \bigr\}
\end{multline*}
where $\phi $ is associated with $\xi $ by the relations $|\xi '|=\cos \phi $,
$|\xi ''|=\sin \phi $ and one can take $\sigma >0$ arbitrarily small.
However, $\mes({\cQ}) =O(\varepsilon ^\sigma )$ obviously.

Therefore for Cartesian products the non-periodicity condition always
is fulfilled.


\item\label{rem-11-3-17-iii}
The above arguments also yield that
$\dist (G^*z,\Psi_t(z))\le \varepsilon ^2$ implies that
$\dist({G^*} ^kz,\Psi_{kt}(z))\le \varepsilon $ for constant $k$ and
the isometry $G^*:S^*\bar{X}\to S^*\bar{X}$ induced by the isometry
$G:\bar{X}\to \bar{X}$. Therefore Definition~\ref{def-11-3-6} is stable under
the above constructions of new manifolds in Remark~\ref{rem-11-3-16}\ref{rem-11-3-16-b} and \ref{rem-11-3-16-c} .
\end{enumerate}
\end{remark}


\subsection{Operators with periodic flows}%
\label{sect-11-3-2}
\index{large eigenvalue asymptotics!periodic trajectory}%
\index{asymptotics!large eigenvalue!periodic trajectory}

\subsubsection{Regular operators on closed manifolds}%
\label{sect-11-3-2-1}

Let us now consider a closed manifold $X$ and a scalar operator $A$ on $X$ with periodic Hamiltonian trajectories of the principal symbol. As before we assume that the manifold and operator are smooth enough; furthermore, as before we divide the operator $A$ by $\tau$, introduce $h=\tau^{-\frac{1}{2m}}$ and obtain an $h$-pseudodifferential operator. Then if all the Hamiltonian trajectories on the energy level  $\Sigma =\{a(x,\xi )=1\}$ are periodic with period $T_0$ then every trajectory is $T$-periodic with $T(x,\xi )=T_0a^{\frac{1}{2m}-1}(x,\xi )$ and then the Hamiltonian flow of the symbol $a^{\frac{1}{2m}}$ is $2mT_0$-periodic.

\emph{Without any loss of the generality we assume that} $2mT_0=1$. According to Section~\ref{sect-6-2} we must replace operator $A$ by operator
$\bar{A}=(\tau ^{-1}A)^{\frac{1}{2m}}$ (one should use this formula only in a neighborhood of $\Sigma$).

Then conditions (\ref{6-2-2}), (\ref{6-2-4}) and (\ref{6-2-7}) with $T_0=1$ are fulfilled with $\Omega_0\supset \Sigma $. Calculating the action by formula (\ref{6-2-6}) we obtain that $\alpha_1=0$ because symbol $\bar{a}$ is positively homogeneous of degree 1 on $\xi $. In what follows all the objects related to the operator $\bar{A}$ are denoted by the same letters as the corresponding objects related to $A$ but equipped with a bar. Then according to (\ref{6-2-12})
\begin{equation}
b_0 (x,\xi )=
{\frac{1}{2mT_0}}\int_0^{T_0}(a^s\circ\Psi_t)(x,\xi )dt -
{\frac{\pi \alpha_0}{2}} \qquad \text{on\ \ }\Sigma
\label{11-3-16}
\end{equation}
and is positively homogeneous of degree $0$ on $\xi $ in a neighborhood of $\Sigma $. Here $\alpha_0$ is the Maslov index.

Then results of Subsubsection \emph{\ref{sect-6-2-3}.3 \nameref{sect-6-2-3-3}\/} and Subsection~\ref{sect-6-4} yield

\begin{theorem}\label{thm-11-3-18}
Let $X$ be a closed compact $\sC^K$ manifold and $A$ an elliptic self-adjoint differential operator\footnote{\label{foot-11-23} Or a classical pseudodifferential operator.
In all cases we assume that $a\ge 0$.} of order $2m$. Let
the Hamiltonian flow of $a(x,\xi)$ be $T_0$-periodic on $\Sigma$.

Let ${\cL}$ be the image of the map
$\Sigma\ni(x,\xi)\to b(x,\xi) \overset{\iota}{\to} \bR/\mu \bZ$
where $\mu = \pi(mT_0)^{-1}$ and $\iota :\bR\to\bR/\mu \bZ$ is a
natural map. Assume ${\cL}$ does not coincide with $\bR/\mu \bZ$;
then $\iota ^{-1}{\cL}$ is a union of intervals $\{I_n\}$ of length
$O(1)$ such that $\omega \in I_n\implies |\omega |\asymp n$ for
$|n|\ge 1$.

It follows that
\begin{equation}
\Spec (A^{\frac{1}{2m}}) \subset \bigcup_{n\ge 1}J_n\cup [-C,C]
\label{11-3-17}
\end{equation}
where $J_n$ are the $Cn^{\delta-1}$-neighborhoods of $I_n$, $\delta >0$
is arbitrarily small and $C=C_\delta$; without loss of generality we assume that $A\ge I$.

Moreover, for $b_0=\const$ one can take $\delta =0$.
\end{theorem}

Theorems \ref{thm-6-3-6} and \ref{thm-6-3-12} yield then

\begin{theorem}\label{thm-11-3-19}
Let the conditions of Theorem~\ref{thm-11-3-18} be fulfilled and let $\omega_0 \in {\cL}$,
\begin{multline}
(x,\xi )\in \Sigma ,b_0(x,\xi )=\omega_0\implies
\text{either} \; \nabla_\Sigma b_0 (x,\xi )\ne 0\\
\text{or}\; \rank \Hess_{\Sigma} b_0 (x,\xi )\ge r.
\label{11-3-18}
\end{multline}
Further, let us assume that \underline{either} the Hamiltonian flow $\Psi_t$ has no subperiodic trajectory on $\Sigma$ \underline{or}
\begin{multline}
\dist \bigl(\Psi_t(x,\xi ),(x,\xi )\bigr)\ge
t(T_0-t)\rho (x,\xi ) \\
\forall t\in (0,T_0)\; (x,\xi )\in\Sigma
\label{11-3-19}
\end{multline}
where
\begin{multline}
|\nabla \rho |\le c\quad \text{and}\quad
\upmu \bigl\{(x,\xi ),\rho (x,\xi )\le h\bigr\} = O(h^q)\quad
\text{as\ }h\to +0.
\label{11-3-20}
\end{multline}

Then for $\tau \to+\infty $ such that
$|\iota \tau ^{\frac{1}{2m}}-\omega_0|\le \epsilon_0$ (where $\epsilon_0>0$ is small enough) asymptotics
\begin{equation}
\N^- (\tau )=\varkappa_0\tau ^{\frac{d}{2m}}+
\bigl(\varkappa_1+F(\tau ^{\frac{1}{2m}})\bigr)\tau ^{\frac{d-1}{2m}}+
O\bigl(\tau ^{\frac{d-1-p}{2m}}\bigr)
\label{11-3-21}
\end{equation}
holds with
\begin{equation}
F(z)=(2mT_0)^{-1}(2\pi )^{-d}\int_\Sigma \Upsilon
\Bigl(2mT_0\bigl(z-b (x,\xi )\bigr)\Bigr)dxd\xi :da,
\label{11-3-22}
\end{equation}
$p=\min (1, \frac{r}{2} -\delta , \frac{q}{2} -\delta )$ with an arbitrary
small exponent $\delta >0$. Here and below $\Upsilon (z)$ is a
$2\pi $-periodic function on $\bR$ equal to $\pi -z$ on $[0,2\pi )$.
\end{theorem}

The following should be rather easy:

\begin{problem}\label{problem-11-3-20}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-3-20-i}
Show that for generic differential and pseudodifferential symbols $a^s$ condition (\ref{11-3-18}) is fulfilled with $r=2d-2$ for all $\omega_0$. In fact the function $b_0(x,\xi )$ is given \emph{on}
$\Sigma '=\Sigma /\Psi_t$ (the factor of $\Sigma $ with respect to
the Hamiltonian flow) which is a $2d-2$-dimensional manifold
\emph{rather than on} $\Sigma$.

\item\label{problem-11-3-20-ii}
 Derive more precise asymptotics are possible as well and improved asymptotics of $\N^-_{(\vartheta)}(\tau)$ with remainder estimates which could be as good as $O(\tau^{(d-2-2\vartheta)/2m})$ (under an appropriate non-degeneracy condition).
\end{enumerate}
\end{problem}

Surely, Theorem~\ref{thm-11-3-19} is applicable to a Laplace-Beltrami operator on a Riemannian manifold with periodic geodesic flow which is perturbed by a first-order operator. For a generic vector $(V_1,\dots ,V_d)$ the field corresponding to the perturbation condition (\ref{11-3-18}) is fulfilled with $r=2d-2$.

In particular, for the Laplace-Beltrami operator on the standard sphere%
\index{Laplace-Beltrami operator!on the sphere}%
\index{operator!Laplace-Beltrami!on the sphere}%
\index{large eigenvalue asymptotics!sphere Laplace-Beltrami operator}%
\index{asymptotics!large eigenvalue!sphere Laplace-Beltrami operator}
$\bS^d$ one can see easily that $\alpha_0\equiv 2(d-1) \mod 4\bZ$ and $T_0=\pi$. Let us consider this operator with perturbation more carefully. Let
$j:\bS^d\to \bS^d$ be the antipodal map $x\to -x$ and let
$j^*:S^*\bS^d\to S^*\bS^d$ be the adjoint map $(x,\xi)\to (-x,-\xi)$. Then (\ref{11-3-16}) yields that $b_0$ depends only on the even part of $a^s$: $a^s_\even = \frac{1}{2} (a^s+a^s\circ j^*)$.
Let us now assume that $a^s$ is skew-symmetric with respect to $j^*$:
\begin{equation}
a^s=-a^s\circ j^*.
\label{11-3-23}
\end{equation}
Then $b_0=0$ and $B$ is a $(-1)$-order operator (i.e.,
$\eta =h=\tau ^{-\frac{1}{2}}$: see Section~\ref{sect-6-2}). Let us calculate then the principal symbol $b_{-1}$ of the operator $B$. Given that the eigenvalues of unperturbed Laplace-Beltrami $A_0$ on $\bS^d$ are $n(n+d-1)$ with $n\in \bZ^+$ it will be more convenient for us to set
\begin{equation}
\bar{A}=h\Bigl(\bigl(A+\frac{1}{4}(d-1)^2\bigr)^{\frac{1}{2}}-
\frac{1}{2}(d-1)\Bigr)
\label{11-3-24}
\end{equation}
here instead of $\bar{A}=A^{\frac{1}{2}}$. Let
\begin{equation}
\bar{A}_0=h\Bigl(\bigl(A_0+\frac{1}{4}(d-1)^2\bigr)^{\frac{1}{2}}-
\frac{1}{2}(d-1)\Bigr)
\label{11-3-25}
\end{equation}
be the corresponding unperturbed operator.

Let $U(t)=\exp (ih^{-1}t\bar{A})$ and $U_0(t)=\exp (ih^{-1}t\bar{A}_0)$. Then
\begin{equation}
U_0(2\pi )=I,\qquad U_0(\pi )=J\quad\text{where\ \ } Jv=v\circ j.
\label{11-3-26}
\end{equation}
So \emph{we want to calculate $U(2\pi)$ modulo operators of order} $(-2)$ because near $\Sigma $ the orders in the sense of standard pseudodifferential operators and in the sense of $h$-pseudodifferential operators coincide. Let us calculate $U(\pi)J$ modulo operators of order $(-1)$ first. To do it we consider
$V(t)=U(t)U_0(-t)$ which is a standard ($h$-)pseudodifferential
operator. Then
\begin{equation*}
\frac{d\ }{dt} V(t)=ih^{-1}U(t)(\bar{A}-\bar{A}_0)U_0(-t)= iV(t)U_0(t)Q U_0(-t)
\end{equation*}
where $Q=h^{-1}(\bar{A}-\bar{A}_0)$ is an operator of order $0$.
Considering principal symbols we obtain that
$\partial_tv=iv(b\circ \Psi_t)$. Since $v|_{t=0}=1$ we obtain that
\begin{equation*}
v(t)=\exp (-i\int_0^t l\circ\Psi_{t'}\,dt')
\end{equation*}
where $q= \frac{1}{2} a^sa^{-\frac{1}{2}}$ is the principal symbol of
$Q$. Therefore (\ref{11-3-26}) yields that

\begin{claim}\label{11-3-27}
$U(\pi)J$ is an $h$-pseudodifferential operator with the principal symbol
$\exp (i\zeta \cdot \int_0^{\pi }q \circ \Psi_t\,dt)$
\end{claim}
with $\zeta=1$.

Let us consider operator $\bar{A}_\zeta =\bar{A}_0+\zeta hQ$ and let us consider the corresponding unitary group $U_\zeta (t)$. Differentiating equalities
\begin{equation*}
(hD_t-\bar{A}_\zeta )U_\zeta (t)=0,\qquad U_\zeta (0)=I
\end{equation*}
with respect to $\zeta $ we obtain that
\begin{equation*}
(hD_t-\bar{A}_\zeta )U'_\zeta (t)=hQ U_\zeta ,\qquad U'_\zeta (0)=0
\end{equation*}
where the prime means the derivative with respect to $\zeta $. Then
\begin{equation*}
U'_\zeta (t)=i\int_0^tU_\zeta (t-t')QU_\zeta (t')\,dt'.
\end{equation*}
Let us set $t=2\pi $ and divide interval $[0,2\pi ]$ of integration into subintervals $[0,\pi ]$ and $[\pi ,2\pi ]$ and replace $t'$ by $t$ in the first subinterval and by $t+\pi $ in the second one. We obtain that
\begin{equation}
U'_\zeta (2\pi )=
iU_\zeta (2\pi )\int_0 ^\pi U_\zeta (-t)\tilde{Q}U_\zeta (t)\,dt
\label{11-3-28}
\end{equation}
with $\tilde{Q}=Q+U_\zeta (-\pi )QU_\zeta (\pi )$. We know that
$U_\zeta (\pi )=V_\zeta J$ and $U_\zeta (-\pi )=JV_\zeta ^*$ where
$V_\zeta$ is a unitary operator. Therefore
\begin{equation*}
\tilde{Q}=Q+JQJ+JV_\zeta ^*[Q,V_\zeta ]J.
\end{equation*}
Then (\ref{11-3-23}) yields that $\tilde{Q}$ is an operator of order
$(-1)$ with the principal symbol
\begin{equation*}
\tilde{q}=2q_{\even}+\zeta \{q,\int_0 ^\pi q\circ \Psi_{t'}\,dt'\}
\end{equation*}
where $q_{\even}$ is the even (with respect to $j^*$) part of $q^s$ and the second term is also even. Therefore (\ref{11-3-28}) yields that
$-iU_\zeta (-2\pi )U'_\zeta (2\pi )$ is an operator of order $(-1)$
with principal symbol
\begin{equation*}
\int_0 ^\pi \tilde{q}\circ \Psi_{-t}\,dt=
\int_0^{2\pi }q^s\circ \Psi_t\,dt+
\zeta \int_0^{\pi }\int_0^{\pi }\{q\circ \Psi_t,q\circ\Psi_{t+t'}\}\,dtdt'
\end{equation*}
where we changed variables in the integration in the obvious way. Integrating over $\zeta \in [0,1]$ we obtain that
\begin{claim}\label{11-3-29}
$U(2\pi )-I$ is an operator of order $(-1)$ with principal symbol $2\pi ib_{-1}$ where
\begin{equation}
b_{-1}={\frac{1}{2\pi }}\bigl(\int_0^{2\pi }q^s\Psi_tdt +
\int_0^{\pi }\!\int_0^{\pi }\{q\circ \Psi_t,q\circ \Psi_{t+t'}\}
\,dtdt'\bigr).
\label{11-3-30}
\end{equation}
\end{claim}

Now theorems \ref{thm-6-3-6} and \ref{thm-6-3-12} yield

\begin{theorem}\label{thm-11-3-21}
Let $A=\Delta +A'+A''$ where $\Delta$ is the (positive) Laplace-Beltrami operator on the standard sphere $\bS^d$, $A'=A'(x,D)$ and $A''=A''(x,D)$ are symmetric operators of first and zero order respectively and $A'$ anti-commutes with $J$ (in which case $a^s$ satisfies \textup{(\ref{11-3-23})}). Let $b_{-1}(x,\xi )$ be defined by \textup{(\ref{11-3-30})} with $q={\frac{1}{2}}a'a^{-\frac{1}{2}}$,
$q^s=\frac{1}{2}a''a^{-\frac{1}{2}}-{\frac{1}{8}}a'{^2}a^{-\frac{3}{2}}$
where $a'$ and $a''$ are the principal symbols of $A'$ and $A''$
respectively.

Let ${\cL}'=[\lambda_1,\lambda_2]$ be the image of the map
$\Sigma \ni (x,\xi )\to b_{-1}(x,\xi )\in\bR$ and let
$f(\tau )=\bigl(\tau +\frac{1}{4}(d-1)^2\bigr)^{\frac{1}{2}}-\frac{1}{2}(d-1)$.
Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-3-21-i}
$f(\Spec A)\subset \bigcup_{n\ge 1}J'_n\cup[-C,C]$ where
\begin{equation}
J'_n=\bigl[n+\lambda_1n^{-1}-Cn^{\delta -2},
n+\lambda_2n^{-1}+Cn^{\delta -2}\bigr],
\label{11-3-31}
\end{equation}
$C=C(\delta )$ is large enough, $\delta >0$ is arbitrarily small and for $\lambda_1=\lambda_2$ one can take $\delta =0$.


\item\label{thm-11-3-21-ii}
Let $\omega_1\in {\cL}'$ and condition \textup{(\ref{11-3-18})} be
fulfilled with $\omega_1$ and $b_{-1}$ instead of $\omega_0$
and $b_0$. Then for $\tau \to +\infty $ such that
\begin{equation*}
f(\tau )\subset\bigcup_{n\ge 1}[n+(\omega_1-\epsilon ){\frac{1}{n}},
n+(\omega_1+\epsilon ){\frac{1}{n}}]
\end{equation*}
with a sufficiently small
constant $\epsilon >0$ asymptotics
\begin{equation}
\N^- (\tau )=\varkappa_0\tau ^{\frac{d}{2}}+
\varkappa_1\tau ^{\frac{d-1}{2}}+F(f(\tau ),\tau )\tau ^{\frac{d-1}{2}}+
O\bigl(\tau ^{\frac{d-1-p}{2}}\bigr)
\label{11-3-32}
\end{equation}
holds with $p=\min(1,{\frac{r}{2}}-\delta )$ with an arbitrarily small
exponent $\delta >0$ and with
\begin{equation}
F(z,\tau )= 2(2\pi )^{-d-1}\int_\Sigma \Upsilon
\Bigl(2\pi \bigl(z-\tau ^{-{\frac{1}{2}}}b_{-1}(x,\xi )\bigr)\Bigr)\,dxd\xi :da.
\label{11-3-33}
\end{equation}
\end{enumerate}
\end{theorem}

The following seems to be easy:

\begin{problem}\label{problem-11-3-22}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-3-22-i}
Prove that for an arbitrary fixed symbol $a''$ and for a generic differential symbol (i.e., vector field) as well as for a generic pseudodifferential symbol $a'$ satisfying (\ref{11-3-23}) the modified\footnote{\label{foot-11-24} I.e., with $\omega_1,b_{-1}$ instead of $\omega_0,b_0$.} condition (\ref{11-3-18}) is fulfilled with $r=2d-2$ for all $\omega_1\in\bR$.

\item\label{problem-11-3-22-ii}
Prove that the same is true for an arbitrary fixed $a''$ satisfying (\ref{11-3-23}) and for a generic differential symbol (i.e., potential) as well as for a generic pseudodifferential symbol $a''$.
\end{enumerate}
\end{problem}

Let us now assume that
\begin{equation}
a'=0,\quad a''\circ j^*=-a''.
\label{11-3-34}
\end{equation}
Then $b_{-1}=0$ and the operator $U(2\pi )-I$ obviously is an operator of order $\le -2$ (we will prove that its order is actually $(-3)$) and our goal is to calculate its principal symbol. Now the calculations are simpler because the perturbation is weaker. Let $\bar{A}$ and $\bar{A}_0$ be defined as above. Then
$\bar{A}=\bar{A}_0+Q'+Q''$\,\footnote{\label{foot-11-25} For the sake of
simplicity we do not write the factor $\tau^{-\frac{1}{2}}$ which in any case is reduced in the final formula.}
where $Q'$ is an operator of order $(-1)$ with principal symbol
$q'=-{\frac{1}{2}}a^{-{\frac{1}{2}}}a''$ anti-commuting with $J$ and $Q''$
is an operator of order $(-3)$ with principal symbol
$q''=-{\frac{1}{8}}a^{-{\frac{3}{2}}}{a''}^{2}$\,\footnote{\label{foot-11-26} In contrast with the above case we did not include a lower order operator
commuting with $J$ in $A$ because we are mainly interested in
differential operators. This generalization is left to the reader.}.
Then the equalities
\begin{equation*}
(D_t-\bar{A}_0)U(t)=QU(t),\qquad U(0)=I
\end{equation*}
with $Q=Q'+Q''$ yield that
\begin{equation*}
U(t)=U_0(t)+i\int_0^tU(t-t')QU(t')\,dt'
\end{equation*}
(this is similar to the calculation of $V$). After iteration we obtain $U(t)$ as an asymptotic series of operators with order decreasing by step $1$. Let us set $t=2\pi $. We then obtain that modulo operators of order $(-4)$
\begin{multline}
U(t)\equiv I+i\int_0^{2\pi }Q(t_1)\,dt_1-
\iint_{\Pi_2}Q(t_1)Q(t_2)\,dt_1dt_2-\\[2pt] i\iiint_{\Pi_3}Q(t_1)Q(t_2)Q(t_3)\,dt_1dt_2dt_3
\label{11-3-35}
\end{multline}
with
$\Pi_k= \{t=(t_1,\dots ,t_k)\in\bR^k,0\le t_1\le \dots \le t_k\le 2\pi \}$
and $Q(t)=U_0(-t)QU_0(t)$. Moreover, in the third and fourth terms we can replace $Q$ by $Q'$.

Dividing the interval of integration in the second term into subintervals $[0,\pi ]$ and $[\pi ,2\pi ]$ and replacing $t_1$ by $t$ and $t+\pi $ on these subintervals respectively we obtain that this term is a pseudodifferential operator with principal symbol $i\int_0^{2\pi }q''\circ \Psi_t\,dt$.

The third term in the right-hand expression is equal to
\begin{equation*}
-{\frac{1}{2}}
\iint_{\Pi_2}\bigl(Q(t_1)Q(t_2)+Q(t_2)Q(t_1)\bigr)\,dt_1dt_2-
{\frac{1}{2}}\iint_{\Pi_2}[Q(t_1),Q(t_2)]\,dt_1dt_2.
\end{equation*}
The first term here equals half of $-Q(t_1)Q(t_2)$ integrated over the square $(t_1,t_2)\in [0,2\pi ]^2$; therefore it is equal to
$-{\frac{1}{2}}(\int_0 ^{2\pi }Q(t)dt)^2$ and therefore is negligible as its principal symbol is $0$.

The second term is an operator of order $(-3)$ and after simple calculations we obtain that its principal symbol is
\begin{equation*}
i\int_0^\pi\int_0^\pi \{q\circ \Psi_t,q\circ \Phi_{t+t'}\}\,dtdt'.
\end{equation*}
Finally, the third term in (\ref{11-3-35}) is obviously an operator of order $(-3)$. Making permutations of $(t_1,t_2,t_3)$ and summing we obtain that modulo an operator of order $(-4)$ this term is one-sixth of $Q(t_1)Q(t_2)Q(t_3)$ integrated over the cube $[0,2\pi ]^3$ and is therefore negligible.

Thus,
\begin{claim}\label{11-3-36}
$(U(2\pi )-I)$ is an operator of order $(-3)$ with the principal symbol
$2\pi ib_{-3}(x,\xi )$ where $b_{-3}$ is given by (\ref{11-3-30}) with $q'={\frac{1}{2}}a''a^{-{\frac{1}{2}}}$ and
$q''=-{\frac{1}{8}}a''{^2}a^{-{\frac{3}{2}}}$ instead of $q$ and $q^s$ respectively.
\end{claim}

Therefore Theorem~\ref{thm-6-2-3} yields

\begin{theorem}\label{thm-11-3-23}
Suppose that conditions of Theorem~\ref{thm-11-3-21} and condition \textup{(\ref{11-3-34})} are fulfilled. Let
${\cL}''=[\lambda_1,\lambda_2]$ be the image of the map
$\Sigma \ni (x,\xi )\to b_{-3}(x,\xi )\in\bR$. Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-3-23-i}
$f(\Spec A)\subset \bigcup_{n\ge 1}J''_n\cup[-C,C]$ where
\begin{equation}
J''_n=\bigl[n+\lambda_1n^{-3}-Cn^{\delta -4},
n+\lambda_2n^{-3}+Cn^{\delta -4}\bigr],
\label{11-3-37}
\end{equation}
$C=C(\delta )$ is small enough, $\delta >0$ is arbitrarily small and
for $\lambda_1=\lambda_2$ one can take $\delta =0$.

\item\label{thm-11-3-23-ii}
Let $\omega_2\in {\cL}''$ and condition \textup{(\ref{11-3-18})} be fulfilled with $\omega_2$ and $b_{-3}$ instead of $\omega_0$ and $b_0$. Then for $\tau \to +\infty $ such that
\begin{equation*}
f(\tau )\subset\bigcup_{n\ge 1}[n+(\omega_2-\epsilon )n^{-3},
n+(\omega_2+\epsilon )n^{-3}]
\end{equation*}
with a sufficiently small constant $\epsilon >0$ asymptotics \textup{(\ref{11-3-32})} holds with the same $p$ as above and with
\begin{equation}
F(z,\tau )= 2(2\pi )^{-d-1}\int_\Sigma \Upsilon
\Bigl(2\pi \bigl(z-\tau ^{-{\frac{3}{4}}}b_{-3}(x,\xi )\bigr)\Bigr)
\,dxd\xi :da.
\label{11-3-38}
\end{equation}
\end{enumerate}
\end{theorem}

We leave to the reader

\begin{problem}\label{problem-11-3-24}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-3-24-i}
Prove that for a generic differential symbol (i.e., potential) as well as for a generic pseudodifferential symbol $a''$ satisfying (\ref{11-3-34}) the modified\footnote{\label{foot-11-27} I.e., with $\omega_2,b_{-3}$ instead of $\omega_0,b_0$.} condition (\ref{11-3-18}) is fulfilled with $r=2d-2$ for all $\omega_2\in\bR$.

\item\label{problem-11-3-24-ii}
Thus, in all the above cases for generic perturbations the remainder estimate is $O\bigl(\tau^{\frac{d-2}{2}}\bigr)$ for $d\ge 3$
and $O\bigl(\tau^{{\frac{1}{2}}(d-2+\delta)}\bigr)$ with an arbitrarily
small exponent $\delta >0$ for $d=2$. Applying the more precise results of Section~\ref{sect-6-2} we obtain that for $d=2$ the remainder estimate is
$O(1)$ if the principal symbol $b$ has no saddle points at the
corresponding level and $O(\log\tau)$ otherwise.

\item\label{problem-11-3-24-iii}
Derive the remainder estimate $O(1)$ in the latter case as well by including in the principal symbol the next symbol too (as we have seen it does
not necessarily vanish even if the principal symbol vanishes
identically).

\item\label{problem-11-3-24-iv} Consider Riesz means asymptotics to the reader. Recall that the best possible remainder estimate is $O\bigl(\tau ^{{\frac{1}{2}}(d-1-n\vartheta )}\bigr)$ where $n=0,1,3$
is the order of $B$ taken with the opposite sign.
\end{enumerate}
\end{problem}

\subsection{Singular operators on closed manifolds}%
\label{sect-11-3-3}

Let us now consider the singular case when not only an operator but also a manifold itself has singularities. Singularities are described by scaling function $\gamma(x)$:

\begin{definition}\label{def-11-3-25}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{def-11-2-25-i}
Let $X$ be a Riemannian manifold (with or without boundary) such that $\bar{X}$ a closure of $X$ in the Riemannian metrics is compact. Then we call $X$ \emph{singular compact Riemannian manifold\/}.

\item\label{def-11-3-25-ii}
If the regular part of the boundary is empty, we call $X$
\emph{singular compact closed Riemannian manifold\/}.


\item\label{def-11-3-25-iii}
Let $\gamma$ be a scaling function on $\bar{X}$, such that $|\gamma(x,y)\le \frac{1}{2}\dist (x,y)$, $\partial X=\{x,\gamma(x)=0\}$, $X=\{x,\gamma(x)>0\}$ and let metrics on $X$ be $\gamma$-admissible. Then we call $X$ (singular)
\emph{$\gamma $-admissible compact Riemannian manifold\/}.
\end{enumerate}
\end{definition}

However we will need also a $\gamma$-admissible function $\zeta(x,\xi)$ describing how close trajectory $\Psi_t(x,\xi)$ can approach $\{\gamma =0\}$ (see condition (\ref{11-3-39}) below):

\begin{theorem}\label{thm-11-3-26}
Let $X$ be a $\gamma $-admissible compact closed Riemannian manifold, $A$ a scalar elliptic $\gamma $-admissible operator of order $2m$ with the lower order
terms satisfying the standard conditions of this section. Let us assume that $\gamma ^{-1-\delta }\in \sL^1(X)$ with $\delta >0$.

Further, let us assume that the Hamiltonian flow of $a(x,\xi )$ is
$T_0$-periodic on $\Sigma $. Furthermore, let us assume that a
$\gamma $-admissible bounded function $\zeta $ is given on
$\Sigma $ such that
\begin{equation}
|D\Psi_t(z)|\le C\zeta ^{-n}(z),\quad \gamma (\Psi_t(z))\ge \epsilon
\zeta ^n(z) \qquad \forall z\in\Sigma \quad \forall t.
\label{11-3-39}
\end{equation}
Finally, let us assume that conditions \textup{(\ref{11-3-18})} with $r\ge 1$ (for some fixed $\omega_0$) and \textup{(\ref{11-3-19})}--\textup{(\ref{11-3-20})} (which is condition to subperiodic trajectories) with $q>0$ are fulfilled.

Then for $\tau \to +\infty $ such that
$|\iota \tau ^{\frac{1}{2m}}-\omega_0|\le \epsilon $ asymptotics
\textup{(\ref{11-3-21})} holds with sufficiently small exponent $p>0$.
\end{theorem}

\begin{proof}
Dividing $\Sigma $ into the zones
$\{\zeta \ge {\frac{1}{2}}\tau ^{-\delta }\}$ and
$\{\zeta \le \tau ^{-\delta }\}$ we can apply results of Section~\ref{sect-6-2} in the former zone and the standard asymptotics in the latter one.
\end{proof}

\begin{Problem}\label{Problem-11-3-27}
We derived asymptotics which is marginally better than the standard one only as $\vartheta \le p$. The problem which is definitely rather difficult and very interesting is to derive asymptotics with the better remainder estimates; ideally one should derive asymptotics with the remainder estimates which are as good as in the regular case (surely one needs to impose more restricting conditions).
\end{Problem}

\begin{example}\label{ex-11-3-28}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-3-28-i}
Consider \emph{Zoll-Tannery manifold\/}\index{Zoll-Tanner manifold} with the rotational symmetry (see Example~\ref{ex-8-3-9}\ref{ex-8-3-9-iii}. Recall that
these manifolds are isometric (up to a factor) to a sphere $\bS^d$ with the metrics $(r+h(\cos(s)))^2\,ds^2 + \sin^2(s)\,d\theta^2$ with $s\in [0,\pi]$, $r=p/q$, $p,q\in \bN$, $\gcd (p,q)=1$ and odd function $h: (-1,1)\to (-r,r)$. Then the length of equator is $2\pi$, the length of meridian $2\pi r$ and the length of general geodesics $2\pi p$. See A.~Besse~\cite{besse:geodesic}, Theorem 4.13.

Then $T_0=2\pi q$. Therefore one can take $A=\Delta^m$ (plus lower order terms) where $\Delta$ is the Laplace-Beltrami operator; these lower order terms must satisfy the standard assumptions of this section and also provide condition (\ref{11-3-12}) with $p\ge 1$. Singularities (if there are any) are located at $s=0,\pi$.

However these singularities do not prevent us from recovering remainder estimate $O(\tau^{(d-2)/2m})$ as long as non-degeneracy condition to the lower order terms is fulfilled. This asymptotics contains non-Weyl correction term.

\item\label{ex-11-3-28-ii}
Consider the same example replace rational $r$ by irrational $r$;
then we are basically in the framework of the Subsection~\ref{sect-11-3-1} and can recover remainder estimate $O(\tau^{(d-1)/2m-\delta})$ without any condition to the lower order terms.
\end{enumerate}
\end{example}


Repeating the arguments of Theorems~\ref{thm-11-3-21} and~\ref{thm-11-3-26} we can generalize them to operators with the singular perturbations on $\bS^d$.

\begin{remark}\label{rem-11-3-29}
Let us consider the Laplace-Beltrami operator of Example~\ref{ex-11-3-28} perturbed by a potential $V\in \sL^s$ such that $\| V\|_{\sL_s}<\epsilon $ with $s>d=2$ or $s=d\ge 3$. Then the standard functional-analytic arguments yield that the cluster
character of the spectrum remains true. The size of a cluster is
$O(\epsilon \tau ^{\frac{d}{2s}})$ and the distance between clusters is
$\asymp \tau ^{\frac{1}{2}}$; here $\epsilon =\|V\|_{\sL^s}$ is assumed
to be small only for $s=d$.
\end{remark}

\subsection{Manifolds with the boundary}%
\label{sect-11-3-4}

The possibility of singularities increases the possibilities even if the boundary is smooth.

\begin{example}\label{ex-11-2-30}
Consider manifolds of Example~\ref{ex-8-3-9} which have boundaries (and these boundaries may also have singularities). Therefore one can take $A=\Delta^m$ (plus lower order terms) where $\Delta$ is the Laplace-Beltrami operator with the appropriate boundary conditions.

Then
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-3-30-i}
If $r$ is rational the lower order terms and boundary conditions must satisfy the standard assumptions of this section and also provide condition (\ref{11-3-12}) with $p\ge 1$.
Then asymptotics with remainder estimate $O(\tau^{(d-1)/2m-\delta})$ holds; this asymptotics contains non-Weyl correction term.

\item\label{ex-11-3-30-ii}
If $r$ is irrational we can recover remainder estimate $O(\tau^{(d-1)/2m-\delta})$ without any condition to the lower order terms and boundary conditions.
\end{enumerate}
\end{example}

\subsection{The indefinite case}%
\label{sect-11-3-5}
\index{indefinite operator}%
\index{operator!indefinite}%
\index{large eigenvalue asymptotics!indefinite operator}%
\index{asymptotics!large eigenvalue!indefinite operator}

In this subsection we discuss the case when the principal symbol is neither positive nor negative definite. We assume that the lower order terms are appropriate: conditions on these terms will be discussed in the next Subsection~\ref{sect-11-3-6}.

All the results of Sections~\ref{sect-11-2} and \ref{sect-11-3} remain true for operators with elliptic principal symbols which are neither positive nor
negative definite. In this case $\N^- (\tau )$ is the number of eigenvalues
in the interval $(0,\tau )$ for $\tau >0$ and $\N^+(\tau)$ is the number of eigenvalues in the interval $(\tau ,0)$ for $\tau <0$ and we consider asymptotics of $\N^\mp(\tau)$ for $\tau \to \pm \infty $.

Surely, for $\tau \to+\infty $ and for $\tau \to-\infty $ we may obtain different asymptotics and the conditions on Hamiltonian trajectories may be different; however in two most interesting examples -- Dirac and Maxwell operators (see Example~\ref{ex-8-4-4}) results should be the same modulo remainder estimate and equal to $\frac{1}{2}\N^- (A^2-\tau^2 )$; this would make those results look trivial.

However it is not the case, at least not for the Maxwell operator which should be considered on the subspace defined by under-defined system and as domain is irregular (for example, if it has edges directed inside, like in $(\bR^d\setminus \bR^{+\,2}\times \bR^{d-2})$) one should be really careful ; in particular formally Maxwell system and system of hydrodynamics\footnote{\label{foot-11-28} Without viscosity.} look the same but in such domains results are different. So, we suggest very difficult and interesting problem

\begin{Problem}\label{Problem-11-3-31}
Accurate analysis with the results of the same sharpness as in this Sections \ref{sect-11-2} and \ref{sect-11-3} for
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{Problem-11-3-31-i}
Maxwell system:
\begin{enumerate}[label=(\alph*), leftmargin=*]
\item\label{Problem-11-3-31-ia}
 isotropic (already difficult);
\item\label{Problem-11-3-31-ib}
anisotropic (much more difficult);
\end{enumerate}
\item\label{Problem-11-3-31-ii}
System of hydrodynamics\footref{foot-11-28}.
\end{enumerate}
\end{Problem}

Further, all the results for $\vartheta >0$ remain true if we set
\begin{equation}
\N^\mp_{(\vartheta)} (\tau )=
\pm \int_0 ^\tau |\tau' |^{\vartheta -1}N(\tau ')d\tau '
\label{11-3-40}
\end{equation}
for $\pm \tau >0$.

Furthermore, the results of Subsection~\ref{11-2-3} should remain true. In this case (instead of the assumption that $A(x,D )$ is a scalar operator) we assume that $a(x,\xi )$ has only one positive (or negative) eigenvalue
$\lambda (x,\xi )$ which is simple provided we treat asymptotics as
$\tau \to +\infty $ ($\tau \to -\infty $ respectively). In this case all the conditions of these subsections are assumed to be fulfilled for the Hamiltonian flow generated by $\lambda (x,\xi )$.

Moreover, to obtain conditions on
lower order terms one should find pseudodifferential operator $Q$
such that
\begin{equation*}
Q^*Q\equiv QQ^*\equiv I\qquad\text{and}\qquad
Q^*AQ\equiv \begin{pmatrix} A_1 &0\\ 0 &A_2\end{pmatrix}
\end{equation*}
where $A_1$ is a scalar operator with principal symbol $\lambda (x,\xi )$ and $A_2$ an operator with principal symbol of the opposite sign. Then all the conditions should be imposed on the lower order terms of $A_1$.

Moreover, we can treat the Dirac operator; nevertheless the eigenvalues of its principal symbol are simple only for $D=2\implies d=1,2,3$ (for $d=3$ one has a principally massless particle). However, one needs to check that all the symbols associated with $A_1$ and taken into account are scalar. Similar notes remain true for isotropic Maxwell and hydrodynamics systems and I suggest another very difficult and interesting problem

\begin{Problem}\label{Problem-11-3-32}
Accurate analysis with the results of the same sharpness as in this subsection \ref{sect-11-3-2} for

\begin{enumerate}[label=(\roman*), leftmargin=*]
\item Dirac operator;
\item Isotropic Maxwell system;
\item System of hydrodynamics\footref{foot-11-28};
\end{enumerate}
\end{Problem}

In order to prove the above statements one should apply the results of Part~\ref{part-2} to the interval $(\frac{1}{2}\tau ,\tau )$ (we consider the case $\tau >0$ for the sake of simplicity). Then the routine remainder estimate $O(\tau ^\nu )$ or $O(\tau ^\nu \log ^{\sigma } \tau)$ is obtained by standard methods. Let us replace $\tau $ by $2^{-j}\tau $ (with $j=0,\dots ,n$ such that $\tau \asymp 2^n$) and sum all these asymptotics; then we obtain asymptotics for the number of eigenvalues lying in $(\tau_1,\tau )$ with the same remainder
estimate for $\nu >0$ and with the remainder estimate $O(\log^{\sigma +1}\tau )$ for $\nu =0, \sigma \ge 0$. On the other hand it is relatively easy to prove that $\N (0,\tau_1)<\infty $.

Moreover, in order to improve the final remainder estimate in the case when it grows slowly, one can apply the following arguments to obtain the remainder estimate $O(\tau ^{-s})$ with arbitrarily chosen $s$ for mollifications of
$\N (\tau ',\tau '')$ (the number of eigenvalues in the interval
$(\tau ',\tau '')$) with respect to $\tau '$ and $\tau ''$ with mollifying functions $\tau ^{-1}\phi_1(\tau ' \tau ^{-1})$ and
$\tau ^{-1}\phi_2(\tau '' \tau ^{-1})$ where $\phi_1$ and $\phi_2$ are supported near $\frac{1}{2}$ and $1$ respectively. Replacing $\tau $ by $2^{-j}\tau $ and making a partition of unity one obtains the remainder estimate $O(1)$ for $\N (0,\tau ')$ mollified near $\frac{1}{2}\tau $. On the other hand,
for $N(\tau ',\tau )$ (even without mollification) we have the appropriate remainder estimate provided $\tau '\asymp \tau $.

So, semiclassical arguments look rather straightforward but there is also analysis in the singular zone and for indefinite operators it may become rather non-trivial. For $\vartheta >0$ one can apply analysis of the same type.


\subsection{Conditions to lower order terms}
\label{sect-11-3-6}

Let us discuss conditions to the lower order terms starting from a series of remarks:

\begin{remark}\label{rem-11-3-33}
All our results were proven for $(\rho,\gamma)$-admissible lower order terms provided
\begin{gather}
\rho ^{d+2m\vartheta }\in \sL^1(X),\label{11-3-41}\\
\rho ^{2m}\in \sL^1(X),\label{11-3-42}\\
\rho ^{2m}\in \sL^2(X),
\tag*{$\textup{(\ref*{11-3-42})}^*$}\label{11-3-42-*}
\end{gather}
where (\ref{11-3-42}) and \ref{11-3-42-*} are conditions in the semi-bounded
and non-semi\-bounded cases respectively. Here $2m$ is the order of the operator and $m\in\frac{1}{2}\bZ$.

Recall that so far $\rho$ was not mentioned at this section.
\end{remark}

We can give a series of admissible lower order terms for all the types of operators treated above. However, it is very simple in the context of $(\rho,\gamma)$-admissibility. We leave this analysis to the reader and discuss how one can weaken these conditions which may be excessive (in contrast to Section~\ref{sect-11-1} because now $\rho$ does not enter in the assumptions on the principal part.

\begin{example}[singularity at origin]\label{ex-11-3-34}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-3-34-i}
Let $\gamma =\epsilon |x|$ and $\rho =|x|^\mu $. Then conditions (\ref{11-3-42}), (\ref{11-3-42}) and \ref{11-3-42-*} mean respectively that
\begin{equation}
\mu >-d(d+2m\vartheta ) ^{-1},\qquad\mu >-{\frac{d}{2m}},\qquad
\mu >-{\frac{d}{4m}}.
\label{11-3-43}
\end{equation}
Let $\mu ^*$ be the maximal forbidden value. Then for $\mu =\mu ^*$ we can treat
$\rho =|x| ^\mu \bigl|\log |x|\bigr|^\nu $ with appropriate $\nu $, etc.

However, arguments associated with estimates (\ref{11-1-66})--(\ref{11-1-67})
imply that it is sufficient to assume that
\begin{equation}
\mu >\max (-1,-\frac{d}{2m}),\qquad\mu >\max (-1,-{\frac{d}{4m}})
\label{11-3-44}
\end{equation}
in the semi-bounded and non-semi-bounded cases respectively, i.e. that one should check (\ref{11-3-43}) only with $\vartheta=0$.

Really, in such vicinity operator $A_0$ or $A_0^2$ (where $A_0$ contains no lower order terms) is larger in operator sense than
$ r^{-2m+\delta}$, $ r^{-4m+\delta}$ with an arbitrarily small exponent $\delta>0$ respectively.

Moreover, for $d>2m$, $d>4m$ respectively in these cases one can even take
$\mu =-1$ assuming that in a neighborhood of $0$
\begin{multline}
|a_{\alpha ',\alpha ''}|\le \epsilon \rho ^{2m-|\alpha '|-|\alpha ''|}
\\ \forall \alpha ',\alpha '':|\alpha '|\le m,|\alpha ''|\le m,
|\alpha '|+|\alpha ''|\ge 1,
\label{11-3-45}
\end{multline}
\begin{equation}
|a_\alpha |\le \epsilon \rho ^{2m-|\alpha |}
\qquad \forall \alpha:1\le |\alpha |\le 2m
\tag*{$\textup{(\ref*{11-3-45})}^*$}\label{11-3-45-*}
\end{equation}
respectively with small enough $\epsilon =\const>0$.

\item\label{ex-11-3-34-ii}
Let us assume that in a neighborhood of $0$ domain $X$ coincides with the cone $\{(r,\theta )\in \bR^+\times U\}$ where $\partial U\in \sC^K$. Further, let us assume that the Dirichlet boundary condition is given on a part of the boundary $\{(r,\theta ):r\le r_0,\theta \in U_1\subset\partial U\}$
and that $r_0>0$ and $U_1\ne \emptyset$ contains the $\partial U$-neighborhood of some point. Then one even does not need condition $\mu >-\frac{d}{2m}$ in the semi-bounded case.

Really, in such vicinity operator $A_0$ is larger in operator sense than
$\epsilon r^{-2m}$ with sufficiently small constant $\epsilon>0$.

\item\label{ex-11-3-34-iii}
 Moreover, for the Schr\"{o}dinger operator with \underline{either} $d\ge 3$ and with the Dirichlet boundary condition \underline{or} with $d\ge 2$ and a domain and boundary conditions of the type described in \ref{ex-11-3-34-ii}, variational arguments yield that one can assume that in a neighborhood of $0$
\begin{equation}
V\ge -\epsilon \rho ^2,\qquad |V_j|\le \epsilon \rho
\label{11-3-46}
\end{equation}
with $\rho =|x|^{-1}$.

\item\label{ex-11-3-34-iv}
 Let us treat the Schr\"{o}dinger operator with $\mu =-1$, $d\ge 3$ assuming that either the Dirichlet boundary condition is given on $\partial X$ or the domain and the boundary condition are of the type described in \ref{ex-11-3-34-ii}. Then
\begin{equation}
(Au,u)\ge \sum_j \epsilon_0 \|(D_j-V_j)u\|^2+(Vu,u).
\label{11-3-47}
\end{equation}
Let us introduce spherical coordinates $(r,\theta )$ and remove the radial component of the magnetic potential by means of a gradient transform. We obtain that for functions supported in the vicinity of $0$
\begin{equation}
(Au,u)\ge \epsilon_0 \|D_ru\|^2+\epsilon_0 \sum_j\|r^{-1}{\cL}_ju\|^2+(Vu,u)-\varepsilon \|r^{-1}u\|^2
\label{11-3-48}
\end{equation}
where ${\cL}_j$ are first-order operators with bounded
coefficients on $\bS^{d-1}$ and $\varepsilon >0$ is arbitrarily small (the vicinity depends on $\varepsilon $). Let us consider
\begin{equation*}
\|D_ru\|^2=\int\int_0^{r_0}r^{d-1}|D_ru|^2\,drd\theta.
\end{equation*}
In order to do this we treat $\|r^\nu D_ru\|^2_1$ where $\|.\|_1$ and $(.,.)_1$ mean respectively $\sL^2$-norm and inner product on $[0,r_0]$, $\nu =\frac{1}{2}(d-1)$. Substituting $u=r^{-\nu }v$ we obtain that
\begin{multline}
\|r^\nu \partial_ru\|_1^2=\|(\partial_r-\nu r^{-1})v\|_1^2=
\|\partial_rv\|_1^2+\nu ^2\|r^{-1}v\|_1^2-\\[2pt]
2\nu \Re (\partial_rv,r^{-1}v)_1=
\|\partial_rv\|_1^2+(\nu ^2-\nu)\|r^{-1}v\|_1^2.
\label{11-3-49}
\end{multline}
Let $d>3$; then $\nu ^2>\nu $ and we conclude that in this case
\begin{equation}
\|r ^\nu \partial_ru\|_1^2\ge \epsilon_1\|r^{\nu -1}u\|_1^2.
\label{11-3-50}
\end{equation}
On the other hand, let $d=3$. Then $\nu =1$ in which case
$\|r ^\nu \partial_ru\|^2= \|\partial_rv\|^2$ but then obviously (\ref{11-3-50}) holds again. Therefore
\begin{claim}\label{11-3-51}
For $d\ge 3$ the second of conditions (\ref{11-3-46}) is not necessary.
\end{claim}

On the other hand, for $d=2$, $\nu =\frac{1}{2}$ and
$\nu ^2-\nu =-\frac{1}{4}$. In this case only one operator
${\cL}_1=D_\theta -w(r,\theta )$ is present and if for $\theta =\theta_1$ a Dirichlet boundary condition is given then
$\|{\cL}_1u\|_2\ge \epsilon_1\|u\|_2$ where $\|.\|_2$ is $\sL^2$-norm with respect to $\theta $.

On the other hand, if $U=\{\theta ,\theta_1<\theta <\theta_2\}$ and if for both $\theta =\theta_1$ and $\theta =\theta_2$ the Neumann boundary condition is given then this estimate fails. However, if $X$ is a complete neighborhood of $0$ then this estimate remains true provided
\begin{equation}
|\int_0^{2\pi }w(\theta ,r)d\theta -2\pi m|\ge \epsilon_0\qquad
\forall m\in\bZ\quad \forall r\in(0,r_0).
\label{11-3-52}
\end{equation}
Conversely, if (\ref{11-3-52}) fails for every $\epsilon_0>0$ then the
previous inequality also fails. We conclude that
\begin{claim}\label{11-3-53}
Let $d=2$ and \underline{either} $U=\{\theta_1<\theta <\theta_2\}$ and for
$\theta_1$ or for $\theta_2$ a Dirichlet boundary condition is given, \underline{or} $X$ contains a complete neighborhood of $0$ and (\ref{11-3-52}) holds. Then the second of conditions (\ref{11-3-46}) is not necessary.
\end{claim}

\item\label{ex-11-3-34-v}
All these arguments remain true in the case $\gamma =\epsilon |x''|$,
$\rho =|x''| ^\mu $ with $d$ replaced by $d''$
in the conditions.
\end{enumerate}
\end{example}

\begin{example}\label{ex-11-3-35}
Using the arguments of Remark~\ref{rem-11-1-13} we see that in the context of Example~\ref{ex-11-2-19} one can assume that $\rho f(|x''|)\le \epsilon $ (with small enough constant $\epsilon >0$) instead of assumption (\ref{11-3-42}).
\end{example}

\begin{remark}\label{rem-11-3-36}
Certain generalizations can be obtained from functional-analytic arguments.
For example, consider Schr\"{o}dinger operator and asymptotics of $\N^-(\tau)$. Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-3-36-i}
Asymptotics with the remainder estimate
$O\bigl(\tau ^{\frac{1}{2}(d-1)}\bigr)$ remain true if one replaces
potentials $V$ and $V_j$ by $V+V'$ and $V_j+V'_j$ with $V'\in \sL^d(X)$, $V'_j\in \sL^\infty (X)$.

\item\label{rem-11-3-36-ii}
 Moreover, asymptotics with the remainder estimate
$O\bigl(\tau ^{\frac{1}{2}(d-1-\sigma )}\bigr)$ remain true provided $V'_j=0$, $V'\in \sL^{d(1-\sigma ) ^{-1}}(X)$.

\item\label{rem-11-3-36-iii}
Therefore approximating $V'\in \sL^d(X)$ by the potentials
$V'_\varepsilon \in \sL^\infty (X)$ we obtain that asymptotics with the remainder estimate $o\bigl(\tau ^{\frac{1}{2}(d-1)}\bigr)$
remain true for such perturbations.

\item\label{rem-11-3-36-iv}
Moreover, similar approximation arguments yield that asymptotics with the the remainder estimate $O\bigl(\tau ^{\frac{1}{2}(d-1)}\log^{-\nu }\tau \bigr)$
remain true provided $V'|\log (|V'|+1)|^\nu \in \sL^d(X)$.

\item\label{rem-11-3-36-v}
On the other hand, remainder estimates weaker than
$O\bigl(\tau ^{\frac{1}{2}(d-1)}\bigr)$ remain true under weaker conditions. However, our weakly singular potentials (i.e., the potentials which we considered in this section) do not necessarily belong to the indicated classes. Thus, a combination of the two methods is the most effective.
\end{enumerate}
\end{remark}


\subsection{Fractional Laplacians}
\label{sect-11-3-7}

Let us discuss fractional Laplacians defined by (\ref{8-5-1}) in domain $X\subset \bR^d$. Then under additional condition
\begin{equation}
\dist (x,y) \le C_0 |x-y|\qquad \forall x,y \in X
\label{11-3-54}
\end{equation}
(where $\dist(x,y)$ is a ``connected'' distance between $x$ and $y$) everything seems to work. We leave to the reader.

\begin{Problem}\label{Problem-11-3-37}
Under assumption (\ref{11-3-54})
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{Problem-11-3-37-i}
Prove the following estimate:
\begin{equation}
\N_\Omega(\lambda )
\le C_{d,m} \mes (\Omega)\lambda ^{d/m}
\label{11-3-55}
\end{equation}
for an arbitrary domain $\Omega\subset \bR^d$. This is the most challenging part.

\item\label{Problem-11-3-37-ii}
Restore results of Chapter~\ref{sect-9}.

\item\label{Problem-11-3-37-iii}
Reconsider examples of Sections~\ref{sect-11-2} and \ref{sect-11-3}.
\end{enumerate}
\end{Problem}

\begin{remark}\label{rem-11-3-38}
Obviously domains with cuts and inner spikes (inner angles of $2\pi$)
\begin{figure}[h]
\centering
\subfloat[]{\label{fig-11-7-a}%
\begin{tikzpicture}
\draw[very thick] (0,0) circle (1.5);
\draw[very thick] (-.5,0)--(1.5,0);
\end{tikzpicture}}\qquad\qquad
\subfloat[]{\label{fig-11-7-b}%
\begin{tikzpicture}
\draw[very thick, domain=-pi:pi,scale=1, smooth] plot[parametric,id=parametric-example]
 function{3*cos(t/2)*cos(t), 2*cos(t/2)*sin(t)};
\end{tikzpicture}}
\caption{\label{fig-11-7} Domain with a cut \protect\subref{fig-11-7-a} and an inner spike \protect\subref{fig-11-7-b}.}
\end{figure}

\noindent
do not fit (\ref{11-3-54}). On the other hand in the case of the domain with the cut due to non-locality of $\Delta^r$ with
$r\in \mathbb{R}^+\setminus \mathbb{Z}$ both sides of the cut ``interact'' and at least coefficient in the second term of two-term asymptotics may be wrong; in the case of the inner spike some milder effects are expected.
\end{remark}

The following problem seems to be very challenging:

\begin{Problem}\label{Problem-11-3-39}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{Problem-11-3-39-i}
Investigate fractional Laplacians in domains with cuts and inner spikes and save whatever is possible.
\item\label{Problem-11-3-39-ii}
Generalize these results to higher dimensions.
\end{enumerate}
\end{Problem}

\section[Large eigenvalues for unbounded domains]{Large eigenvalues for operators in essentially unbounded domains}
\label{sect-11-4}

\subsection{Coercivity condition and standard asymptotics}
\label{sect-11-4-1}

In this section, under the assumptions of the previous section concerning the domain $X$ and the principal symbol, we consider operators with the lower order terms essential from the point of view of the domain of the operator and asymptotics\footnote{\label{foot-11-29} Thus, it would be better to speak about senior symbols and junior terms.}. These terms could be more singular than those studied before but they must satisfy \emph{coercivity condition}\index{coercivity condition}.

We start with operators with positive principal symbol. In this case the coercivity condition is
\begin{equation}
\blangle A(x,\xi )v,v\brangle \ge \epsilon_0(|\xi |+\rho )^{2m}\1v\1^2
\qquad \forall \xi \quad \forall v,
\label{11-4-1}
\end{equation}
\begin{multline}
\sum_{\alpha ,\beta:|\alpha | \le m,|\beta |\le m}
\blangle a_{\alpha ,\beta }w_\alpha ,w_\beta \brangle \ge
\epsilon_0 \sum_{\alpha :|\alpha |\le m}\1w_\alpha \1^2 \rho ^{2m-2|\alpha |}\\
\forall w=(w_\alpha )_{\{|\alpha |\le m\} }
\label{11-4-2}
\end{multline}
where $\epsilon_0>0$,
\begin{equation}
A(x,\xi )=\sum_{\alpha ,\beta:|\alpha | \le m,|\beta |\le m}
a_{\alpha ,\beta }\xi ^{\alpha +\beta }
\label{11-4-3}
\end{equation}
is the complete (symmetric) symbol of an operator $A$ of the form (\ref{11-1-1}) with $h=1$ and the first condition (\ref{11-4-1}) is assumed to be fulfilled for all $x\in X$ while the second condition (\ref{11-4-2}) (which is surely stronger) is assumed to be fulfilled only in
$\{x\in X,\rho \gamma \ge \epsilon_0,\gamma \le \epsilon_0\}$.
However, in the certain cases this condition is assumed to be fulfilled in a part of $X$ which larger than this. Again we have assumed that
\begin{equation}
\varrho =\rho ^{2m}
\label{11-4-4}
\end{equation}
for the sake of simplicity. We leave to the reader to consider the more general case. In what follows we treat lower order terms which are sums of coercive and admissible indefinite (lower order) terms. For the Schr\"{o}dinger operator (\ref{11-1-6}) conditions (\ref{11-4-1}) and (\ref{11-4-2}) coincide with the condition
\begin{equation}
V\ge \epsilon_0\rho ^2\qquad \forall x
\label{11-4-5}
\end{equation}
provided condition (\ref{11-1-6}) is fulfilled.

\begin{figure}[h]
\centering
\subfloat[]{\label{fig-11-8-a}%
\begin{tikzpicture}
\begin{scope}
\foreach \y in {-4,-3.75,...,-1} \draw [very thin, cyan] (-1,\y)--(1,\y);
\fill[white ,domain=-1:-.2,scale=1, smooth] plot function{1/x }--(-1,-5);
\fill[white ,domain=1:.2,scale=1, smooth] plot function{-1/x }--(1,-5);
\end{scope}
\draw[thick,  domain=-1:-.2,scale=1, smooth] plot function{1/x };
\draw[thick,  domain=1:.2,scale=1, smooth] plot function{-1/x };
\end{tikzpicture}}
\qquad\qquad
\subfloat[]{\label{fig-11-8-b}%
\begin{tikzpicture}
\begin{scope}
\foreach \y in {1.1,1.35,...,4.85} \draw [very thin, cyan] (-1.5,\y)--(1.5,\y);
\fill[white ,domain=-1:-.2,scale=1, smooth] plot function{-1/x }--(0,5)--(0,1);
\fill[white ,domain=1:.2,scale=1, smooth] plot function{1/x }--(0,5)--(0,1);
\end{scope}
\draw[thick,  domain=-1:-.2,scale=1, smooth] plot function{-1/x };
\draw[thick,  domain=1:.2,scale=1, smooth] plot function{1/x };
\end{tikzpicture}}
\caption{\label{fig-11-8} Non-coercive weakly singular potential \protect\subref{fig-11-8-a} and coercive singular potential \protect\subref{fig-11-8-b}; blue lines show symbolically energy levels of the corresponding Schr\"odinger operator. For weakly singular  potential the lowest energy level on \protect\subref{fig-11-8-a} exists.}
\end{figure}


As before we set $\gamma_\tau=\gamma $ and
$\rho_\tau=\rho +\tau ^{\frac{1}{2}}$ and consider domain
\begin{equation*}
X_\reg=\bigl\{x\in X,\ \tau ^{\frac{1}{2m}}\gamma (x)\ge 1,\
\exists
\xi \, \exists v \ne 0: \ \ \blangle A(x,\xi )v,v\brangle \le
(1+\epsilon_1)\tau \1v\1^2\bigr\}
\end{equation*}
with an arbitrarily small constant $\epsilon_1>0$. Then condition (\ref{11-4-1}) yields that $\rho \le C\tau ^{\frac{1}{2m}}$.

As before we apply the results of Part~\ref{part-2} in $X_\reg$ to obtain local
semiclassical spectral asymptotics for $\N^-(\tau)$ (case $\vartheta>0$ will be considered later) in the ball $\cB\bigl(x,\gamma (x),X\bigr)$ with the remainder estimate $O\bigl(\tau ^{\frac{1}{2m}(d-1)}\gamma ^{d-1}\bigr)$ provided
$\rho \le \epsilon_2\tau ^{\frac{1}{2m}}$, in which case operator is $\xi$-microhyperbolic.

Moreover, under condition to the Hamiltonian flow generated by the senior symbol this remainder estimate can be improved to
$o\bigl(\tau ^{\frac{1}{2m}(d-1)}\gamma ^{d-1}\bigr)$ or sharper.

On the other hand, for balls with $\rho \ge \epsilon_2\tau ^{\frac{1}{2m}}$ the remainder estimate (as well as the principal part of the asymptotics) is
$O\bigl(\tau ^{\frac{d}{2m}}\gamma ^d\bigr)$ in the general case; however it could be improved to
$O\bigl(\tau ^{{\frac{1}{2m}}(d-1+\delta )} \gamma ^{d-1+\delta }\bigr)$ with an arbitrarily small exponent $\delta>0$ for the scalar operators.

In order to obtain the remainder estimate
$O\bigl(\tau ^{{\frac{1}{2m}}(d-1)}\gamma ^{d-1}\bigr)$ in the local
spectral asymptotics in this zone one should check microhyperbolicity or another non-degeneracy condition there. In particular, for the Schr\"{o}dinger operator with $d\ge 2$ we obtain this remainder estimate without any additional conditions. This improvement and condition will be important in the next sections but not now.

On the other hand, in the zone
\begin{equation*}
X_+=\bigl\{x\in X,\ \rho \gamma \ge \epsilon_1,\forall \xi \
\forall v \ \blangle A(x,\xi )v,v\brangle \ge
(1+\epsilon_1)\tau \1v\1^2\bigr\}
\end{equation*}
we obtain the remainder estimate\footnote{\label{foot-11-30} The principal part vanishes here.} $O(\rho ^{-s}\gamma ^{-s})$ with arbitrarily chosen exponent $s$ provided either $B\bigl(x,\gamma (x)\bigr)$ does not intersect $\partial X$, or $m$-th order Dirichlet boundary condition is given on $\partial X$.

Moreover, one can obtain the same answer provided\footnote{\label{foot-11-31} This inequality is a restriction on the boundary conditions.}
\begin{equation}
(Au,u)\ge \sum_{\alpha ,\beta :|\alpha |,|\beta |\le m}
(a_{\alpha ,\beta }D ^\alpha u,D ^\beta u)\quad \forall u\in\fD (A).
\label{11-4-6}
\end{equation}
Let us note that
$X_\reg\cup X_+\supset\bigl\{x\in X,\tau^{\frac{1}{2m}}\gamma\ge C_0\bigr\}$. Thus we include $X_+$ either into semiclassical zone $X_\reg$ or into variational zone $X_\sing$.

Let us assume that condition (\ref{11-4-2}) is fulfilled in the domain
\begin{equation*}
{\cX}\supset\{x\in X,\ \rho\gamma\le\epsilon_1,\ \gamma\le\epsilon_1\}.
\end{equation*}
Then for $u$ supported in ${\cX}$ the following estimate
\begin{equation*}
\bigl((A-\tau I)u,u\bigr)\ge -C\tau \int_{\cX_-}\1u\1^2dx
\end{equation*}
holds with $\cX_-={\cX}\setminus \cX_+$,
\begin{equation*}
\cX_+=\bigl\{x\in \cX,\sum_{\alpha ,\beta :|\alpha |\le m,|\beta |\le m}
\blangle a_{\alpha ,\beta }(x)w_\alpha ,w_\beta \brangle \ge
\tau \sum_{\alpha :|\alpha |\le m}\1w_\alpha \1^2
\quad \forall w_\alpha \bigr\}.
\end{equation*}
Surely
$\cX_+\supset\bigl\{x\in X,\rho \ge C\tau ^{\frac{1}{2m}}\bigr\}$.
Therefore we conclude that
\begin{claim}\label{11-4-7}
Contribution of ${\cX}$ to the remainder does not exceed
$C\tau ^{\frac{d}{2m}}\mes (\cX_-)$ provided either the Dirichlet boundary condition or any other condition providing (\ref{11-4-6}) on
$\partial X\cap{\bar{\cX}}$ is given; in the latter case we assume that the cone condition is fulfilled.
\end{claim}

Let us note that
\begin{remark}\label{rem-11-4-1}
${\cX}$ and $X_+$ overlap and therefore we can subtract from
$X_+$ and add to ${\cX}$ zone
\begin{equation*}
\tilde{\cX}=\bigl\{x\in X,
\dist(x,X\setminus {\cX})\ge \epsilon_1\gamma \bigr\}.
\end{equation*}
\end{remark}

So we arrive to the estimate
\begin{equation}
\bigl|\N^- (\tau )-\N^\W (\tau )\bigr|\le
C\bigl(R_1(\tau )+ R_2(\tau )+R_3(\tau )\bigr)
\label{11-4-8}
\end{equation}
with
\begin{equation}
\N^\W (\tau )=(2\pi )^{-d}\iint_{X_\reg\times \bR^d}
\boldsymbol{n}(x,\xi ;\tau )dxd\xi
\label{11-4-9}
\end{equation}
where $\boldsymbol{n}(x,\xi ;\tau )$ is now the eigenvalue counting function for
the complete symbol $A(x,\xi )$,
\begin{align}
&R_1(\tau )=\int_{X_\reg}\tau ^{\frac{d-1}{2m}}\gamma ^{-1}\,dx,
\label{11-4-10}\\[3pt]
&R_2(\tau )=\tau ^{\frac{d}{2m}}\mes (\cX_-\cup \tilde{\cX}),
\label{11-4-11}\\[3pt]
&R_3(\tau )=\int_{X_+\setminus \tilde{\cX}}\rho ^{d-s} \gamma ^{-s}\, dx,
\label{11-4-12}
\end{align}
$\tilde{\cX}=
\bigl\{x\in X_\reg,\ \rho \ge \epsilon_2 \tau ^{\frac{1}{2m}}\bigr\}$
in the general case. This zone can be reduced (or even voided) under
microhyperbolicity or other non-degeneracy condition; in particular $\tilde{\cX}=\emptyset$ for the Schr\"{o}dinger operator with $d\ge 2$.

Similarly, for $\vartheta >0$ estimate
\begin{equation}
\bigl|\N^-_{(\vartheta)} (\tau )-\N^\W _{(\vartheta)} (\tau )\bigr|
\le C\bigl(R_{1(\vartheta)}(\tau )+R_{2(\vartheta)}(\tau )+
R_{3(\vartheta)} (\tau )\bigr)
\label{11-4-13}
\end{equation}
holds with $\N^-_{(\vartheta)}(\tau) =\tau_+^{\vartheta -1}*\N^-(\tau) $,
$\N^\W_{(\vartheta)} (\tau)=\tau_+^{\vartheta -1}*\N^\W (\tau) $, $\N^\W (\tau)$ containing now lower order terms as well,
\begin{align}
&R_{1(\vartheta)}(\tau )=
\int_{X_\reg}\tau ^{{\frac{1}{2m}}(d-1-\vartheta )+\vartheta }
\gamma ^{-1-\vartheta}\,dx,
\label{11-4-14}\\[3pt]
&R_{2(\vartheta )}(\tau )=\tau ^{{\frac{d}{2m}}+\vartheta }
\mes (\cX_-\cup \tilde{\cX}),
\label{11-4-15}\\[3pt]
&R_{3(\vartheta )}(\tau )=\int_{X_+\setminus \tilde{\cX}}\rho ^{2m\vartheta+d-s} \gamma ^{-s}\,dx.
\label{11-4-16}
\end{align}

In particular, we have proven
\begin{proposition}\label{prop-11-4-2}
Let
\begin{gather}
\gamma ^{-1-\vartheta }\in \sL^1(X)\label{11-4-17},\\[2pt]
\rho ^{2m\vartheta+d-s}\gamma ^{-s}\in \sL^1(X\setminus \tilde{\cX})\label{11-4-18}\\
\shortintertext{and}
\mes(\cX_-\cup \tilde{\cX})=O\bigl(\tau ^{-{\frac{1}{2m}}(\vartheta +1)}\bigr);
\label{11-4-19}\\
\shortintertext{then}
\N^-_{(\vartheta)} (\tau )=\N^\W_{(\vartheta)} (\tau )+
O\bigl(\tau ^{{\frac{1}{2m}}(d-1-\vartheta )+\vartheta }\bigr)\qquad
\text{as\ \ }\tau \to+\infty.
\label{11-4-20}
\end{gather}
\end{proposition}

For the Schr\"{o}dinger operator with $d\ge 2$ and other scalar operators with $\vartheta >0$ condition (\ref{11-4-19}) is fulfilled automatically, but in the general case this condition is very unpleasant and it is best to check the microhyperbolicity condition for $(A-\tau )$ in $\tilde{\cX}_-$ and then reduce this zone.

\begin{remark}\label{rem-11-4-3}
Let us discuss the principal differences between weakly and strongly singular potentials:
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-4-3-i}
For strongly singular potentials coercivity condition is required; without it operator may be even not essentially self-adjoint;

\item\label{rem-11-4-3-ii}
For weakly singular potentials small vicinity of the singular point is a singular zone; for strongly singular potential it belongs to a classically forbidden (due to coercivity) part of regular zone;

\item\label{rem-11-4-3-iii}
Finally, in the general case the principal parts of the asymptotics $\N^\W (\tau)$ and $\N^\W_{(\vartheta)}(\tau) $ cannot be decomposed into a power series of $\tau ^{\frac{1}{2m}}$ as in the previous section. Usually this decomposition leads to much worse remainder estimate than the original one.
\end{enumerate}
\end{remark}


\subsection{Sharp remainder estimates}
\label{sect-11-4-2}

Let us discuss an improvement of the remainder estimate in the zone
$X_\reg \cap \{\rho \le C\tau ^{\frac{1}{2m}}\}$; thus we consider the term
$R_1(\tau )$ or $R_{1(\vartheta) }(\tau )$. Let us write our results as a series of remarks:

\begin{remark}\label{rem-11-4-4}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-4-4-i}
Let the standard non-periodicity condition to the (billiard) Hamiltonian
trajectories is fulfilled in $X_\reg$ for the symbol $a(x,\xi )$ on the energy level  $1$.

Then for any fixed $\bar{\gamma}>0$ one can replace the contribution of zone $\{X,\gamma(x)\ge \bar{\gamma}\}$ to the remainder by
$R_{1(\vartheta)}^*(\tau)=o\bigl(R_{1(\vartheta)}(\tau)\bigr)$.

\item\label{rem-11-4-4-ii}
 Further, let condition (\ref{11-4-17}) be fulfilled; then $R_{1(\vartheta)}(\tau)\asymp\tau^{\frac{1}{2m}(d-1-\vartheta)+\vartheta}$) and we can replace it by $R_{1(\vartheta)}^*(\tau) =o\bigl(\tau^{\frac{1}{2m}(d-1-\vartheta)+\vartheta}\bigr)$.

So, under condition (\ref{11-4-17}) and improved assumption (\ref{11-4-19})
\begin{gather}
\mes(\cX_-\cup \tilde{\cX})=o\bigl(\tau ^{-{\frac{1}{2m}}(\vartheta +1)}\bigr)
\tag*{$\textup{(\ref*{11-4-19})}^*$}\label{11-4-19-*}
\\
\intertext{we can improve asymptotics (\ref{11-4-20}) to}
\N^-_{(\vartheta)} (\tau )=\N^\W_{(\vartheta)} (\tau )+
o\bigl(\tau ^{{\frac{1}{2m}}(d-1-\vartheta )+\vartheta }\bigr)
\qquad \text{as\ \ }\tau \to+\infty.
\tag*{$\textup{(\ref*{11-4-20})}^*$}\label{11-4-20-*}
\end{gather}
In particular, for $\vartheta=0$ the two-term asymptotics holds with the remainder estimate $o(\tau^{(d-1)/2m})$.

\item\label{rem-11-4-4-iii}
All the examples of Subsection~\ref{sect-11-3-1} remain true. However, the
principal part of these asymptotics should be given by the formulas of
the present section.
\end{enumerate}
\end{remark}

\begin{remark}\label{rem-11-4-5}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-4-5-i}
Let the enhanced non-periodicity condition to the (billiard) Hamiltonian
trajectories is fulfilled in $X_\reg$ for the symbol $a(x,\xi )$ on the energy level  $1$. Namely, let us assume that this flow is of either exponential or power type and that the corresponding non-periodicity condition is fulfilled. Then one can replace $R_{1(\vartheta)}(\tau)$ by
\begin{gather}
R^{**}_{1(\vartheta)}(\tau )=
\int_{X_\reg}\tau ^{{\frac{1}{2m}}(d-1-\vartheta )+\vartheta }
\gamma ^{-1-\vartheta}\bigl(\log (\tau^{1/2m}\gamma)\bigr)^{-1-\vartheta}\,dx,
\tag*{$\textup{(\ref*{11-4-14})}^{**}$}\label{11-4-14-**}\\
\shortintertext{or}
R^{***}_{1(\vartheta)}(\tau )=
\int_{X_\reg}\tau ^{{\frac{1}{2m}}(d-1-\vartheta )+\vartheta }
\gamma ^{-1-\vartheta} (\tau^{1/2m}\gamma)^{-\delta}\,dx
\tag*{$\textup{(\ref*{11-4-14})}^{***}$}\label{11-4-14-***}
\end{gather}
respectively.

\item\label{rem-11-4-5-ii}
So, under condition (\ref{11-4-17}) and further improved assumption (\ref{11-4-19})
\begin{gather}
\mes(\cX_-\cup \tilde{\cX})=
O\bigl(\tau ^{-{\frac{1}{2m}}(\vartheta +1)}|\log \tau|^{-1-\vartheta}\bigr)
\tag*{$\textup{(\ref*{11-4-19})}^{**}$}\label{11-4-19-**}\\
\shortintertext{or}
\mes(\cX_-\cup \tilde{\cX})=
O\bigl(\tau ^{-{\frac{1}{2m}}(\vartheta +1)-\delta}\bigr)
\tag*{$\textup{(\ref*{11-4-19})}^{***}$}\label{11-4-19-***}\\
\intertext{we can improve asymptotics (\ref{11-4-20}) to}
\N^-_{(\vartheta)} (\tau )=\N^\W_{(\vartheta)} (\tau )+
O\bigl(
\tau ^{\frac{1}{2m}(d-1-\vartheta )+\vartheta }|\log\tau|^{-1-\vartheta}\bigr)
\tag*{$\textup{(\ref*{11-4-20})}^{**}$}\label{11-4-20-**}%
\shortintertext{or}
\N^-_{(\vartheta)} (\tau )=\N^\W_{(\vartheta)} (\tau )+
O\bigl(\tau ^{{\frac{1}{2m}}(d-1-\vartheta )+\vartheta -\delta}\bigr)
\tag*{$\textup{(\ref*{11-4-20})}^{***}$}\label{11-4-20-***}
\end{gather}
respectively.

In particular, for $\vartheta=0$ the two-term asymptotics holds with the remainder estimate $O(\tau^{(d-1)/2m}(\log\tau)^{-1})$ or
$O(\tau^{(d-1)/2m-\delta})$ respectively.
\end{enumerate}
\end{remark}

\begin{remark}\label{rem-11-4-6}
In the context of Subsection~\ref{sect-11-3-2} (periodic billiard Hamiltonian flow) under condition \ref{11-4-19-***} asymptotics
\begin{equation}
\N^- (\tau)=\N^\W (\tau)+\tau^{\frac{d-1}{2m}}
\bigl(\varkappa_1+F(\tau^{\frac{1}{2m}})\bigr)+
O\bigl(\tau^{\frac{d-1}{2m}-\delta})
\label{11-4-21}
\end{equation}
holds as $\tau \to +\infty$.
\end{remark}

\begin{remark}\label{rem-11-4-7}
Non-periodicity condition may be useful even with weakened assumptions
(\ref{11-4-17})--(\ref{11-4-19}).
\end{remark}

\subsection{Examples}
\label{sect-11-4-3}

Let us consider some examples. We start from the Schr\"odinger operator
$\Delta + V(x)$ with potential $V(x)=\kappa |x|^{2\mu}$, $\kappa=\const\ne 0$, $\mu \le -1$, singular at origin, gradually adding the complexity. Note that as $\mu<-1$ operator $V$ is not $\Delta$-bounded (see Definition~\ref{def-10-2-4}) and as $\mu=-1$ it may be $\Delta$-bounded\footnote{\label{foot-11-32} It is the case unless $d=2$ and $0$ is surrounded by $X$.} but it's $\Delta$-bound is not $0$.

So, as $\mu <-1$, we \emph{must\/} assume that $0\notin X$ and $\kappa> 0$, defining operator $\Delta+V$ through quadratic form; as $\mu=-1$ we
may\footref{foot-11-32} allow $\kappa \ge \kappa_0$ with $\kappa_0<0$.

Then we can consider the case of singularity at origin when
$\gamma(x)\asymp |x|$ and $\rho \asymp |x|^\mu$ with $\mu \le -1$ and to generalize it to singularity at $\{x, x''=0\}$ of codimension $d''$.

\begin{example}[Power singularities]\label{ex-11-4-8}%
\index{power singularity!large eigenvalue asymptotics of}%
\index{singularity!power!large eigenvalue asymptotics of}%
\index{large eigenvalues asymptotics!power singularity}%
\index{asymptotics!large eigenvalue!power singularity}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-4-8-i}
Let all the conditions be fulfilled with $\gamma \asymp |x''|$,
$\rho \asymp |x''|^\mu $, $\mu \le -1$. There one can take
${\cX}=\emptyset$ for $\mu <-1$ and
${\cX}=\{x\in X, |x''|\le \epsilon_0\}$ for $\mu =-1$.

Then in the general case we should take the transitional zone\\
$\tilde{\cX} =\{\epsilon \tau \le |x''| ^{2m\mu }\le C\tau \}$ arriving to

\begin{enumerate}[label=(\alph*), wide, labelindent=0pt]
\item\label{ex-11-4-8-ia}
 For $d''>\vartheta +1$, $\mu \ge -d''(\vartheta +1) ^{-1}$
asymptotics (\ref{11-4-20}) holds.

Moreover, for $\mu >-d''(\vartheta +1) ^{-1}$ under the standard non-periodicity condition to the Hamiltonian trajectories asymptotics \ref{11-4-20-*} holds.

Note that for $\vartheta =0$ and $\mu >-d''$ one can replace full Weyl expression (including all terms of $A$) $\N^\W (\tau )$ by the standard two-term expression (one needs the second term only for sharp asymptotics)
$\varkappa_0\tau ^{\frac{d}{2m}}+\varkappa_1\tau ^{\frac{d-1}{2m}}$
with the standard coefficients $\varkappa_0,\varkappa_1$ and
with the same remainder estimate as above.

On the other hand, for $\mu =-d''$, $\N^\W (\tau)= \varkappa_0\tau^{\frac{d}{2m}}+O\bigl(\tau^{\frac{d-1}{2m}}\log\tau\bigr)$
in the general case and
$\N^\W (\tau)=\varkappa_0\tau^{\frac{d}{2m}}+O\bigl(\tau^{\frac{d-1}{2m}}\bigr)$
in the case of a scalar principal symbol.

\item\label{ex-11-4-8ib}
For $d''=\vartheta +1$, $\mu =-1$ asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau )=\N^\W_{(\vartheta)} (\tau )+
O\bigl(\tau ^{{\frac{1}{2m}}(d-1-\vartheta )+\vartheta }
\log \tau \bigr)
\label{11-4-22}
\end{equation}
holds and for $\vartheta =0$, $d''=1$, $\mu =-1$ one can replace $\N^\W (\tau )$ by $\varkappa_0\tau ^{\frac{d}{2m}}$.

\item\label{ex-11-4-8-ic}
 If $\mu <-d''(\vartheta +1) ^{-1}$ then asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau )=\N^\W _{(\vartheta)} (\tau ) +
O\bigl(\tau ^{{\frac{d}{2m}}+ {\frac{d''}{2m\mu }}+\vartheta}\bigr)
\label{11-4-23}%\tag{10.3.16}
\end{equation}
holds.
\end{enumerate}

Let us note that $\mu \ge -d''(\vartheta +1) ^{-1}$, $\mu \le -1$ yield $d''\le \vartheta +1$ and therefore only the listed cases are possible.

\item\label{ex-11-4-8-ii}
One can slightly improve the above results in the number of cases. For the Schr\"{o}dinger operator with $d\ge 2$ and general scalar operators with $\vartheta >0$ one can extend $X_\reg$ and take $\tilde{\cX}=\emptyset$. Moreover, one can easily see that if
$X$ is a conic with respect to the $x''$ domain in a neighborhood
of $\{x''=0\}$ and
\begin{multline}
D ^\alpha (a_{\beta', \beta ''}-a^0_{\beta ',\beta ''})=
o(\rho ^{2m-|\beta '|-|\beta''|} \gamma^{-|\alpha |})\\
\forall \beta ',\beta ''\quad \forall \alpha :|\alpha |\le 1
\label{11-4-24}
\end{multline}
as $|x''|\to 0$ with functions $a^0_{\beta',\beta''}$ which are positively homogeneous of degrees $(2m-|\beta '|-|\beta ''|)\mu $ then\footnote{\label{foot-11-33} We call conditions similar to (\ref{11-4-24}) \emph{stabilization conditions\/}\index{stabilization condition}.} checking the microhyperbolicity condition with
\begin{equation*}
\ell =\langle \xi ,\partial_\xi\rangle +
\mu ^{-1}\langle x'',\partial_{x''}\rangle
\end{equation*}
we see that we can take $\tilde{X}=\emptyset$ as well.

In all these we obtain that

\begin{enumerate}[label=(\alph*), wide, labelindent=0pt]
\item\label{ex-11-4-8-iia}
 For $d''>\vartheta+1$ asymptotics (\ref{11-4-20}) holds.
Moreover, under the standard non-periodicity condition to Hamiltonian
trajectories asymptotics \ref{11-4-20-*} holds.

\item\label{ex-11-4-8-iib}
For $d''=\vartheta+1$ asymptotics (\ref{11-4-22}) holds and for
$d''<\vartheta+1$ asymptotics (\ref{11-4-23}) holds.
\end{enumerate}
Let us note that in both cases for $\mu \le -d''$, even for the Schr\"{o}dinger operator, it is possible that
\begin{equation*}
\N^\W (\tau)-\varkappa_0\tau^{\frac{d}{2m}} -
\varkappa_1 \tau^{\frac{d-1}{2m}}\asymp
\tau^{\frac{d}{2m}+\frac{d''}{2m\mu}}
\end{equation*}
and therefore for $\mu <-d''$ we cannot replace $\N^\W (\tau)$ by $\varkappa_0\tau^{\frac{d}{2m}}$ and preserve the remainder estimate. Moreover, for $\mu =-d''$ we cannot replace $\N^\W (\tau)$ by
$\varkappa_0\tau^{\frac{d}{2m}}+\varkappa_1\tau^{\frac{d-1}{2m}}$
and preserve the remainder estimate $o\bigl(\tau^{\frac{d-1}{2m}}\bigr)$.
\end{enumerate}
\end{example}

\begin{example}[Power singularities again]\label{ex-11-4-9}
Let us consider Schr\"{o}\-din\-ger operator with
$d\ge 2$\,\footnote{\label{foot-11-34} One can consider general scalar
operators for $\vartheta>0$.} and let us assume that in a neighborhood of $\{x''=0\}$ domain $X$ coincides with
$X^0=\{x=(x',r,\theta )\in \bR^{d''}\times \bR^+\times U\}$ where
$U\subset\bS^{d''-1}$ is a $\tilde{\gamma}$-admissible domain with
$\tilde{\gamma}=\tilde{\gamma}(x',\theta )$.

Let us assume that $g^{jk}=g^{jk}(x',\theta )$, $V_j=v_j(x',\theta )|x''|^\mu $,
$V=v(x',\theta )|x''|^{2\mu }$ and $\mu \le -1$. Further, let us assume that
$v\ge 0$ and the functions $g^{jk}$, $v_j$ and $v$ on
$\bR^{d'}\times \bS^{d''-1}$
satisfy standard conditions (\ref{11-1-6})--(\ref{11-1-8}) and (\ref{11-4-5})
with $\tilde{\rho}=\sqrt v$ and with $\tilde{\gamma}$ instead of $\rho $ and $\gamma $. Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-4-9-i}
Under additional assumption $|v_j|\le c\tilde{\rho }$ one can take
$\rho =\tilde{\rho }|x''| ^\mu $ and $\gamma =\epsilon_1\tilde{\gamma }|x''|$ with small enough constant $\epsilon_1>0$.

\begin{enumerate}[label=(\alph*), wide, labelindent=0pt]
\item\label{ex-11-4-9-ia}
Then we obtain that under assumption
\begin{equation}
\tilde{\gamma }^{-1-\vartheta }\in \sL^1(\bR^{d'}\times U)
\label{11-4-25}
\end{equation}
asymptotics (\ref{11-4-20}) holds for $d''>\vartheta +1$.

\item\label{ex-11-4-9-ib}
 Moreover, under the standard non-periodicity condition to the Hamiltonian trajectories asymptotics \ref{11-4-20-*} holds.

\item\label{ex-11-4-9-ic}
 On the other hand, under condition (\ref{11-4-25}) for
$d''=\vartheta +1$ and $d''<\vartheta +1$ we obtain asymptotics
(\ref{11-4-22}) and (\ref{11-4-23}) respectively.
\end{enumerate}

\item\label{ex-11-4-9-ii}
Without condition $|v_j|\le c\tilde{\rho }$ we cannot use variational estimates. In this case we should assume that
$\mu <-1$ and
\begin{equation}
\tilde{\rho}\tilde{\gamma }\ge \epsilon_0>0.
\label{11-4-26}
\end{equation}
These conditions forbid the degeneration of $v$ but permit certain
singularities. Then all the statements of the previous assertion
remain true.

\item\label{ex-11-4-9-iii}
Let $\mu <-1$, condition (\ref{11-4-26}) be fulfilled and
$V_j=v_j(x', \theta )|x''|^{\mu '}$ with $\mu '<\mu $ (the case
$\mu '>\mu $ is trivial).

Then one can take $\rho =\tilde{\rho}|x'|^\mu$,
$\gamma =\epsilon_1\tilde{\gamma }|x''| ^{-\mu '+\mu +1}$. Then
$\rho \gamma \ge \epsilon_2|x''|^{-\sigma }$ with $\sigma >0$
provided $2\mu +1<\mu '$.

\begin{enumerate}[label=(\alph*), wide, labelindent=0pt]
\item\label{ex-11-4-9-iiia}
Then, under assumption (\ref{11-4-25}) we obtain asymptotics (\ref{11-4-20}) for $d''>(1+\vartheta )(1+\mu -\mu ') ^{-1}$.

\item\label{ex-11-4-9-iiib}
 Moreover, under the standard non-periodicity condition to Hamiltonian trajectories we obtain asymptotics \ref{11-4-20-*}.

\item\label{ex-11-4-9-iiic}
 On the other hand, for $d''=(1+\vartheta )(1+\mu -\mu ') ^{-1}$ we obtain asymptotics (\ref{11-4-22}) and for $d''<(1+\vartheta )(1+\mu -\mu ') ^{-1}$ we obtain asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau )=\N^\W_{(\vartheta)} (\tau )+
O\bigl(\tau ^{{\frac{d-\eta }{2}}+\vartheta }\bigr)
\label{11-4-27}
\end{equation}
with $\eta=\mu^{-1}\bigl((1+\vartheta)(1+2\mu-\mu')-d''\bigr)\in
(0,1+\vartheta)$.

Here we cannot consider the case $\mu' \le 2\mu +1$ because the magnetic field is too strong near the origin. This case is left to the next part.
\end{enumerate}
\end{enumerate}
\end{example}

Let us note that every time assertions with large enough $s$ are used, $K$ (in the conditions on coefficients) depends on $\mu$, $\mu '$, etc.\ (via $s$).

\begin{example}[Exponential singularities]\label{ex-11-4-10}%
\index{exponential singularity!large eigenvalue asymptotics of}%
\index{singularity!exponential!large eigenvalue asymptotics of}%
\index{large eigenvalue asymptotics!exponential singularity}%
\index{asymptotics!large eigenvalue!exponential singularity}
Let $X$, $g^{jk}=g^{jk}(x',\theta)$, $v_j=v_j(x',\theta)$ and $v=v(x',\theta)$ be as in statements \ref{ex-11-4-9-i} or \ref{ex-11-4-9-ii} of the previous Example~\ref{ex-11-4-9}. Let $V_j=v_j\exp (|x''|^{-\nu })$,
$V=v\exp (2|x''|^{-\nu })$ with $\nu >0$.

Then all the conditions will be fulfilled with
$\rho =\tilde{\rho}\exp (|x''|^{-\nu })$ and
$\gamma =\epsilon_1\tilde{\gamma}|x''|^{\nu +1}$. We obtain that

\begin{enumerate}[label=(\alph*), wide, labelindent=0pt]
\item\label{ex-11-4-10-a}
For $(1+\nu )(1+\vartheta )<d''$ asymptotics (\ref{11-4-20}) holds and
under the standard non-periodicity condition to Hamiltonian
trajectories asymptotics \ref{11-4-20-*} holds.

\item\label{ex-11-4-10-b}
 Further, for $(1+\nu )(1+\vartheta )=d''$ asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau )=\N^\W_{(\vartheta)} (\tau ) +
O\bigl(\tau ^{\frac{d-1+\vartheta }{2}}\log\log\tau \bigr)
\label{11-4-28}
\end{equation}
holds and

\item\label{ex-11-4-10-c}
For $(1+\nu )(1+\vartheta )>d''$ asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau )=\N^\W_{(\vartheta)} (\tau )+
O\bigl(\tau ^{\frac{d-1+\vartheta }{2}}\log ^\sigma \tau \bigr)
\label{11-4-29}
\end{equation}
holds with
$\sigma =\nu^{-1}\bigl((1+\nu)(1+\vartheta)-d''\bigr)$.
\end{enumerate}
\end{example}

We leave it to the reader the following series of rather easy exercises:

\begin{problem}\label{problem-11-4-11}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-4-11-i}
Consider examples in the spirit of Example~\ref{ex-11-4-9}(iii) with exponential singularities, i.e., with
$V_j=v_j|x''|^{-l}\exp(|x''|^{-\nu})$ or with $V_j=v_j\exp(k|x''|^{-\nu})$,
$k\in (1,2)$.

\item\label{problem-11-4-11-ii}
For different examples estimate
$\bigl(\N^\W (\tau)-\varkappa_0\tau^{\frac{d}{2}}\bigr)$ from above and
below.

\item\label{problem-11-4-11-iii}
Consider quasi-conical domains and domains with cusps for potentials which grow at $0$ or infinity.


\item\label{problem-11-4-11-iv}
Consider general scalar operators with $\vartheta >0$.
\end{enumerate}
\end{problem}

\subsection{Indefinite perturbations}
\label{sect-11-4-4}

Now we consider the case when a strongly singular coercive potential is perturbed by a less singular indefinite potential. Let us assume that conditions (\ref{11-1-3})--(\ref{11-1-4}) are fulfilled with $\rho +\rho '$ instead of $\rho $ and with $\varrho =(\rho +\rho ') ^{2m}$ where $\rho $ and $\rho '$ are
$\gamma $-admissible weight functions. We denote such conditions by $\textup{(\ref{11-1-3})}'$--$\textup{(\ref{11-1-4})}'$.

Meanwhile we replace conditions (\ref{11-4-1}) and (\ref{11-4-2}) by conditions
\begin{equation}
\blangle A(x,\xi )v,v\brangle \ge
\epsilon_0\bigl((|\xi |+\rho )^{2m}-C\rho ^{\prime\,2m}\bigr)\1v\1^2
\qquad \forall \xi \quad \forall v
\tag*{$\textup{(\ref*{11-4-1})}'$}\label{11-4-1-'}
\end{equation}
and
\begin{multline}
\sum_{\alpha ,\beta :|\alpha |\le m,|\beta |\le m}
\blangle a_{\alpha ,\beta }(x)v_\alpha ,v_\beta \brangle \ge \\
\epsilon_0\sum_{\alpha :|\alpha |\le m} \rho^{2m-2|\alpha |}
\1v_\alpha \1^2 -C\sum_{\alpha :|\alpha |\le m-1}
\rho^{\prime\,2m-2|\alpha |}\1v_\alpha \1^2\\
\forall v=(v_\alpha )_{\{|\alpha |\le m\} }
\tag*{$\textup{(\ref*{11-4-2})}'$}\label{11-4-2-'}%\tag*{$(10.3.2)'$}
\end{multline}
respectively.

\begin{remark}\label{rem-11-4-12}
Then the arguments of this and previous sections show that all the estimates of this section remain true with all domains defined by $\rho $ if to their right-hand expressions we add
\begin{equation}
R'(\tau )=C\bigl(\int_{\cZ }(\rho^{\prime\,2m})_+^q\,dx\bigr)^{\frac{d}{2mq}}
\times \bigl(\mes(\cZ)\bigr)^{1-{\frac{d}{2mq}}}
\label{11-4-30}
\end{equation}
for $\vartheta =0$, and
\begin{equation}
R'_{(\vartheta)} (\tau )= C\int_0 ^\infty t^{\vartheta -1}
\bigl( \int_{\cZ} (\rho ^{\prime\,2m}-t)_+^q\,dx\bigr)^{\frac{d}{2mq}}\,dt
\times \bigl(\mes(\cZ)\bigr)^{1-{\frac{d}{2mq}}}
\label{11-4-31}
\end{equation}
for $\vartheta >0$ where $q\ge \frac{d}{2m}$, $q\ge 1$ and one of
these inequalities is strict, and
\begin{equation*}
\cZ=\{x\in X, \rho \le C\rho '\}.
\end{equation*}
\end{remark}

\begin{example}\label{ex-11-4-13}
Consider a power singularity under the assumptions of Example~\ref{ex-11-4-9}(i) with potentials $V$, $V_j$ replaced by $V+V'$, $V_j+V'_j$ respectively where $V'=w(x',\theta )|x''|^{2\nu }$, $V'_j=w_j(x',\theta )|x''| ^\nu $, $w$ and $w_j$ are also functions on $\bS^{d''-1}\times \bR^{d'}$ satisfying conditions
(\ref{11-1-6})--(\ref{11-1-8}) with $\tilde{\rho}'$, $\tilde{\gamma}$.

Here $\tilde{\rho}'$ is a $\tilde{\gamma}$-admissible weight function on
$\bS^{d''-1}\times \bR^{d'}$ and $\nu >\mu $, $\mu \le -1$, $\nu <0$. Let us set $\gamma =\epsilon_1\tilde{\gamma}|x''|$, $\rho =\tilde{\rho}|x''|^\mu $,
$\rho '=\tilde{\rho}'|x''| ^\nu $ with $\tilde{\rho}=\sqrt v$. Then term (\ref{11-4-30}) or (\ref{11-4-31}) should be added to the right-hand expressions of our estimates, and one can see easily that this term does not exceed existing remainder estimate provided one of the following conditions is
fulfilled:\begin{phantomequation}\label{11-4-32}\end{phantomequation}
\begin{align}
&\iint_{\{\tilde{\rho}^{\prime\,2}\ge \epsilon v\}}
\tilde{\rho} ^{\prime\,-a} v^{\frac{b}{2}}\,d \theta dx'<\infty
&\qquad \text{if\ \ } b&<0,\;d\ge 3
\tag*{$\textup{(\ref*{11-4-32})}_1$}\label{11-4-32-1}\\
\intertext{with $a=(d''+d\mu+2\vartheta \mu )(\nu -\mu ) ^{-1}$,
$b=(d''+d\nu +2\vartheta \nu )(\nu -\mu ) ^{-1}$,}
&\iint_{\{\tilde{\rho}^{\prime\,2}\ge \epsilon v\}}
\tilde{\rho}^{\prime\,d+2\vartheta}
\bigl(\log \frac{\tilde{\rho}^{\prime\,2}}{v} \bigr)_+\,d\theta dx'<\infty
&\qquad
\text{if\ \ } b&=0,\;d\ge 3
\tag*{$\textup{(\ref*{11-4-32})}_2$}\label{11-4-32-2}\\[2pt]
&\iint_{\{\tilde{\rho}^{\prime\,2}\ge \epsilon v\}}\tilde{\rho}
^{\prime\,d+2\vartheta }\,d\theta dx'<\infty
&\qquad
\text{if\ \ }b&>0,\;d\ge 3,
\tag*{$\textup{(\ref*{11-4-32})}_3$}\label{11-4-32-3}\\[2pt]
&\iint_{\{\tilde{\rho}^{\prime\,2}\ge \epsilon v\}}
\tilde{\rho} ^{\prime\,-a-\delta \bar{a}}v^{\frac{b}{2}+\delta}\, d\theta
dx'<\infty
&\qquad
\text{if\ \ } b&\le 0,\;d=2,
\tag*{$\textup{(\ref*{11-4-32})}_4$}\label{11-4-32-4}\\[2pt]
&\iint_{\{ \tilde{\rho}^{\prime\,2}\ge \epsilon v\}}
\tilde{\rho}^{\prime\,d+2\vartheta+\delta}\, d\theta dx'<\infty
&\qquad
\text{if\ \ } b&>0,\;d=2,
\tag*{$\textup{(\ref*{11-4-32})}_5$}\label{11-4-32-5}
\end{align}
where $\delta >0$ is arbitrarily small,
$\bar{a}=\mu (\nu -\mu ) ^{-1}$, ${\bar b}=\nu (\nu -\mu ) ^{-1}$.
\end{example}

We leave to the reader

\begin{problem}\label{problem-11-4-14}
Modify and analyze the same way the other examples of this section.
\end{problem}

\subsection{Operators with indefinite principal symbols}
\label{sect-11-4-5}

We leave to the reader

\begin{problem}\label{problem-11-4-15}
Analyze operators with indefinite principal symbols.
\end{problem}

In this case one should replace conditions (\ref{11-4-1}), (\ref{11-4-2}) by
\begin{equation}
\1A(x,\xi )v\1\ge \epsilon_0(|\xi |+\rho )^{2m}\1v\1\qquad
\forall \xi \quad \forall v
\tag*{$\textup{(\ref{11-4-1})}^*$}\label{11-4-1-*}
\end{equation}
and
\begin{equation}
\1\sum_{\alpha :|\alpha |\le 2m}a_\alpha (x)v_\alpha \1\ge
\epsilon_0
\sum_{\alpha :|\alpha |\le 2m}\rho ^{2m-|\alpha |}\1v_\alpha \1
\qquad \forall v=(v_\alpha )_{\{\alpha :|\alpha |\le 2m\}}
\tag*{$\textup{(\ref{11-4-2})}^*$}\label{11-4-2-*}
\end{equation}
respectively. Moreover, one should replace conditions \ref{11-4-1-'}, \ref{11-4-2-'} by\enlargethispage{\baselineskip}
\begin{equation}
\1A(x,\xi )v\1\ge
\epsilon_0\bigl((|\xi |+\rho )^{2m}-C \rho ^{\prime\, 2m}\bigr)\1v\1
\qquad \forall \xi \quad \forall v
\tag*{$\textup{(\ref{11-4-1})}^{*\prime}$}\label{11-4-1-*'}
\end{equation}
and
\begin{multline}
\1\sum_{\alpha :|\alpha |\le 2m}a_\alpha (x)v_\alpha \1\ge\\
\epsilon_0\sum_{\alpha :|\alpha |\le 2m}\rho ^{2m-|\alpha |}
\1v_\alpha \1-
C\sum_{\alpha :|\alpha |\le 2m-1}\rho ^{\prime\,2m}\1v_\alpha \1\\
\forall v=(v_\alpha )_{\{\alpha :|\alpha |\le 2m\}}
\tag*{$\textup{(\ref{11-4-2})}^{*\prime}$}\label{11-4-2-*'}
\end{multline}
respectively.

Unfortunately we are not aware of any examples of this type which are interesting from the physical point of view. The reader can easily construct artificial examples (like generalized Dirac operator) and analyze them.


\section[Large eigenvalues for unbounded domains. II]{Large eigenvalues for operators in essentially unbounded domains}
\label{sect-11-5}

Now we consider \emph{essentially unbounded domains\/}%
\index{essentially unbounded domain}%
\index{domain!essentially unbounded}
which are domains containing massive\footnote{\label{foot-11-35} E.g., conical. Domains with cusps even having infinite volume do not qualify as essentially unbounded and will be treated in the next chapter.} exits to infinity. In domains of this type the spectrum of the operator in question is discrete only because the operator contains lower degree terms which are coercive with the function $\rho$ tending to $\infty $ at infinity (in almost all directions).

\begin{figure}[th]
\centering
\begin{tikzpicture}[xscale=1.2]
\draw[thick,  domain=-4.6:4.6,scale=1, smooth] plot function{x**2/4};
\clip[domain=-4.6:4.6,scale=1, smooth] plot function{x**2/4};
\foreach \y in {0, .5,...,5} \draw [thin, cyan] (-4.6,\y)--(4.6,\y);
\end{tikzpicture}
\caption{\label{fig-11-9}  Coercive at infinity potential; blue lines show symbolically energy levels of the corresponding Schr\"odinger operator.}
\end{figure}
\enlargethispage{3\baselineskip}

Therefore even the order of the asymptotics of $\N^\W(\tau )$ depends on the lower degree terms (which are not anymore ``lower order terms'' from our point of view).

We treat here only operators with positive definite senior symbols and leave the indefinite case to the reader.


\subsection{Standard results}
\label{sect-11-5-1}

We begin with potentials of the power growth at infinity. As the first example we use only the results of Part~\ref{part-2} to obtain the following well known assertion:

\begin{theorem}\label{thm-11-5-1}%
\index{power growth potential!large eigenvalue asymptotics}%
\index{potential!power growth!large eigenvalue asymptotics}%
\index{large eigenvalue asymptotics!power growth potential}%
\index{asymptotics!large eigenvalue!power growth potential}
Let $X$ be an unbounded connected domain in $\bR^d$ and let conditions \textup{(\ref{11-1-1})}--\textup{(\ref{11-1-3})}, \textup{(\ref{11-4-1})} and \textup{(\ref{11-4-4})} be fulfilled with $\gamma =\epsilon_1\langle x\rangle$,
$\rho =\langle x\rangle^\mu$, $\mu >0$ where here and below
$\langle x\rangle =(|x|^2+1)^{\frac{1}{2}}$.

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-5-1-i}
Let us assume that for every $\tau >c$ one of the non-degeneracy conditions
is fulfilled after rescaling for the symbol $A(x,\xi)\tau^{-1}$ on the energy level $1$ uniformly with respect to $\tau ,x,\xi $ (this assumption is only restrictive for $|x|\ge C_0$). Then asymptotics
\begin{equation}
\N^- (\tau )=\N^\W (\tau )+O\bigl(\tau ^{l(d-1)}\bigr)
\label{11-5-1}
\end{equation}
holds as $\tau \to +\infty $ where $\N^\W (\tau )$ is given by
\textup{(\ref{11-4-9})} and $\N^\W \asymp \tau ^{ld}$,
$l={\frac{1}{2m\mu }}(\mu +1)$.

\item\label{thm-11-5-1-ii}
Let us assume that for every $\tau >c$ one of the corresponding non-degeneracy conditions\footnote{\label{foot-11-36} Recall that for operators with the scalar symbols some very weak non-degeneracy condition is needed only as $\vartheta=0$.} is fulfilled for the symbol
$A(x,\xi )\tau^{-1}$ on the energy level $1$ uniformly with respect to
$\tau ,x,\xi $. Then for $\vartheta \ge 0$ asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau )=\N^\W_{(\vartheta)} (\tau)+
O\bigl(R_{(\vartheta)} (\tau )\bigr)
\label{11-5-2}
\end{equation}
holds as $\tau \to+\infty $ with
\begin{equation}
R_{(\vartheta)} (\tau )=\left\{\begin{aligned}
\tau ^{l(d-1)+\vartheta (1-l)}\qquad &\text{for\ \ }\vartheta <d-1, \\
\tau ^{d-1}\log \tau \qquad &\text{for\ \ }\vartheta =d-1, \\
\tau ^{{\frac{1}{2m}}(d-1-\vartheta )+\vartheta }\qquad
&\text{for\ }\vartheta >d-1
\end{aligned}\right.
\label{11-5-3}
\end{equation}
where $\N^\W_{(\vartheta)} (\tau )\asymp \tau ^{ld+\vartheta }$.
\end{enumerate}
\end{theorem}

\begin{proof}
Proof trivially follows from the corresponding results of Part~\ref{part-2} (also see \nameref{sect-0}).
\end{proof}

\begin{remark}\label{rem-11-5-2}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-5-2-i}
Obviously domain $\{|x|\asymp \tau^{1/(2m\mu)}\}$ provides the main contribution to the asymptotics. Further, as $\vartheta<\vartheta^*=(d-1)$ this domain also provides the main contribution to the remainder estimate.

\item\label{rem-11-5-2-ii}
 However as $\vartheta>\vartheta^*$ inner domain $\{|x|\asymp 1\}$ provides the the main contribution to the remainder estimate while for
 $\vartheta =\vartheta^*$ intermediate domain
 $\{\epsilon^{-1}\le |x|\le \epsilon \tau^{1/(2m\mu)}\}$ provides the main contribution to the remainder estimate.

Therefore to improve remainder estimate one needs non-periodicity assumption for the corresponding Hamiltonian flow.
\end{enumerate}
\end{remark}

\begin{theorem}\label{thm-11-5-3}
Let assumptions of Theorem~\ref{thm-11-5-1} be fulfilled. Moreover, let
$X\cap \{x\ge c_1\}=X^0\cap \{x\ge c_1\}$ where $X^0$ is a conical (with respect to $x$) domain with $\partial X^0\setminus 0\in \sC^K$ and let the stabilization conditions
\begin{equation}
D^\alpha (a_\beta -a^0_\beta )=
o\bigl(|x|^{(2m-|\beta |)\mu -|\alpha |}\bigr)
\qquad \forall \beta :|\beta |\le 2m\quad
\forall \alpha :|\alpha |\le 1
\label{11-5-4}
\end{equation}
be fulfilled as $|x|\to \infty $ with functions
$a ^0_\beta \in \sC^K(\bar{X} ^0\setminus 0)$ which are positive homogeneous of
degrees $(2m-|\beta |)\mu $ with respect to $x$.

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-5-3-i}
Further, let us assume that on the energy level  $\tau =1$ for the quasi-homogeneous symbol
\begin{equation}
A^0(x,\xi )=\sum_{|\beta |\le 2m}a^0_\beta (x)\xi ^\beta
\label{11-5-5}
\end{equation}
the standard non-periodicity condition to the Hamiltonian trajectories in $T^*X^0$ is fulfilled and that these permitted trajectories\footnote{\label{foot-11-37} I.e. trajectories originated at $\{A^0(x,\xi)=1\}\setminus \Lambda $ where $\Lambda$ is an exceptional set.} never hit $0\times \bR^d$.

Then for $\vartheta < \vartheta^*=(d-1)$ asymptotics
\begin{equation}
\N_{(\vartheta)}^- (\tau )=\N^\W_{(\vartheta)} (\tau )+
o\bigl(R_{(\vartheta)} (\tau )\bigr)
\label{11-5-6}
\end{equation}
holds $\tau \to+\infty $ with $R_{(\vartheta)}(\tau)=\tau^{l(d-1)+\vartheta(1-l)}$ according to \textup{(\ref{11-5-3})}.

\item\label{thm-11-5-3-ii}
On the other hand, let $\vartheta > \vartheta^*$, and the standard non-periodicity condition to Hamiltonian trajectories be fulfilled on the energy level  $\tau =1$ for the symbol
\begin{equation}
a(x,\xi )=\sum_{|\beta |=2m}a_\beta (x)\xi ^\beta
\label{11-5-7}
\end{equation}
in the domain $X$. Then asymptotics \textup{(\ref{11-5-6})} also holds as $\tau\to+\infty$ but this time with $R_{(\vartheta)}(\tau)=\tau^{\frac{1}{2m}(d-1-\vartheta)+\vartheta}$ according to \textup{(\ref{11-5-3})}.

\item\label{thm-11-5-3-iii}
Finally, let $\vartheta =\vartheta^*$ and stabilization condition \textup{(\ref{11-5-4})} and the standard non-periodicity condition to Hamiltonian trajectories is fulfilled on the energy level  $\tau =1$ for the symbol
\begin{equation}
a^0(x,\xi )=\sum_{|\beta |=2m}a^0_\beta (x)\xi ^\beta
\label{11-5-8}
\end{equation}
in the domain $X^0$ and these permitted\footref{foot-11-37} trajectories never hit $0\times \bR^d$. Then asymptotics \textup{(\ref{11-5-6})} holds as $\tau\to+\infty$ but this time with $R_{(\vartheta)}(\tau)=\tau^{d-1}\log\tau$ according to \textup{(\ref{11-5-3})}.
\end{enumerate}
\end{theorem}

\begin{remark}\label{rem-11-5-4}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-5-4-i}
If only stabilization condition (\ref{11-5-4}) is fulfilled then the
microhyperbolicity condition is automatically fulfilled for the symbol
$A(x,\xi )\tau ^{-1}$ on the energy level $1$ and
\begin{equation}
\N^\W_{(\vartheta)} (\tau )=
\varkappa_{0(\vartheta)}\tau ^{ld}\bigl(1+o(1)\bigr)
\label{11-5-9}
\end{equation}
as $\tau \to+\infty $.

\item\label{rem-11-5-4-ii}
As $\vartheta=0$ asymptotics must include the second term
$\varkappa_1\tau ^{l(d-1)}$ where for the Schr\"{o}dinger operator,
\begin{equation}
\varkappa_0=(2\pi )^{-d}\omega_d
\int_{X^0}\bigl(1-V^0\bigr)_+^{\frac{d}{2}}\sqrt{g^0}\,dx
\label{11-5-10}
\end{equation}
and
\begin{equation}
\varkappa_1=\mp \frac{1}{4}(2\pi)^{1-d}\omega_{d-1}
\int_{\partial X^0}\bigl(1-V^0\bigr)_+^{\frac{d-1}{2}} \,dS^0
\label{11-5-11}
\end{equation}
for Dirichlet and Neumann boundary conditions respectively, $dS^0$ is the Riemannian density on $\partial X^0$ generated by the induced Riemannian metrics, $g^0=\det (g^{jk0})^{-1}$.
\end{enumerate}
\end{remark}

\begin{proof}[Proof of Theorem~\ref{thm-11-5-3}]
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{proof-11-5-3-i}
One can see easily that as $\vartheta<\vartheta^*$ the contribution of zone
$\{|x|\le \varepsilon \tau^{\frac{1}{2m\mu}}\}$ to the remainder does not exceed
$\varepsilon^\delta R_{(\vartheta)}(\tau)$ and therefore only zone
$\{ \varepsilon \tau^{\frac{1}{2m\mu}}\le |x|\le C_0\tau^{\frac{1}{2m\mu}}\}$ should be considered: in all cases zone $\{ |x|\ge C_0\tau^{\frac{1}{2m\mu}}\}$ is elliptic.

Let us apply the theorems of Part~\ref{part-2} and we examine the behavior of
the billiards generated by the symbol
$A(x,\xi)$ on $\Sigma_\tau=\{(x,\xi),\tau\in\Spec A(x,\xi)\}$.
We take
\begin{multline}
\Lambda_1=\Lambda_{1,\tau ,\epsilon ,T}=
\bigl\{(x,\xi )\in\Sigma_\tau ,
|x|\ge \varepsilon \tau ^{\frac{1}{2m\mu }}, \\
|x\tau ^{-{\frac{1}{2m\mu }}}-y|+|\xi \tau ^{-{\frac{1}{2m}}}-\eta |\ge
\epsilon \quad \forall (y,\eta )\in \Lambda ^0_T\bigr\}
\label{11-5-12}
\end{multline}
where $\Lambda ^0_T=\Sigma ^0\setminus \Lambda ^1_T$,
$\Sigma ^0=\{(y,\eta ), 1\in\Spec A^0(y,\eta )\}$ and for every point of
$\Lambda ^1_T$ the Hamiltonian frow of $A^0$ (with reflection from $\partial X^0$) for time $T$ in an appropriate time direction does not enter $\varepsilon$-vicinity of $0\times \bR^d$ and periodicity is violated with at least divergence $\varepsilon$; we fix arbitrary small $\varepsilon$ in advance.

By assumption $\mes(\Lambda ^0_T)=0$, on the other hand, $\Lambda ^0_T$ is a relatively closed subset of $\Sigma ^0\setminus \{x=0\}$ for every $T$. The remaining arguments repeat those in the proof of Theorem~\ref{thm-11-1-1}: we check that the conditions on billiards generated by $A^0(x,\xi )$ and
$A(x,\xi )$ coincide provided $\tau \ge C_{\varepsilon ,T}$.

\item\label{proof-11-5-3-ii}
On the other hand, for $\vartheta >\vartheta^*$ the principal contribution to the remainder estimate is given by the zone $\{x\in X,|x|\le r\}$ (with arbitrarily large fixed $r$) in the sense that the contribution of the remaining part does not exceed $r^{-\delta} R_{(\vartheta)} (\tau )$.

Therefore, to prove Statement~\ref{thm-11-5-3-ii} one should treat Hamiltonian billiards in this zone, in which one can replace $A(x,\xi)$ by $a(x,\xi)$ for large $\tau$.

\item\label{proof-11-5-3-iii}
Finally, for $\vartheta =\vartheta^*$ the principal contribution to the remainder estimate is given by the zone
$\{r\le |x|\le \varepsilon\tau^{\frac{1}{2m\mu}}\}$ for every fixed
$\varepsilon$ and $r$ in the sense that the contribution of the remaining part does not exceed $(\varepsilon^\delta+r^{-\delta}) R_{(\vartheta)} (\tau )$.

Therefore, to prove Statement~\ref{thm-11-5-3-iii} one should treat Hamiltonian billiards in this zone, in which one can replace $A(x,\xi)$ by $a^0(x,\xi)$ for large $\tau$, $|x|$.
\end{enumerate}
\end{proof}

Let us consider scalar operators. Observing that the microhyperbolicity condition is automatically fulfilled for $|x|\le \epsilon\tau^{\frac{1}{2m\mu}}$ and recalling the results of Chapter~\ref{sect-5} we arrive immediately to

\begin{theorem}\label{thm-11-5-5}
Let $X$ be an unbounded connected domain in $\bR^d$ and let conditions
\textup{(\ref{11-1-1})}--\textup{(\ref{11-1-3})}, \textup{(\ref{11-4-1})}, \textup{(\ref{11-4-4})} be fulfilled with $\gamma =\epsilon_1\langle x\rangle $,
$\rho =\langle x\rangle ^\mu $, $\mu >0$.

Moreover, let $A$ be a scalar operator. Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-5-5-i}
Asymptotics
\begin{equation}
\N^- (\tau )=\N^\W (\tau)+
O\bigl(\tau ^{l(d-1)+\delta }\bigr)
\label{11-5-13}
\end{equation}
holds as $\tau \to+\infty$ with an arbitrarily small exponent $\delta >0$ and asymptotics \textup{(\ref{11-5-2})} holds for $\vartheta >0$.

\item\label{thm-11-5-5-ii}
Moreover, for $0<\vartheta<\vartheta^*=(d-1)$, $\vartheta >\vartheta^*$, $\vartheta =\vartheta^*$ respectively Statements \ref{thm-11-5-3-i}--\ref{thm-11-5-3-iii} of Theorem~\ref{thm-11-5-3} remain true.
\end{enumerate}
\end{theorem}

\subsection{Strongly non-periodic Hamiltonian flow}%
\label{sect-11-5-2}
\index{potential!power growth (non-periodic)!large eigenvalue asymptotics}%
\index{power growth potential!non-periodic!large eigenvalue asymptotics}%
\index{large eigenvalue asymptotics!power growth potential!non-periodic}%
\index{asymptotics!large eigenvalue!power growth potential, non-periodic}

In what follows we consider homogeneous coefficients with singularities and (what is more essential here) with degenerations. However, we now improve the remainder estimates under stronger conditions to Hamiltonian trajectories.

\begin{theorem}\label{thm-11-5-6}
Let the conditions of Theorem~\ref{thm-11-5-1} be fulfilled. Let $A$ be a scalar operator. Assume that
\begin{claim}\label{11-5-14}
Either $X^0=\bR^d$ or $A$ is the Schr\"{o}dinger operator or its power.
\end{claim}
Further, let the strong stabilization condition
\begin{multline}
D^\alpha (a_\beta -a^0_\beta )=
O\bigl(|x|^{2m-|\beta |)\mu -|\alpha |-\delta }\bigr) \\
\forall \beta :|\beta |\le 2m\quad \forall \alpha :|\alpha |\le 1
\tag*{$\textup{(\ref{11-5-4})}^*$}\label{11-5-4-*}%\tag*{$(10.4.3)^*$}
\end{multline}
be fulfilled as $|x|\to \infty $ with some $\delta >0$. Furthermore, let us assume that the Hamiltonian flow (with reflections at $\partial X^0$) is of
non-periodic power type\footnote{\label{foot-11-38} We are aware of no example when the flow is of non-periodic exponential type but is not of
non-periodic power type. We would appreciate construction of such example. We leave to the reader to formulate the statement in the case of non-periodic exponential type.}
and that along trajectories $(x(t),\xi (t))$ with
$(x(0),\xi (0))\in \Lambda ^0_{\varepsilon ,T}\subset\Sigma_1$,
$|x(0)|=1$, $\varepsilon =T^{-M}$, condition $|x(t)|\ge T^{-M_1}$ is
fulfilled.\enlargethispage{\baselineskip}

Then asymptotics
\begin{equation}
\N^- (\tau)=\N^\W (\tau)+
\bigl(\varkappa_1+O(\tau^{-\delta'})\bigr)\tau^{l(d-1)}
\label{11-5-15}
\end{equation}
holds as $\tau\to+\infty$. Moreover, for $0<\vartheta \le d-1-\delta$ asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau )= \N^\W_{(\vartheta)} (\tau ) +
O\bigl(\tau ^{l(d-1)+\vartheta (1-l)-\delta '}\bigr)
\label{11-5-16}
\end{equation}
holds as $\tau \to +\infty $ with $\delta '=\delta '(d,m,\delta ,l)>0$.
\end{theorem}

\begin{example}\label{ex-11-5-7}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-5-7-i}
Growth and non-periodicity conditions of Theorem~\ref{thm-11-5-6} to the Hamiltonian flow are fulfilled for the Schr\"{o}dinger operator with $X^0=\bR^d$ and $A^0(x,\xi )=\bigl(|\xi |^2+|x| ^{2\mu}\bigr)$, $0<\mu \ne 1$.

\item\label{ex-11-5-7-ii}
Therefore the statement of Theorem~\ref{thm-11-5-6} is true for this operator (provided all the other conditions of this theorem, including
\ref{11-5-4-*}, are fulfilled) and for the $2m$-order operator with
$A^0(x,\xi )=(|\xi |^2+|x|^{2\mu })^m$, and one can replace $X^0=\bR^d$ by the $X^0$ obtained after (a sequence of) the following transformations:

\begin{enumerate}[label=(\alph*), wide, labelindent=0pt]
\item\label{ex-11-5-7-iia}
We take the factor manifold of $X^0$ with respect to a finite
rotation group (with center at the origin),

\item\label{ex-11-5-7-iib}
 We consider the reflection $S:\bar{X} ^0\to\bar{X} ^0 $ with respect to a hyperplane and remove from $X^0$ some subset ${\cK}$ of this plane provided
$\tilde{\gamma}^{-1-\vartheta }\in \sL^1(\bS^{d-1})$ with
$\tilde{\gamma}=\dist (x,{\cK})$.
\end{enumerate}
\end{enumerate}
\end{example}

\begin{proof}
Obviously it is sufficient to prove Statement \ref{ex-11-5-7-i}. Moreover, the potential $V^0=|x|^{2\mu}$ is spherically symmetric and therefore an angular momentum is constant along every Hamiltonian trajectory and therefore the $x$-projection of this trajectory lies in some 2-dimensional plane. Therefore it is sufficient to treat only the case $d=2$. We introduce polar coordinates $(r,\theta)$ and use
the fact that the \emph{angular momentum\/} $M=\dot{\theta }r^2$\index{angular momentum} is constant where $\dot{\theta }=\frac{d\theta}{dt}$, etc.

Therefore the energy is equal to
\begin{equation}
E=\frac{1}{2}\dot{r}^2+{\frac{1}{2}}M^2r^{-2}+r^{2\mu}= \frac{1}{2}\dot{r}^2+W(r,M)
\label{11-5-17}
\end{equation}
and is also constant and therefore $r$ obeys equation of oscillations \begin{equation}
\overset{..}r = -W'(r,M)
\label{11-5-18}
\end{equation}
with the \emph{effective potential\/}\index{potential!effective} $W(r)= {\frac{1}{2}}M^2r^{-2}+r^{2\mu}$.

Then a trajectory with $|M|\ge \varepsilon$ lies permanently in the zone $\{(\theta,r), r\ge M\sqrt{\frac{2}{E}}\}$. One can easily see that
\begin{equation}
|M|\le M_0(E)=(2\mu)^{\frac{1}{2}}
\bigl(\frac{E}{\mu+1}\bigr)^{\frac{1}{2\mu}(\mu+1)}
\label{11-5-19}
\end{equation}
and every trajectory oscillates between the largest and the smallest values $r=r_2(E,M)$ and $r=r_1(E,M)$ respectively where $r_1<r_2$\,\footnote{\label{foot-11-39} And $r_1(E,M)=r_2(E,M)$ if and only if $|M|=M_0(E)$.}
are roots of the equation $W(r,M)=E$ (i.e.
${\frac{1}{2}}M^2r^{-2}+r^{2\mu }=E$) and the period of the oscillation is
\begin{equation}
T_\Pi=T_\Pi(E,M)=2\int_{r_1(E,M)}^{r_2(E,M)}
\bigl(2E-2W(r,M)\bigr)^{-\frac{1}{2}}\,dr
\label{11-5-20}
\end{equation}
while the increment of $\theta$ during a period is
\begin{equation}
\theta_\Pi = 2\int_{r_1(E,M)}^{r_2(E,M)}
Mr^{-2}\bigl(2E-2W(r,M)\bigr)^{-{\frac{1}{2}}}\,dr.
\label{11-5-21}
\end{equation}
One can easily see that
\begin{claim}\label{11-5-22}
If $\varepsilon \le |M|\le M_0(E)-\varepsilon $ and $E\asymp 1$ then
\begin{equation*}
|r_2(E,M)-r_1(E,M)|\ge \epsilon \varepsilon ^p,\quad r_1(E,M)\ge \epsilon\varepsilon^p, \quad
T_\Pi (E,M)\ge \epsilon \varepsilon ^p, \quad
\theta_\Pi \ge \epsilon \varepsilon ^p
\end{equation*}
and the functions $f(E,M)=r_1(E,M),r_2(E,M),T_\Pi(E,M),\theta_\Pi (E,M)$ satisfy the inequalities
\begin{equation*}
|D_{E,M}^\beta f|\le C_{|\beta |}\varepsilon ^{-p|\beta |}\qquad
\forall \beta
\end{equation*}
with appropriate constants $p,\epsilon >0$ and $C_{|\beta |}$;
$\varepsilon >0$ is a small parameter here.
\end{claim}
On the other hand,
\begin{claim}\label{11-5-23}
The $dxd\xi :dA^0$-measure of the set of points
\begin{equation*}
\bigl\{(r,\theta ):
E=1,|M|\le \varepsilon\;\text{or\ } E=1,|M|\ge M_0(E)-\varepsilon \bigr\}
\end{equation*}
is less than $C\varepsilon ^\delta $ with $\delta >0$.
\end{claim}
These assertions (\ref{11-5-22}) and (\ref{11-5-2}) yield that the Hamiltonian flow is of power type. Let us prove that as $\mu \ne 1$ this flow is of non-periodic power type.

The arguments above yield that it is sufficient to prove that
\begin{claim}\label{11-5-24}
For $k,n\in \bZ^+, m\le \varepsilon ^{-1},n\le \varepsilon ^{-1}$ the
measure of the set of points $(x,\xi )$ with $E(x,\xi )=1$ such that
\begin{equation}
|\theta_\Pi (1,M(x,\xi ))-2\pi{\frac{k}{n}}|\le \varepsilon ^L
\label{11-5-25}
\end{equation}
does not exceed $O(\varepsilon ^{\frac{L}{q}})$ where $L$ is arbitrarily
large.
\end{claim}
Obviously, $\theta_\Pi (1,M)$ is an analytic function of $M\in (0,M_0(1))$; further, $\theta_\Pi (1,M_0(1)-\eta ^2)$ is an analytic function of
$\eta \in (-\epsilon_0, \epsilon_0)$.%

Furthermore, it is well known (see, e.g., V.~I.~Arnold~\cite{arnold:classical}) that
\begin{claim}\label{11-5-26}
For $\mu >0, \mu \ne 1$ function $\theta_\Pi (1,M)$ is not constant.
\end{claim}
Therefore the measure of points $(x,\xi)$ with $E(x,\xi)=1$ and
$|M(x,\xi)|\ge \epsilon_1$, satisfying (\ref{11-5-25}) is $O(\varepsilon^{\frac{L}{q}})$ as $\varepsilon\to +0$. Here $\epsilon_1>0$ is an arbitrary constant.

On the other hand, one can easily see that $\theta_\Pi$ is continuous at $[0,M_0(1)]$ and $\theta_\Pi(+0)=\pi$. Therefore in the zone $\{(x,\xi), 0<M(x,\xi) \le \epsilon \epsilon_0\}$ inequality (\ref{11-5-25}) can be fulfilled only with $k\asymp n$.

Further, one can easily see that for $M\in (0,\epsilon_0)$,
$\theta_\Pi (1,M)={\cF}(M,M^{2\mu })$ where ${\cF}$ is an analytic function of two variables in a neighborhood of $(0,0)$.
Furthermore, $\theta_\Pi (1,M)\ne \const$ and therefore
$|\nabla_M \theta_\Pi (1,M)|\ge \epsilon_1 M^p$ for $M \in (0,\epsilon_1)$ with appropriate $\epsilon_1>0$ and $p$ and therefore the measure of the set of points with $E(x,\xi)=1$ and $M(x,\xi)\in (0,\epsilon_1)$ satisfying (\ref{11-5-25}) is $O(\varepsilon^{\frac{L}{p}})$.
\end{proof}

\begin{remark}\label{rem-11-5-8}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-5-8-i}
For $\vartheta > d-1+\delta $ one can easily improve the remainder estimate
$O(\tau ^{{\frac{1}{2m}}(d-1\vartheta )+\vartheta })$ to
$O(\tau ^{{\frac{1}{2m}}(d-1\vartheta )+\vartheta -\delta '})$ under a corresponding condition on the Hamiltonian flow of $a(x,\xi )$.

In order to reach uniformity one can assume that stabilization condition \ref{11-5-4-*} is fulfilled only for terms with $|\alpha |=2m$. In this case only these terms should be scalar but if some junior terms are not scalar one should check that some non-degeneracy condition is fulfilled.

\item\label{rem-11-5-8-ii}
Moreover, one can consider the case $\vartheta =d-1$. It is easy
to replace the factor $\log \tau $ by $\log ^{1-\delta '}\tau $ but better
improvements are possible only under much more complicated and
restrictive conditions.
\end{enumerate}
\end{remark}


\subsection{Periodic Hamiltonian flow}%
\label{sect-11-5-3}
\index{power growth potential!periodic!large eigenvalue asymptotics}%
\index{potential!power growth (periodic)!large eigenvalue asymptotics}%
\index{large eigenvalue asymptotics!power growth potential!periodic}%
\index{asymptotics!large eigenvalue!power growth potential, periodic}

Let $A$ be a scalar operator and condition (\ref{11-5-14}) be fulfilled. Further, let us assume that
\begin{claim}\label{11-5-27}
The Hamiltonian trajectories of $A^0(x,\xi )$ are periodic with period $T(A^0(x,\xi ))$ and
\end{claim}
\begin{equation}
A=A^{0\w}(x,D)+A ^{\prime \w}(x,D),
\label{11-5-28}
\end{equation}
where
\begin{multline}
D ^\beta (a'_\alpha -a^1_\alpha )=
O\bigl(|x|^{(2m-| \alpha |)\mu -\delta_1-\delta' -|\beta |}\bigr)\\
\forall \alpha :|\alpha |\le 2m\quad \forall \beta :|\beta |\le K
\qquad \text{as\ \ }|x|\to \infty
\label{11-5-29}
\end{multline}
where $a^1_\alpha (x)$ are positively homogeneous of degrees
$(2m-|\alpha |)\mu -\delta_1$ with respect to $x$ and are smooth away from $0$,
$0<\delta_1<2(\mu +1)$, $\delta' >0$.

Let us introduce function
\begin{equation}
b(x,\xi )={\frac{l}{T_0}}\int_0^{T_0}A^1\circ \Psi_tdt \qquad\text{with\ \ }
A^1(x,\xi)=\sum_{|\alpha |\le 2m}a^1_\alpha (x)\xi ^\alpha
\label{11-5-30}
\end{equation}
on the surface $\Sigma ^0=\bigl\{(x,\xi ), A^0(x,\xi )=1\bigr\}$;
recall that $l=\frac{1}{2m\mu}(\mu +1)$ and $T_0=T(1)$.

It follows from the quasi-homogeneity of $A^0$ with respect to $(x,\xi )$ that the action vanishes\footnote{\label{foot-11-40} In fact, the action is equal to
\begin{equation*}
{\frac{1}{T_0}}\int_0^{T_0}\bigl(k\langle \xi ,A^0_\xi \rangle +
(1-k)\langle x,A^0_x\rangle -A\bigr)\circ \Psi_tdt
\end{equation*}
with an arbitrary constant $k$. Let us take $k=\mu (\mu +1) ^{-1}$.
Then the Euler identity yields that the integrand vanishes for $l=1$.
On the other hand, we must assume that $l=1$: otherwise we should
replace $A$ by $A^l$ in order to obtain $T=T_0$ for all $(x, \xi )$.}.

Then the results of Sections~\ref{sect-6-2},~\ref{sect-8-3} immediately yield the following theorem:

\begin{theorem}\label{thm-11-5-9}
Let conditions \textup{(\ref{11-5-14})} and \textup{(\ref{11-5-27})}--\textup{(\ref{11-5-30})} be fulfilled. Further, let us assume that
\begin{equation}
\mes_\Sigma \bigl(\bigl\{(x,\xi )\in \Sigma ,
|b(x,\xi )-\omega |\le \varepsilon\bigr\}\bigr)=
O(\varepsilon ^\delta )\qquad \text{as\ \ }\varepsilon \to+0
\label{11-5-31}
\end{equation}
with $\delta >0$ and
\begin{multline}
\dist (\Psi_t(x,\xi ),(x,\xi ))\ge t(T_0-t) \gamma (x,\xi ) \\[2pt]
\forall
(x,\xi )\in\Sigma \quad \forall t\in (0,T_0)\\[2pt]
\text{ with $\gamma \ge 0$ such that
$\mes\bigl(\{(x,\xi ),\gamma (x,\xi )\le \varepsilon \}\bigr)=
O(\varepsilon ^\delta )$ as $\varepsilon \to+0$.}
\label{11-5-32}
\end{multline}
Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-5-9-i}
If $\delta_1<\mu +1$ and condition \textup{(\ref{11-5-31})} is fulfilled for
every $\omega \in\bR$ then asymptotics
\begin{equation}
\N^- (\tau )=\N^\W (\tau )+\kappa_1 \tau^{l(d-1)}+
O\bigl(\tau ^{l(d-1) -\delta ''}\bigr)
\label{11-5-33}
\end{equation}
holds as $\tau \to +\infty $ with $\delta ''>0$.

\item\label{thm-11-5-9-ii}
If $\delta_1\in [\mu +1,2\mu +2)$ then for $\tau \to +\infty $
such that $\tau ^l\in \bigcup_{n\in \bZ^+}J_n$ asymptotics
\begin{equation}
\N^- (\tau )=\N^\W (\tau )+\bigl(\kappa_1+F(\tau )\bigr)\tau ^{l(d-1)}+
O\bigl(\tau ^{l(d-1)-\delta ''}\bigr)
\label{11-5-34}
\end{equation}
holds with $\delta ''>0$ where
\begin{equation*}
J_n=\bigl[\nu (n+{\frac{1}{4}}\omega_0)+(\omega -\epsilon_1)
(\nu n)^{l-{\frac{\delta_1}{2m\mu }}},
\nu (n+{\frac{1}{4}}\omega_0)+
(\omega +\epsilon_1)(\nu n)^{l-{\frac{\delta_1}{2m\mu }}}\bigr],
\end{equation*}
$\omega_0$ is the Maslov index of the trajectory $\Psi_t(x,\xi )$
with $t\in (0,T_0)$, $\nu =\frac{2\pi l}{T_0}$ and $\epsilon_1>0$ is
small enough,
\begin{multline}
F(\tau )=
(2\pi )^{-d}lT_0^{-1}\int_\Sigma \Upsilon
\Bigl(T_0l^{-1}\bigl((\tau ^l-{\frac{1}{4}}\pi \omega_0)-
\tau ^{l-{\frac{\delta_1}{2m\mu }}}b\bigr)\Bigr)\times\\
dxd\xi :dA^0.
\label{11-5-35}
\end{multline}
\end{enumerate}
\end{theorem}

Let us consider the perturbed harmonic oscillator $A_0=\frac{1}{2}(|D|^2+|x|^2)$ in $\bR^d$ more carefully. In this case $\mu =l=m=1$, $T_0=2\pi $,
$\omega_0\equiv 2d \mod 4\bZ$ and the $x$-projections of the Hamiltonian trajectories are ellipses centered at the origin.

Moreover,
\begin{claim}\label{11-5-36}
$\Spec A_0=\{\tau_n=\frac{d}{2}+n, n\in \bZ^+\}$. The multiplicity of $\tau_n$ is $P(n)$ where $P(.)$ is a polynomial of degree $d-1$.
\end{claim}
Functional-analytic arguments yield that
\begin{claim}\label{11-5-37}
If the perturbing operator is a potential $V$ with $\|V\|_{\sL^\infty }\le \epsilon $ then the spectrum consists of clusters of length $\le \epsilon $.
\end{claim}\enlargethispage{\baselineskip}

We leave to the reader
\begin{problem}\label{problem-11-5-10}
Prove that for generic functions $a^1_\alpha $ ($|\alpha |\le k$) which are positively homogeneous of degree $(2-|\alpha |-\delta_1)$ condition (\ref{11-5-31}) is fulfilled for every $\omega $.
\end{problem}

For such perturbations the theory of Section~\ref{sect-6-2} yields that
\begin{claim}\label{11-5-38}
Asymptotics (\ref{11-5-33}) holds for $0<\delta_1<2$ and asymptotics (\ref{11-5-34})--(\ref{11-5-35}) holds for $\delta_1\ge 2$ where $\delta_k>0$ ($k=0,1,2$) are now arbitrary.
\end{claim}
In particular, one can take $k=0$ and a perturbing potential
$V'=v_0r^{2\mu -\delta_1 }$ with arbitrary $v_0\ne 0$ and $0< \delta_1\ne 2$.

Let us consider the case $b\equiv 0$. Then we have two possibilities.

The first (rather trivial) possibility is to assume that
$A=A^{0\w}+A^{1\w}+A^{\prime\prime \w}$ where $A''$ (instead of $A'$) satisfies condition (\ref{11-5-29}) with $a^2_\alpha ,\delta_2$ instead of
$a^1_\alpha ,\delta_1$ respectively, $\delta_2\in (\delta_1,2\delta_1)$. Then one can construct the symbol $b(x,\xi )$ by formula (\ref{11-5-30}) with $A^2$ instead of $A^1$, assume that condition (\ref{11-5-31}) is fulfilled and obtain asymptotics (\ref{11-5-33}) or (\ref{11-5-34})--(\ref{11-5-35}) with $\delta_2$ instead of $\delta_1$.

However, for $\delta_2=2\delta_1$ the situation is more complicated because in this case $b$ contains a term which is quadratic with respect to $A^1$.

So, let us assume that
\begin{equation}
A^1\circ j^*=-A^1
\label{11-5-39}
\end{equation}
where $j^*$ is the antipodal map $(x,\xi )\to (-x,-\xi )$. Repeating the arguments of the proof of Theorem~\ref{thm-11-3-21} we again obtain formula
(\ref{11-3-27}):
\begin{equation}
b= \frac{1}{2\pi} \Bigl( \int_0^{2\pi}A^2\circ \Psi_t\,dt+
\int_0^\pi\int_0^\pi \{A^1\circ \Psi_t,A^1\circ \Psi_{t+t'}\}\,dtdt'\Bigr)
\label{11-5-40}
\end{equation}
is a positive homogeneous symbol of degree $(2-2\delta_1)$ with respect
to $(x,\xi)$.

Therefore we have proven

\begin{theorem}\label{thm-11-5-11}
Let $X^0=\bR^d$, $A=A^{0\w}+A^{1\w}+A^{\prime\prime \w}$ where $A''$ satisfies
\textup{(\ref{11-5-29})} with $a^2_\alpha $ and $\delta_2>0$ instead of $a^1_\alpha $ and $\delta_1$. Here $a^1_\alpha $ and $a^2_\alpha $ are functions smooth for $x\ne 0$ and positively homogeneous of degrees $(2-|\alpha |-\delta_1)$, $(2-|\alpha|-\delta_2)$, and $\delta_2=2\delta_1$.

Further, let condition \textup{(\ref{11-5-39})} be fulfilled and let the symbol $b$ be defined by \textup{(\ref{11-5-40})}. Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-5-11-i}
If $\delta_2<2$ and condition \textup{(\ref{11-5-31})} is fulfilled for every $\omega \in\bR$ then asymptotics \textup{(\ref{11-5-33})} holds for
$\tau\to +\infty$.

\item\label{thm-11-5-11-ii}
If $\delta_2\ge 2$ and condition \textup{(\ref{11-5-31})} is fulfilled for
some $\omega\in\bR$ then asymptotics \textup{(\ref{11-5-34})}--\textup{(\ref{11-5-35})} holds for $\tau\to +\infty$ and belonging to the intervals $J_n$ indicated in Theorem~\ref{thm-11-5-9}\ref{thm-11-5-9-ii} with $\omega_0=2(d-1)$, $\nu=1$. In these
asymptotics as well as in the definition of the intervals $J_n$ one should
replace $\delta_1$ with $\delta_2$.
\end{enumerate}
\end{theorem}

We leave to the reader

\begin{problem}\label{problem-11-5-12}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-5-12-i}
Prove that for generic positively homogeneous functions $a^2_\alpha$ ($|\alpha|\le k$) with $k=0,1,2$ condition (\ref{11-5-33}) is fulfilled for all $\omega\in\bR$.

\item\label{problem-11-5-12-ii}
Consider Riesz means with $\vartheta <\vartheta^*=(d-1)$.
\end{enumerate}
\end{problem}


\begin{remark}\label{rem-11-5-13}
It does not look right that in our results here $\delta''>0$ is unspecified small exponent. Later under certain conditions we will bring our results to be more sharp (up to being consistent with results of Section~\ref{sect-6-2}.
\end{remark}

\subsection{Singularities and degenerations}%
\label{sect-11-5-4}
\index{power growth potential!degenerate!large eigenvalue asymptotics}%
\index{potential!power growth (degenerate)!large eigenvalue asymptotics}%
\index{large eigenvalue asymptotics!power growth potential!degenerate}%
\index{asymptotics!large eigenvalue!power growth potential, degenerate}

Let us consider operators with homogeneous terms with singularities and
(what is now more interesting) degenerations. In order to avoid non-degeneracy conditions we consider only the Schr\"{o}dinger operator.

\begin{theorem}\label{thm-11-5-14}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-5-14-i}
Let $d\ge 3$, $X=\{x=(r,\theta )\in \bR^+\times U\}$ where $U\subset\bS^{d-1}$. Let $g^{jk}=g^{jk}(\theta )$, $V_j=v_j(\theta )r ^\mu $,
$V=v(\theta )r ^{2\mu }$ with $\mu >0$.

Further, let $v\ge 0$ and let $U,g^{jk},v_j,v$ and $\tilde{\rho}=\sqrt v$,
$\tilde{\gamma}=\tilde{\gamma}(\theta )$ satisfy conditions
\textup{(\ref{11-1-6})}--\textup{(\ref{11-1-6})} and \textup{(\ref{11-4-5})}.

Finally, let
\begin{equation}
v^{-{\frac{d}{2\mu}}},
v^{-{\frac{d-1}{2\mu }}}\tilde{\gamma}^{-1}\in \sL^1(U).
\label{{11-5-41}}
\end{equation}
Then asymptotics \textup{(\ref{11-5-1})} holds and one can substitute $\N^\W(\tau)$ by $\varkappa_0\tau ^{ld}$ with $l={\frac{1}{2\mu}}(\mu +1)$ and
with the coefficient $\varkappa_0$ given by \textup{(\ref{11-5-10})}.

Moreover, if $0<\vartheta <\vartheta^*=(d-1)$ and
\begin{equation}
v^{-\frac{1}{2\mu}(d-1-\vartheta)}\tilde{\gamma}^{-1-\vartheta}\in \sL^1(U)
\label{11-5-42}
\end{equation}
then asymptotics \textup{(\ref{11-5-2})}--\textup{(\ref{11-5-3})} holds.

\item\label{thm-11-5-14-ii}
Let us assume that there exists a set\ \
$\Xi \subset\Sigma =\{(x,\xi ),a(x,\xi )=1\}$ such that $\mes_\Sigma (\Xi) =0$ and through every point of $\Sigma \setminus \Xi $ there passes an infinitely long non-periodic Hamiltonian billiard generated by the Hamiltonian
\begin{equation}
H^0=
\tilde{\gamma}|x|\bigl(g^{jk}(\xi_j-V_j)(\xi_k-V_k)+V-1\bigr).
\label{11-5-43}
\end{equation}
Then asymptotics \textup{(\ref{11-5-6})} holds and one can substitute $\N^\W(\tau)$ by $\varkappa_0\tau ^{ld}$.

Moreover, if $0<\vartheta <\vartheta^*$ and
\begin{equation}
v^{-\frac{1}{2\mu}(d-1-\vartheta)}\tilde{\gamma}^{-1-\vartheta}\in \sL^1(U)
\label{11-5-44}
\end{equation}
then asymptotics \textup{(\ref{11-5-6})}, \textup{(\ref{11-5-3})} holds.
\end{enumerate}
\end{theorem}

\begin{proof}
One can easily prove this theorem by the same method as Theorem~\ref{thm-11-5-1} but also with analysis in the zone
$X_\sing=\{\gamma \cdot (\tau ^{\frac{1}{2}}+\rho)\le C_0\}$ with $\gamma=\tilde{\gamma}r$, $\rho=\tilde{\rho}r^\mu$.

In the calculation of $\N^\W (\tau)$ we use spherical coordinates and the change of variable $r=\tau^{\frac{1}{2\mu}}r'$.
\end{proof}

\begin{remark}\label{rem-11-5-15}
It should be noted that if in (\ref{11-5-43}) we skip the regularizing factor $\tilde{\gamma}r$ in $H^0$ (i.e., replace $H^0$ by $H^0_{\st}$) then the conditions of the Statement~\ref{thm-11-5-14-ii} do not change because it follows from the assumptions of the Statement \ref{thm-11-5-14-i} that the set of the points through which pass Hamiltonian billiards generated by $H^0_{\st}$ and reaching $\{\tilde{\gamma}r=0\}$ in a finite time is a set of measure 0.
\end{remark}

We leave to the reader the following rather easy

\begin{problem}\label{problem-11-5-16}
Generalize Theorem~\ref{thm-11-5-14} to operators different from the Schr\"odinger operator.
\end{problem}

\begin{example}\label{ex-11-5-17}
Let $X=\bR^d$, $d\ge 3$ and as $|x|\ge 1$\ \
$V\asymp |x''|^{2\nu }|x|^{2\mu -2\nu }$ where
$x=(x';x'')=(x_1,\dots ,x_{d'};x_{d'+1}\dots ,x_d)$, $d''=d-d'$, $0<d''<d$
(in which case one should try $\rho (x) =|x''| ^\nu \cdot |x|^{\mu -\nu }$,
$\gamma (x) =\frac{1}{2}|x''|$).

Let us assume that the conditions to $g^{jk},V_j,V$ are fulfilled with the indicated $\gamma $ and $\rho $. Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-5-17-i}
$v^{-\frac{d}{2\mu}}\in \sL^1(\bS^{d-1})$ and
$v^{-\frac{1}{2\mu }(d-1-\vartheta )}\tilde{\gamma}^{-1-\vartheta }\in \sL^1(\bS^{d-1})$ if and
only if
\begin{gather}
\nu <\nu_0^*=\mu {\frac{d''}{d}}
\label{11-5-45}\\
\shortintertext{and}
\nu <\nu_{1+\vartheta}^*=\mu (d''-1-\vartheta )(d-1-\vartheta ) ^{-1}
\label{11-5-46}
\end{gather}
respectively.

Therefore for $\nu <\mu (d''-1 )(d-1) ^{-1}$ asymptotics (\ref{11-5-1})\footnote{\label{foot-11-41} As well as asymptotics (\ref{11-5-6}) under the standard condition on Hamiltonian trajectories.} holds, and for $0<\vartheta <d''-1$ under assumption (\ref{11-5-46}) asymptotics
(\ref{11-5-2})--(\ref{11-5-3})\,\footnote{\label{foot-11-42} As well as asymptotics (\ref{11-5-6}), (\ref{11-5-3}) under the standard condition on Hamiltonian trajectories. Both these footnotes remain true below.} holds.

\item\label{ex-11-5-17-ii}
Let $\vartheta=0$. In order to treat the case
$\nu \in [\nu ^*_1,\nu ^*_0]$ when condition (\ref{11-5-45}) holds (or reaches the borderline value) and (\ref{11-5-46}) fails, recall that the original remainder estimate was
\begin{equation*}
R(\tau )=\int_{\{V\le C\tau ,\sqrt \tau \gamma \ge 1\}}
\tau ^{\frac{d-1}{2}}\gamma ^{-1}\,dx+
\int_{\{V\le C\tau ,\sqrt \tau \gamma \le 1\}}\tau ^{\frac{d}{2}}\,dx.
\end{equation*}
Introducing spherical coordinates and integrating over $r$ we obtain the remainder estimate
\begin{equation*}
R(\tau )=\tau ^{l(d-1)}\int_{\{v\le C\tau ^{\mu +1}
\tilde{\gamma}^{2\mu }\}}v^{-{\frac{d-1}{2\mu }}}
\tilde{\gamma}^{-1}\,d\theta +
\tau ^{ld}\int_{\{v\ge C\tau^{\mu+1}\tilde{\gamma}^{2\mu}\}}
v^{-\frac{d}{2\mu}}\,d\theta.
\end{equation*}
We can replace $v$ by $|x''|^{2\nu }\cdot|x|^{2\mu -2\nu }$ here in which case
we arrive to asymptotics
\begin{equation}
\N^- (\tau )=\N^\W (\tau )+ O\bigl(\tau ^{l(d-1)}\log \tau \bigr)
\label{11-5-47}%\tag{10.4.20}
\end{equation}
as $\tau \to+\infty $ provided $\nu =\nu^*_1 $ and the asymptotics
\begin{equation}
\N^- (\tau )=\N^\W (\tau )+O\bigl(\tau ^{l(d-\eta )}\bigr)
\label{11-5-48}%\tag{10.4.21}
\end{equation}
as $\tau \to+\infty $ provided $\nu \in (\nu ^*_1,\nu ^*_0)$ and
$\eta = (-\nu d+\mu d'')(\mu -\nu ) ^{-1}\in (0,1)$.

Here again one can replace $\N^\W (\tau )$ by $\varkappa_0\tau ^{ld}$ with
$\varkappa_0$ given by (\ref{11-5-10}).

\item\label{ex-11-5-17-iii}
Similarly, for $\nu =\nu^*_{\vartheta+1} =
\mu (d''-\vartheta -1)(d-\vartheta -1) ^{-1}$ asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau )=\N^\W_{(\vartheta)} (\tau )+
O\bigl(\tau ^{l(d-1-\vartheta )+\vartheta }\log \tau \bigr)
\label{11-5-49}
\end{equation}
holds as $\tau \to+\infty $ and for
$\nu \in (\nu ^*_{\vartheta +1}, \nu ^*_0)$ asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau )=\N^\W_{(\vartheta)} (\tau )+
O\bigl(\tau ^{l(d-\eta )+\vartheta }\bigr)
\label{11-5-50}
\end{equation}
holds as $\tau \to+\infty $ with
$\eta =\bigl((d''-\vartheta )\mu -(d-\vartheta )\nu \bigr)(\mu -\nu )^{-1}
\in (0,\vartheta +1)$.

\item\label{ex-11-5-17-iv}
Finally, for $\nu =\nu ^*_0$ asymptotics
\begin{equation}
\N^- (\tau)=\N^\W (\tau)+O(\tau^{ld})
\label{11-5-51}
\end{equation}
holds as $\tau \to+\infty $ where
\begin{equation}
\N^\W (\tau )=(2\pi )^{-d}\omega_d
\int_{\gamma \ge \epsilon \tau ^{-\frac{1}{2}}}
(\tau -V)_+^{\frac{d}{2}}\sqrt g \,dx
\label{11-5-52}
\end{equation}
and $\N^\W (\tau )\asymp \tau ^{ld}\log \tau $\,\footnote{\label{foot-11-43} Moreover, under stabilization condition (\ref{11-5-4})
\begin{equation}
\N^\W (\tau)=\bigl(\bar{\varkappa}+o(1)\bigr)\tau^{ld}\log\tau.
\label{11-5-53}
\end{equation}
This statement remains true below.}. The results for $\vartheta >0$ obviously follow from this statement.

In order to prove this statement one needs only note that in the domain
$X_\sing=\{x, |x''|\le \epsilon \tau ^{-\frac{1}{2}}\}$ one can take
$\tilde{\rho} =0$ in the inequality
\begin{equation}
((Au-\tau ),u)\ge \epsilon \|u\|_m^2-C\| \tilde{\rho} ^mu\|^2
\label{11-5-54}
\end{equation}
for all $u\in \fD (A)$ supported in $\bar{X}_\sing$.
Moreover, this estimate yields that

\item\label{ex-11-5-17-v}
All the results of Statements \ref{ex-11-5-17-i}--\ref{ex-11-5-17-iv} remain true for $d=2$.
\end{enumerate}
\end{example}

\begin{figure}[ht]
\centering
\subfloat[]{\label{fig-11-10-a}%
\begin{tikzpicture}
\draw[thick, domain=0.000:6.28,scale=1, smooth] plot[parametric,id=parametric-cusp] function{cos(t), sin(t)};
\draw[thick, dashed, domain=0.0:6.28,scale=1, smooth] plot[parametric,id=parametric-cusp] function{1.5*cos(t), 1.5*sin(t) };
\draw[domain=0.0:6.28,scale=1, smooth] plot[parametric,id=parametric-cusp] function{2*cos(t) , 2*sin(t) };
\end{tikzpicture}}
\quad
\subfloat[]{\label{fig-11-10-b}%
\begin{tikzpicture}[scale=.9]
\draw[thick, domain=0.007:6.276,scale=1, smooth] plot[parametric,id=parametric-cusp] function{cos(t) / (sin(t/2) ** 0.333), sin(t) / (sin(t/2) **0.333)};
\draw[thick, dashed, domain=0.023:6.26,scale=1, smooth] plot[parametric,id=parametric-cusp] function{1.5*cos(t) / (sin(t/2) ** 0.333), 1.5*sin(t) / (sin(t/2) **0.333)};
\draw[domain=0.055:6.23,scale=1, smooth] plot[parametric,id=parametric-cusp] function{2*cos(t) / (sin(t/2) ** 0.333), 2*sin(t) / (sin(t/2) **0.333)};
\end{tikzpicture}}
\caption{\label{fig-11-10} Level lines for non-degenerate \protect\subref{fig-11-10-a} and degenerate in one direction \protect\subref{fig-11-10-b} potential. In the latter case $V\le \tau$ forms a cusp but in contrast to cusps studied in Section~\ref{sect-11-2} and \ref{sect-11-3} this cusp grows and fattens as $\tau\to +\infty$.}
\end{figure}

It is interesting to perturb the potentials treated above by potentials which have a lesser ``average'' growth at infinity bet does not have this degeneration. Namely, we can take perturbing potentials satisfying condition $\textup{(\ref{11-1-7})}_3$ with the same $\gamma $ as above and with
$\rho' =(|x|+1)^{\mu '}$, $0<\mu '<\mu $ instead of $\rho $:
\begin{equation}
|D ^\alpha V'|\le c\rho ^{\prime 2}\gamma ^{-|\alpha |}
\label{11-5-55}
\end{equation}

Then two different situations may arise:

\begin{enumerate}[label=(\alph*), wide, labelindent=0pt]
\item\label{sect-11-5-4-a}
The perturbing potential is also coercive i.e., satisfies (\ref{11-4-5})
with $\rho $ replaced by $\rho '$
\begin{equation}
V'\ge \epsilon_0\rho ^{\prime 2}\qquad \forall x
\label{11-5-56}
\end{equation}
in which case the perturbing potential ``helps'' to the unperturbed one. In this case the above analysis can be applied with no change.

\item\label{sect-11-5-4-b}
 The perturbing potential is indefinite.
\end{enumerate}

In the former case~\ref{sect-11-5-4-a} we leave the detailed analysis to the reader and formulate the following statements:

\begin{theorem}[Coercive perturbations]\label{thm-11-5-18}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-5-18-i}
Let $d\ge 3$ and $X$, $g^{jk}$, $V_j^0$ and $V^0$ be as in Theorem~\ref{thm-11-5-14}. Let $V_j=V_j^0+V'_j$, $V=V^0+V'$ where $V'_j$ and $V'$ satisfy \textup{(\ref{11-5-55})} and \textup{(\ref{11-5-56})} with
$\rho '=\langle x\rangle ^{\mu ' }$, $0<\mu ' <\mu $. Then asymptotics
\textup{(\ref{11-5-1})} holds with
$\N^\W (\tau)=\varkappa_0\tau^{ld}\bigl(1+o(1)\bigr)$ as $\tau \to +\infty$.

\item\label{thm-11-5-18-ii}
Moreover, if the Hamiltonian $H^0$ given by \textup{(\ref{11-5-43})} satisfies the conditions of the Statement~\ref{thm-11-5-14-ii} of Theorem~\ref{thm-11-5-14} then asymptotics \textup{(\ref{11-5-6})}, \textup{(\ref{11-5-3})} holds as $\vartheta=0$.

\item\label{thm-11-5-18-iii}
Finally, if $0<\vartheta <(d-1)$ and \textup{(\ref{11-5-42})} is fulfilled
then in the frameworks of \ref{thm-11-5-18-i} and \ref{thm-11-5-18-ii} asymptotics \textup{(\ref{11-5-2})}--\textup{(\ref{11-5-3})} and
\textup{(\ref{11-5-6})}, \textup{(\ref{11-5-3})} hold respectively.
\end{enumerate}
\end{theorem}

\begin{example}\label{ex-11-5-19}
Let $X$, $g^{jk}$, $V_j^0$ and $V^0$ be as in Example~\ref{ex-11-5-17}. Let $V_j=V_j^0+V'_j$, $V=V^0+V'$ where $V'_j$ and $V'$ satisfy (\ref{11-5-55}) and (\ref{11-5-56}) with $\rho '=\langle x\rangle ^{\mu '}$, $0<\mu '<\mu$, and $\gamma =\epsilon |x''|$. Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-5-19-i}
If $\nu<\nu_{\vartheta+1}$ defined by (\ref{11-5-46}),
$0\le \vartheta <(d''-1)$ then asymptotics (\ref{11-5-2})--(\ref{11-5-3}) holds.

\item\label{ex-11-5-19-ii}
In the case of threshold value
$\nu =\nu_{\vartheta+1}$,
$0\le \vartheta <(d''-1)$ asymptotics (\ref{11-5-47}) holds.

\item\label{ex-11-5-19-iii}
In the case of above threshold value
$\nu_{\vartheta+1} <\nu < \nu_{0}$, with $\nu_0$ defined by (\ref{11-5-45}),
$0\le \vartheta <(d''-1)$ asymptotics (\ref{11-5-50})
holds with $\eta $ given in Example~\ref{ex-11-5-17}(ii)$'$ provided
$\mu '\le \mu '_*=(\mu -\nu )(\nu +1) ^{-1}$.

\item\label{ex-11-5-19-iv}
On the other hand, for $\mu '>\mu '_*$ the remainder estimate is $O(\tau ^q)$ with
\begin{equation*}
q=\frac{1}{2}(d-\vartheta -1)+{\frac{1}{2\mu '\nu }}
\bigl(d'\nu -(\mu -\nu +\mu ')(d''-\vartheta -1)\bigr)
\end{equation*}
for $\vartheta <(d''-1)$ and with
$q=\frac{d'}{2}+\frac{d'}{2\mu '}+\vartheta $ for
$\vartheta >d''-1$.

For $\vartheta =(d''-1)$ the remainder estimate i $O(\tau ^q\log \tau )$ with the same $q$.

\item\label{ex-11-5-19-v}
All these results remain true for $\nu =\nu_0$ and
$\vartheta =0$ with $\N^\W (\tau)\asymp \tau^{lq}\log\tau$.

\item\label{ex-11-5-19-vi}
 Moreover, for $\nu >\nu_0$, $\vartheta =0$ and
$\mu'>\mu'_*$ these results remain true with
$\N^\W (\tau)\asymp \tau^p$ with
$p=\frac{1}{2}(d+\frac{d}{\mu'}-\frac{d''\mu}{\mu'\nu}+\frac{d''}{\nu})$.
Then
$p-q=\frac{1}{2\nu}\bigl(\nu+1-\frac{1}{\mu'}(\mu-\nu)\bigr)>0$.
\end{enumerate}
\end{example}

Let us now consider indefinite perturbations. In this case the perturbation
cannot be too strong.

\begin{theorem}[Indefinite perturbations]\label{thm-11-5-20}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-5-20-i}
Let $d\ge 3$ and let $X$, $g^{jk}$, $V_j^0$ and $V^0$ be as in Theorem~\ref{thm-11-5-14}. Let $V_j=V_j^0+V'_j$, $V=V^0+V'$ where $V'_j$
and $V'$ satisfy \textup{(\ref{11-5-55})} with $\rho '=\langle x\rangle ^{\mu'}$, $0<\mu ' <\mu $ and $\gamma =\tilde{\gamma}|x|$. Then, if
\begin{gather}
v^{-nd-\mu '\vartheta (\mu -\mu ') ^{-1}}\in \sL^1(U)
\label{11-5-57}\\
\shortintertext{and}
v^{-n(d-\vartheta-1)-\mu'\vartheta(\mu-\mu')^{-1}}\tilde{\gamma}^{-\vartheta-1}
\in \sL^1(U)
\label{11-5-58}
\end{gather}
with
$n=\frac{1}{2}(\mu '+1)(\mu -\mu ') ^{-1}$, $0\le \vartheta <(d-1)$
then asymptotics \textup{(\ref{11-5-2})}--\textup{(\ref{11-5-3})} holds and for $\vartheta =0$ \ $\N^\W (\tau )=\varkappa_0\tau ^{ld}+o(\tau ^{l(d-1)})$.

\item\label{thm-11-5-20-ii}
Moreover, if the Hamiltonian $H^0$ given by \textup{(\ref{11-5-43})} satisfies the conditions of Theorem~\ref{thm-11-5-14}\ref{thm-11-5-14-ii}, then asymptotics
\textup{(\ref{11-5-6})}, \textup{(\ref{11-5-3})} holds.
\end{enumerate}
\end{theorem}

\begin{proof}
The proof is similar to the proof of Theorem~\ref{thm-11-5-14} but the domain $\{V\le\tau\}$ consists of two overlapping zones
$\{V^0\le C\tau, \rho'\le C\tau^{\frac{1}{2}}\}$ and
$\{V^0\le C\rho ^{\prime 2}, \tau \le C\rho ^{\prime 2}\}$.


Then $\tilde{\rho}(\tau)\asymp\tau^{\frac{1}{2}}$ and
$\tilde{\rho}(\tau)\asymp\rho'$ in the first and second zones respectively.
\end{proof}

%\renewcommand{\thetheorem}{10.4.13}
\begin{example}\label{ex-11-5-21}
Let $X$, $g^{jk}$, $V_j^0$ and $V^0$ be as in Example~\ref{ex-11-5-17}. Let $V_j=V_j^0+V'_j$, $V=V^0+V'$ where $V'_j$ and $V'$ satisfy (\ref{11-5-55}) with $\rho '=\langle x\rangle ^{\mu '} $, $0<\mu ' <\mu $ and
$\gamma =\epsilon |x''|$.

Let $\mu >\mu '+\nu $ (otherwise the potential $V$ can be semi-bounded from
above or even tend to $-\infty$ in the pipe $\{|x''|\le \epsilon \}$). Moreover, let us assume that
\begin{equation}
\nu < \frac{\mu-\mu'}{\mu'+1}.
\label{11-5-59}%\tag{10.4.25}
\end{equation}
Then considering the zone
\begin{equation*}
X''=\bigl\{x:|x''|\le z(x,\tau )=
\epsilon \min\bigl(\tau^{-\frac{1}{2}},|x|^{-(\mu-\nu)(\nu+1)^{-1}}\bigr)\bigr\}
\end{equation*}
we see that we can take
$\tilde{\rho}(\tau)=(\rho'-\epsilon_1 z^{-1})_+$ in condition (\ref{11-5-54})
where $\epsilon_1>0$ does not depend on $\epsilon$. Then (\ref{11-5-54}) yields
that we can take $\tilde{\rho}(\tau)=0$ in $X''$ for $\tau\ge\epsilon^{-1}$
and small enough $\epsilon$.

On the other hand, (\ref{11-5-59}) yields that
\begin{equation*}
(\tau^{\frac{1}{2}}+\rho)\gamma \ge \epsilon_2>0,\ \
\rho'\le C(\tau^{\frac{1}{2}}+\rho)^{1-\delta}
\end{equation*}
outside of $X''$ where $\delta>0$, $\rho =|x''|^\nu \cdot |x|^{\mu\mu-\nu}$, $\gamma =\epsilon_3|x''|$. Using these assertions one can easily prove that under condition (\ref{11-5-59}) all the statements of Example~\ref{ex-11-5-17} remain true.
\end{example}

We leave to the reader
\begin{problem}\label{problem-11-5-22}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-5-22-i}
Consider the Schr\"{o}dinger operator with coefficients satisfying conditions (\ref{11-1-6})--(\ref{11-1-8}), (\ref{11-4-5}) with
$\rho =\langle x\rangle ^\mu $,
$\gamma =\epsilon \langle x\rangle ^{1-\delta }$, $\mu >0$,
$\delta >0$, $\mu+1>\delta$.

In this case the asymptotics
$\N^-_{(\vartheta)}(\tau)=\N^\W_{(\vartheta)}(\tau)+O(\tau^q)$ appear with
$\N^\W (\tau )\asymp \tau ^p$ in domains conical at infinity.

\item\label{problem-11-5-22-ii}
Consider domains or Riemannian manifolds of type (\ref{11-5-69}) (see below). Then asymptotics appear with other exponents $p$ and $q$. In this example the magnetic field can grow strongly enough at infinity.
\end{enumerate}
\end{problem}

\subsection{Quasi-homogeneous potentials}%
\label{sect-11-5-5}
\index{quasi-homogeneous potential!large eigenvalue asymptotics}%
\index{potential!quasi-homogeneous!large eigenvalue asymptotics}%
\index{large eigenvalue asymptotics!quasi-homogeneous potential}%
\index{asymptotics!large eigenvalue!quasi-homogeneous potential}

Let us now consider the quasi-homogeneous case.

\begin{example}\label{ex-11-5-23}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-5-23-i}
Let $X$ be an $L$-quasi-conical domain in $\bR^d$ and let $g^{jk}$, $V_j$, $V$ be $L$-quasi-homogeneous on $x$ of degrees $0$, $\mu $ and $2\mu $
respectively. Here $\mu >0$ and $L=(L_1,\dots ,L_d)$ with $L_j=1$
for $1\le j\le d'$ and $L_j>1$ for $d'+1\le j\le d$, $0<d'<d$.

Let us assume that $\partial X\setminus 0\in \sC^K$ and
$g^{jk},V_j,V\in \sC^K(\bar{X}\setminus 0)$ satisfy (\ref{11-1-8}) and
$V(x)>0$ for $x\ne 0$.

Then all of the conditions (\ref{11-1-6})--(\ref{11-1-8}) and (\ref{11-4-5}) are fulfilled with
\begin{gather}
\rho =[x]_L^\mu ,\qquad \gamma =\epsilon [x]_L
\label{11-5-60}\\
\shortintertext{for}
[x]_L\coloneqq
\bigl(\sum_j|x|^{\frac{\bar{L}}{L_j}}\bigr)^{\frac{1}{\bar{L}}}\ge 1;
\label{11-5-61}
\end{gather}
for $[x]_L<1$ one should take $\gamma =[x]_L^{\bar{L}}$ with $\bar{L}=\max_jL_j$ here.

Then asymptotics
\begin{equation}
\N^- (\tau )=\varkappa_0\tau ^p+O(\tau ^q)
\label{11-5-62}
\end{equation}
holds with $p={\frac{d}{2}}+{\frac{L^*}{2\mu }}$,
$q=\frac{1}{2} (d-1)+ \frac{1}{2\mu }(L^*-1)$, $L^*=\sum_jL_j$ and with the coefficient
\begin{equation}
\varkappa_0=
(2\pi )^{-d}\omega_d\int (1-V)_+^{\frac{d}{2}}\sqrt g \,dx.
\label{11-5-63}
\end{equation}

We leave the analysis for $\vartheta >0$ to the reader.

\item\label{ex-11-5-23-ii}
In order to improve these asymptotics let us consider the Hamiltonian
billiards generated by the Hamiltonian
\begin{equation}
H=[x]_L^{1-\mu }\bigl(\sum_{j,k} g^{jk}(\xi_j-V_j)(\xi_k-V_k)+V- \tau \bigr).
\label{11-5-64}
\end{equation}
Obviously, the contribution of the zones
$\{x\in X,|x_i|\le \epsilon \tau ^{\frac{L_j}{2\mu }}\}$ to the remainder estimate does not exceed $\epsilon_1\tau ^q$ with $\epsilon_1\to 0$ as
$\epsilon \to +0$ ($i=1,\dots ,d$). So we consider billiards starting from complements to these zones.

One can easily see that along Hamiltonian trajectories
\begin{equation}
{\frac{d\xi_i}{dt\ }}=o\bigl(\tau ^{\frac{1}{2}}\bigr),\qquad
{\frac{dx_i}{dt\ }}= o\bigl(\tau ^{\frac{L_i}{2\mu}}\bigr)
\label{11-5-65}
\end{equation}
as $\tau \to +\infty $ for $i \ge d'+1$ provided
$[x]_L\ge \epsilon \tau ^{\frac{1}{2\mu }}$. Let us fix arbitrarily large $T$ and arbitrarily small $\epsilon >0$ and treat billiards of the length $T$.

Let us assume that $x'\ne 0$, $\nu '\ne 0$ on $\partial X\setminus 0$ where $x'=(x_1,\dots ,x_{d'})$ and $\nu '=(\nu_1,\dots ,\nu_{d'})$,
$\nu =(\nu_1,\dots , \nu_d)=(\nu ',\nu '')$ is a unit normal to $\partial X$. Then in the indicated zone $|\nu ''|=o(1)$ and therefore the increment of $\xi_i$ when a billiard reflects from $\partial X$ is $o(\tau ^{\frac{1}{2}})$ for $i\ge d'+1$.

Therefore $\tau ^{-\frac{1}{2}}\xi_i$ and $\tau ^{-{\frac{L_i}{2\mu }}}x_i$ with $i\ge (d'+1)$ are almost constant along billiards (if the length and the number of reflections are bounded).

Therefore if $(\bar{x}',\bar{\xi}')$ is a good starting point for a billiard generated by the Hamiltonian
$H_{(\bar{x}'', \bar{\xi}'')}= H(x',\bar{x}'',\xi ',\bar{\xi }'')$ in the
cross-section domain $X_{(\bar{x}'')}= \{x':(x',\bar{x}'')\in X\}$ then
$(\bar{x},\bar{\xi})$ is a good starting point for the original Hamiltonian.

Therefore the phase space measure of points which cannot be starting points does not exceed $\epsilon_2\tau ^q$ with arbitrarily small $\epsilon_2>0$. Here
$\tau \ge \tau_0(\epsilon_2)$.

Let us treat the non-periodicity. Let us assume that
\begin{equation}
g^{jk}=0,\quad V_k=0\quad \text{for\ }j\le d',\ k\ge d'+1.
\label{11-5-66}
\end{equation}
Then one can easily show that
$|x''(0)-x''(t)|\ge \varepsilon |t|\tau ^{\frac{1}{2\mu }}$ provided
$t\in [-T,T]$, $|\xi ''|\ge C_{\epsilon ,T}\varepsilon \tau ^{\frac{1}{2}}$,
$\tau \ge \tau_0(\epsilon ,\varepsilon ,T)$ where $\epsilon $ is defined by the above conditions including the transversality condition. Therefore the non-periodicity condition is also fulfilled if we exclude a subset of measure $\epsilon_2\tau ^q$ from the starting point set.

Therefore asymptotics
\begin{equation}
\N^- (\tau )= \N^\W (\tau )+\bigl(\varkappa_1+o(1)\bigr)\tau ^q
\label{11-5-67}
\end{equation}
holds with the coefficient
\begin{equation}
\varkappa_1=\mp {\frac{1}{4}}(2\pi )^{1-d}
\omega_{d-1}\int_{\partial X}(1-V)_+^{\frac{d-1}{2}}\,dS'\sqrt{g''}\,dx''
\label{11-5-68}
\end{equation}
where $dS'$ and $\sqrt{g''}dx''$ are Riemannian densities on the projections $(\partial X)_{x''}=\{x':(x',x'')\in \partial X\}$ and
$X_{x'}=\{x'':(x',x'')\in X\}$ generated by the metrics $(g^{jk})_{j,k\le d'}$
and $(g^{jk})_{j,k\ge d'+1}$ respectively (these metrics and densities depend on $x$). Here the sign ``$\mp$'' corresponds to Dirichlet and Neumann boundary condition respectively.
\end{enumerate}
\end{example}

\begin{remark}\label{rem-11-5-24}
Surely, these statements remain true in the case when the operator tends to an $L$-quasi-homogeneous operator or if assumptions are fulfilled with $\rho $ and $\gamma $ defined by (\ref{11-5-60})--(\ref{11-5-61}); in the latter case only Statement \ref{ex-11-5-23-i} remains true. In the former case
$\N^\W (\tau )=\bigl(\varkappa_0+o(1)\bigr)\tau ^p$ without exact equality.
\end{remark}


\subsection{Quickly growing potentials}%
\label{sect-11-5-6}
\index{quickly growing potential!large eigenvalue asymptotics}%
\index{potential!quickly growing!large eigenvalue asymptotics}%
\index{large eigenvalue asymptotics!quickly growing potential}%
\index{asymptotics!large eigenvalue!quickly growing potential}

In this subsection we consider potentials with more than power growth at infinity. Then the volume of the domain $\{x:V(x)\le \tau\}$ grows slowly as $\tau\to +\infty$ and one should expect that
\begin{equation}
N^\W_{(\vartheta)} \asymp \mes( \{x:V(x)\le \tau\})\cdot \tau^{\frac{d}{2}}
\label{11-5-69}
\end{equation}
have slightly larger magnitude than in the case of the essentially bounded domain.

\begin{figure}[h]
\centering
\subfloat[]{%
\begin{tikzpicture}
\fill[cyan!20, domain=1:5,scale=1, smooth]  plot function{sqrt(x)}
-- plot[domain=5:1] function{-sqrt(x)};
\end{tikzpicture}}\qquad\qquad
\subfloat[]{%
\begin{tikzpicture}
\fill[cyan!20, domain=1:6.25,scale=1, smooth]  plot function{2.25/x}
-- plot[domain=6.25:1] function{-2.25/x};
\end{tikzpicture}}
\caption{\label{fig-11-Y} Domains of the type (\ref{11-5-69})}
\end{figure}

\begin{theorem}\label{thm-11-5-25}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-5-25-i}
Let $d\ge 2$ and let $X$ be a domain in $\bR^d$ such that
\begin{equation}
\Vol(\{x\in X, |x|\asymp  r\}) \asymp r^n\quad \text{as\ \ } r\to+\infty ,
\label{11-5-70}
\end{equation}
$n\le d$.



Let conditions \textup{(\ref{11-1-6})}--\textup{(\ref{11-1-8})} and \textup{(\ref{11-4-5})} be
fulfilled with $\gamma =\epsilon_1\langle x\rangle ^{1-\mu }$,
$\rho =\exp \langle x\rangle ^\mu $, $\mu >0$.

Then asymptotics \textup{(\ref{11-5-2})} holds with the principal part
\begin{gather}
\N^\W_{(\vartheta)}(\tau)\asymp
\tau^{\frac{d}{2}+\vartheta}\sigma (\tau),\\
\sigma  (\tau )=\left\{\aligned
\log^n\tau \qquad &
\text{for\ }n>0 ,\\
\log\log\tau \qquad &\text{for\ }n=0,\\
1\qquad &\text{for\ }n<0.\endaligned\right.
\label{11-5-71}\\
\intertext{and remainder estimate}
R_{(\vartheta)}(\tau)=
\tau^{\frac{1}{2}(d+\vartheta-1)}\omega_{(\vartheta)}(\tau),
\label{11-5-72}\\
\omega_{(\vartheta)} (\tau )=\left\{\aligned
\log^q\tau \qquad &
\text{for\ }q\coloneqq  (n-(1-\mu )(1+\vartheta ))/\mu >0,\\
\log\log\tau \qquad &\text{for\ }q=0,\\
1\qquad &\text{for\ }q<0.\endaligned\right.
\label{11-5-73}
\end{gather}

\item\label{thm-11-5-25-ii}
Moreover, let $q\ge 0$ and for every fixed $k>0$ let condition
\begin{multline}
\Vol \bigl\{x\in X,|x|\le r,\
\dist (x,\partial X)\le k \gamma (x)\bigr\}=o(r^n)\\
\text{as\ \ } r\to +\infty
\label{11-5-74}
\end{multline}
be fulfilled. Furthermore, let
\begin{gather}
|D ^\alpha g^{jk}|=o(\gamma ^{-1})\qquad \text{as\ }|x|\to+\infty \quad
\forall j,k,\alpha :|\alpha |=1,
\label{11-5-75}\\
\shortintertext{and}
|D ^\alpha V_j|\le C\rho \gamma ^{-|\alpha |}\qquad
\forall j, \alpha :|\alpha |\le 1.
\label{11-5-76}
\end{gather}
Then asymptotics \textup{(\ref{11-5-6})} holds with $R_{(\vartheta)} (\tau )$
defined above and with $\varkappa_1=0$ for $\vartheta =0$.
\end{enumerate}
\end{theorem}

\begin{proof}
One can easily prove Statement~\ref{thm-11-5-25-i} in the standard way.

In order to prove Statement~\ref{thm-11-5-25-ii} let us note that if $q>0$ then for $\tau \ge \tau_0(\varepsilon )$ the contributions of the zones
$\{x\in X, |x|\le \varepsilon \log^{\frac{1}{\mu}}\tau^{\frac{1}{2}}\}$
and
$\{x\in X, |x|\ge (1-\varepsilon)\log^{\frac{1}{\mu}}\tau ^{\frac{1}{2}}\}$
to the remainder do not exceed $\varepsilon_1R_{(\vartheta)} (\tau )$ with
$\varepsilon_1\to 0$ as $\varepsilon \to 0$.

Moreover, condition (\ref{11-5-74}) yields that the contribution of the zone
$\{X,\dist (x,\partial X)\le k\gamma (x)\}$ to the remainder is $o(R_{(\vartheta)} (\tau ))$ and therefore one need consider only billiards generated by the improved Hamiltonian and starting in
the zones
\begin{equation*}
X_{k,\varepsilon ,\tau }=\bigl\{X\in X,
\varepsilon \le |x|\log^{-{\frac{1}{\mu }}}\tau ^{\frac{1}{2}}\le
1-\varepsilon , \dist(x,\partial X)\ge
k(\log \tau ^{\frac{1}{2}})^{\frac{1}{\mu }-1}\bigr\}.
\end{equation*}
Then for $t\in [-T,T]$ and $\tau \ge \tau_0(T,k,\varepsilon )$,
$k\ge k_0(T,\varepsilon )$ these billiards lie in $X_{\frac{k}{2},\frac{\varepsilon}{2},\tau}$, they do not hit $\partial X$,
and along them
\begin{multline*}
\tau^{-\frac{1}{2}}V_j \equiv \tau ^{-1}V\equiv 0,\quad
g^{jk}\equiv \const,
\quad \gamma (\log \tau )^{1-\frac{1}{\mu }}\equiv \const,\\
\tau ^{-\frac{1}{2}}\xi_j\equiv \const,\quad
\gamma ^{-1} \frac{dx_j}{dt\ } \equiv
2\tau ^{-\frac{1}{2}}\sum_k g^{jk}\xi_k,
\quad \tau ^{-1}\sum_{j,k} g^{jk}\xi_j\xi_k\equiv 1
\end{multline*}
modulo $o(1)$ as $\tau \to +\infty $.

The rest of the proof is similar to the proof of Theorems~\ref{thm-11-2-7} and~\ref{thm-11-2-8}. The case $q=0$ is treated in the same way with the removal of the zones $\{x\in X,|x|\le R\}$,
$\{x\in X, |x|\ge \epsilon \log^{\frac{1}{\mu }}\tau \}$ and
$\{x\in X, \dist(x,\partial X)\le k\gamma (x)\}$ with arbitrarily small $\epsilon >0$ and arbitrarily large $R$.
\end{proof}

This theorem could be improved.

\begin{theorem}\label{thm-11-5-25a}
In the framework of the previous Theorem~\ref{thm-11-5-25} assume that $g^{jk}$ and  the boundary satisfy smoothness assumptions with
$\gamma(x)=\epsilon \langle x\rangle$ (then $n=d$). Then one can redefine \textup{(\ref{11-5-73})}
\begin{equation}
\omega_{(\vartheta)} (\tau )=
\log^q\tau \qquad
\text{for\ }q\coloneqq  (d-1-(1-\mu )\vartheta )/\mu.
\label{11-5-73a}
\end{equation}
\end{theorem}

\begin{proof}
One can see easily that we can then replace $\gamma(x)=\langle x\rangle^{1-\mu}$ by
\begin{equation}
\gamma_1 (x)=
\epsilon \min\bigl( (\tau/\rho^2)^\delta \gamma(x),\ \langle x\rangle\bigr).
\label{11-5-73b}
\end{equation}
Indeed, one can check easily that it is scaling function
($|\nabla \gamma |\le \epsilon_1$) and that
$|\nabla ^\alpha V|\le C\tau \gamma_1^{-|\alpha|}$,
$|\nabla ^\alpha V_j|\le C\tau^{1/2} \gamma_1^{-|\alpha|}$ for $|\alpha|\le K$.

Then contribution of the zone $\{x: V(x)\le 2\tau\}$ to the remainder does not exceed  $C\int \tau^{(d-1-\theta )/2} \gamma_1^{-1-\theta}\,dx$. Plugging $\gamma_1(x)=(\tau/\rho^2)^\delta \gamma(x)$ and $dx=r^{d-1}\,dr$ we get (\ref{11-5-73}) with $q= d-1-(1-\mu)\vartheta$ and plugging
$\gamma_1=\langle x\rangle$ we get even better remainder estimate.
\end{proof}


In the same way  the following theorem is proven:


\begin{theorem}\label{thm-11-5-26}
Let $d\ge 2$, $X=\bR^+\times X'$ where $X'$ is a bounded domain in
$\bR^{d-1}\ni x'$ with $\sC^K$ boundary. Let all the conditions \textup{(\ref{11-1-6})}--\textup{(\ref{11-1-8})} and \textup{(\ref{11-4-5})} be
fulfilled with $\rho =\exp x_1$ and $\gamma =\epsilon_0>0$ and let
\begin{equation}
g^{jk}-g^{jk0}=o(1),\qquad D_1g^{jk}=o(1)\qquad \text{as\ \ } x_1\to +\infty
\label{11-5-77}
\end{equation}
where $g^{jk0}=g^{jk0}(x')$ and $g^{1k0}=0$ for $k\ge 2$.

Further, let conditions \textup{(\ref{11-5-75})}--\textup{(\ref{11-5-76})} be fulfilled. Then for every $\vartheta >0$ asymptotics \textup{(\ref{11-5-6})} holds with
\begin{equation}
R_{(\vartheta)} (\tau )=\tau ^{\frac{1}{2}(d+\vartheta -1)}\log\tau.
\label{11-5-78}%\tag{10.4.35}
\end{equation}

Further, for $\vartheta =0$ the principal part is
\begin{gather}
\N^\W (\tau )+\varkappa_1\tau ^{\frac{1}{2}(d-1)}\log \tau \label{11-5-79}\\
\intertext{with coefficient}
\varkappa_1=\mp {\frac{1}{8}}(2\pi )^{1-d}\omega_{d-1}
\int_{\partial X'} \frac{dS'}{\sqrt{g^{110}}}
\label{11-5-80}
\end{gather}
where $dS'$ is the Riemannian density on $\partial X'$ generated by
the metric $(g^{jk0})_{j,k\ge 2}$.

Furthermore,
\begin{gather}
\N^\W (\tau)=\bigl({\bar\varkappa}_0+o(1)\bigr)\tau^{\frac{d}{2}}\log\tau
\label{11-5-81}\\
\intertext{with the coefficient}
\bar{\varkappa}_0= \frac{1}{2} (2\pi)^{-d} \omega_{d}
\int_{X'} \sqrt{g^{0\prime}} \frac{dx'}{\sqrt{g^{110}}}
\label{11-5-82}
\end{gather}
where $\sqrt{g^{0\prime}}dx'$ is a Riemannian density on $X'$
generated by the same metric.
\end{theorem}

The following problems look rather interesting but not very difficult:

\begin{Problem}\label{Problem-11-5-27}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{Problem-11-5-27-i}
Consider more general operators than the Schr\"odinger operator.

\item\label{Problem-11-5-27-ii}
 Consider $X=\bR^+\times X'$, where $X'$ is a bounded domain in $\bR^{d-1}$ with $\sC^K$-boundary, $\rho= exp (x_1^\mu)$,
$\gamma \asymp x_1^\sigma$, $\sigma=\max (0,1-\mu)$, $\mu>0$.

\item\label{Problem-11-5-27-iii}
Consider potentials with the degenerations and singularities (in the spirit of Section~\ref{sect-11-5-4}.

\item\label{Problem-11-5-27-iv}
Consider other types of super-power growth.
\end{enumerate}
\end{Problem}


\subsection{Slowly growing potentials}%
\label{sect-11-5-7}
\index{slowly growing potential!large eigenvalue asymptotics}%
\index{potential!slowly growing!large eigenvalue asymptotics}%
\index{large eigenvalue asymptotics!slowly growing potential}%
\index{asymptotics!large eigenvalue!slowly growing potential}

Finally, let us consider potentials with slow growth at infinity. Here we should be very careful and specific since even formula (\ref{11-5-69}) may be not valid anymore.

Namely, let $V=v(\theta )\log r$ in spherical coordinates
$(r,\theta )$. We use $\rho_\tau =(\tau -V)_+^{\frac{1}{2}}$
and $\gamma_\tau =\epsilon_0r\min(1,(\tau -V)_+\log ^{-1}r)$.
Then we obtain

\begin{theorem}\label{thm-11-5-28}
Let $d\ge 3$ and let $g^{jk}=g^{jk}(\theta )$, $V_j=0$, $V=v(\theta )\log r$,
$X=\{\theta \in U\}$ for $r\ge c$ where $(r,\theta )$ are spherical coordinates, $g^{jk}, v, \partial U\in \sC^K$ and $(g^{jk})$ is a positive definite matrix. Let $v_0=\min_Uv>0$. Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-5-28-i}
Asymptotics \textup{(\ref{11-5-2})} holds with
\begin{gather}
\N^\W_{(\vartheta)} \asymp \int_U\exp ({\frac{\tau d}{v}}) \,d\theta ,
\label{11-5-83}\\[3pt]
R_{(\vartheta)} (\tau )=\tau ^{1+\vartheta }\int_{U'}
\exp ({\frac{\tau (d-1-\vartheta )}{v}})\, d\theta
\qquad \text{for\ }\vartheta <d-1.
\label{11-5-84}\\
\intertext{Moreover,}
\N^\W (\tau )=
a\int_{U'}v^{\frac{d}{2}}\exp ({\frac{\tau \ d}{v}}) \sqrt g \,d\theta
\label{11-5-85}
\end{gather}
with
$a=(2\pi)^{-d}\omega_dd^{-(1+\frac{d}{2})}\Gamma(1+\frac{d}{2})=2^{1-d}\pi^{-\frac{d}{2}} d^{-(1+\frac{d}{2})}$ and
$U'= \{\theta \in U, v\le v_0+\varepsilon \}$ with arbitrarily small
$\varepsilon >0$.

\item\label{thm-11-5-28-ii}
In particular, if $v=\const =v_0$ then the principal part is
$\varkappa \exp({\frac{\tau d}{v_0}})$ and the remainder estimate is
$O\bigl(\tau^{1+\vartheta}\exp(\tau(d-\vartheta-1)v_0^{-1})\bigr)$\,\footnote{\label{foot-11-44} One can take
$\gamma_\tau =\epsilon_0r\min(1,(\tau -V)_+)$ in this
case and drop factor $\tau^{1+\vartheta}$ in the remainder estimate.}.

On the other hand, if $v(\theta )=v_0\implies \theta \in \partial U, \nabla v(\theta )\ne 0$ and $\rank\Hess v|_{\partial U}(\theta )=d-2$ then the principal part is $\asymp \tau ^{-{\frac{d}{2}}}\exp(\tau dv_0 ^{-1})$ and the
remainder estimate is
$O\bigl(\tau^{1+\vartheta-\frac{d}{2}}\exp(\tau(d-\vartheta-1)v_0^{-1}))\bigr)$.

In other cases the principal part of the asymptotics and the remainder estimate have intermediate orders.
\end{enumerate}
\end{theorem}

We leave to the reader

\begin{problem}\label{problem-11-5-29}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-5-29-i}
Investigate the case $\vartheta \ge (d-1)$. Note that one can take $\tilde{\rho}(\tau )=\tau ^{\frac{1}{2}}+(\log r)^{\frac{1}{2}}$,
$\tilde{\gamma}(\tau )=\epsilon_0r$ and for $d\ge 2$ and smooth
$\partial X$, $g^{jk}$, $V_j$ and $V$ we obtain the remainder estimate
$R_{(\vartheta)} (\tau )=C\tau ^d$ for $\vartheta =d-1$ and
$R_{(\vartheta)} (\tau )=C\tau ^{\frac{1}{2}(d+\vartheta -1)}$ for
$\vartheta >(d-1)$.

\item\label{problem-11-5-29-ii}
Consider potential $V=v(\theta )\log ^\mu r$.

\item\label{problem-11-5-29-iii}
Consider potentials with degenerations and singularities. Obviously in this case the degeneration should be very weak, something like
\begin{equation*}
(\log (|x|^2+2))^\mu \cdot (\log (|x''|^2+2))^{-\nu}.
\end{equation*}
\end{enumerate}
\end{problem}


\subsection{Non-Dirichlet boundary conditions}
\label{sect-11-5-8}

All our results have been obtained for Dirichlet boundary conditions. Surely, they remain true for other boundary conditions provided these conditions are regular in the obvious sense and the domain satisfies the cone condition. In particular, for the Schr\"{o}dinger operator Neumann conditions (and Robin conditions provided the free term coefficient is regular in the obvious sense) are regular.

Then we obtain that if the domain satisfies the cone condition and if the asymptotics do not distinguish Dirichlet and Neumann boundary conditions then the asymptotics remain true for mixed boundary condition when Dirichlet and Neumann boundary conditions are given on $Y_0\subset \partial X$ and
$Y=\partial X\setminus Y_0$ respectively.

Let us consider more accurate asymptotics distinguishing Dirichlet
and Neumann the boundary conditions. Then, repeating arguments of
Subsection~\ref{sect-11-2-3} we obtain that these asymptotics remain true for mixed boundary conditions with properly defined second coefficient provided either

\begin{enumerate}[label=(\alph*), wide, labelindent=0pt]
\item\label{sect-11-5-8-a}
We are in the frameworks of Theorems~\ref{thm-11-5-3},~\ref{thm-11-5-14}\ref{thm-11-5-14-ii}), \ref{thm-11-5-18}\ref{thm-11-5-18-ii} and
\begin{equation}
\mes_{\partial X}\bigl( (\bar{Y}_0\cap {\bar Y}_1\cap
\{|x|\ge c\})_\cone\bigr)=0
\label{11-5-86}
\end{equation}
or
\item\label{sect-11-5-8-b}
we are in the framework of Example~\ref{ex-11-5-23}\ref{ex-11-5-23-ii} and
\begin{equation}
\mes_{\Pi '\partial X}
\bigl(\Pi ' ( \bar{Y}_0\cap \bar{Y}_1\cap\{|x|\ge c\})_\cone\bigr)=0
\label{11-5-87}
\end{equation}
where $\Pi '$ is the projection $\bR^d\ni x\to x'\in \bR^{d'}$ or

\item\label{sect-11-5-8-c}
We are in the framework of Theorem~\ref{thm-11-5-26} and
\begin{equation}
\mes_{\partial X'}
\bigl(\Pi ' (\bar{Y}_0\cap \bar{Y}_1\cap \{|x|\ge c\})\bigr)=0
\label{11-5-88}
\end{equation}
with the same $\Pi '$. Here $M_\cone$ is the conical hull of the set
$M$.

Moreover, applying the arguments of Example~\ref{ex-11-2-27} we obtain that
asymptotics (\ref{11-5-16}) remains true in the context of Example~\ref{ex-11-5-7} provided
\begin{equation}
\mes_{\partial X}\{x\in \partial X,
\dist (x,Y) \le \varepsilon \}=O(\varepsilon ^\delta ) \qquad
\text{as\ \ }\varepsilon \to +0
\label{11-5-89}
\end{equation}
with $\delta >0$ and $Y=(\bar{Y}_0\cap \bar{Y}_1\cap\{|x|\ge c\})_\cone$.

Finally, we would like to note that in almost all the above examples
the remainder estimate is $O(\tau ^{\frac{1}{2}(d+\vartheta -1)})$ for large enough $\vartheta$ (for the Schr\"{o}dinger operator). In this case the principal contribution to the remainder estimate is provided by the zone
$\{x\in X, |x|\le R\}$ with arbitrarily large $R$. In this case the standard non-periodicity condition to the Hamiltonian $\sum_{j,k}g^{jk}\xi_j\xi_k$ on the energy level  $\tau =0$ provides the remainder estimate
$o(\tau ^{{\frac{1}{2}}(d+\vartheta -1)})$ (see, e.g., Theorem~\ref{thm-11-5-3}).

The situation in which the principal contributions to the principal part of the asymptotics and to the remainder estimate are provided by different zones is not very exotic.
\end{enumerate}


\section{Asymptotics of eigenvalues near $-0$}
\label{sect-11-6}
In this section we consider Schr\"{o}dinger operators with potentials decaying at infinity. Under certain rather general assumptions its continuous spectrum is $[0,\infty)$ and the point $-0$ is the only possible limit point of the discrete spectrum. Moreover, there are no positive eigenvalues.

\begin{figure}[th]
\centering
\begin{tikzpicture}[xscale=1.2]
\draw[thick, domain=-4.6:4.6,scale=1, smooth] plot function{-6/(x**2+1)**.3};
\clip[domain=-4.6:4.6,scale=1, smooth] plot function{-6/(x**2+1)**.3};
\foreach \y in {-5, -4, -3.25, - 2.75, -2.5} \draw[thin, cyan] (-4.6,\y)--(4.6,\y);
\end{tikzpicture}
\caption{\label{fig-11-11}  Slowly decaying at infinity potential; blue lines show symbolically energy levels of the corresponding Schr\"odinger operator.}
\end{figure}

Further, as potential is negative (at least in massive zones so that
$\mes (\{x, V(x)<0\})=\infty$ and potential decays slowly ($|x|^{-2}$ is a threshold) $-0$ is a limit point of the discrete spectrum. In this case we obtain asymptotics of $\N^- (\tau)$ as $\tau \to-0$.

We treat more general higher-order operators and non-semi-bounded operators as well. In particular, we treat the Dirac operator with positive mass $M$ where a spectral gap $(-M,M)$ appears in the case of $V=0$ (while continuous spectrum occupies $(-\infty,-M]\cup[M,\infty)$ and in the general case of decaying potential there could be a discrete spectrum inside the spectral gap and if $V$ decays slowly enough these eigenvalues accumulate to $-M+0$ and/or $M-0$. So we will treat \emph{asymptotics of eigenvalues accumulating to the border of the essential spectrum}\index{eigenvalues accumulating to the border of the essential spectrum}.

Later we consider much more subtle mechanism when the similar situation appears: Schr\"odinger and Dirac operators with magnetic field or operator with periodic coefficients. Essential spectrum may occupy spectral bands or separate points (separating spectral gaps). In both cases adding decaying potential one may create discrete spectrum inside the spectral gap and these eigenvalues may accumulate to its borders.

\subsection{Standard results}
\label{sect-11-6-1}

We start with semi-bounded operators. First of all the following
statement holds:

\begin{theorem-foot}\label{thm-11-6-1}\footnotetext{\label{foot-11-45} Cf. Theorem~\ref{thm-11-5-1}.}
\index{power decay potential!asymptotics of eigenvalues tending to $-0$}%
\index{potential!power decay!asymptotics of eigenvalues tending to $-0$}%
\index{eigenvalues tending to $-0$!asymptotics of!power decay potential}%
\index{asymptotics!eigenvalues tending to $-0$!power decay potential}
Let $X$ be an unbounded connected domain in $\bR^d$ and let
conditions \textup{(\ref{11-1-1})}--\textup{(\ref{11-1-3})} be fulfilled with
$\gamma =\epsilon_1\langle x\rangle $,
$\rho =\langle x\rangle ^\mu $, $\mu \in (-1,0)$.

Let us assume that
\begin{equation}
\blangle a(x,\xi )v,v\brangle \ge \epsilon_0|\xi |^{2m}\1v\1 ^2
\qquad \forall \xi \;\forall v
\label{11-6-1}
\end{equation}
where $a(x,\xi )$ is the senior symbol of $A$.

Further, let us assume that for every $\tau \in (-\epsilon ,0]$ one of non-degeneracy conditions is fulfilled for the symbol $(A(x,\xi )\tau^{-1}-1)$ uniformly with respect to $(\tau ,x,\xi )$ (this condition is restrictive
only for $|x|\ge C_0$). Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-6-1-i}
Asymptotics
\begin{equation}
\N^- (\tau )=\N^\W (\tau )+O\bigl(\tau ^{l(d-1)}\bigr)
\label{11-6-2}
\end{equation}
holds as $\tau \to -0$, where $\N^\W (\tau)$ is given by \textup{(\ref{11-4-9})} and $\N^\W =O(\tau^{ld})$ with $l=\frac{1}{2m\mu}(\mu+1) <0$.

\item\label{thm-11-6-1-ii}
Moreover, for $0<\vartheta \le \vartheta^*_0=-ld$ asymptotics
\begin{equation}
\N^-_{(\vartheta)}(\tau )=
\N^\W_{(\vartheta)} (\tau )+ O\bigl(R_{(\vartheta)} (\tau )\bigr)
\label{11-6-3}
\end{equation}
holds as $\tau\to -0$ with $\N^\W_{(\vartheta)}(\tau)=\tau_+^{\vartheta-1}*\N^\W$ where in this case
$\N^\W$ should contain also lower order terms and
\begin{equation}
R_{(\vartheta)} (\tau )= \left\{\begin{aligned}
|\tau |^{l(d-1)+\vartheta (1-l)}\qquad &
\text{for\ }\vartheta <\vartheta^*_1, \\
\log |\tau |\qquad &\text{for\ }\vartheta =\vartheta^*_1, \\
1 \qquad &\text{for\ }\vartheta >\vartheta^*_1\end{aligned}\right.
\label{11-6-4}
\end{equation}
where $\vartheta^*_1=-l(d-1)(1-l) ^{-1}$.

One can see easily that $0<\vartheta^*_1<\vartheta^*_0$ and that
\begin{equation}
\N^\W_{(\vartheta)} (\tau )=\left\{\begin{aligned}
O\bigl(|\tau |^{ld+\vartheta }\bigr)\qquad
&\text{for\ }\vartheta <\vartheta^*_0\\
O\bigl(\log |\tau |\bigr) \qquad &\text{for\ }\vartheta = \vartheta^*_0
\end{aligned}\right.
\label{11-6-5}
\end{equation}
as $\tau \to -0$ while for $\vartheta >\vartheta^*_0$ we have estimate
$\N^\W_{(\vartheta)} =O(1)$.

\item\label{thm-11-6-1-iii}
Furthermore, if
\begin{multline}
\mes\bigl(\{x\in X: |x|\le r\;\And\exists \xi \in \bR^d:\\
\Spec A(x,\xi )\cap (-\infty , -\epsilon_1\rho ^{2m}]\ne
\emptyset \}\bigr) \asymp r^d\qquad \text{as\ }r \to +\infty
\label{11-6-6}%\tag{10.5.4}
\end{multline}
for some $\epsilon_1>0$ then
\begin{equation}
\N^\W_{(\vartheta)} (\tau )\asymp \left\{\begin{aligned} |\tau
|^{ld+\vartheta } \qquad &\text{for\ }\vartheta <\vartheta^*_0\\
\log |\tau | \qquad &\text{for\ }\vartheta =\vartheta^*_0\end{aligned}\right.
\label{11-6-7}
\end{equation}
as $\tau \to -0$.

For the Schr\"{o}dinger operator condition \textup{(\ref{11-6-7})} is equivalent to
\begin{equation}
\mes \bigl(\{x\in X: |x|\le r,V\le -\epsilon_1\rho ^2\}\bigr)\asymp
r^d \qquad \text{as\ }r\to+\infty.
\label{11-6-8}
\end{equation}
\end{enumerate}
\end{theorem-foot}

\begin{theorem-foot}\label{thm-11-6-2}\footnotetext{\label{foot-11-46} Cf. Theorem~\ref{thm-11-5-3}.}
Let assumptions of Theorem~\ref{thm-11-6-1} be fulfilled.

Further, let us assume that $X\cap \{|x|\ge r_0\}=X^0\cap \{|x|\ge r_0\}$ where $X^0$ is a non-empty conical domain with $\partial X^0\setminus 0\in \sC^K$ and that stabilization conditions \textup{(\ref{11-5-4})} are fulfilled. Let us assume that as $\tau =-1$ the standard non-periodicity condition to Hamiltonian trajectories for the quasi-homogeneous symbol
\begin{equation}
A^0(x,\xi )=\sum_{|\beta |\le 2m}a^0_\beta (x)\xi ^\beta
\label{11-6-9}
\end{equation}
satisfies, and the permitted\footref{foot-11-37} trajectories never hit
$0\times \bR^d$. Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-6-2-i}
Asymptotics
\begin{equation}
\N^- (\tau )=\N^\W (\tau )+
\bigl(\varkappa_1+o(1)\bigr)|\tau| ^{l(d-1)}
\label{11-6-10}
\end{equation}
holds as $\tau \to -0 $. In particular, for the Schr\"{o}dinger operator
\begin{equation}
\varkappa_1=\mp{\frac{1}{4}}(2\pi )^{1-d}\omega_{d-1}
\int_{\partial X^0}\bigl(-1-V^0\bigr)_+^{\frac{d-1}{2}}dS^0
\label{11-6-11}
\end{equation}
for Dirichlet or Neumann  boundary conditions respectively where
the notation of \textup{(\ref{11-5-10})}--\textup{(\ref{11-5-11})} is used.

\item\label{thm-11-6-2-ii}
Moreover, for $0<\vartheta < \vartheta^*_1$
asymptotics
\begin{equation}
\N_{(\vartheta)}^- (\tau )=\N^\W_{(\vartheta)} (\tau )+
o\bigl(R_{(\vartheta)} (\tau )\bigr)\qquad \text{as\ \ } \tau \to-0.
\label{11-6-12}
\end{equation}
holds.


\item\label{thm-11-6-2-iii}
Finally, let $\vartheta =\vartheta^*_1$; the condition on the domain
and the stabilization condition remain true. Moreover, let the non-periodicity condition to Hamiltonian trajectories be fulfilled for the symbol $A^0(x,\xi)$ on the energy level  $0$ and let the permitted\footref{foot-11-37} trajectories never hit $0\times \bR^d$.

Then asymptotics \textup{(\ref{11-5-6})} also holds (so the remainder estimate is $o(\log |\tau|)$ rather than $O(\log |\tau|)$).
\end{enumerate}
\end{theorem-foot}

\begin{proof}[Proof of Theorems \ref{thm-11-6-1} and \ref{thm-11-6-2}]
The proof is similar to the proof of theorems \ref{thm-11-5-1} and \ref{thm-11-5-3} but now in the zone $X'_\reg$, $\rho _\tau \asymp \rho$
(instead of $\rho_\tau \asymp |\tau|^{\frac{1}{2m}}$) and
$X'_\reg \subset \{\rho \ge \epsilon_2 |\tau|^{\frac{1}{2m}}\}$ with
appropriate $\epsilon_2>0$.

Further, every bounded domain gives a finite contribution to the remainder estimate (and therefore in the contrast to \ref{thm-11-5-3} there is no assertion about improved asymptotics as $\vartheta>\vartheta^*_1$), Furthermore, the reduced Hamiltonian is now $|x|^{1-2m\mu +\mu }A^0 (x,\xi )$.

We would like to emphasize that for $\vartheta >\vartheta^*_0$ we obtain the estimate $\N^-_{(\vartheta)} (-0 )<\infty $ instead of asymptotics. This remark remains true in many examples below.

In the framework of Theorem~\ref{thm-11-6-2} the remainder estimate is
$o(|\tau | ^{l(d-1)+\vartheta (1-l)})$ and $o(\log |\tau |)$ in asymptotics (\ref{11-5-6}) for $\vartheta <\vartheta^*_1$ and $\vartheta =\vartheta^*_1$ respectively.

Finally, the main contributions to the remainder estimate are made by the zones
$\{x,|x|\ge \varepsilon |\tau|^{\frac{1}{2m}}\}$ and
$\{x,R\le |x|\le \varepsilon |\tau|^{\frac{1}{2m}}\}$ for
$\vartheta <\vartheta^*_1$ and $\vartheta =\vartheta^*_1$ respectively with arbitrarily small $\varepsilon >0$ and arbitrarily large $R$. This difference leads to different non-periodicity conditions.
\end{proof}


\begin{remark}\label{rem-11-6-3}
If only stabilization conditions \textup{(\ref{11-5-4})}
(including the condition $X\cap\{|x|\ge r_0\}=X^0\cap\{|x|\ge r_0\}$) are
fulfilled then the non-degeneracy condition is automatically fulfilled and
$\N^\W (\tau )= \varkappa_0|\tau |^{ld}\bigl(1+o(1)\bigr)$ as $\tau \to -0$ where for the Schr\"{o}dinger operator
\begin{equation}
\varkappa_0= (2\pi )^{-d}\omega_d
\int_{X^0} \bigl(-1-V^0\bigr)_+^{\frac{d}{2}} \sqrt{g^0}dx
\label{11-6-13}
\end{equation}
in the notation of \textup{(\ref{11-5-10})}--\textup{(\ref{11-5-11})}.
\end{remark}

For scalar operators we get the following\enlargethispage{\baselineskip}

\begin{theorem-foot}\label{thm-11-6-4}\footnotetext{\label{foot-11-47} Cf. Theorem~\ref{thm-11-5-5}.}
Let $X$ be an unbounded connected domain in $\bR^d$ and let conditions \textup{(\ref{11-1-1})}--\textup{(\ref{11-1-3})} be fulfilled with
$\gamma =\epsilon_1\langle x\rangle $,
$\rho =\langle x\rangle ^\mu $, $\mu \in (-1,0)$.

Let condition \textup{(\ref{11-6-1})} be fulfilled and let $A$ be a scalar operator. Then asymptotics
\begin{equation}
\N (\tau )=\N^\W (\tau )+O\bigl(\tau ^{l(d-1)-\delta }\bigr)
\label{11-6-14}
\end{equation}
hold as $\tau \to -0 $, and for $\vartheta >0$ asymptotics
\textup{(\ref{11-6-3})} holds.
\end{theorem-foot}


\subsection{Strongly non-periodic Hamiltonian flow}
\label{sect-11-6-2}
\index{Hamiltonian!flow!non-periodic}%
\index{non-periodic!Hamiltonian flow!asymptotics of eigenvalues tending to $-0$}%
\index{eigenvalues tending to $-0$!asymptotics of!non-periodic Hamiltonian flow}%
\index{asymptotics!eigenvalues tending to $-0$!non-periodic Hamiltonian flow}

In what follows we consider homogeneous potentials with singularities. Now we obtain a more precise remainder estimate under more restrictive conditions on the Hamiltonian flow. One can prove easily the following

\begin{theorem-foot}\label{thm-11-6-5}\footnotetext{\label{foot-11-48} Cf. Theorem~\ref{thm-11-5-6}.}
Let the conditions of Theorem~\ref{thm-11-6-1} be fulfilled and let $A$ be a scalar operator. Moreover, let us assume \textup{(\ref{11-5-14})} is fulfilled i.e. that \underline{either} $X^0=\bR^d$ \underline{or} $A$ is the Schr\"{o}dinger operator or its power.

Further, let stabilization condition \ref{11-5-4-*} be fulfilled. Furthermore, let us assume that the Hamiltonian flow (with reflections at $\partial X^0$) is of non-periodic power type\footnote{\label{foot-11-49} Footnote \footref{foot-11-38} of the previous section remains true.} at negative energy levels and that along the trajectories $(x(t),\xi (t))$ with
$(x(0),\xi (0))\in \Lambda ^0_{\varepsilon ,T}\subset\Sigma_{-1}$,
$|x(0)|=1$, $\varepsilon =T^{-M}$ condition $|x(t)|\ge T^{-M_1}$ is fulfilled.

Then asymptotics
\begin{equation}
\N^- (\tau )=\N^\W (\tau )+
\bigl(\varkappa_1+ O(|\tau |^{\delta'})\bigr)\tau ^{l(d-1)}
\label{11-6-15}
\end{equation}
holds as $\tau \to -0$ with $\delta '>0$. Moreover, for
$0<\vartheta \le \vartheta^*_1-\delta $ with $\delta >0$ asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau )= \N^\W_{(\vartheta)} (\tau )+
O\bigl(|\tau |^{l(d-1)+\vartheta (1-l)+\delta '}\bigr)
\label{11-6-16}
\end{equation}
holds as $\tau \to -0 $ with $\delta '=\delta '(d,m,\delta ,L)>0$.
\end{theorem-foot}

Let us consider the following\enlargethispage{\baselineskip}

\begin{example-foot}\label{ex-11-6-6}\footnotetext{\label{foot-11-50} Cf. Example~\ref{ex-11-5-7}.}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-6-6-i}
The condition of Theorem~\ref{thm-11-6-5} to the Hamiltonian flow is
fulfilled for the Schr\"{o}dinger operator with $X^0=\bR^d$ and
$A^0(x,\xi )=|\xi |^2-|x| ^{2\mu}$ with $\mu\ne -\frac{1}{2}$. So we consider
$\mu \in (-1,-\frac{1}{2}) \cup (-\frac{1}{2},0)$.

\item\label{ex-11-6-6-ii}
Therefore the statement of Theorem~\ref{thm-11-6-5} is true for this operator (provided all the other conditions of this theorem, including
\ref{11-5-4-*}, are fulfilled) and for any $2m$-order operator with
$A^0(x,\xi )=(|\xi |^2-|x|^{2\mu })^m$, and one can replace $X^0=\bR^d$ by the $X^0$ obtained after (a sequence of) the transformations (a),(b) of Example~\ref{ex-11-5-7}\ref{ex-11-5-7-ii}.
\end{enumerate}
\end{example-foot}

\subsection{Periodic Hamiltonian flow}%
\label{sect-11-6-3}
\index{Hamiltonian!flow!periodic}%
\index{periodic Hamiltonian flow!asymptotics of eigenvalues tending to $-0$}%
\index{eigenvalues tending to $-0$!asymptotics of!periodic Hamiltonian flow}%
\index{asymptotics!eigenvalues tending to $-0$!periodic Hamiltonian flow}

As in the previous section let us consider the case of periodic Hamiltonian flow:

\begin{theorem-foot}\label{thm-11-6-7}\footnotetext{\label{foot-11-51} Cf. Theorem~\ref{thm-11-5-9}.}
Let $X^0=\bR^d$ and conditions \textup{(\ref{11-5-27})}--\textup{(\ref{11-5-27})}, \textup{(\ref{11-5-32})} with $\mu \in (-1,0)$ be fulfilled in the domain of negative energies. Let
us introduce the symbol
\begin{equation}
b(x,\xi )=-\frac{l}{T_0} \int_0^{T_0}A^1\circ \Psi_tdt
\label{11-6-17}
\end{equation}
where $T_0$ is the period on the energy level $-1$ (compare with
\textup{(\ref{11-5-30})}; we have changed sign because $A^0(x,\xi )=-1$ now). Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-6-7-i}
If $\delta_1<(\mu +1)$ and condition \textup{(\ref{11-5-31})} is fulfilled for all $\omega $ then asymptotics
\begin{equation}
\N^- (\tau )=
\N^\W (\tau )+O\bigl(|\tau |^{l(d-1)+\delta ''}\bigr)
\label{11-6-18}
\end{equation}
holds as $\tau \to -0$ with $\delta ''>0$.

\item\label{thm-11-6-7-ii}
If $\delta_1\in [\mu +1,2\mu +2]$ then for $\tau \to-0$ such
that $|\tau |^l\in \bigcup_{n\in \bZ^+}J_n$ asymptotics
\begin{equation}
\N^- (\tau )=\N^\W (\tau )+F(\tau ) |\tau |^{l(d-1)}+
O\bigl(|\tau |^{l(d-1)+\delta ''}\bigr)
\label{11-6-19}
\end{equation}
holds with $\delta ''>0$ and
\begin{multline}
F(\tau )=\\
(2\pi )^{-d}lT_0^{-1}\int_{\Sigma_{-1}} \Upsilon
\Bigl(T_0l^{-1}\bigl((|\tau |^l-{\frac{\pi }{4}}\omega_0)-
|\tau |^{l-{\frac{\delta_1}{2m\mu }}}b\bigr)\Bigr) dxd\xi :dA^0.
\label{11-6-20}
\end{multline}
The intervals $J_n$ are defined in Theorem~\ref{thm-11-5-9}(ii) with
$\nu = -\frac{2\pi l}{T_0}$, $\omega_0$ replaced by $-\omega_0$ where $\omega_0$ is the Maslov index of the trajectory $\Psi_t$ with $t\in (0,T_0)$.
\end{enumerate}
\end{theorem-foot}

Let us treat the perturbed Schr\"{o}dinger operator with the Coulomb potential more carefully. In this case $A_0=|D|^2-|x|^{-1}$ and $\mu =-\frac{1}{2}$, $l=-\frac{1}{2}$, $T_0=\frac{\pi}{2}$, $\nu =2$ and the Hamiltonian trajectories are Keplerian ellipses (with one focus located at the origin). Moreover,
$\omega_0\equiv\- 2(d-1) \mod 4\bZ$ and
\begin{equation}
\Spec (A_0)=\{\tau_n= -1(d+1+2n)^2,\;n\in\bZ^+\}
\label{11-6-21}
\end{equation}
and the multiplicity of $\tau_n$ is $P(n)$ where $P(n)$ is a polynomial of
degree $(d-1)$ in $n$. Let us introduce the function
$f(\tau )=\frac{1}{2}(-\tau )^{-\frac{1}{2}}-\frac{1}{2}$.

We leave to the reader

\begin{problem}\label{problem-11-6-8}
Prove that for generic positively homogeneous functions $a^1_\beta$ (with $|\beta|\le k$) of degree $(-1+2|\beta|-\delta_1)$ condition (\ref{11-5-31}) is fulfilled for all $\omega \in \bR$ and therefore asymptotics (\ref{11-6-18}) holds for $0<\delta_1<\frac{1}{2}$ while asymptotics (\ref{11-6-19})--(\ref{11-6-20}) holds for $\delta_1\ge \frac{1}{2}$, and now there is no restriction of the type ``$\delta_1\le 2\mu +2$'' on $\delta_1$ and $k=0,1,2$ is arbitrary.

Moreover, prove that one can take $V'=v_0|x|^{-1-\delta }$ with an
arbitrary exponent $\delta >0$ and an arbitrary constant $v_0\ne 0$.
\end{problem}

Let us assume that $b=0$. There are two possibilities in this case: the trivial possibility is to take $\delta_2\in (\delta_1,2\delta_1)$ and the non-trivial one is to take $\delta_2=2\delta_1$. In the first case all the previous
statements remain true with $\delta_1$ replaced by $\delta_2$ etc.

In the second case we assume that condition (\ref{11-5-39}) is fulfilled in which case the symbol $b(x,\xi )$ is given by formula (\ref{11-3-27}) with $b$ and $b^s$ replaced by $-{\frac{1}{2}}A^1(-A^0)^{-\frac{1}{2}}$ and
$-\frac{1}{2}A^2(-A^0)^{-\frac{1}{2}}+\frac{3}{4}(A^1)^2(-A^0)^{-\frac{3}{2}}$
respectively and with integration from 0 to $\pi$, $\frac{\pi}{2}$ instead of $2\pi$, $\pi$ respectively.

Further, the numerical factor on every integral is $\frac{1}{\pi}$ instead of $\frac{1}{2\pi}$. Furthermore, one can move $A^0$ out of the Poisson brackets and then take $A^0=-1$. Therefore
\begin{multline}
b(x,\xi )={\frac{1}{2\pi }}\int_0 ^\pi
\bigl(A^2-{\frac{3}{2}}(A^1)^2\bigr)\circ \Psi_tdt+\\
{\frac{1}{2\pi }}\int_0 ^{\frac{\pi}{2}}\int_0 ^{\frac{\pi}{2}}
\{A^1\circ \Psi_t,A^1\circ \Psi_{t+t'}\}dtdt'.
\label{11-6-22}
\end{multline}

Therefore the following assertion has been proven:

\begin{theorem}\label{thm-11-6-9}
Let $x^0=\bR^d$, $A=A^{0\w}+A^{1\w}+A ^{\prime\prime \w}$ where $A''$ satisfies
condition \textup{(\ref{11-5-29})} with $a^2_\beta ,\delta_2$ instead of
$a^1_\beta ,\delta_1$, $\delta_2=2\delta_1$ and $a^j_\beta $ are
functions which are positively homogeneous of degrees $(-1+2|\beta |-\delta_j)$ with respect to $x$, smooth for $x\ne 0$. Let condition \textup{(\ref{11-5-39})} be fulfilled and let us define the symbol $b$ by \textup{(\ref{11-6-22})}.
Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-6-9-i}
If $\delta_2< \frac{1}{2}$ and condition \textup{(\ref{11-5-31})} is fulfilled for every $\omega \in \bR$ then asymptotics \textup{(\ref{11-6-18})} hold as $\tau \to-0$.

\item\label{thm-11-6-9-ii}
If $\delta_2\ge \frac{1}{2}$ and condition \textup{(\ref{11-5-31})} is
fulfilled for some $\omega \in \bR$ then asymptotics
\textup{(\ref{11-6-19})}--\textup{(\ref{11-6-20})} holds as $\tau \to-0$ and
$(-\tau )^{-{\frac{1}{2}}}\in\bigcup_{n\in \bZ^+}$ where $J_n$ are
given in Theorem~\ref{thm-11-5-9}\ref{thm-11-5-9-ii} with
$\omega_0=2(d-1),\mu =2$ and with $\delta_1$ replaced by $\delta_2$ everywhere.
\end{enumerate}
\end{theorem}

One can easily prove that for fixed $a^1_\beta $ with $|\beta |\le 2$
satisfying (\ref{11-5-39}) and for generic $a^2_\beta $ with $|\beta |\le k$
condition (\ref{11-5-33}) is fulfilled for all $\omega \in \bR$; here
$k=0,1,2$ is arbitrary.


\subsection{Singularities}
\label{sect-11-6-4}
Let us consider homogeneous lower order terms with singularities (for the Schr\"{o}dinger operator only):

\begin{theorem-foot}\label{thm-11-6-10}\footnotetext{\label{foot-11-52} Cf. Theorem~\ref{thm-11-5-14}.}
Let $d\ge 2$, $X=\{(r,\theta )\in \bR^+\times U\}$ where
$U\subset\bS^{d-1}$ and let $g^{jk}=g^{jk}(\theta )$, $V_j=v_j(\theta )r^\mu $, $V=v(\theta )r^{2\mu }$, $\mu \in (-1,0)$. Further, let $\tilde{\rho}=\tilde{\rho}(\theta )$ and
$\tilde{\gamma}=\tilde{\gamma}(\theta )$ be functions on $U$ and let conditions \textup{(\ref{11-1-6})}--\textup{(\ref{11-1-8})} be fulfilled.

Furthermore, assume that \underline{either} $d\ge 3$ \underline{or}
$\tilde{\rho}\tilde{\gamma}\ge \epsilon_0>0$. Finally, let
\begin{gather}
\tilde{\rho}^{-\frac{d}{\mu}}\in \sL^1(U),\label{11-6-23}\\[2pt]
\tilde{\rho}^{-\frac{1}{\mu}(d-1)}\tilde{\gamma}^{-1}\in \sL^1(U).\label{11-6-24}
\end{gather}
Moreover, let $v(\bar{\theta})<0$ for some $\bar {\theta }\in U$.

\item\label{thm-11-6-10-i}
Then asymptotics \textup{(\ref{11-6-2})} holds and
$\N^\W (\tau )=\varkappa_0| \tau |^{ld}$ with the coefficient $\varkappa_0$ given by \textup{(\ref{11-6-13})}.

\item\label{thm-11-6-10-ii}
Further, if $\vartheta \in (0,\vartheta^*_1)$,
$\vartheta^*_1=-l(d-1)(1-l) ^{-1}=(1+\mu )(d-1)(1-\mu ) ^{-1}$ and if
\begin{equation}
\tilde{\rho}^{-\frac{1}{\mu}(d-1-\vartheta)}\tilde{\gamma}^{-1-\vartheta}\in \sL^1(U)
\label{11-6-25}
\end{equation}
then asymptotics \textup{(\ref{11-6-3})}--\textup{(\ref{11-6-4})} holds.

\item\label{thm-11-6-10-iii}
Furthermore, let us assume that there exists a set
$\Lambda \subset\Sigma =\Sigma_{-1}$ with $\mes_\Sigma (\Lambda )=0$ such that through every point of $(\Sigma \setminus \Lambda )$ there passes an infinitely long non-periodic billiard generated by the Hamiltonian
\begin{equation}
H^0=\tilde{\gamma}r^{1-\mu }(\tilde{\rho}+ r^{-\mu })^{-1}
\bigl( \sum_{j,k} g^{jk}(\xi_j-V_j)(\xi_k-V_k)+V+1\bigr)
\label{11-6-26}
\end{equation}
which never hits $0\times \bR^d \cup \Lambda $. Then asymptotics \textup{(\ref{11-6-10})} holds with the coefficient $\varkappa_0$ given by
\textup{(\ref{11-6-11})}.

Moreover, let $\vartheta \in (0,\vartheta^*_1)$ and \textup{(\ref{11-6-25})} be fulfilled. Then asymptotics \textup{(\ref{11-6-12})} holds.
\end{theorem-foot}

\begin{example-foot}\label{ex-11-6-11}\footnotetext{\label{foot-11-53} Cf. Example~\ref{ex-11-5-17}.}
Let $x=\bR^d$, $d\ge 2$ and $\rho =|x''| ^\nu \cdot |x|^{\mu -\nu }$,
$\gamma ={\frac{1}{2}}|x''|$ with $\mu \in (-1,0)$, $\nu \in (\mu ,0)$. Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-6-11-i}
Conditions (\ref{11-6-23}) and (\ref{11-6-25}) are fulfilled if and only if
$\nu >\nu_0=\mu d'' d ^{-1}$ and
$\nu >\nu_{\vartheta +1}=\mu (d''-1-\vartheta )(d-1-\vartheta )^{-1}$ respectively.

Therefore for $\nu >\nu_1$ asymptotics (\ref{11-6-2}) holds while for
$\nu >\nu_{\vartheta +1}$, $\vartheta <\vartheta^*_1$ asymptotics
(\ref{11-6-3}) holds\footnote{\label{foot-11-54} And under non-periodicity condition on the Hamiltonian flow asymptotics (\ref{11-6-10}) holds. Further, asymptotics (\ref{11-6-12}) (for $\nu >\nu_{\vartheta +1})$ holds.}.

\item\label{ex-11-6-11-ii}
The case $\nu \in [\nu_0,\nu_1)$ is treated in the same way as
case \ref{ex-11-5-17-ii} of Example~\ref{ex-11-5-17}. We obtain that for $\nu =\nu_1$ asymptotics
\begin{equation}
\N^- (\tau )=
\N^\W (\tau )+O\bigl(|\tau |^{l(d-1)}\log |\tau |\bigr)
\label{11-6-27}
\end{equation}
holds as $\tau \to -0$ and for $\nu \in (\nu_0,\nu_1)$ asymptotics
\begin{equation}
\N (\tau )=\N^\W (\tau )+O\bigl(|\tau |^q\bigr)
\label{11-6-28}
\end{equation}
holds as $\tau \to -0$ with
$q=-\frac{1}{2}(\mu +1)d'(\nu -\mu )^{-1} =l(d-\eta )$,
$\eta =(\mu d''-\nu d)(\mu -\nu ) ^{-1}\in (0,1)$.

In these asymptotics $\N^\W (\tau )=\varkappa_0 |\tau |^{ld}$.

\item\label{ex-11-6-11-iii}
Similarly, for $\nu =\nu_{\vartheta +1}$, $\vartheta \in (0,\vartheta^*_1)$ asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau )=\N^\W_{(\vartheta)} (\tau )+
O\bigl(|\tau |^{l(d-1-\vartheta )+\vartheta }\log |\tau |\bigr)
\label{11-6-29}
\end{equation}
holds as $\tau \to -0$ and for $\nu \in (\nu_0,\nu_{\vartheta +1})$
asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau )=
\N^\W_{(\vartheta)} (\tau )+O\bigl(|\tau | ^{q+\vartheta }\bigr)
\label{11-6-30}
\end{equation}
holds as $\tau \to -0$ with the same $q$ as before.

\item\label{ex-11-6-11-iv}
Finally, for $\nu =\mu d''d ^{-1}$ asymptotics
\begin{equation}
\N (\tau )=\N^\W (\tau )+O\bigl(|\tau |^{ld}\bigr)
\label{11-6-31}
\end{equation}
holds as $\tau \to -0$ with $\N^\W (\tau )$ given by (\ref{11-5-52}) and moreover $\N^\W (\tau )\asymp |\tau |^{ld}\log |\tau |$. Moreover, footnotes \footref{foot-11-41}, \footref{foot-11-42} section hold.
\end{enumerate}
\end{example-foot}

We now have no need of the coercivity condition and therefore Theorems \ref{thm-11-5-18} and \ref{thm-11-5-20} and Examples \ref{ex-11-5-19} and \ref{ex-11-5-21} are almost senseless. However, the following problems make sense:

\begin{problem}\label{problem-11-6-12}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-6-12-i}
Examine potentials of the type $V^0+V'$ where $V^0$ is a slowly decreasing and not very singular
potential and $V'$ decreases faster and is more singular, etc.

\item\label{problem-11-6-12-ii}
Let us note that for $d\ge 3$ in the zone $\{V\ge 0\}$ no condition excluding $|V_j|\le c\sqrt V$ is necessary. Consider examples with
$\rho =\langle x\rangle^\mu$, $\gamma =\langle x\rangle ^{1-\sigma}$ with
$\mu <0$, $\sigma \in (0,1+\mu)$, where asymptotics with a worse
remainder estimate may be obtained. In this case the magnetic field can decrease more slowly at infinity.
\end{enumerate}
\end{problem}


\subsection{Quasi-homogeneous potentials}%
\label{sect-11-6-5}
\index{non-homogeneous potential!asymptotics of eigenvalues tending to $-0$}%
\index{potential!non-homogeneous!asymptotics of eigenvalues tending to $-0$}%
\index{eigenvalues tending to $-0$!asymptotics of!non-homogeneous potential}%
\index{asymptotics!eigenvalues tending to $-0$!non-homogeneous potential}

Let us consider non-homogeneous operators. Repeating the arguments of Example~\ref{ex-11-5-23} with obvious modifications we obtain

\begin{example}\label{ex-11-6-13}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{ex-11-6-13-i}
Let $X$ be an $L$-quasi-conical domain in $\bR^d$ and let $g^{jk}$, $V_j$, $V$ be positively $L$-quasi-homogeneous with respect to $x$ of degrees $0$, $\mu$, $2\mu$ respectively where $\mu \in (-1,0)$, $L=(L_1,\dots ,L_d)$ with $L_j=1$ for $1\le j\le d'$ and $L_j>1$ for $d'+1\le j\le d$, $1\le d'<d$.

Let us assume that $g^{jk},V_j,V\in \sC^K(\bar{X}\setminus 0)$ satisfy condition
(\ref{11-1-8}) and that $V( \bar{\theta})<0$ for some $\bar{\theta}\in X$. Then conditions (\ref{11-1-7}) are fulfilled with $\rho =[x]_L ^\mu $,
$\gamma =\epsilon [x]_L$ for $[x]_L\ge 1$; for $[x]_L\le 1$ one should take $\gamma =\epsilon [x]_L^{\bar{L}}$ with $\bar{L}=\max_jL_j$.
Then the asymptotics
\begin{equation}
\N^- (\tau )=\varkappa_0|\tau |^p+O\bigl(|\tau |^q\bigr)
\label{11-6-32}
\end{equation}
holds as $\tau \to-0$ with $p=\frac{d}{2}+\frac{L^*}{2\mu}$,
$q=\frac{1}{2}(d-1)+\frac{1}{2\mu}(L^*-1)$, $L^*=\sum_jL_j$ and
\begin{equation}
\varkappa_0 =
(2\pi )^{-d}\omega_d\int \bigl(-1-V\bigr)_+^{\frac{d}{2}}\sqrt g\, dx.
\label{11-6-33}
\end{equation}

\item\label{ex-11-6-13-ii}
Moreover, let us assume that $x'\ne 0$, $\nu '\ne 0$ on $\partial
X\setminus 0$ where $\nu $ is a unit normal to $\partial X$ and
$x'=(x_1,\dots ,x_{d'})$, $\nu '=(\nu_1,\dots ,\nu_{d'})$. Let us assume that $g^{jk}=0$, $V_k=0$ for $j\le d'$, $k\ge d'+1$. Then asymptotics
\begin{equation}
\N^- (\tau )=\varkappa_0|\tau |^p+
\bigl(\varkappa_1+o(1)\bigr)|\tau |^q
\label{11-6-34}
\end{equation}
holds with
\begin{equation}
\varkappa_1 =\mp {\frac{1}{4}}(2\pi )^{1-d}\omega_{1-d}
\int \bigl(-1-V\bigr)_+^{\frac{d-1}{2}}\, dS'\sqrt{g''} dx''
\label{11-6-35}
\end{equation}
where $dS'$ and $\sqrt{g''} dx''$ are the Riemannian densities introduced
in Example~\ref{ex-11-5-23}.
\end{enumerate}
\end{example}


\subsection{Quickly decreasing potentials}%
\label{sect-11-6-6}
\index{quickly decreasing potential!asymptotics of eigenvalues tending to $-0$}%
\index{potential!quickly decreasing!asymptotics of eigenvalues tending to $-0$}%
\index{eigenvalues tending to $-0$!asymptotics of!quickly decreasing potential}%
\index{asymptotics!eigenvalues tending to $-0$!quickly decreasing potential}

Let us consider potentials which decrease rather quickly. We considered homogeneous potentials decreasing as $\langle x\rangle^{2\mu}$ with
$\mu \in (-1,0)$ and $N^-(0)<\infty$ as either $\mu <-1$ or $\mu =-1$,
$V\ge -\epsilon \langle x\rangle^{2\mu}$ with sufficiently small $\epsilon>0$. So ``rather quickly'' should mean ``a bit slower than $\langle x\rangle^{-2}$'' .

\begin{theorem}\label{thm-11-6-14}

Let $X$ be an unbounded domain in $\bR^d$ and let conditions \textup{(\ref{11-1-1})}--\textup{(\ref{11-1-3})} and \textup{(\ref{11-6-1})} be fulfilled with
\begin{equation}
\gamma =\epsilon \langle x\rangle ,\qquad
\rho =\langle x\rangle ^{-1}\log ^\nu \langle x\rangle
\label{11-6-36}
\end{equation}
where we now take $\langle x\rangle =(|x|^2+4)^{\frac{1}{2}}$, $\nu >0$.

Further, let us assume that for every $\tau \in (-\epsilon ,0]$ one of non-degeneracy conditions is fulfilled for the symbol $(A(x,\xi )\tau^{-1}-1)$ uniformly with respect to $(\tau ,x,\xi )$ (this condition is restrictive
only for $|x|\ge C_0$). Then


\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-6-14-i}
Asymptotics
\begin{equation}
\N^- (\tau )=\N^\W (\tau )+
O\bigl(\bigl|\log|\tau |\bigr| ^{\nu (d-1)+1}\bigr)
\label{11-6-37}
\end{equation}
holds as $\tau \to -0$ where
$\N^\W (\tau )=O\bigl(\bigl|\log|\tau |\bigr| ^{\nu d+1}\bigr)$ and
under condition \textup{(\ref{11-6-8})}
$\N^\W (\tau )\asymp \bigl|\log|\tau |\bigr| ^{\nu d+1}$.

\item\label{thm-11-6-14-ii}
Moreover, let $X\cap \{|x|\ge r_0\}=X^0\cap \{|x|\ge r_0\}$ where
$X^0$ is a conical domain with $\partial X^0\setminus 0\in \sC^K$
and let stabilization conditions \textup{(\ref{11-5-4})} be fulfilled for
functions $\;a_\beta \log^{-\nu (2m-|\beta |)}\;$ where the functions
$a^0_\beta \in \sC^K(\bar{X} ^0\setminus 0)$ are positively
homogeneous of degrees $-(2m-|\beta|)$ on $x$.

Then the microhyperbolicity condition is fulfilled automatically. Further, if the non-periodicity condition is fulfilled for the quasi-homogeneous symbol
\begin{equation}
A ^0(x,\xi )=|x|^{2m}\sum_{|\beta |\le 2m}a^0_\beta (x)\xi ^\beta
\label{11-6-38}
\end{equation}
on the energy level  $0$ then the asymptotics
\begin{equation}
\N^- (\tau )=\N^\W (\tau )+
\bigl(\varkappa_1+o(1)\bigr)\bigl|\log|\tau |\bigr| ^{\nu (d-1)+1}
\label{11-6-39}
\end{equation}
holds where, for the Schr\"{o}dinger operator,
\begin{equation}
\varkappa_1=\mp 2^{-\nu (d-1)-3}(2\pi)^{1-d} \omega_{d-1}
\int_{\partial U}\bigl(V^0\bigr)_-^{\frac{d-1}{2}} \,dS,
\label{11-6-40}
\end{equation}
$U=X^0\cap\bS^{d-1}$ is a domain on $\bS^{d-1}$, $dS=dS^0:dr$ is the
natural density on $\partial U$, $dS^0$ is the Riemannian density on
$\partial X^0$ generated by the metric $g^{jk0}$ (compare with
(\textup{(\ref{11-6-12})}).

\item\label{thm-11-6-14-iii}
On the other hand, if only the stabilization condition is fulfilled then
$\N^\W (\tau)=\bigl(\varkappa_0+o(1)\bigr)\bigl|\log|\tau|\bigr|^{\nu d+1}$
where, for the Schr\"{o}dinger operator,
\begin{equation}
\varkappa_0= 2^{-\nu d-1}(2\pi )^{-d}\omega_d
\int_U\bigl(V^0\bigr)_-^{\frac{d}{2}}\sqrt{g^0}\,d\theta ,
\label{11-6-41}
\end{equation}
$d\theta =dx:dr$, $g^0=\det (g^{jk0})^{-1}$ (compare with
(\textup{(\ref{11-6-11})}).
\end{enumerate}
\end{theorem}

\begin{proof}
Statement~\ref{thm-11-6-14-i} follows immediately from our previous arguments; moreover, now $\rho \gamma =\log ^\nu \langle x\rangle \to \infty $ as
$|x|\to \infty $ and $X''=\emptyset$.

In order to prove Statement~\ref{thm-11-6-14-ii} let us note that the principal contribution to the remainder estimate is given by the zone
$\{R\le |x|\le \epsilon \tau ^{-\frac{1}{2m}}\}$ with arbitrary fixed $R$ and $\epsilon >0$. We need to examine the Hamiltonian trajectories starting in this zone and associated with the symbol
\begin{equation}
A_\tau (x,\xi )=\langle x\rangle ^{2m}\log ^{-\nu }\langle x\rangle
\bigl(A(x,\xi )+\tau \bigr)
\label{11-6-42}
\end{equation}
on $\Sigma_\tau =\{\det A_\tau (x,\xi )=0\}$. Let $\Sigma ^0\supset \Lambda_T$ be a closed set of measure $0$ such that through every point of
$(\Sigma ^0\setminus \Lambda_T)$ there passes a non-periodic Hamiltonian trajectory (with reflections) of length $2T$ associated with the symbol $A^0$. Then one can take
\begin{multline*}
\Lambda_{1,T,\epsilon,\varepsilon ,\tau ,R}=
\bigl\{(x,\xi )\in \Sigma_\tau ,
R\le |x|\le \epsilon \tau ^{-{\frac{1}{2m}}},\\
\dist ({\frac{x}{|x|}}, \partial X^0)>0,
\dist \bigl(({\frac{x}{|x|}}, \xi |x| \log^{-\nu }|x|),
\Lambda_T\bigr) > \varepsilon \bigr\}
\end{multline*}
with $R=R(\epsilon ,\varepsilon ,T)$. Moreover, one can see that
$\log |x(t)|\log ^{-1}|x(0)|=1+o(1)$ as $|x(0)|\to \infty $ uniformly
with respect to $\tau$ and $t\in [-2T,2T]$ with arbitrary fixed
$T$. We leave the details to the reader.
\end{proof}
We leave to the reader the following set of rather easy problems:\enlargethispage{\baselineskip}

\begin{problem}\label{problem-11-6-15}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-6-15-i}
Prove a statement similar to Theorem~\ref{thm-11-6-10} with
\begin{equation*}
g^{jk}=g^{jk}(\theta ),\qquad V_j=v_j(\theta )r ^{-1}\log ^\nu r,\qquad
V=v(\theta )r ^{-2}\log^{2\nu }r,
\end{equation*}
$X=(1,\infty )\times U$.

\item\label{problem-11-6-15-ii}
Consider the case when
\begin{equation}
\rho =\langle x\rangle ^\mu \log ^\nu \langle x\rangle ,
\label{11-6-43}
\end{equation}
$\vartheta \ge 0$ with \underline{either} $\mu >-d(d+2m\vartheta ) ^{-1}$ \underline{or} $\mu =-d(d+2m\vartheta ) ^{-1}$,
$\nu \ge -1(d+2m\vartheta ) ^{-1}$.

Prove that under these conditions the principal part of the asymptotics is $\asymp I$ with either $I=|\tau |^p$ (with $p<0$) or
$I=\bigl|\log |\tau |\bigr| ^q$ (with $q>0$) or $I=\log\bigl|\log |\tau |\bigr|$ and the remainder estimate is either from the same list or $O(1)$.

\item\label{problem-11-6-15-iii}
Moreover, consider the case of potentials decreasing
even more quickly when
\begin{equation}
\rho =\langle x\rangle ^{-1}\bigl({\underbrace{\log \dots\log}_{\text{$r$ times}}} \langle x\rangle \bigr) ^\nu
\label{11-6-44}
\end{equation}
when the principal part of the asymptotics and the remainder estimate are of the orders $\log |\tau | \times\zeta (\tau ) ^{\nu d}$ and
$\log |\tau | \times \zeta (\tau ) ^{\nu (d-1)}$ respectively with
$\zeta(\tau)={\underbrace{\log\dots\log}_{\text{$r$ times}}} |\tau|$.

\item\label{problem-11-6-15-iv}
Prove that in the framework of Theorem~\ref{thm-11-6-14}
$\N^-_{(\vartheta)} (-0)<\infty $ for $\vartheta >0$.
\end{enumerate}
\end{problem}


\subsection{Slowly decreasing potentials}%
\label{sect-11-6-7}
\index{slowly decreasing potential!asymptotics of eigenvalues tending to $-0$}%
\index{potential!slowly decreasing!asymptotics of eigenvalues tending to $-0$}%
\index{eigenvalues tending to $-0$!asymptotics of!slowly decreasing potential}%
\index{asymptotics!eigenvalues tending to $-0$!slowly decreasing potential}

Let us consider the slowly decreasing potential $V=v(\theta )\log^{-1}r$ in the spherical coordinate system $(r,\theta )$. Using\enlargethispage{\baselineskip}
\begin{equation}
\tilde{\rho}_\tau =(\tau -V)_+^{\frac{1}{2}},\qquad
\tilde{\gamma}_\tau =\epsilon_0r\min (1, (\tau -V)_+\log r)
\label{11-6-45}
\end{equation}
for $r\ge 2$ we easily prove

\begin{theorem}\label{thm-11-6-16}
Let $d\ge 3$ and $X\cap\{r\ge r_0\}=\{r\ge r_0,\theta \in U\}$. For $|x|\ge r_0$ let
\begin{equation}
g^{jk}=g^{jk}(\theta ),\qquad V_j=0,\qquad V=v(\theta )\log^{-1}r
\label{11-6-46}
\end{equation}
where $(r,\theta )$ are spherical coordinates, $g^{jk},v, \partial X\in \sC^K$ and the matrix $(g^{jk})$ is positive definite. Let $v_0=\min_U v<0$.
Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-6-16-i}
Asymptotics \textup{(\ref{11-6-3})} holds with
\begin{gather}
\N^\W_{(\vartheta)} (\tau )\asymp |\tau |^{d+2\vartheta }
\int_U\exp\bigl({\frac{vd}{\tau }}\bigr)\,d\theta ,\label{11-6-47}\\[2pt]
R_{(\vartheta)} (\tau )= |\tau |^{d-2}\int_U
\exp\bigl({\frac{v}{\tau }}(d-\vartheta -1)\bigr)\, d\theta\label{11-6-48}
\end{gather}
for $\vartheta <d-1$. Moreover, one can take
\begin{equation}
\N^\W (\tau )= a\int_{U'}|\tau |^dv_-^{-{\frac{d}{2}}}
F_d(-{\frac{\tau }{v_-}})\exp \bigl(-{\frac{vd}{\tau }}\bigr)\sqrt g
\,d\theta
\label{11-6-49}
\end{equation}
where $U'=U\cap \{v<v_0+\varepsilon \}$ with arbitrarily small
fixed $\varepsilon >0$,
$a=2^{1-d}\pi ^{-{\frac{d}{2}}}d^{-{\frac{d}{2}}+1}$,
\begin{equation}
F_d(s)=\frac{1}{\Gamma({\frac{d}{2}}+1)}
\int_0 ^{{\frac{d}{s}}-\varepsilon }t^{\frac{d}{2}}
\bigl(1-{\frac{s t}{d}}\bigr)^{-{\frac{d}{2}}}e^{-t}dt=1+O(s)
\label{11-6-50}
\end{equation}
as $s\to +0$.

\item\label{thm-11-6-16-ii}
In particular, for $v=v_0=\const$ the principal part of the
asymptotics is $\asymp |\tau |^{d+2\vartheta }\exp ({\frac{v_0d}{\tau}})$ and the remainder estimate is
$O(|\tau |^{d-2}\exp ({\frac{v_0}{\tau}}(d-1-\vartheta )))$.

Moreover, in this case one can take
\begin{equation*}
\gamma_\tau = \epsilon_0r\min\bigl(1,(\tau-V)_+\log^2r\bigr)
\end{equation*}
and obtain a remainder estimate with the factor $|\tau |^{d+\vartheta -1}$
instead of $|\tau |^{d-2}$.

On the other hand, if $v=v(\theta )=v_0\implies \theta \in \partial U,
\nabla v(\theta )\ne 0$ and $\rank\Hess v|_{\partial U}=d-1$ then
the principal part is
$\asymp |\tau|^{\frac{3}{2}+2\vartheta}\exp(\frac{v_0d}{\tau})$
and the remainder estimate is
$O(|\tau|^{\frac{3}{2}d-3}\exp\bigl(\frac{v_0}{\tau}(d-1-\vartheta))\bigr)$.
In other cases the principal part and the remainder estimate are of intermediate
orders.
\end{enumerate}
\end{theorem}

\begin{problem}\label{problem-11-6-17}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-6-17-i}
Consider the case $\vartheta \ge (d-1)$. Then one can take $\rho_\tau=\log^{-\frac{1}{2}}r+|\tau|$ and $\gamma_\tau=\epsilon_0r$ and for $d\ge 2$ one can derive the remainder estimates $O(|\tau|^d)$ for $\vartheta=(d-1)$ and $O(1)$ for $\vartheta >(d-1)$.

\item\label{problem-11-6-17-ii}
Consider potential $V=v(\theta)\log^{-\nu}r$ with arbitrary $\nu >0$.
\end{enumerate}
\end{problem}


\subsection{General boundary conditions}
\label{sect-11-6-8}

\begin{remark}\label{rem-11-6-18}
All the above results remain true for the Neumann boundary condition provided the domain satisfies the cone condition. Let us assume that this (cone) condition is fulfilled. Moreover, all the above results remain true for mixed boundary conditions (provided the asymptotics do not distinguish Dirichlet and Neumann boundary conditions) and also in the following cases:


\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-6-18-i}
 We are in the frameworks of Theorem~\ref{thm-11-6-2} or \ref{thm-11-6-10}\ref{thm-11-6-10-iii}, and condition (\ref{11-5-86}) is fulfilled.

\item\label{rem-11-6-18-ii}
We are in the frameworks of Example~\ref{ex-11-6-13}\ref{ex-11-6-13-ii}, and condition (\ref{11-5-87}) is fulfilled.

Moreover, in the context of Theorem~\ref{thm-11-6-5} asymptotics (\ref{11-6-16})
remain true if condition (\ref{11-5-88}) is fulfilled.
\end{enumerate}
\end{remark}


\subsection{Non-semi-bounded operators}
\label{sect-11-6-9}
\index{Dirac operator!asymptotics of eigenvalues tending to border of spectral gap}%
\index{operator!Dirac!asymptotics of eigenvalues tending to border of spectral gap}%
\index{eigenvalues tending to border of spectral gap!asymptotics of!Dirac operator}%
\index{asymptotics!eigenvalues tending to border of spectral gap!Dirac operator}

Finally, let us consider non-semi-bounded operators. We consider the Dirac operator with mass $M>0$ (otherwise in the context of this section the spectrum coincides with $\bR$). Moreover, let $V\to 0$, $V_j\to 0$ as $|x|\to\infty $.

Then
$\Spec_\ess (A)= (-\infty ,M]\cup[M,\infty )$ and the spectral gap
$(-M,M)$ contains either a finite or infinite number of eigenvalues. In
the second case these eigenvalues tend to $-M+0$ and (or) to $M-0$
and we can consider the corresponding eigenvalue asymptotics. Let us
consider $M-0$. In order to replace it by $-0$ we replace the operator
$A$ by $A-M\cdot I$. Let us fix $\tau_1\in (-2M,0)$ and let us consider
\begin{equation}
\N^- (\tau )\coloneqq   \N (\tau_1,\tau )
\label{11-6-51}
\end{equation}
with $\tau \to -0$. Then

\begin{remark}\label{rem-11-6-19}
Under described modifications

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-6-19-i}
Theorems \ref{thm-11-6-1}, \ref{thm-11-6-2}, \ref{thm-11-6-14} and \ref{thm-11-6-5} and Examples \ref{ex-11-6-13}, \ref{ex-11-6-6} remain true and one can check conditions on the Hamiltonian flow for the corresponding Schr\"{o}dinger operator with the symbol
\begin{equation}
H=\sum_{j,k} g^{jk}(\xi_j-V_j)(\xi_k-V_k)+(V+M)^2-M^2.
\label{11-6-52}
\end{equation}
In this Hamiltonian one can skip the term $V^2$ which is negligible at infinity (as far as non-periodicity condition is concerned) in which case one can consider the Hamiltonian
\begin{equation}
H=\sum_{j,k} g^{jk}(\xi_j-V_j)(\xi_k-V_k)+2MV.
\label{11-6-53}
\end{equation}

Now, however, due to term $V^2$
\begin{equation}
\N^\W (\tau)=\varkappa_0|\tau|^p\bigl(1+O(|\tau|^\delta)\bigr)
\label{11-6-54}
\end{equation}
with
$\delta >0$ instead of $\N^\W (\tau )=\varkappa_0|\tau |^p$.

\item\label{rem-11-6-19-ii}
 Theorem \ref{thm-11-6-10} (and Example~\ref{ex-11-6-11}\ref{ex-11-6-11-i} for $d\ge 3$) remain true. In order to prove this let us note that only the analysis in the zone $\{\tilde{\rho}r^\mu \ge 1\}$ should be changed. In this zone
instead of $\rho=\tilde{\rho}r^\mu$ one should set $\rho=\tilde{\rho}^2r^{2\mu}$.

We include this zone in $X_\sing$. In this zone $\rho ^d\in \sL ^1$ due to assumption $\tilde{\rho}^{-\frac{d}{2\mu}}\in \sL^1(U)$. Therefore the
contribution of this zone to the asymptotics and to the remainder estimate is $O(1)$.

\item\label{rem-11-6-19-iii}
 Theorem \ref{thm-11-6-16} also remains true. However, $\N^\W (\tau)$ should be calculated for the Dirac operator, i.e., for the Schr\"{o}dinger operator with the symbol (\ref{11-6-52}) and with the spectral parameter equal to $0$.

In the proof one should replace $\rho_\tau =(\tau -V)_+^{\frac{1}{2}}$ by
\begin{equation}
\rho_\tau =\bigl(\tau -V+C_1r^{-1} \log^{-2}r\bigr)_+^{\frac{1}{2}}
\label{11-6-55}
\end{equation}
with large
enough $C_1$ in the zone
$X_\sing\cap \{\tau-V \le C |\tau|^{\frac{2}{3}} r^{-\frac{2}{3}}\}$.
This does not increase the remainder estimate.
\end{enumerate}
\end{remark}

Let us consider Theorems~\ref{thm-11-5-9} and \ref{thm-11-6-9}. For simplicity we assume that
\begin{equation}
|v|\le 2M-\epsilon_0\qquad \forall x.
\label{11-6-56}
\end{equation}\label{problem-11-6-20}
We leave to the reader the following easy
\begin{problem}
Conduct analysis below without assumption (\ref{11-6-56}).
\end{problem}

Under assumption (\ref{11-6-56}) for
appropriate $\tau_1$,
\begin{equation}
\N^- (\tau )=\tilde{\N}^-(\tau )- \tilde{\N}^-(\tau_1)
\label{11-6-57}
\end{equation}
where $\tilde{\N}^-(\tau )$ is the number of the negative eigenvalues
for the operator
\begin{gather}
A(\tau )={\cL}^*(2M-V+\tau )^{-1}{\cL}+V-\tau\label{11-6-58}\\
\shortintertext{with}
{\cL}=
\sum_j\bigl(\sum_k\omega ^{jk}(D_k-V_k)-{\frac{i}{2}}\omega ^j\bigr)\upsigma '_j
\label{11-6-59}
\end{gather}
where we assume that
\begin{equation*}
\upsigma_0=\begin{pmatrix} I &0\\ 0 &-1\end{pmatrix} ,\qquad
\upsigma_j=\begin{pmatrix} 0& \upsigma '_j{^*}\\
\upsigma '_j& 0\end{pmatrix} \quad (j\ge 1)
\end{equation*}
and use the notation $\omega ^j=\sum_k\partial_k\omega ^{jk}$.

If we could take $\rho=\langle x\rangle^{-\frac{1}{2}}$, $\gamma=\epsilon_0\langle x\rangle$ for the original Dirac operator and if
\begin{gather}
D ^\alpha (\omega ^{jk}-\updelta ^{jk})=
O\bigl(|x|^{-\delta_0-|\alpha |}\bigr),
\label{11-6-60}\\[3pt]
D ^\alpha F_{jk}=O\bigl(|x|^{-{\frac{3}{2}}-\delta_3-|\alpha |} \bigr)
\qquad \text{as\ }|x|\to \infty \quad \forall \alpha :|\alpha |\le K
\label{11-6-61}
\end{gather}
(where $F_{jk}=i(\partial_j V_k-\partial_k V_j)$ is the tensor magnetic intensity) then the operator $A(\tau)$ is a scalar operator plus perturbation $\sum_j A'_j(D_j-V_j)+A'_0$ where
\begin{align}
&D ^\alpha A'_j=O\bigl(|x|^{\max (-1-\delta_0,-2)-|\alpha|}\bigr),
\label{11-6-62}\\[3pt]
&D ^\alpha A'_0=
O\bigl(|x|^{\max (-1-\delta_0,-2,
-\frac{1}{2}-\delta_3)-|\alpha|-1}\bigr)
\quad \text{as\ \ }|x|\to \infty\label{11-6-63}
\end{align}
and in the context of the previous subsections this error does not matter provided that under the assumptions of Theorems~\ref{thm-11-6-7} and \ref{thm-11-6-9}\begin{phantomequation}\label{11-6-64}\end{phantomequation}
\begin{equation}
\delta_\iota <{\frac{3}{2}},\quad \delta_\iota <{\frac{1}{2}}+\delta_0,
\quad \delta_\iota< {\frac{1}{2}}+\delta_3
\tag*{$\textup{(\ref*{11-6-64})}_{1,2,3}$}\label{11-6-64-*}
\end{equation}
respectively with $\iota =1,2$ (because the ``order'' of the operator $D_j-V_j$ is $-\frac{1}{2}+\delta '$ with arbitrarily small $\delta '>0$ if we take the ``order'' of $|x|$ equal to $1$). Then the operator $A(\tau )$ differs by negligible terms from the Schr\"{o}dinger operator
\begin{equation}
B(\tau )=\sum_{j,k}(D_j-V_j)g^{jk}(2M-V+\tau )^{-1}(D_k-V_k)+V-\tau
\label{11-6-65}
\end{equation}
and moreover, for
\begin{equation}
\delta_\iota <1 \qquad (\iota =1,2)
\label{11-6-66}%\tag{10.5.28}
\end{equation}
one can replace this operator by the operator
\begin{equation}
B'(\tau )=(2M)^{-1}\sum_{j,k} (D_j-V_j)g^{jk}(D_k-V_k) +V-\tau.
\label{11-6-67}
\end{equation}

So we arrive to

\begin{theorem}\label{thm-11-6-21}
Let conditions \textup{(\ref{11-6-60})}--\textup{(\ref{11-6-63})}, \ref{11-6-64-*} and \textup{(\ref{11-6-66})} be fulfilled.

Furthermore, let assumptions of some statement of Theorem~\ref{thm-11-6-7} or Theorem~\ref{thm-11-6-9} be fulfilled for the Schr\"{o}dinger operator
$B'(\tau)$ defined by \textup{(\ref{11-6-65})} (or equivalently by \textup{(\ref{11-6-67})}); then $\iota =1,2$ respectively.

Then the corresponding asymptotics holds for the Dirac operator. Namely, asymptotics \textup{(\ref{11-6-18})}) holds for $\delta_\iota < \frac{1}{2}$ (then condition \textup{(\ref{11-6-64})}) is fulfilled automatically) and asymptotics \textup{(\ref{11-6-19})}) holds for
$\delta_\iota \in (\frac{1}{2},1)$.

In these asymptotics $\N^\W (\tau)$ is calculated for the Dirac operator and $F(\tau)$ is calculated for the Schr\"{o}dinger operator and then it is multiplied by $\frac{1}{2}\D$.
\end{theorem}

On the other hand, let condition (\ref{11-6-66}) be violated but condition $\textup{(\ref{11-6-63})}_{1,2,3}$ be (almost) fulfilled. Then one should replace $B(\tau)$ by
\begin{multline}
B''(\tau)=\\
(2M)^{-1}\sum_{j,k}(D_j-V_j)g^{jk} (D_k-V_k)+V-\tau -(2M)^{-1}(V-\tau )^2
\label{11-6-68}
\end{multline}
and in the last term one can replace $V$ by $V^0$ where $V^0$ is a smooth function equal to $-1(2M|x|) ^{-1}$ for $|x|\ge c$. Changing variables
$x\to \zeta x$ and multiplying by $2M\zeta ^2$ with $\zeta =1-\tau M^{-1}$ we obtain, modulo negligible terms, operator
\begin{gather}
B''' (\tau ')=\sum_{j,k} (D_j-V_j)g^{jk}(D_k-V_k)+W-\tau '
\label{11-6-69}\\
\intertext{with the new potential}
W=2MV-(V^0)^2\label{11-6-70}
\intertext{and with the modified spectral parameter}
\tau'=\tau \bigl(1-\frac{3\tau}{2M}\bigr)\label{11-6-71}
\end{gather}

This yields that

\begin{theorem}\label{thm-11-6-22}
Let assumptions of some statement of either Theorem~\ref{thm-11-6-7} or Theorem~\ref{thm-11-6-9} be fulfilled for the Schr\"{o}dinger operator $B'''(0)$
defined by \textup{(\ref{11-6-69})}.

Let conditions \textup{(\ref{11-6-60})}--\textup{(\ref{11-6-63})}, $\textup{(\ref{11-6-63})}_{1,2,3}$ be fulfilled but
$\delta_\iota \in [1,\frac{3}{2})$.

Then asymptotics \textup{(\ref{11-6-19})} remains true where $\N^\W (\tau )$ is calculated for the Dirac operator and $F(\tau ')$ is calculated for the Schr\"{o}dinger operator $B'''(\tau ')$ and is then multiplied by $\frac{1}{2}\D$, and $\tau'$ is defined by \textup{(\ref{11-6-71})}.
\end{theorem}

Let us weaken condition \ref{11-6-64-*}.

\begin{remark}\label{rem-11-6-23}
For $d=2$ one can assume without any loss of the generality that $\D=2$. Then $A(\tau)$ is surely a scalar operator but we have not taken into account some terms. Taking them into account and applying the above analysis we can discard
condition \ref{11-6-64-*} completely (in which case we have additional corrections for $W$ and $\tau'$).
\end{remark}\enlargethispage{\baselineskip}

In the general case we assume that conditions (\ref{11-6-60})--(\ref{11-6-62}) are fulfilled. If $\delta_1 \ge 1$ then the non-scalar terms in $A(\tau)$ are
\begin{equation}
\frac{1}{2}(2M)^{-3}r^{-3}\sum_{l\ne k}\upsigma '_l{^*} \upsigma'_k F_{lk}
\label{11-6-72}
\end{equation}
modulo operators of the form $\sum_j b'_jD_j+b'_0$ where $b'_j,b'_0$ satisfy condition (\ref{11-6-60}), (\ref{11-6-61}) with ``$-2$'' replaced by ``$-3$.'' Here we used the skew-symmetry of the matrices $\upsigma'_l{^*} \upsigma'_k$ with $l\ne k$; recall that $F_{lk}=(\partial_k A_l-=\partial_l A_k)$.

This statement remains true for $\delta_2\ge 1$ (i.e., for
$\delta_1\ge \frac{1}{2}$) in the framework of Theorem~\ref{thm-11-6-7}. However, in this case the operator $A(\tau)$ also contains terms of type
$b''_jD_j+b''_0$ with $b''_j,b''_0$ satisfying conditions (\ref{11-6-62})--(\ref{11-6-63}) with ``$-2$'' replaced by ``$-2-\delta_1$'' and this operator skew-commutes with the antipodal map. In both cases these terms are negligible provided \begin{phantomequation}\label{11-6-73}\end{phantomequation}
\begin{equation}
\delta_\iota <2,\quad \delta_\iota < \frac{1}{2}+\delta_3\quad
(\iota =1,2).
\tag*{$\textup{(\ref{11-6-73})}_{1,2}$}\label{11-6-73-*}
\end{equation}

However, the second inequality is not necessary: for $\iota =1$ it is fulfilled automatically and for $\iota =2$ it is associated with terms of the type
\begin{equation*}
-i\,\const \sum_{l\ne k}\upsigma '_l{^*}\upsigma '_lF_{lk}.
\end{equation*}
However, in this case $V_l\circ j^*=V_l$ and therefore $F_{lk}\circ j^*=-F_{lk}$ and the same is true for this extra term. Then one should check the condition $-2-\delta_1 < -1 < -2\delta_1$ which follows from the first inequality.

Let us consider Schr\"odinger operator with a (perturbed) Coulomb potential. Let us consider
\begin{equation*}
\int_0^{T_0}r^{-3}(x_j\xi_k-x_k\xi_j)\circ \Psi_t\, dt
\end{equation*}
where $\Psi_t$ is the Hamiltonian flow generated by $|\xi|^2-|x|^{-1}$. One can easily see that this integral is equal to $\pi \mu_{jk} \mu^{-3}$ where
$\mu_{jk}$ are components of the angular momentum tensor
\begin{equation}
\mu_{jk}=(x_j\xi_k-x_k\xi_j)\qquad\text{and}\qquad
\mu =(\sum_{j<k}\mu_{jk}^2)^{\frac{1}{2}}.
\label{11-6-74}
\end{equation}
This calculation is easy for trajectories lying in the $(x_1,x_2)$-plane and then one can change coordinates.

Then we obtain that the contribution of the non-scalar terms to the operator $U(\pi,\tau)$\,\footnote{\label{foot-11-55} Here $U(\pi,\tau)=\exp\bigl(i\pi(-A(\tau)\bigr)^{-\frac{1}{2}})$ and
$\pi$ is the period of the corresponding Hamiltonian flow for
$\tau=0$.}
is the multiplication by
\begin{equation*}
I-i\pi \sum_{j,k}\upsigma'_j{^*}\upsigma '_k\mu_{jk}\mu ^{-3}+
O\bigl(|\tau| ^{{\frac{3}{2}}-\delta '}\bigr)
\end{equation*}
with arbitrarily small $\delta '>0$. Applying corollary \ref{cor-5-A-7} and
calculating the eigenvalues of $\mu_{jk}$ we obtain that in order to
take into account non-scalar terms for $d\ge 3$ we can treat the
family of operators
\begin{equation}
B'''(\tau ')+k\nu |\tau |^{\frac{3}{2}}\boldsymbol{M}^{-2}
\label{11-6-75}
\end{equation}
with an appropriate constant $k$ and with $\nu \in \{-1,0,1\}$ of
the corresponding multiplicities where $\boldsymbol{M}^s$ is an operator
with the symbol $\mu ^s$ with $\mu =\mu (x,\xi )$ defined by (\ref{11-6-74}).
One should check conditions for every such operator, calculate and
sum $\N^-_\nu(\tau)$ with the corresponding multiplicities.

For $d=2$ and $\D=2$ we have $\nu =0,1$ and the operators
\begin{equation}
B'''(\tau ')+
3\varsigma \nu |\tau '|^{\frac{3}{2}}{\cM} \boldsymbol{M}^{-3}
\label{11-6-76}
\end{equation}
with ${\cM}=x_1D_2-x_2D_1$,
$\varsigma =i\upsigma_0\upsigma_1\upsigma_2=\pm 1$.

We leave the following rather easy problem to the reader:

\begin{problem}\label{problem-11-6-24}
Analyze the Schr\"odinger operator with a (perturbed) Coulomb potential in details.
\end{problem}



\section{Multiparameter asymptotics}%
\label{sect-11-7}
\index{multiparameter asymptotics}%
\index{asymptotics!multiparameter}

\subsection{Problem set-up}%
\label{sect-11-7-1}

In this section we consider operators depending on more than one parameter. First of all, we consider semiclassical asymptotics in the case when the scalar semiclassical parameter $h$ is replaced by a vector
$\boldsymbol{h}=(h_1,\dots ,h_d)$ with $h_j\to+0$.

Next we assume that there are two parameters: the semiclassical parameter $h\to+0$ and the spectral parameter $\tau $. Let us recall that each of the semiclassical asymptotics of Section~\ref{sect-11-1} was uniform with respect to the energy level $\tau $ lying in the interval in which conditions of the corresponding theorem were fulfilled\footnote{\label{foot-11-56} In this subsection for the sake of simplicity we consider only the Schr\"{o}dinger and Dirac operators and we no not need to check non-degeneracy conditions.}
uniformly. Therefore there are two principally different situations in which non-trivial results are possible. We will explain them for the Schr\"{o}dinger operator.

In the first situation $\tau$ increases and tends to a value $\tau^*$ such that the conditions of the corresponding theorem of Section~\ref{sect-11-1} are violated for $\tau =\tau ^*$ and therefore the asymptotics are no longer uniform. There are two cases:

\begin{enumerate}[label=(\alph*), wide, labelindent=0pt]
\item\label{sect-11-7-1-a}
$\tau\to+\infty$ as in Sections~\ref{sect-11-2}--\ref{sect-11-5} or

\item\label{sect-11-7-1-b}
 $\tau\to\tau^*-0$ with $\tau^*<\infty$ as in Section~\ref{sect-11-6} where in the this case $\tau^* =\liminf_{|x|\to\infty } V$. In this case $\tau^*$ is the bottom of the essential spectrum and $\tau^*-0$ is either a limit point of the discrete spectrum for every fixed $h>0$ or there is only a finite discrete spectrum for every fixed $h>0$ and in the second case the number of eigenvalues and (or) the remainder estimate near $\tau ^*-0$ are unusually large
($\gg \const\cdot h^{-d}$ and $\gg \const\cdot h^{1-d}$ respectively).

In all these cases we obtain estimates for the number of eigenvalues and for the remainder which are \emph{worse\/} than for ``normal'' $\tau $.
\end{enumerate}



In the second situation $\tau $ decreases to the special value $\tau ^*=\inf V$ and we obtain estimates for the number of eigenvalues and for the remainder which are \emph{better\/} than for ``normal'' $\tau $. Again there are two different cases:

\begin{enumerate}[label=(\alph*), wide, labelindent=0pt, resume]
\item\label{sect-11-7-1-c}
either $\inf V$ is finite in which case $\tau \to \tau ^*+0$ or

\item\label{sect-11-7-1-d}
$\inf V=-\infty $ but $-\infty $ is not a limit point of the spectrum for every fixed $h>0$. Then for $h\to+0$ the bottom eigenvalues of the operator ``fall'' to $-\infty $ and we consider this process. Only the last case is
impossible for the Dirac operator.
\end{enumerate}


\subsection{Semiclassical asymptotics with a vector semiclassical parameter}
\label{sect-11-7-2}

Let us consider the Schr\"{o}dinger operator\enlargethispage{\baselineskip}
\begin{equation}
A=A_{\boldsymbol{h}}=\sum_{j,k}P_jg^{jk}P_k+V,\qquad P_j=h_j-V_j
\label{11-7-1}
\end{equation}
or the Dirac operator of the same type as before. Changing coordinates $x_{j\,\new}=x_{j\,\old}h_j^{-1}$ we obtain operator
\begin{equation}
A'=A'_{\boldsymbol{h}}=\sum_{j,k}
(D_j-V_{j \boldsymbol{h}})g^{jk}_{\boldsymbol{h}}
(D_k-V_{k \boldsymbol{h}})+V_{\boldsymbol{h}}
\label{11-7-2}
\end{equation}
in the domain $X_{\boldsymbol{h}}=\{x, f_{\boldsymbol{h}}(x)\in X\}$ where $X$ is the original domain and $v_{\boldsymbol{h}}=v\circ f_{\boldsymbol{h}}$ for every function $v$ where $f_{\boldsymbol{h}}(x)=h\bullet x\coloneqq  (h_1x_1,\dots ,h_dx_d)$,
${\boldsymbol{h}}=(h_1,\dots ,h_d)$. One can easily see that if (some of) the
conditions (\ref{11-1-6})--(\ref{11-1-8}), (\ref{11-4-5}) were fulfilled for
$X,\rho ,\gamma ,g^{jk},V_j,V$ then the same conditions remain true
for $X_{\boldsymbol{h}},\rho_{\boldsymbol{h}},h^{-1}\gamma_{\boldsymbol{h}},
V_{j{\boldsymbol{h}}},V_{\boldsymbol{h}}$ where $h=\max_jh_j$. Moreover, if the
cone condition was fulfilled for the domain $X$ then it remains true
for $X_{\boldsymbol{h}}$ provided $h\le 1$. This immediately yields

\begin{theorem}\label{thm-11-7-1}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-7-1-i}
Let $d\ge 3$ and let conditions \textup{(\ref{11-1-6})}--\textup{(\ref{11-1-8})} be fulfilled for $g^{jk},V_j,V,\rho ,\gamma$. Let $\gamma >0$ a.e.\ and $V_-^{\frac{d}{2}}$, $\rho ^{d-1}\gamma ^{-1}\in \sL^1(X)$. Then asymptotics
\begin{gather}
\N^-(A_{\boldsymbol{h}})= (h_1\dots h_d)^{-1}\bigl(\N^\W +O(h)\bigr)
\label{11-7-3} \\
\intertext{holds as $h=\max_jh_j\to+0$ where as usual}
\N^\W =(2\pi )^{-d}\omega_d\int V_-^{\frac{d}{2}}\sqrt g\, dx.
\label{11-7-4}
\end{gather}

\item\label{thm-11-7-1-ii}
Moreover, let us assume that
\begin{gather}
g^{jk}=V_j=0\qquad \text{for\ \ } j\ge d'+1, k\le d',
\label{11-7-5}\\
\intertext{$0<d'<d$ and that }
|\nu '|\ge \epsilon_0>0\qquad \text{on\ \ } \partial X\cap \{V\le 0\}
\label{11-7-6}
\end{gather}
where $\nu = (\nu_1,\dots ,\nu_{d'};\nu_{d'+1},\dots ,\nu_d)=(\nu ';\nu '')$ is a unit normal to $\partial X$. Then asymptotics
\begin{equation}
\N^-(A_{\boldsymbol{h}})=
(h_1\dots h_d)^{-1}\bigl(\N^\W +\varkappa_1h+o(h)\bigr)
\label{11-7-7}
\end{equation}
holds as $h=\max_jh_j\to+0$, $h_j=o(h)$ \ $\forall j\ge d'+1$ where
\begin{equation}
\varkappa_1=\mp {\frac{1}{4}}(2\pi )^{1-d}\omega_{d-1}
\int_{\partial X}V_-^{\frac{d-1}{2}}\, dS'\sqrt {g''}dx''
\label{11-7-8}%\tag{10.6.4}
\end{equation}
for Dirichlet and Neumann boundary conditions respectively and
the Riemannian densities $dS'$, $\sqrt{g''} dx''$ were introduced in
Example~\ref{ex-11-5-23}\ref{ex-11-5-23-ii} (see \textup{(\ref{11-5-68})}).

\item\label{thm-11-7-1-iii}
Furthermore, if $\vartheta >0$, $V_- ^{{\frac{d}{2}}+\vartheta },
\rho ^{d-1+\vartheta }\in \sL^1(X)$ we have, in the frameworks of Statements \ref{thm-11-7-1-i} and \ref{thm-11-7-1-ii}, asymptotics
\begin{gather}
\N^-_{(\vartheta)} (A_{\boldsymbol{h}})=
(h_1\dots h_d)^{-1}\bigl(\N^\W_{\vartheta ,{\boldsymbol{h}}}+
O(h^{1+\vartheta })\bigr)
\label{11-7-9}\\
\shortintertext{and}
\N^-_{(\vartheta)} (A_{\boldsymbol{h}})=
(h_1\dots h_d)^{-1}\bigl(\N^\W_{\vartheta ,{\boldsymbol{h}}}+
o(h^{1+\vartheta })\bigr)
\label{11-7-10}
\end{gather}
respectively.

\item\label{thm-11-7-1-iv}
 The same results remain true for $d=2$, $d'=d''=1$ under additional restrictions $\mes(Y)<\infty$ where $Y=\{X, \rho \gamma \le h_0\}<\infty $ for some $h_0>0$ and $V_-^{p+\vartheta }\in \sL^1(X'')$ for some $p>1$.

\item\label{thm-11-7-1-v}
 Under the cone condition all these results remain true for Neumann boundary conditions and also for the Dirac operator (with the reasonable boundary conditions). In the case of Dirac operator we consider eigenvalues lying in the interval $[\tau_1,\tau_2]$ with arbitrary fixed $\tau_1,\tau_2$.
\end{enumerate}
\end{theorem}

\begin{proof}
Statement~\ref{thm-11-7-1-i} follows immediately from Theorem~\ref{thm-9-1-7}.

Statement~\ref{thm-11-7-1-ii} follows from Theorem~\ref{thm-9-1-7} with an improved remainder estimates under non-periodicity assumption. Analysis of the Hamiltonian billiards is based on the same arguments as in Example~\ref{ex-11-5-23}\ref{ex-11-5-23-ii}; namely $\xi_j$ and $h_jx_j$ with $j\ge d'+1$ are ``almost constant'' (constant modulo $o(1)$) along these billiards (which is not true for $j\le d'$). But then
$\frac{d\ }{dt}x_j \equiv\sum_{k\ge d'+1} g^{jk}\xi_k \mod o(1)$ as $j\ge d'+1$ and for generic $\xi$ non-periodicity condition is fulfilled automatically.

The other Statements~\ref{thm-11-7-1-iii}--\ref{thm-11-7-1-v} are proven by a similar method.
\end{proof}

\subsection{Asymptotics of eigenvalues near \texorpdfstring{$+\infty$}{+\textinfty}}
\label{sect-11-7-3}

Here and below we consider the Schr\"{o}dinger operator $A_h$ and consider the number of its eigenvalues lesser than $\tau$. For the Dirac operator $A_h$ (we use the same notation) we consider the number of eigenvalues lying in the interval $[\tau_1,\tau)$ with fixed $\tau_1$.

Applying the arguments of Sections~\ref{sect-11-2}--\ref{sect-11-5} with
$\rho_{\tau,h}=h^{-1}(\rho+\sqrt{\tau})$ and $\gamma_{\tau,h}=\gamma$ we obtain modifications of the statements of these sections. However, we cannot anymore replace $\N^\W (\tau)$ by $\varkappa_0 \tau^{\frac{d}{2m}}$ in these assertions. In particular, we obtain the following statements:

\begin{theorem}\label{thm-11-7-2}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-7-2-i}
For the Schr\"{o}dinger operator, let conditions \textup{(\ref{11-1-6})}--\textup{(\ref{11-1-8})} be fulfilled with auxiliary functions $\rho,\gamma$. Let $\vartheta \ge 0$ and
\begin{equation}
\rho^{d+2\vartheta},1,\gamma^{-\vartheta-1}\in \sL^1(X).
\label{11-7-11}
\end{equation}
For $d=2$ let us assume also that
\begin{equation}
\rho ^{2p+2\vartheta }\in \sL^1(X)\qquad \text{with some\ \ }p>1.
\label{11-7-12}
\end{equation}
Moreover, in the case of the Neumann condition let us in addition assume that the cone condition is also fulfilled\,\footnote{\label{foot-11-57} We leave the analysis of mixed boundary conditions to the reader.}.
Then asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau ,h)=\N^\W_{(\vartheta)} (\tau ,h)
+O\bigl(\tau^{\frac{1}{2}(d+\vartheta-1)}h^{1-d+\vartheta}\bigr)
\label{11-7-13}
\end{equation}
holds as $\tau\to +\infty, h\to +0$. In particular, for $\vartheta=0$
\begin{equation}
\N^\W (\tau ,h)=\N^\W (\tau )h^{-d}.
\label{11-7-14}
\end{equation}

\item\label{thm-11-7-2-ii}
Further, if the set of all points which are periodic with respect to the
geodesic flow with reflections is of measure $0$ then asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau ,h)=\N^\W_{(\vartheta )} (\tau ,h) +
o_\tau \bigl(\tau ^{{\frac{1}{2}}(d+\vartheta -1)}
h^{1-d+\vartheta }\bigr)
\label{11-7-15}
\end{equation}
holds as $\tau \to+\infty ,h\to+0$ where $M'=o_\zeta (M)$ means that $M'M^{-1}\le \varepsilon (\zeta )$ with $\varepsilon (\zeta )=o(1)$ as $\zeta $ tends to the described limit.\enlargethispage{\baselineskip}

In particular, for $\vartheta =0$ asymptotics
\begin{equation}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+
\bigl(\varkappa_1+o_\tau (1)\bigr)\tau ^{\frac{1}{2}(d-1)}h^{1-d }
\label{11-7-16}
\end{equation}
holds as $\tau \to+\infty ,h\to+0$ with the coefficient
\begin{equation}
\varkappa_1=\mp {\frac{1}{4}}(2\pi )^{1-d}\omega_{d-1}
\Vol '\bigl(\partial X\cap \{\gamma >0\}\bigr)
\label{11-7-17}
\end{equation}
for Dirichlet and Neumann boundary conditions respectively.

\item\label{thm-11-7-2-iii}
Furthermore, let us assume that $\gamma^{-1-\theta}\in \sL^1(X)$ with
$\theta >\vartheta $ and that the geodesic flow is \underline{either} of non-periodic power type \underline{or} of non-periodic exponential type. Then these asymptotics hold the remainder estimates
\begin{gather}
O\bigl(\tau^{\frac{1}{2}(d+\vartheta-1-\delta')}h^{1-d+\vartheta}\bigr)
\label{11-7-18}\\
\shortintertext{or}
O\bigl(\tau^{\frac{1}{2}(d+\vartheta-1)}h^{1-d+\vartheta}
\log^{-1-\vartheta}\tau\bigr) \label{11-7-19}
\end{gather}
respectively.

\item\label{thm-11-7-2-iv}
 All these asymptotics remain true if we drop condition
$\rho ^{d+2\vartheta }\in \sL^1(X)$ replacing it by the coercivity condition
\textup{(\ref{11-4-5})}.

\item\label{thm-11-7-2-v}
Statements \ref{thm-11-7-2-i}--\ref{thm-11-7-2-iii} remain true for
$\vartheta =0$ for the Dirac
operator\,\footnote{\label{foot-11-58} For $\vartheta >0$ one should modify
$\N_{(\vartheta)} (\tau_1,\tau_2 ,h)$ in the obvious manner.}.
In these assertions one should replace $\N^-(\tau ,h)$ and $\N^\W (\tau_2)$ by $\N (\tau_1,\tau_2,h)$ and $\N^\W (\tau_1,\tau_2)$ respectively and take
$\tau=|\tau_1|+|\tau_2|\to \infty $. One should assume that
the boundary conditions are elliptic and the domain satisfies the cone
condition.
\end{enumerate}
\end{theorem}

We leave to the reader the following easy set of problems

\begin{problem}\label{problem-11-7-3}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-7-3-i}
Modify in the same way the complete set of Theorems \ref{thm-11-2-7}, \ref{thm-11-2-8}, \ref{thm-11-2-12} and Corollary \ref{cor-11-2-9}.

\item\label{problem-11-7-3-ii}
Consider Examples \ref{ex-11-2-13}, \ref{ex-11-2-14}, \ref{ex-11-2-15}, \ref{rem-11-2-17}, \ref{ex-11-2-18}, \ref{ex-11-2-19}, \ref{ex-11-2-21}, \ref{ex-11-2-22}, \ref{ex-11-2-25}, \ref{ex-11-2-26}, \ref{ex-11-2-27},
\ref{ex-11-3-34}, \ref{ex-11-3-35}, \ref{ex-11-4-8}, \ref{ex-11-4-9}, \ref{ex-11-4-10} and translate them into the framework of the present two-parameter theory (automatically or with minor modifications). The same for all other results of this type.

\item\label{problem-11-7-3-iii}
Modify Theorems \ref{thm-11-3-7}, \ref{thm-11-3-18}, \ref{thm-11-3-19}, \ref{thm-11-3-21}, \ref{thm-11-3-23}, \ref{thm-11-3-26} etc.

Here one should assume that $h\ge \tau ^{-n}$, and the principal part of the
asymptotics is of the form $\N^\W (\tau )h^{-d}$ and the second term is of the form
\begin{equation}
\bigl(\varkappa_1+F(\tau h^{-m})\bigr)
h^{1-d} \tau^{\frac{1}{2m}(d-1)}
\label{11-7-20}
\end{equation}
and there is additional factor $h^{1-d}$ in the remainder estimate.
\end{enumerate}
\end{problem}

Let us consider the statements of Section~\ref{sect-11-5}. For the sake of simplicity let us consider only the Schr\"{o}dinger operator. Then the following statements hold:

\begin{theorem}\label{thm-11-7-4}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-7-4-i}
In the framework of Theorem~\ref{thm-11-5-1} (with the additional assumption that $A$ is the Schr\"{o}dinger operator) asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau,h)= \N^\W_{(\vartheta)} (\tau,h)+
O\bigl(R_{(\vartheta)} (\tau) h^{1-d+\vartheta}\bigr)
\label{11-7-21}
\end{equation}
holds as $\tau\to +\infty, h\to +0$ where $R_{(\vartheta)} (\tau )$ is
defined by \textup{(\ref{11-5-3})}.

\item\label{thm-11-7-4-ii}
Further, under the additional assumptions of Theorem~\ref{thm-11-5-3}\ref{thm-11-5-3-i} asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau ,h)=\N^\W_{(\vartheta)} (\tau ,h)+ o_\tau
\bigl(R_{(\vartheta)} (\tau )h^{1-d+\vartheta }\bigr)
\label{11-7-22}
\end{equation}
holds as $\tau \to+\infty ,h\to+0$.

\item\label{thm-11-7-4-iii}
Furthermore, in the framework of Theorem~\ref{thm-11-5-3}\ref{thm-11-5-3-ii} asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau ,h)= \N^\W_{(\vartheta)} (\tau ,h)+
o_{\tau h^{-2}}\bigl(R_{(\vartheta)} (\tau )h^{1-d+\vartheta }\bigr)
\label{11-7-23}
\end{equation}
holds as $\tau \to+\infty ,h\to+0$. Moreover, the principal part in
asymptotics \textup{(\ref{11-7-21})} with $\vartheta =0$ is
$\N^\W (\tau )h^{-d}$ and in \textup{(\ref{11-7-22})}, \textup{(\ref{11-7-23})} the principal part is $\N^\W (\tau )h^{-d}+\varkappa_1\tau ^{l(d-1)}h^{1-d}$
with the coefficient $\varkappa_1$ given by \textup{(\ref{11-5-11})}.

\item\label{thm-11-7-4-iv}
 In the framework of Theorem~\ref{thm-11-5-6} for $\vartheta \le d-1-\delta $ with $\delta >0$ asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau ,h)=\N^\W_{(\vartheta)} (\tau ,h)+
O\bigl(\tau ^{l(d-1)+\vartheta (1-l)-\delta '}h^{1-d}\bigr)
\label{11-7-24}
\end{equation}
holds as $\tau \to+\infty ,h\to+0$. Here for $\vartheta =0$ the
principal part is the same as in \textup{(\ref{11-7-22})}. In particular, Example~\ref{ex-11-5-7} applies.

\item\label{thm-11-7-4-v}
In the frameworks of Theorems \ref{thm-11-5-14}, \ref{thm-11-5-18} and \ref{thm-11-5-20} asymptotics \textup{(\ref{11-7-21})} remains true. Moreover, under the conditions of these theorems on the Hamiltonian trajectories with reflections asymptotics \textup{(\ref{11-7-22})} remains true.

\item\label{thm-11-7-4-vi}
In the frameworks of Example~\ref{ex-11-5-23}\ref{ex-11-5-23-i} and \ref{ex-11-5-23-ii} asymptotics
\begin{gather}
\N (\tau ,h)=\N^\W (\tau )h^{-d}+O(\tau ^qh^{1-d}),
\label{11-7-25}\\%\tag{10.6.10}\\
\shortintertext{and}\N (\tau ,h)=\N^\W (\tau )h^{-d}+
\bigl(\varkappa_1+o_\tau (1)\bigr)\tau ^qh^{1-d},
\label{11-7-26}%\tag{10.6.11}
\end{gather}
hold respectively with the coefficient $\varkappa_1$ given by
\textup{(\ref{11-5-68})}.

\item\label{thm-11-7-4-vii}
 In the frameworks of Theorem~\ref{thm-11-5-25}\ref{thm-11-5-25-i} and \ref{thm-11-5-25-ii} the asymptotics
\begin{gather}
\N^-_{(\vartheta)} (\tau ,h)=\N^\W_{(\vartheta)} (\tau )h^{-d}+
O\bigl(\tau ^{{\frac{1}{2}}(d+\vartheta -1)}h^{1-d+\vartheta }
\omega (\tau )\bigr),
\label{11-7-27}\\
\shortintertext{and}
\N^-_{(\vartheta)} (\tau ,h)= \N^\W_{(\vartheta)} (\tau )h^{-d}+
o\bigl(\tau ^{{\frac{1}{2}}(d+\vartheta -1)}h^{1-d+\vartheta }
\omega (\tau )\bigr)
\label{11-7-28}
\end{gather}
hold respectively with
\begin{equation}
N^\W_{(\vartheta)} (\tau ,h)\asymp \tau ^{ \frac{d}{2} +\vartheta }
\log^{\frac{n}{\mu }}\tau h^{-d}
\label{11-7-29}
\end{equation}
and $\omega (\tau )$ defined by \textup{(\ref{11-5-73})}. For $\vartheta =0$ we
have $\N^\W (\tau ,h)= \N^\W (\tau )h^{-d}$.

Moreover, asymptotics \textup{(\ref{11-7-28})} remains true in the framework of Theorem~\ref{thm-11-5-26} and for $\vartheta =0$
\begin{equation}
\N^\W_{(0)}(\tau, h )=\N^\W (\tau )h^{-d}+\varkappa_1
\tau ^{{\frac{1}{2}}(d-1)}h^{1-d}\log \tau
\label{11-7-30}
\end{equation}
where the coefficient $\varkappa_1$ is defined by \textup{(\ref{11-5-80})}.

\item\label{thm-11-7-4-viii}
In the framework of Theorem~\ref{thm-11-5-28}\ref{thm-11-5-28-i} asymptotics with the principal part
\begin{equation}
\N^\W_{(\vartheta)} (\tau ,h)\asymp \N^\W (\tau )h^{-d},\qquad
\N_{(0)}^w(\tau ,h)=\N^\W (\tau )h^{-d}
\label{11-7-31}
\end{equation}
and with remainder estimate $h^{1-d+\vartheta} R_{(\vartheta)} (\tau)$ holds where $\N^\W (\tau)$ and $R_{(\vartheta)} (\tau)$ are defined in the theorem.

Moreover, the improvements made in Statement \ref{thm-11-5-28-ii} and in footnote \footref{foot-11-44} remain true.
\end{enumerate}
\end{theorem}

We leave to the reader the following easy set of problems:

\begin{problem}\label{problem-11-7-5}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-7-5-i} Analyze Examples \ref{ex-11-5-17}, \ref{ex-11-5-19} and \ref{ex-11-5-21}.

\item\label{problem-11-7-5-ii} Modify Theorems \ref{thm-11-5-5}, \ref{thm-11-5-9} and \ref{thm-11-5-11}.

Note that remark in Problem~\ref{problem-11-7-3}\ref{problem-11-7-3-iii} also remains true in this case.
\end{enumerate}
\end{problem}


\subsection{Asymptotics of eigenvalues near $-0$ and related
asymptotics}
\label{sect-11-7-4}

Applying the arguments of Section~\ref{sect-11-6} with
$\rho_{\tau ,h}=h^{-1}(\rho +\sqrt |\tau |)$ and $\gamma_{\tau ,h}=\gamma $ we obtain

\begin{theorem}\label{thm-11-7-6}
Again, we treat only the Schr\"{o}dinger operator.
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-7-6-i}
In the framework of Theorem~\ref{thm-11-6-1} asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau ,h)= \N^\W_{(\vartheta)} (\tau ,h)
+O\bigl(h^{1-d+\vartheta } R_{(\vartheta)} (\tau )\bigr)
\label{11-7-32}
\end{equation}
holds as $\tau \to -0$, $h\to+0$ with $R_{(\vartheta)} (\tau )$ defined by \textup{(\ref{11-6-4})}.

\item\label{thm-11-7-6-ii}
Moreover, in the framework of Theorem~\ref{thm-11-6-2}\ref{thm-11-6-2-i} asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau ,h)=\N^\W_{(\vartheta)} (\tau ,h)+
o_\tau \bigl(h^{1-d+\vartheta }R_{(\vartheta)} (\tau )\bigr)
\label{11-7-33}
\end{equation}
holds as $\tau \to -0$, $h\to+0$.

For $\vartheta =0$ the principal parts of these asymptotics are
$\N^\W (\tau )h^{1-d}$ and
\begin{equation}
\N^\W (\tau )h^{1-d}+\varkappa_1|\tau |^{l(d-1)}h^{1-d}
\label{11-7-34}
\end{equation}
respectively with the coefficient $\varkappa_1$ given by \textup{(\ref{11-6-11})}.

\item\label{thm-11-7-6-iii}
In the framework of Theorem~\ref{thm-11-6-5} with
$\vartheta \le \vartheta_1-\delta $, $\delta >0$ asymptotics
\begin{equation}
\N^-_{(\vartheta)} (\tau ,h)=\N^\W_{(\vartheta)} (\tau ,h) +
O(h^{1-d+\vartheta }|\tau |^{l(d-1)+\vartheta (1-l)+\delta '})
\label{11-7-35}
\end{equation}
holds with $\delta '>0$. In these asymptotics the principal part for
$\vartheta =0$ is $\N^\W (\tau )h^{1-d}+\varkappa_1 |\tau|^{l(d-1)} h^{1-d}$. In
particular, Example~\ref{ex-11-6-6} applies.

\item\label{thm-11-7-6-iv}
In the framework of Theorem~\ref{thm-11-6-10} asymptotics \textup{(\ref{11-7-32})} remains true and under a condition on Hamiltonian trajectories with reflection asymptotics \textup{(\ref{11-7-33})} also remains true.

\item\label{thm-11-7-6-v}
In the frameworks of Example~\ref{ex-11-6-13}\ref{ex-11-6-13-i} and \ref{ex-11-6-13-ii} asymptotics
\begin{gather}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+ O(|\tau |^qh^{1-d}),
\label{11-7-36}\\
\shortintertext{and}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+
\bigl(\varkappa_1+o_\tau (1)\bigr)|\tau |^qh^{1-d}
\label{11-7-37}
\end{gather}
hold with the coefficient $\varkappa_1$ given by \textup{(\ref{11-6-35})}.

\item\label{thm-11-7-6-vi}
In the frameworks of Theorems~\ref{thm-11-6-14}\ref{thm-11-6-14-i} and \ref{thm-11-6-14-ii} asymptotics
\begin{gather}
\N (\tau ,h)=\N^\W (\tau )h^{-d}+
O\bigl(\bigl|\log |\tau |\bigr|^{\nu (d-1)+1}h^{1-d}\bigr),
\label{11-7-38}\\
\shortintertext{and}
\N (\tau ,h)=\N^\W (\tau )h^{-d}+
\bigl(\varkappa_1+o_\tau (1)\bigr)
\bigl|\log |\tau |\bigr|^{\nu (d-1)+1}h^{1-d}
\label{11-7-39}
\end{gather}
respectively hold with the coefficient $\varkappa_1$ given by \textup{(\ref{11-6-40})}.

\item\label{thm-11-7-6-vii}
 Moreover, Statement \ref{thm-11-7-6-vi} remains true for $\nu =0$ with $o_\tau (1)$ replaced by $o(1)$ in asymptotics \textup{(\ref{11-7-39})}.
\end{enumerate}
\end{theorem}

\begin{remark}\label{rem-11-7-7}
Statement Statement \ref{thm-11-7-6-vii} dealing with potentials decaying as $|x|^{-2}$ has no analog in Section~\ref{sect-11-6} because for $\nu =0$ for every small enough fixed $h>0$ the eigenvalues of $A_h$ tend to $-0$ but in \textup{(\ref{11-7-38})} both the principal part and the remainder estimate are of the same order $\log|\tau|$ and \textup{(\ref{11-7-38})} is only an estimate (or a couple of estimates: from above and below), not asymptotics.
\end{remark}

We leave to the reader

\begin{problem}\label{problem-11-7-8}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-7-8-i}
 Modify Example~\ref{ex-11-6-11}.

\item\label{problem-11-7-8-ii}
In the framework of Problem~\ref{problem-11-6-15} derive asymptotics with the principal parts
\begin{equation*}
N^\W_{(\vartheta)} (\tau ,h)\asymp
\N^W_{\vartheta ,h}(\tau )h^{-d},
\qquad N_{(0)}^\W (\tau,h )=\N^\W (\tau )h^{-d}
\end{equation*}
and remainder estimate $O\bigl(h^{1-d+\vartheta} R_{(\vartheta)} (\tau)\bigr)$ where $\N^\W (\tau)$, $R_{(\vartheta)} (\tau)$ are defined in that problem.

\item\label{problem-11-7-8-iii}
Modify Theorems \ref{thm-11-6-4}, \ref{thm-11-6-7} and \ref{thm-11-6-9}.

Note that remark in Problem~\ref{problem-11-7-3}\ref{problem-11-7-3-iii} also remains true in this case as $h\ge |\tau|^n$.
\end{enumerate}
\end{problem}

Let us consider the situation in which the conditions of Theorem~\ref{thm-11-6-14} are fulfilled with $\nu <0$ instead of $\nu >0$.

In this case for every fixed $h>0$ the discrete spectrum is finite. However,
$V_-^{\frac{d}{2}}\notin \sL^1(X)$ for $\nu \ge -d^{-1}$ provided condition (\ref{11-6-8}) is fulfilled. In this case the above arguments
lead us to the following

\begin{theorem}\label{thm-11-7-9}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-7-9-i}
Under the assumptions of Theorem~\ref{thm-11-6-14}\ref{thm-11-6-14-i} with
$\nu \in (-d ^{-1},0)$ asymptotics \textup{(\ref{11-7-38})} holds for the Schr\"{o}dinger operator for $\tau \to -0$, $h\to +0$ provided
\begin{equation}
h=o\bigl(\bigl|\log|\tau |\bigr| ^\nu \bigr).
\label{11-7-40}
\end{equation}
In this asymptotics
$\N^\W (\tau )=O\bigl(\bigl|\log|\tau |\bigr| ^{\nu d+1}\bigr)$ and under condition \textup{(\ref{11-6-8})}
$\N^\W (\tau )\asymp \bigl|\log|\tau |\bigr| ^{\nu d+1}$.

\item\label{thm-11-7-9-ii}
Under the assumptions of Theorem~\ref{thm-11-6-14}\ref{thm-11-6-14-i} with
$\nu =-d ^{-1}$ asymptotics \textup{(\ref{11-7-38})} holds for the Schr\"{o}dinger operator for
$\tau \to -0$, $h\to +0$ provided
\begin{equation}
h=O\bigl(\bigl|\log|\tau |\bigr| ^\nu \bigr).
\label{11-7-41}
\end{equation}
In this asymptotics $\N^\W (\tau )=O\bigl(\log\bigl|\log|\tau |\bigr|\bigr)$ and under condition \textup{(\ref{11-6-8})}
$\N^\W (\tau )\asymp \log\bigl|\log|\tau |\bigr|$.

\item\label{thm-11-7-9-iii}
 Under the assumptions of Theorem~\ref{thm-11-6-14}\ref{thm-11-6-14-ii} with
$\nu \in [-d ^{-1},0)$ asymptotics \textup{(\ref{11-7-39})} holds for the Schr\"{o}dinger operator for $\tau \to -0 $, $h\to +0$ satisfying \textup{(\ref{11-7-40})}. In this asymptotics coefficient $\varkappa_1$ is given by \textup{(\ref{11-6-40})}.
\end{enumerate}
\end{theorem}

Let us consider the case
\begin{equation}
h\ge \epsilon_0\bigl|\log|\tau|\bigr|^\nu.
\label{11-7-42}
\end{equation}
Then the singular zone
$X_\sing =\bigl\{(\rho +\sqrt{|\tau |})\gamma \le \epsilon h\bigr\}$
is not necessarily empty. Considering only the lower estimate we
obtain that under condition (\ref{11-6-8})
\begin{alignat}{2}
\N^- (\tau,h) &\ge \epsilon_1 h^{\frac{1}{\nu}}
\qquad &\text{for\ }\nu &\in (-\frac{1}{d},0),
\label{11-7-43}\\
\shortintertext{and}
\N^- (\tau ,h) &\ge \epsilon_1 h^{\frac{1}{\nu}} |\log h|
\qquad &\text{for\ }\nu &=-\frac{1}{d}
\label{11-7-44}
\end{alignat}
with $\epsilon_1>0$.

On the other hand, for $d\ge 3$ one can apply a variational estimate in $X_\sing$ (with $\rho =0$ for $\log ^\nu r\le \epsilon_2h$. Then we obtain estimate
\begin{equation}
\N^- (\tau ,h)=O(h^{\frac{1}{\nu }})\qquad \text{for\ \ }
\nu \in (-{\frac{1}{d}},0),
\label{11-7-45}
\end{equation}
and even asymptotics
\begin{equation}
\N^- (\tau ,h)=\bigl(\N^\W_h(\tau ) +O(1)\bigr)h^{-d}\qquad
\text{for\ }\nu =-{\frac{1}{d}}
\label{11-7-46}
\end{equation}
for $\tau \to-0$, $h\to+0$ with
\begin{equation}
\N^\W_h(\tau )=(2\pi )^{-d}\omega_d
\int_{\{|\log|x||\le Ch^{-{\frac{1}{\nu }}}\} }
\bigl(-\tau -V\bigr)_+^{\frac{d}{2}}\sqrt g\, dx
\label{11-7-47}%\tag{10.6.25}
\end{equation}
with an arbitrarily chosen constant $C$. Under condition (\ref{11-6-8})
this expression is
$\asymp \min \bigl(\log \bigl|\log|\tau |\bigr|, |\log h|\bigr)$ for
$\nu =-d ^{-1}$.

Let us recall that the asymptotics and estimates (\ref{11-7-43})--(\ref{11-7-46}) were obtained under the restriction (\ref{11-7-42}).

Thus we arrive to

\begin{remark}\label{rem-11-7-10}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{rem-11-7-10-i}
If $d\ge 3$, $\nu \in (-d ^{-1},0)$ then under condition (\ref{11-6-8})
$\N^- (\tau ,h)\asymp h^{\frac{1}{\nu}}$ for $\tau\to-0$, $h\to+0$ satisfying
(\ref{11-7-42}). One can easily obtain this result by purely variational arguments.

\item\label{rem-11-7-10-ii}
For $d\ge 3$, $\nu =-d ^{-1}$ we combine Statement~\ref{thm-11-7-9-ii} of Theorem~\ref{thm-11-7-9} and (\ref{11-7-46}) to obtain
\begin{equation}
\N^- (\tau ,h)=\N^\W_h(\tau )h^{-d}+ O\Bigl(\min \bigl(h^{-d},
h^{1-d}\bigl|\log |\tau |\bigr|^{\frac{1}{d}}\bigr)\Bigr)
\label{11-7-48}
\end{equation}
with $\N^\W_h(\tau )$ given by (\ref{11-7-47}) and $\tau \to -0$, $h\to +0$.
\end{enumerate}
\end{remark}

We leave to the reader the following

\begin{problem}\label{problem-11-7-11}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-7-11-i}
Treat the case $\nu \in [-(d-1) ^{-1},-d ^{-1})$. In this case the principal part is standard and $\asymp h^{-d}$ but the remainder estimate is worse
than usual. In this case we also obtain asymptotics for $\tau=0$
in the context of Section~\ref{sect-11-1}.

\item\label{problem-11-7-11-ii}
rove that all the results of this subsection remain true for the Dirac operator with
\begin{equation}
\tau^0_1=-M+\limsup_{|x|\to\infty} V<\tau^0_2=M+\liminf_{|x|\to\infty} V.
\label{11-7-49}
\end{equation}
One need only to replace $\N^- (\tau;h )$ by $\N (\tau_1,\tau ;h)$ with fixed
$\tau_1\in (\tau ^0_1,\tau ^0_2)$ and respectively modify the formulas for
$\N^\W $, $\N^\W_h$, $\varkappa_0$ and $\varkappa_1$; without any loss of the generality one can assume that $\tau ^0_2=0$ and then $\tau \to -0$.\end{enumerate}
\end{problem}


\subsection{Asymptotics of eigenvalues near $+0$}
\label{sect-11-7-5}

Arguments of the same type as above permit us also to treat the case
$\tau \to +0$, $h\to +0$ and to obtain asymptotics of $\N^- (\tau ,h)$ assuming that $\inf V=0$ for the Schr\"{o}dinger operator.

Similar results may be obtained for the Dirac operator for $\N (\tau_1,\tau ;h)$ provided (\ref{11-7-49}) holds, $\tau_1\in (\tau ^0_1,\tau ^0_2)$ and
\begin{equation*}
\tau ^0_1=-M+\sup V<\tau_1\le \tau ^0_2=M+\inf V;
\end{equation*}
without any loss of the generality one can assume that $\tau ^0_2=0$ and then $\tau \to +0$.

We formulate our statements only for the Schr\"{o}dinger operator with Dirichlet boundary conditions.  For the the Schr\"{o}dinger operator with Neumann boundary conditions and for the Dirac operator with any self-adjoint boundary conditions
these statements remain true as long as the domain $X$ satisfies the cone condition.

It is easy to prove the following

\begin{theorem}\label{thm-11-7-12}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-7-12-i}
Let $X$ be a bounded domain and let $Y$ a $\sC^1$ manifold of codimension $d''$ in $\bR ^d$, $2\le d''\le d$ such that $\bar{X}\cap Y\ne \emptyset$.
\enlargethispage{2\baselineskip}

Let conditions \textup{(\ref{11-1-6})}--\textup{(\ref{11-1-8})}, \textup{(\ref{11-4-5})} be fulfilled with $\gamma =\epsilon r(x)$,
$\rho (x)=r ^\mu (x)$, $\epsilon >0$, $\mu >0$, $r(x)=\dist (x,Y)$.
Then asymptotics
\begin{equation}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+O\bigl(\tau ^qh^{1-d}\bigr)
\label{11-7-50}
\end{equation}
holds for $\tau \to +0$, $h\to+0$ with
$\N^\W (\tau )=O(\tau ^p)$, $p=\frac{1}{2}d+ \frac{1}{2\mu} d'' $ and
$q=\frac{1}{2}(d-1)+ \frac{1}{2\mu} (d''-1)$\,\footnote{\label{foot-11-59} Surely we obtain asymptotics only for $h=o(\tau^l)$ with
$l={\frac{1}{2\mu}}(\mu +1)$, i.e., only if $\tau $ tends to $+0$ slowly
enough. Otherwise we obtain only an upper estimate and for
$h\ge \epsilon_0\tau ^l$ with a small enough constant $\epsilon_0$
we obtain a lower estimate for $\N^- (\tau ,h)$. This remark
remains true for other asymptotics of this subsection.}\footnote{\label{foot-11-60} We did not study the lowest eigenvalue but under rather general assumptions one can prove that it is $\tau_1>0: \,\tau_1\asymp h^{1/l}$.}.

Moreover, $\N^\W (\tau )\asymp \tau ^p$ provided
\begin{equation}
\Vol \bigl(X\cap \{r(x)<{\bar r}\}\bigr)\asymp r^n \quad \text{as\ }r\to 0
\label{11-7-51}
\end{equation}
with $n=d''$.

\item\label{thm-11-7-12-ii}
Further, let us assume that $Y=\{0\}$,
$X\cap \{|x|\le r_0\}=X^0\cap \{|x|\le r_0\}$ where $r_0>0$ and $X^0$ is the non-empty open cone with $\partial X^0\setminus 0\in \sC^K$.

Let stabilization conditions \textup{(\ref{11-5-4})} be fulfilled for $|x|\to 0$ with functions $g^{jk0}$, $V_j^0$ and $V^0$ positively homogeneous of degrees $0$, $\mu $ and $2\mu $ respectively.

Finally, let the standard non-periodicity condition be fulfilled for the domain $X^0$ and the Hamiltonian
\begin{equation}
H^0_\st= \sum_{j,k} g^{jk0}(\xi_j-V_j^0)(\xi_k-V_k^0)+V^0-1
\label{11-7-52}
\end{equation}
on the energy level $0$. Then the asymptotics
\begin{equation}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+
\bigl(\varkappa_1+o(1)\bigr)\tau ^{l(d-1)}h^{1-d}
\label{11-7-53}
\end{equation}
holds as $\tau \to +0$, $h=o(\tau ^l)$ with the coefficient $\varkappa_1$ given by \textup{(\ref{11-5-11})}.

Note that under the stabilization
conditions alone, $\N^\W =\bigl(\varkappa_0+o(1)\bigr)\tau ^{ld}$
with the coefficient $\varkappa_0$ given by \textup{(\ref{11-5-10})}.


\item\label{thm-11-7-12-iii}
Finally, let the stabilization conditions
\begin{multline}
D^\alpha (a_\beta -a^0_\beta )=
O\bigl(|x|^{(2m-|\beta |)\mu -|\alpha |+\delta }\bigr) \\
\forall \beta :|\beta |\le 2m\quad \forall \alpha :|\alpha |\le 1
\label{11-7-54}
\end{multline}
be fulfilled as $|x|\to 0$ with some $\delta >0$. Let the Hamiltonian
flow generated by $H^0_\st$ near $0$ be of non-periodic power
type. Then the asymptotics
\begin{equation}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+
\bigl(\varkappa_1+O(h^{\delta '}\tau ^{-l\delta '})\bigr)
h^{1-d}\tau ^{l(d-1)}
\label{11-7-55}
\end{equation}
with $\delta '>0$ holds for $\tau \to +0$, $h=o(\tau ^l)$.
\end{enumerate}
\end{theorem}

We leave to the reader the following easy Problem~\ref{problem-11-7-13} and the proofs of Theorems~\ref{thm-11-7-14}--\ref{thm-11-7-16} below.\enlargethispage{\baselineskip}

\begin{problem}\label{problem-11-7-13}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{problem-11-7-13-i}
Generalize Statement~\ref{thm-11-7-12-ii} of Theorem~\ref{thm-11-7-12} to the case $d''<d$. The arguments of Example~\ref{ex-11-5-23}(ii) should be applied here.

\item\label{problem-11-7-13-ii}
Consider the case of periodic Hamiltonian flow.

\item\label{problem-11-7-13-iii}
Consider the case $d''=1$ when the logarithmic factor appears in the remainder estimate.

\item\label{problem-11-7-13-iv}
Consider the general operators and the case $\vartheta >0$.
\end{enumerate}
\end{problem}

\begin{theorem}\label{thm-11-7-14}
Let $X$ be a bounded domain, $0\in X$ and
\begin{equation}
X\cap \{|x|\le r_0\}=X ^0\cap \{|x|\le r_0\}
\label{11-7-56}
\end{equation}
where $X^0$ is an $L$-quasi-conical domain in $\bR^d$. Let $g^{jk}$, $V_j$ and $V$ be $L$-quasi-homogeneous with respect to $x$ of degrees $0$, $\mu $, $2\mu $ respectively with $\mu >0$, $L=(L_1,\dots ,L_d)$, $L_j=1$ for $j\le d'$ and $L_j<1$ for $j\ge d'+1$, $0<d'<d$.

Let us assume that $\partial X\setminus 0 \in \sC^K$ and
$g^{jk},V_j,V\in \sC^K(\bar{X}\setminus 0)$ satisfy condition
\textup{(\ref{11-1-8})}\,\footnote{\label{foot-11-61} Then one can take
$\gamma =\epsilon [x]_L$, $\rho =\epsilon [x]_L ^\mu $.}
Finally, let us assume that
\begin{equation}
V(x)>0\qquad \forall x\in \bar{X}\setminus 0.
\label{11-7-57}
\end{equation}
Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-7-14-i}
Asymptotics
\begin{equation}
\N^- (\tau ,h)=\varkappa_0 \tau ^ph^{-d}+O(\tau ^qh^{1-d})
\label{11-7-58}
\end{equation}
holds for $\tau \to+0$, $h\to+0$ with $p=\frac{1}{2}d+ \frac{1}{2\mu } L^*$,
$q=\frac{1}{2}(d-1)+ \frac{1}{2\mu } (L^*-1)$, $L^*=L_1+\ldots +L_d$ and
with the coefficient $\varkappa_0$ given by \textup{(\ref{11-5-63})} with $X$
replaced by $X^0$.

\item\label{thm-11-7-14-ii}
Under the additional conditions of Example~\ref{ex-11-5-23}\ref{ex-11-5-23-ii}
asymptotics
\begin{equation}
\N^- (\tau ,h)=\varkappa_0 \tau ^ph^{-d}+
\bigl(\varkappa_1+o(1)\bigr)\tau ^qh^{1-d}
\label{11-7-59}
\end{equation}
holds for $\tau \to-0$, $h=o(\tau ^{\frac{1}{2}+\frac{1}{2\mu}})$ with the coefficient $\varkappa_1$ given by \textup{(\ref{11-5-67})}.
\end{enumerate}
\end{theorem}

\begin{theorem}\label{thm-11-7-15}
Let $X$ be a bounded domain and let $Y$ be a $\sC^1$ manifold of codimension $d''$ in $\bR^d$, $2\le d''\le d$, $\bar{X}\cap Y\ne \emptyset$.

Let conditions
\textup{(\ref{11-1-6})}--\textup{(\ref{11-1-8})}, \textup{(\ref{11-4-5})} be fulfilled with $\gamma =\epsilon r(x)$, $\rho =\exp \bigl(-r(x) ^\nu \bigr)$ with $\nu <0$, $r(x)=\dist (x,Y)$.

Let us assume that condition \textup{(\ref{11-7-51})} is fulfilled with an
exponent $n$ which is now not necessarily equal to $d''$. Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-7-15-i}
Asymptotics
\begin{equation}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+
O\bigl(\tau ^{{\frac{1}{2}}(d-1)}|\log \tau |^{(\nu +n-1)\nu ^{-1}}
h^{1-d}\bigr)
\label{11-7-60}
\end{equation}
holds for $\tau \to+0$, $h\to +0$ and
$\N^\W (\tau )\asymp \tau ^{ \frac{1}{2} d}|\log \tau |^{n\nu ^{-1}}$.

\item\label{thm-11-7-15-ii}
 Moreover, let $Y=\{0\}$, $n=d$. Let condition \textup{(\ref{11-7-59})} be
fulfilled for $r\to +0$ and every fixed $k$ and let conditions
\textup{(\ref{11-5-75})}--\textup{(\ref{11-5-76})} be fulfilled for $|x|\to 0$. Then asymptotics
\begin{equation}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+
o\bigl(\tau ^{{\frac{1}{2}}(d-1)}|\log \tau |^{(\nu +n-1)\nu ^{-1}}
h^{1-d}\bigr)
\label{11-7-61}
\end{equation}
holds for $\tau \to+0$,
$h=o\bigl(\tau ^{\frac{1}{2}}|\log \tau |^{(1-\nu )\nu ^{-1}}\bigr)$.
\end{enumerate}
\end{theorem}

\begin{theorem}\label{thm-11-7-16}
Let $d\ge 3$, $X=(0,\frac{1}{2} )\times U$ where $U$ is a domain on $\bS^{d-1}$
with $\sC^K$ boundary, $g^{jk}=g^{jk}(\theta )\in \sC^K(\bar{U})$ satisfy
\textup{(\ref{11-4-5})}. Let $V_j=0$, $V=v(\theta )|\log r|^{-1}$ with
$v\in \sC^K(\bar{U})$ and $\min_{\bar{U}} v=v_0>0$. Then asymptotics
\begin{equation}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+O\Bigl(h^{1-d}\tau ^{d-2}
\int_U\exp \bigl(-v(d-1)\tau ^{-1}\bigr)\,d\theta \Bigr)
\label{11-7-62}
\end{equation}
holds as $\tau \to+0$, $h\to+0$ with
\begin{equation}
\N^\W (\tau )=a\int_{U'}\tau ^dv^{-{\frac{d}{2}}}
F_d({\frac{\tau }{v}})\exp (-vd\tau ^{-1})\sqrt g\,d\theta
\label{11-7-63}
\end{equation}
where $U'=U\cap \{v <v_0+\varepsilon \}$, $\varepsilon >0$ is arbitrarily small, and $a$ and $F_d$ are introduced in Theorem~\ref{thm-11-6-14}
in which the orders of $\N^\W (\tau)$ and the remainder estimate are also discussed.
\end{theorem}

\subsection{Asymptotics of eigenvalues near \texorpdfstring{$-\infty $}{-\textinfty}}
\label{sect-11-7-6}

Let us consider asymptotics of $\N (\tau ,h)$ for $\tau \to -\infty $, $h\to+0$. Recall that we consider the Schr\"{o}dinger operator and now we assume that
\begin{equation}
\inf V=-\infty;
\label{11-7-64}
\end{equation}
thus it is still the case``$\tau \searrow \inf V$''. The results of this subsection surely do not make any sense for the Dirac operator. The same arguments as above give us the following

\begin{theorem}\label{thm-11-7-17}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-7-17-i}
Let $X$ be a bounded domain in $\bR^d$, $0\in \bar{X}$ and let conditions \textup{(\ref{11-1-6})}--\textup{(\ref{11-1-8})} be fulfilled with $\gamma=\epsilon|x|$, $\rho=|x|^\mu$, $\mu \in (-1,0)$. Then asymptotics\footref{foot-11-59}\footref{foot-11-60}
\begin{equation}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+
O\bigl(|\tau |^{l(d-1)}h ^{1-d}\bigr)
\label{11-7-65}
\end{equation}
holds for $\tau \to-\infty $, $h\to+0$ and $\N^\W (\tau)=O(|\tau |^{ld})$.

Moreover,
$\N^\W (\tau )\asymp |\tau |^{ld}$ provided
\begin{equation}
\mes\bigl(\bigl\{x\in X,|x|\le r, V\le -\epsilon_0\rho ^2(x)\bigr\}\bigr)
\asymp r^d \qquad \text{for\ \ } r\to +0.
\label{11-7-66}
\end{equation}

\item\label{thm-11-7-17-ii}
Further, let $X\cap \{|x|\le r_0\}=X^0\cap \{|x|\le r_0\}$ with
some $r_0>0$ and an open non-empty cone $X^0$ such that
$\partial X^0\setminus 0\in \sC^K$. Let stabilization conditions
\textup{(\ref{11-5-4})} be fulfilled for $|x|\to 0$ with functions
$g^{jk0},V_j^0,V^0\in \sC^K(\bar{X} ^0\setminus 0)$.

Let the standard non-periodicity condition to the Hamiltonian flow be fulfilled on the energy level  $0$ for the Hamiltonian
\begin{equation}
H^0(x,\xi )=
|x|^{1-\mu }\bigl(\sum_{j,k}  g^{jk0}(\xi_j-V_j^0)(\xi_k-V_k^0)+V^0+1\bigr).
\label{11-7-67}
\end{equation}
Then asymptotics
\begin{equation}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+
\bigl(\varkappa_1+o(1)\bigr)|\tau |^{l(d-1)}h^{1-d}
\label{11-7-68}
\end{equation}
holds for $\tau \to -\infty $, $h=o(|\tau |^l)$ with the coefficient
$\varkappa_1$ given by \textup{(\ref{11-6-11})}.

\item\label{thm-11-7-17-iii}
 Furthermore, let stabilization conditions \textup{(\ref{11-7-54})} with
$\delta >0$ be fulfilled for $x\to 0$ and let the Hamiltonian flow
corresponding to the Hamiltonian
\begin{equation}
H^0_\st(x,\xi )=\sum_{j,k} g^{jk0}\bigl(\xi_j-V_j^0)(\xi_k-V_k^0)+V^0+1
\label{11-7-69}
\end{equation}
be of power non-periodic type near the energy level $0$. Then
asymptotics
\begin{equation}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+
\bigl(\varkappa_1+O(h^{\delta '}|\tau |^{-l\delta '})\bigr)
|\tau |^{l(d-1)}h^{1-d}
\label{11-7-70}
\end{equation}
with $\delta '>0$ holds for $\tau \to -\infty $, $h\to+0$.
\end{enumerate}\end{theorem}

We leave to the reader the following easy Problem~\ref{problem-11-7-18} and Theorems~\ref{thm-11-7-19},  \ref{thm-11-7-20} and \ref{thm-11-7-22} below.

\begin{problem}\label{problem-11-7-18}
Treat the case of a singularity at a manifold of codimension less than $d$.
\end{problem}

\begin{theorem}\label{thm-11-7-19}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-7-19-i}
Let conditions of Theorem~\ref{thm-11-7-14} be fulfilled with $\mu \in (-1,0)$. Then asymptotics
\begin{equation}
\N^- (\tau ,h)=\varkappa_0|\tau |^ph^{-d}+
O\bigl(|\tau |^qh^{1-d}\bigr)
\label{11-7-71}
\end{equation}
holds as $\tau \to-\infty $, $h\to +0$ with the same exponents $p$, $q$ and coefficient $\varkappa_0$ as in Theorem~\ref{thm-11-7-14} (i.e. given by \textup{(\ref{11-5-63})} with $X$ replaced by $X^0$).

\item\label{thm-11-7-19-ii}
Further, under the additional restrictions of Theorem~\ref{thm-11-7-14}\ref{thm-11-7-14-ii} asymptotics
\begin{equation}
\N^- (\tau ,h)=\varkappa_0|\tau |^ph^{-d}+
\bigl(\varkappa_1+o(1)\bigr)|\tau |^qh^{1-d}
\label{11-7-72}
\end{equation}
holds for $\tau \to -\infty $, $h=o(|\tau |^{{\frac{1}{2\mu}}(\mu +1)})$
with the coefficient $\varkappa_1$ given by \textup{(\ref{11-5-68})}.
\end{enumerate}
\end{theorem}

\begin{theorem}\label{thm-11-7-20}
Let $X$ be a bounded domain in $\bR^d$, $0\in\bar{X}$ and let conditions \textup{(\ref{11-1-6})}--\textup{(\ref{11-1-8})} be fulfilled with
$\gamma =\epsilon |x|$,
$\rho =|x| ^{-1}\bigl(\bigl|\log |x|\bigr|+1\bigr) ^\nu $,
$\nu \le -d ^{-1}$. Then


\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-7-20-i}
For $\nu <-(d-1) ^{-1}$ asymptotics
\begin{equation}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+
O\bigl((\log |\tau |)^{\nu (d-1)+1}h ^{1-d}\bigr)
\label{11-7-73}
\end{equation}
holds for $\tau \to-\infty $, $h\to+0$.

\item\label{thm-11-7-20-ii}
For $\nu =-(d-1) ^{-1}$ the asymptotics
\begin{equation}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+
O\bigl(\log(\log|\tau |\cdot h^{-\nu ^{-1}})h^{1-d}\bigr)
\label{11-7-74}
\end{equation}
holds for $\tau \to -\infty $, $h=o(\log ^\nu |\tau |)$.

\item\label{thm-11-7-20-iii}
Furthermore, let $X\cap\{|x|\le r_0\}= X^0\cap\{|x|\le r_0\}$ with
$r_0>0$ and a non-empty open cone $X^0$ with
$\partial X^0\setminus 0\in \sC^K$. Let the
functions $g^{jk}$, $V_j\bigl|\log|x|\bigr|^{-\nu}$,
$V\bigl|\log|x|\bigr|^{-2\nu}$ satisfy stabilization conditions
\textup{(\ref{11-5-4})} for $|x|\to 0$ with $\mu =-1$ and with functions
$g^{jk0}$, $V_j^0$, $V^0$ positively homogeneous of degrees $0$,
$-1$, $-2$ respectively.

Moreover, let the standard non-periodicity condition be fulfilled with the Hamiltonian
\begin{equation}
H^0(x,\xi )=|x|^2\bigl(\sum_{j,k} g^{jk0}(\xi_j-V^0_j)(\xi_k-V^0_k)+V^0\bigr)
\label{11-7-75}
\end{equation}
on the energy level  $0$. Then in the framework of Statement  \ref{thm-11-7-20-i} asymptotics
\begin{equation}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+
\bigl(\varkappa_1+o(1)\bigr)(\log |\tau |)^{\nu (d-1)+1}h^{1-d}
\label{11-7-76}
\end{equation}
holds for $\tau \to -\infty $, $h=o(\log ^\nu |\tau |)$ and in the framework of Statement \ref{thm-11-7-20-ii} asymptotics
\begin{equation}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+
\bigl(\varkappa_1+o(1)\bigr)
\log(\log|\tau |\cdot h^{-\nu ^{-1} })h^{1-d}
\label{11-7-77}
\end{equation}
holds for $\tau \to -\infty $, $h=o(\log ^\nu |\tau |)$.

\item\label{thm-11-7-20-iv}
 Furthermore, for $\nu \in (-(d-1) ^{-1},-d ^{-1})$ asymptotics
\begin{equation}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+O\bigl(h^{\nu ^{-1}}\bigr)
\label{11-7-78}
\end{equation}
holds for $\tau \to -\infty $, $h=o(\log ^\nu |\tau |)$.

In all these asymptotics $\N^\W (\tau )=O(\log^{\nu d+1} |\tau |)$ and
$\N^\W (\tau )\asymp \log ^{\nu d+1}|\tau |$
under condition \textup{(\ref{11-7-66})}.

\item\label{thm-11-7-20-v}
Let $\nu =-d ^{-1}$. Furthermore, suppose that \underline{either} $d\ge 3$ \underline{or} $0\in \partial X$ and a Dirichlet condition is given on
$\partial X$. Then asymptotics
\begin{equation}
\N^- (\tau ,h)=\bigl(\N^\W(\tau,h )+O(1)\bigr)h^{-d}
\label{11-7-79}
\end{equation}
holds for $\tau \to -\infty $, $h=o(\log ^\nu |\tau |)$ and
$\N^\W(\tau,h )$ is give by \textup{(\ref{11-7-47})},
$\N^\W(\tau,h )= O\bigl(\log(\log|\tau |\cdot h^{\nu ^{-1}})\bigr)$.

Moreover, under condition \textup{(\ref{11-7-66})}
$\N^\W(\tau,h )\asymp \log(\log|\tau |\cdot h^{\nu ^{-1}})$.
\end{enumerate}
\end{theorem}

\begin{remark}\label{rem-11-7-21}
In the proof of the last statement of this theorem
we also use the arguments of Remark \ref{rem-11-1-13}\ref{rem-11-1-13-i}.
\end{remark}

\begin{theorem}\label{thm-11-7-22}
Let $d\ge 3$, $X$ be a conical domain with $\partial X\setminus 0\in \sC^K$, and let $g^{jk}=g^{jk}(\theta )\in \sC^K(\bS^{d-1})$ satisfy condition
\textup{(\ref{11-4-5})}. Let $V_j=0$, $V=v(\theta )|\log r|$ with
$v\in \sC^K(\bS^{d-1})$ and $\min_{\bar{X}} v=v_0<0$. Then asymptotics
\begin{equation}
\N^- (\tau ,h)=\N^\W (\tau )h^{-d}+
O\Bigl(h^{1-d}\tau
\int_U\exp \bigl(-\tau (d-1)v^{-1}\bigr)\,d\theta \Bigr)
\label{11-7-80}
\end{equation}
holds as $\tau \to -\infty $, $h\to+0$ with
\begin{equation}
\N^\W (\tau )=a\int_U\exp (-\tau dv ^{-1})\sqrt g\, d\theta
\label{11-7-81}
\end{equation}
where $U=X\cap \bS^{d-1}$ and the coefficient $a$ is introduced in
Theorem~\ref{thm-11-5-28}. The orders of $\N^\W (\tau )$ and the remainder
estimate and more accurate results are discussed in Statement \ref{thm-11-5-28-ii} of that theorem.
\end{theorem}

\section[Negative order operators]{Distributions of spectra for negative order operators}
\label{sect-11-8}
Let $A=A^\W(x,D)$ be a classical pseudodifferential operator of order $m<0$ on a compact closed manifold $X$. We are interested in the asymptotics of the eigenvalue counting function\enlargethispage{\baselineskip}
\begin{equation}
\N^\pm (\tau )=\#\bigl\{\lambda >\tau ,\; \pm \lambda\;
\text{is an eigenvalue of}\; A\bigr\}
\label{11-8-1}
\end{equation}
and
\begin{equation}
\N_{(\vartheta)} ^\pm (\tau )=
\int(\lambda -\tau )_+^\vartheta d_\lambda \N^\pm (\lambda )
\label{11-8-2}
\end{equation}
as $\tau \to +0$. First of all, the following theorem holds:

\begin{theorem}\label{thm-11-8-1}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-8-1-i}
Let $a(x,\xi )$ be a microhyperbolic symbol on the energy level  $0$ (in a direction depending on the point). Then asymptotics
\begin{equation}
\N^\pm (\tau )=\varkappa ^\pm \tau ^{\frac{d}{m}}+
O\bigl(\tau ^{\frac{d-1}{m}}\bigr)
\label{11-8-3}
\end{equation}
holds as $\tau \to +0$ with
\begin{equation}
\varkappa ^\pm =(2\pi )^{-d}\int \boldsymbol{n} ^\pm (x,\xi ;1)\,dxd\xi
\label{11-8-4}
\end{equation}
where $\boldsymbol{n} ^\pm (x,\xi ;\tau )$ is an eigenvalue counting function for $a(x,\xi)$ i.e. the number of eigenvalues of the symbol $\pm a(x,\xi )$ greater than $\tau$ and $a$ is the principal symbol of $A$.

\item\label{thm-11-8-1-ii}
 Moreover, asymptotics
\begin{equation}
\N^\pm _{(\vartheta)} (\tau )= \N^{\W,\pm} _{(\vartheta)}(\tau)
+O\bigl(R_{(\vartheta)} (\tau )\bigr)
\label{11-8-5}
\end{equation}
holds with
\begin{equation}
\N^{\W,\pm} _{(\vartheta)} (\tau )=
\sum_k\varkappa_{\vartheta k} ^\pm\tau ^{\frac{d-k}{m}}
\label{11-8-6}
\end{equation}
and
\begin{equation}
R_{(\vartheta)} (\tau )=\left\{\begin{aligned}
\tau ^{{\frac{1}{m}}(d-1-\vartheta )+\vartheta }\qquad
\text{for\ }&\vartheta (1-m) <d-1,\\
|\log \tau |\qquad \text{for\ }&\vartheta (1-m)=d-1,\\
1 \qquad \text{for\ }&\vartheta (1-m)>d-1.
\end{aligned} \right.
\label{11-8-7}
\end{equation}

\item\label{thm-11-8-1-iii}
Further, let $\vartheta (1-m)<d-1$ and let the standard non-periodicity condition be fulfilled for the Hamiltonian trajectories of the symbol $\pm a$ on the energy level  $1$. Then asymptotics
\begin{equation}
\N^\pm (\tau )=\varkappa ^\pm \tau ^{\frac{d}{m}}+
\bigl(\varkappa_1+o(1)\bigr)\tau ^{\frac{d-1}{m}}
\label{11-8-8}
\end{equation}
and asymptotics
\begin{equation}
\N^\pm _{(\vartheta)} (\tau )= \N^{\W,\pm}_{(\vartheta)} (\tau )
+o\bigl(R_{(\vartheta)} (\tau )\bigr)
\label{11-8-9}
\end{equation}
hold as $\tau \to +0$.

\item\label{thm-11-8-1-iv}
Furthermore, let $\vartheta (1-m)=d-1$ and the standard non-periodicity condition be fulfilled for the Hamiltonian trajectories of the symbol
$\pm a$ on the energy level  $0$. Then asymptotics \textup{(\ref{11-8-9})}
holds.

\item\label{thm-11-8-1-v}
 On the other hand, if the symbol $\pm a(x,\xi )$ is negative-definite for every $(x,\xi )$ (which under the microhyperbolicity condition means precisely that $\varkappa ^\pm=0$) then
\begin{equation}
\N^\pm (\tau )=O(1).
\label{11-8-10}
\end{equation}
\end{enumerate}
\end{theorem}

\begin{proof}
We leave all the details of the proof to the reader and indicate only the rescaling which should be applied in this proof: namely, we apply the rescaling
$(\epsilon ,\epsilon r)$ with respect to $(x,\xi )$ where $r=|\xi |$
and $h_\eff=r+|\tau | ^{\frac{1}{m}}$ afterwards.
\end{proof}

\begin{remark}\label{rem-11-8-2}
Asymptotics (\ref{11-8-3}) and (\ref{11-8-5}) are standard results under ellipticity condition
\begin{equation}
|a(x,\xi )v|\ge \epsilon_0|v|\cdot |\xi | ^m\qquad
\forall (x,\xi )\quad \forall v\in \bH
\label{11-8-11}
\end{equation}
and asymptotics (\ref{11-8-8}) and (\ref{11-8-9}) for $\vartheta (1-m)<d-1$ under this condition and non-periodicity condition on the energy level  $1$.
\end{remark}

Let us get rid of the microhyperbolicity condition. In the general case we can do nothing better than introduce the rescaling
\begin{equation}
(x_1,x',\xi_1,\xi') \mapsto (\zeta ^{-2}x_1, \zeta^{-1}x', r ^{-1}\xi_1, \zeta^{-1}r^{-1}\xi')\qquad \text{with\ \ } r\asymp |\xi |
\label{11-8-12}
\end{equation}
where the coordinate system is taken such that
$\xi '=0$ at some point of the element of the partition and
\begin{equation}
\zeta =\min_j(|\alpha_j|+\tau r ^{-m}+r ^{-\frac{1}{2}})\qquad\text{for\ \ }
\tau \le Cr^m
\label{11-8-13}
\end{equation}
and $\alpha_j=\alpha_j(x,\xi )$ are eigenvalues of $a(x,\xi |\xi | ^{-1})$. Further

\begin{claim}\label{11-8-14}
Here and below we set $\zeta=1$ for $\tau \ge r^m$.
\end{claim}

Then $h_\eff=r ^{-1}\zeta ^{-2}$ and the contribution of the zone
$\{(x,\xi):\ h_\eff \ge 1\}$ to the asymptotics does not exceed $CR'_{(\vartheta)}$ with
\begin{equation}
R'_{(\vartheta)} =\left\{\begin{aligned}
\tau ^{l+\vartheta }\qquad &\text{for\ }\vartheta <-l,\\
|\log \tau | \qquad &\text{for\ \ }\vartheta =-l,\\
1\qquad &\text{for\ \ }\vartheta >-l,\end{aligned} \right.
\quad \qquad l=- \frac{2d}{1-2m} .
\label{11-8-15}
\end{equation}

Then one can easily obtain the following\enlargethispage{\baselineskip}


\begin{theorem}\label{thm-11-8-3}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-8-3-i}
In the general case the following asymptotics holds:
\begin{equation}
\N^\pm _{(\vartheta)} (\tau )= \N^{\W,\pm}_{(\vartheta)} (\tau )+
O\bigl(R_{(\vartheta)} (\tau )+R'_{(\vartheta)} (\tau )\bigr)
\label{11-8-16}
\end{equation}
where $R_{(\vartheta)}$ and $R'_{(\vartheta)} $ are defined by
\textup{(\ref{11-8-7})} and \textup{(\ref{11-8-16})} respectively.

\item\label{thm-11-8-3-ii}
Moreover, suppose that
$\vartheta< (d(1-2m)^{-1}-1)$\,\footnote{\label{foot-11-62} Which implies that $d>1-2m$ and $\vartheta(1-m)<(d-1)$ i.e. $R_{(\vartheta)} \gg R'_{(\vartheta)} $.}
and let the standard non-periodicity condition be fulfilled for the Hamiltonian trajectories of the symbol $\pm a$ on the energy level  $1$. Then asymptotics \textup{(\ref{11-8-8})} and \textup{(\ref{11-8-9})} hold.


\item\label{thm-11-8-3-iii}
On the other hand, if the symbol $\pm a(x,\xi )$ is non-positive
definite for every $(x,\xi ) (\Leftrightarrow \varkappa ^\pm =0$) then estimate
\begin{equation}
\N^\pm (\tau )=O(\tau ^l)
\label{11-8-17}
\end{equation}
holds.
\end{enumerate}
\end{theorem}

To improve results of Theorem~\ref{thm-11-8-3} let us assume that
\begin{gather}
|D ^\alpha_{(x,\xi )}a(x,\xi )|\le c\gamma ^{\mu -|\alpha |}
\qquad \forall \alpha :|\alpha |\le \mu \quad \forall (x,\xi ):|\xi |=1,
\label{11-8-18}\\[2pt]
|a(x,\xi )v|\ge \epsilon_0 \gamma ^\mu |v|
\quad \forall v\in \bH \quad \forall (x,\xi ):|\xi |=1,
\label{11-8-19}
\end{gather}
where $\gamma (x,\xi )=\dist \bigl((x,\xi ),\Lambda \bigr)$ and $\Lambda$ is the union of a finite number of $\sC^K$ manifolds of codimension $\ge p$. Then one can make rescalings
\begin{gather}
(x,\xi )\mapsto (\zeta ^{-1}x,\zeta ^{-1}r ^{-1}\xi )\label{11-8-20}\\
\shortintertext{with}
\zeta=\epsilon(\gamma+\tau^{\frac{1}{\mu}}r^{-\frac{m}{\mu}}+r^{-\frac{1}{2}})
\label{11-8-21}
\end{gather}
and obtain
\begin{theorem}\label{thm-11-8-4}
Under assumptions \textup{(\ref{11-8-18})}--\textup{(\ref{11-8-19})} Statements \ref{thm-11-8-3-i}--\ref{thm-11-8-3-ii} of Theorem~\ref{thm-11-8-3} hold with $R'_{(\vartheta)}$ defined by \textup{(\ref{11-8-15})} but this time with $l=-(2d-p)(\mu-2m)^{-1}$.
\end{theorem}

Let us now treat the scalar case. First of all, for $\vartheta >0$ one can apply exactly the construction of the proof of Theorem~\ref{thm-11-8-1} (no microhyperbolicity-type condition is necessary at all). On the other hand, for $\vartheta =0$ one can apply rescaling (\ref{11-8-20}) with
\begin{equation}
\zeta =\epsilon \bigl(\sum_{|\alpha |< M}
|D ^\alpha a| ^{\frac{M}{M-|\alpha |}}
+ |\tau r ^{-m}|\bigr) ^{\frac{1}{M}}+
\epsilon r ^{-\frac{1}{2}}
\label{11-8-22}
\end{equation}
with $M=2$. Then microhyperbolicity is fulfilled for $h_\eff\le h_0$. After calculations one gets the remainder estimate
$O\bigl(\tau ^{\frac{d-1}{m}}+\tau ^l\bigr)$ where this time $l=-d(1-m) ^{-1}$ which is good for $m<(1-d)$.

On the other hand, taking arbitrarily large $M$ one can refer to the weakest possible non-degeneracy condition (\ref{5-2-126}) and after easy calculations
get the remainder estimate $O(\tau ^{{\frac{1}{m}}(d-1+\delta )})$ with
arbitrarily small $\delta >0$. Therefore the following statement
holds:

%\renewcommand{\thetheorem}{H.3}
\begin{theorem}\label{thm-11-8-5}
Let $A$ be a scalar operator. Then

\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{thm-11-8-5-i}
For $\vartheta=0$ asymptotics \textup{(\ref{11-8-3})} hold if $m\le (1-d)$; further, asymptotics
\begin{equation}
\N^\pm (\tau )=\varkappa ^\pm \tau ^{\frac{d}{m}}+
O(\tau ^{ \frac{1}{m} (d-1+\delta )})
\label{11-8-23}
\end{equation}
holds with arbitrarily small exponent $\delta >0$ if $m>(1-d)$.

\item\label{thm-11-8-5-ii}
For $\vartheta>0$ asymptotics \textup{(\ref{11-8-5})} holds.

\item\label{thm-11-8-5-iii}
Suppose that either $\vartheta >0$ or $m\le (1-d)$ and and that the standard non-periodicity condition is fulfilled for the Hamiltonian trajectories of the symbol $\pm a$ on the energy level  $1$. Then asymptotics
\textup{(\ref{11-8-8})}, \textup{(\ref{11-8-9})} hold.
\end{enumerate}
\end{theorem}




\section{Spectral asymptotics for the semiclassical Dirichlet to Neumann operator}
\label{sect-11-9}


In this section we demonstrate how Birman-Schwinger principle combined with our ``main'' results allows us to derive some rather non-standard asymptotics.


%Paper \href{http://arxiv.org/abs/1505.04894}{http://arxiv.org/abs/1505.04894} of Andrew Hassell \& Victor Ivrii (in a more general framework) will be here;

%Let $X$ be a compact Riemannian manifold with smooth boundary, and let $R(\lambda)$ be the Dirichlet-to-Neumann operator at frequency $\lambda$. The Dirichlet-to-Neumann operator $R (\lambda)$ is defined to be $\lambda^{-1} R(\lambda)$. We obtain a leading asymptotic for the spectral counting function for $R_{\scl}(\lambda)$ in an interval $[a_1, a_2)$ as $\lambda \to \infty$, under the assumption that the measure of periodic billiards on $T^*M$ is zero.
%The asymptotic takes the form
%\begin{equation*}
%\N(\lambda; a_1,a_2) = \bigl( \kappa(a_2)-\kappa(a_1)\bigr)\Vol'(\partial M) \lambda^{d-1}+o(\lambda^{d-1}),
%\label{11-9-16}
%\end{equation*}
%where $\kappa(a)$ is given explicitly by
%\begin{multline*}
%\kappa(a) = \frac{\omega_{d-1}}{(2\pi)^{d-1}} \bigg( -\frac{1}{2\pi} \int_{-1}^1 (1 - \eta^2)^{(d-1)/2} \frac{a}{a^2 + \eta^2} \, d\eta \\
%- \frac{1}{4} + H(a) (1+a^2)^{(d-1)/2} \bigg) .
%\label{11-9-17}
%\end{multline*}

\subsection{Problem set-up}
\label{sect-11-9-1}

Let $X$ be a compact Riemannian manifold with the boundary $\partial X$. The Dirichlet-to-Neumann operator is a family of operators defined on $\sL^2(\partial X)$ depending on the parameter $\lambda \ge 0$. It is defined as follows: given $f \in \sL^2(\partial X)$, we solve the equation (if possible)
\begin{equation}
(\Delta - \lambda^2) u = 0 \quad \text{on\ \ } X, \qquad u |_{\partial X} = f.
\label{11-9-1}
\end{equation}
Then the \emph{Dirichlet-to-Neumann operator\/}\index{Dirichlet-to-Neumann operator} at frequency $\lambda$ is the map
\begin{equation}
R (\lambda) : f \mapsto -\partial_\nu u |_{\partial X}
\label{11-9-2}
\end{equation}
where as usual $\partial_\nu$ is the interior unit normal derivative, and $\Delta$ is the positive Laplacian on $X$.

It is well known that $R(\lambda)$ is a self-adjoint, semi-bounded from below pseudodifferential operator of order $1$ on $\sL^2(\partial X)$, with the domain $\fD(R(\lambda))=\sH^1(\partial X)$. It therefore has discrete spectrum accumulating only at $+\infty$. The Dirichlet-to-Neumann operator and closely related operators are important in a number of areas of mathematical analysis including inverse problems (such as Calder\'on's problem A.~P.~Calder\'on~\cite{Cal}), domain decomposition problems (such as the determinant gluing formula of D.~Burghelea, L.~Friedlander and T.~Kappeler \cite{BFK}), and spectral asymptotics (see e.g. L.~Friedlander~\cite{Fried}).

In this section, we are interested in the spectral asymptotics of $R(\lambda)$ in the high-frequency limit, $\lambda \to \infty$. Nanmely, let us consider
\begin{equation}
\N(\lambda; a_1,a_2)\coloneqq   \#\{\beta\colon  \beta \text{\ is an eigenvalue of \ }
R(\lambda),\ a_1\le \beta <a_2\},
\label{11-9-3}
\end{equation}
the number of eigenvalues of $R (\lambda)$ in the interval $[a_1, a_2)$.

Both $R(\lambda)$ has the disadvantage that it is undefined whenever $\lambda^2$ is a Dirichlet eigenvalue, since then (\ref{11-9-1}) is not solvable for arbitrary $f \in \sH^1(X)$. Indeed, when $\lambda^2$ is a Dirichlet eigenvalue, a necessary condition for solvability of (\ref{11-9-1}) is that $f$ is orthogonal to the normal derivatives of Dirichlet eigenfunctions at frequency $\lambda$. To overcome this issue, we introduce the \emph{Cayley transform\/}\index{Cayley transform} of $R (\lambda)$: we define
\begin{equation}
C(\lambda) = (\lambda^{-1}R(\lambda)- i)(\lambda^{-1}R (\lambda)+ i)^{-1}.
\label{11-9-4}
\end{equation}
This family of operators is related to the Robin boundary conditions: we have
$C(\lambda) f = g$ if and only if there is a function $u$ on $X$ satisfying
\begin{gather}
(\Delta - \lambda^2) u = 0
\label{11-9-5}\\
\shortintertext{and}
\frac{1}{2} (\lambda^{-1} \partial_\nu u- i u) = f,
\qquad \frac{1}{2} (\lambda^{-1} \partial_\nu u + i u) = g.
\label{11-9-6-*}\tag*{$\textup{(\ref*{11-9-6})}_{1,2}$}
\end{gather}
\begin{phantomequation}\label{11-9-6}\end{phantomequation}%

\begin{remark}\label{rem-11-9-1}
As observed in A.~Barnett and A.~Hassell~\cite{BH}, $C(\lambda)$ is a well-defined analytic family of operators for $\lambda$ in a neighbourhood of the positive real axis, which is unitary on the real axis. In particular, it is well-defined even when $\lambda^2$ is a Dirichlet eigenvalue of the Laplacian on $X$. As a unitary operator, $C(\lambda)$, $\lambda > 0$, has its spectrum on the unit circle, and as $R (\lambda)$ has discrete spectrum accumulating only at $\infty$, it follows that the spectrum of $C(\lambda)$ is discrete on the unit circle except at the point $1$.
\end{remark}

Our question can be formulated in terms of $C(\lambda)$: given two angles $\theta_1, \theta_2$ satisfying $0 < \theta_1 < \theta_2 < 2\pi$, what is the asymptotic for
\begin{multline}
\tilde{\N}(\lambda; \theta_1,\theta_2)\coloneqq   \\
\# \{ e^{i\theta}\colon  e^{i\theta} \text{\ is an eigenvalue of \ } C(\lambda),\ \theta_1\le \theta <\theta_2\}
\label{11-9-7}
\end{multline}
the number of eigenvalues of $C(\lambda)$ in the interval
$\{ e^{i\theta}\colon  \theta \in [\theta_1, \theta_2) \}$ of the unit circle, as $\lambda \to \infty$.

Clearly, we have
\begin{multline}
\tilde{\N}(\lambda; \theta_1,\theta_2) =\\
 \N(\lambda; a_1\lambda,a_2\lambda), \
\text{where\ \ } e^{i\theta_j} = \frac{a_j - i}{a_j + i}, \text{\ \ i.e.\ \ }
a_j = - \cot \bigl(\frac{\theta_j}{2}\bigr) .
\label{11-9-8}
\end{multline}

\subsection{Problem reduction}
\label{sect-11-9-2}

To answer this question we relate it to a standard semiclassical eigenvalue counting problem on $X$. To state the next result, we first define the self-adjoint operator $P_{a,h}$ on $\sL^2(X)$ by
\begin{gather}
\fD (P_{a,h})= \{ u \in H^2(M) \colon  (h \partial_\nu + a ) u = 0\quad
\text{at\ \ } \partial X\},
\label{11-9-9}\\[2pt]
P_{a,h}(u) = (h^2 \Delta - 1) u, \quad u \in \fD (P_{a,h}).
\label{11-9-10}
\end{gather}
It is the self-adjoint operator associated to the semi-bounded quadratic form
\begin{equation}
h^2 \|\nabla u\|_X ^2 - \|u\|_X ^2 - h a \|u\|^2_{\partial X} .
\label{11-9-11}
\end{equation}
This operator $P_{a,h}$ is linked with the Dirichlet-to-Neumann operator as follows: if $f$ is an eigenfunction of $R (\lambda)$ with eigenvalue
$\lambda a$, then the corresponding Helmholtz function $u$ defined by (\ref{11-9-1}) is in the domain (\ref{11-9-9}) of $P_{a,h}$, and $P_{a,h} u = 0$ (where $h = \lambda^{-1}$).

Then we have the following

\begin{proposition}\label{prop-11-9-2}
Let $h = \lambda^{-1}$. Assume $0 < \theta_1 < \theta_2 < 2\pi$. Then the number of eigenvalues of $C(\lambda)$ in the interval
$J_{\theta_1, \theta_2} := \{ e^{i\theta}\colon  \theta \in [\theta_1, \theta_2) \}$ is equal to
\begin{gather}
\tilde{\N}(\lambda; \theta_1,\theta_2) = \N(\lambda; \lambda a_1,\lambda a_2)= \N_h^- (a_2) - \N^-_h(a_1) ,
\label{11-9-12}\\
\intertext{where $a_j = - \cot (\theta_j/2)$ and}
\N_h^- (a)\coloneqq   \# \{\mu <0\colon  \mu \text{\ is an eigenvalue of\ \ } P_{a,h} \}
\label{11-9-13}.
\end{gather}
\end{proposition}

\begin{proof}
We begin by recalling that the operator $P_{a, h}$ is the self-adjoint operator associated to the quadratic form (\ref{11-9-11})

We recall the min-max characterization of eigenvalues: the $n$-th eigenvalue $\mu_n(a, h)$ of $P_{a,h}$ is equal to the infimum of
\begin{equation*}
\sup_{ v \in V, \| v \| = 1 } Q_{a,h}(v)
\end{equation*}
over all subspaces $V \in\sH^1(M)$ of dimension $n$.
The monotonicity of $Q_{a,h}$ in $a$, for fixed $h$, shows that the eigenvalues are monotone nonincreasing with $a$. In fact, they are strictly decreasing, which follows from the fact that eigenfunctions of $P_{a, h}$ cannot vanish at the boundary. Indeed, the eigenfunctions satisfy the boundary condition
$h \partial_\nu u = -a u$, which shows that if $u$ vanishes at the boundary, so does $\partial_\nu u$, which is impossible.

The eigenvalues $\mu_n(a, h)$ are thus continuous, strictly decreasing functions of $a$. Let $a_1 < a_2$ be real numbers. The Birman-Schwinger principle (Theorem~\ref{thm-10-2-8}) says that the number of negative eigenvalues of $P_{a_2, h}$ is equal to the number of negative eigenvalues of $P_{a_1, h}$, plus the number of eigenvalues $\mu_n(a,h)$ of $P_{a, h}$ that change from nonnegative to negative as $a$ varies from $a_1$ to $a_2$. We illustrate it by the following offshoot of Figure~\ref{fig-10-2-a}:
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=1.1]
\clip(-1.6,-1) rectangle (6.2,5);
\draw [ultra thin,->](0,0)--(5.5,0) node[below]{$t$};
\draw [ultra thin,->](0,0)--(0,4.5) node[right]{$\tau$};
\draw[ultra thick] (0,4)--(0,-.5) ;
\draw[thick] (5,4)--(0,4) node[left]{$\tau=\bar{\tau}_2$};
\draw[ultra thick] (5,4)--(5,-.5);
\draw [red,->] (0.5,4.5) ..controls (1.3,4.5).. (1.5,3.5) node[below]{$\tau'_1$};
\draw [red,->] (1.5,4.5) ..controls (2.3,4.5).. (2.5,3.5);
\draw [red,->] (2.5,4.5) ..controls (3.3,4.5).. (3.5,3.5) ;
\draw [red,->] (3.5,4.5) ..controls (4.3,4.5).. (4.5,3.5) node[below]{$\tau'_n$};
\draw[red,<-] (.3,.5)--(-.3,.5) node[left] {$\tau_1$};
\draw[red,<-] (.3,1.5)--(-.3,1.5);
\draw[red,<-] (.3,2.5)--(-.3,2.5);
\draw[red,<-] (.3,3.5)--(-.3,3.5) node[left] {$\tau_N$};
\node at (-.6,2) {\rotatebox{90}{$\Spec(P_{a_1,h})$}};
\draw[blue,->] (4.5,.5)--(5.3,.5) node[right] {$\tau_1$};
\draw[blue,->] (4.5,1.5)--(5.3,1.5) ;
\draw[blue,->] (4.5,2.5)--(5.3,2.5) ;
\draw[blue,->] (4.5,3.5)--(5.3,3.5) node[right] {$\tau_M$};
\node at (5.7,2) {\rotatebox{90}{$\Spec(P_{a_2,h})$}};
\end{tikzpicture}
\caption{\label{fig-11-12} Birman-Schwinger principle as applied in this section}
\end{figure}

The strict monotonicity of $\mu(a, h)$ in $a$ shows that the number of eigenvalues $\mu_n(a,h)$ of $P_{a, h}$ that change from nonnegative to negative as $a$ varies from $a_1$ to $a_2$ is the same as the number of
$\mu(a, h)$ (counted with multiplicity) equal to zero, for $a \in [a_1, a_2)$.

Next, we observe that the space of eigenfunctions $u_n(a, h)$ of $P_{a, h}$ with zero eigenvalue, i.e. $\mu_n(a, h) = 0$ is in one-to-one correspondence with the space of eigenfunctions of $C(\lambda)$, $\lambda = h^{-1}$, with eigenvalue $(a-i)(a+i)^{-1}$, or equivalently $e^{i\theta}$ where $a=-\cot(\theta/2)$. Indeed, whenever $u_n$ is such an eigenfunction of
$P_{a, h}$, then
\begin{equation}
f \coloneqq   \frac1{2} (h \partial_\nu u - iu) \big|_{\partial M}
\label{11-9-14}
\end{equation}
is an eigenfunction of $C(\lambda)$, with eigenvalue $(a-i)(a+i)^{-1}$.

Conversely, if $f$ is an eigenfunction of $C(\lambda)$ with eigenvalue $(a-i)(a+i)^{-1}$, then by definition there exists a Helmholtz function $u$ such that $u$ is related to $f$ according to (\ref{11-9-14}), and we have
$(h \partial_\nu + a)u = 0$ at $\partial X$.
\end{proof}

\begin{remark}\label{rem-11-9-3}
We can apply similar arguments for $\lambda^{-\delta}\rho^{-1} R(\lambda)$ as $\rho>0$ is a smooth function on $\partial X$ and then plug corresponding
parameters in the boundary conditions coming again to equality (\ref{11-9-12}).
\end{remark}

We next digress to prove that the eigenvalues of $C(\lambda)$ are monotonic (that is, they move monotonically around the unit circle) in $\lambda$. This plays no role in the our analysis, but is (in the authors' opinion) of independent interest.

\begin{proposition}\label{prop-11-9-4}
The eigenvalues of $C(\lambda)$ rotate clockwise around the unit circle as $\lambda$ increases.
\end{proposition}

\begin{remark}\label{rem-11-9-5}
 This implies that the eigenvalues of $\lambda^{-1}R(\lambda)$ are monotone decreasing in $\lambda$.
\end{remark}

\begin{proof}[Proof of Proposition~\ref{prop-11-9-4}]
As discussed in the proof of Proposition~\ref{prop-11-9-2}, $C(\lambda)$ has eigenvalue $e^{i\theta}$ if and only if $P_{a, h}$ has a zero eigenvalue, where $a = a(\theta) = - \cot (\theta/2)$. Thus, as a function of $h = \lambda^{-1}$, $\theta(h)$ is defined implicitly by the condition
\begin{equation*}\mu(a(\theta), h) = 0.
\end{equation*}
Since $a$ is a strictly increasing function of $\theta$, and we have just seen that $\mu$ is a strictly decreasing function of $a$, it suffices to show that when $\mu = 0$, $\mu$ is a strictly increasing function of $h$, hence a strictly decreasing function of $\lambda$.

We now compute the derivative of $\mu$ with respect to $h$, at a value of $a$ and $h$ where $\mu(a, h) = 0$. We have
\begin{multline*}
\frac{d}{dh}\mu(a,h) = \frac{d}{d h} ( (h^2 \Delta - 1) u(h), u(h) )_X \\[3pt]
= 2h (\Delta u, u )_X + ((h^2 \Delta - 1) u'(h), u(h))_X +
((h^2\Delta - 1)u(h), u'(h) )_X \\[3pt]
= 2h (\Delta u, u)_X +( (h^2\Delta - 1)u', u)_X - (u' ,(h^2 \Delta - 1) u)_X.
\end{multline*}
In the third line, we used the fact that $(h^2\Delta - 1)u = 0$ when $\mu(h)=0$.
Note the second term is not zero, as $u'$ is not in the domain of the operator due to the changing boundary condition, so we cannot move the operator to the right hand side of the inner product without incurring boundary terms.
We use the Gauss-Green formula to express the last two terms as a boundary integral:
\begin{align*}
\mu'(h) &= 2h (\Delta u, u)_X + h(h\partial_\nu u', u)_{\partial X} -
h(u', h\partial_\nu u)_{\partial X}\\
&= 2h ( \Delta u, u )_X +h(h\partial_\nu u', u)_{\partial X} + ha(u', u)_{\partial X}.
\end{align*}
Differentiating the boundary condition we find that
\begin{equation*}
(h\partial_\nu + a ) u' = -h\partial_\nu u \qquad\text{at\ \ } \partial X.
\end{equation*}
Substituting that in we get
\begin{gather*}
\mu'(h) = 2h ( \Delta u, u )_X - h(u, \partial_\nu u)_{\partial X}. \\
\intertext{Applying Gauss-Green again, we get }
\mu'(h) = h ( \Delta u, u )_X + h \| \nabla u\|_X^2
= h^{-1} \Bigl( \| u \| ^2 + \| h\nabla u\|^2 \Bigr) > 0.
\end{gather*}
\end{proof}


\subsection{Main Theorem}
\label{sect-11-9-3}


Having thus reduced the original problem to a standard one for semiclassical spectral asymptotics, we obtain our main result. Since operators $P_{a_1,h}$ and $P_{a_2,h}$ differ only by boundary conditions, the principal terms of these asymptotics coincide and the difference appear only in the second terms and we arrive either to estimate or to asymptotics (after calculations in Subsection~\ref{sect-11-9-4}:

\begin{theorem}\label{thm-11-9-6}
\begin{enumerate}[fullwidth, label=(\roman*)]
\item\label{thm-11-9-6-i}
The following estimate holds:
\begin{equation}
\N(\lambda; \lambda a_1, \lambda a_2) = O(\lambda^{d-1}).
\label{11-9-15}
\end{equation}
\item\label{thm-11-9-6-ii}
Further, if the set of periodic billiards on $X$ has measure $0$ then the following asymptotic holds as $\lambda \to +\infty$:
\begin{equation}
\N(\lambda; \lambda a_1,\lambda a_2) =
\bigl( \kappa(a_2)-\kappa(a_1)\bigr)\Vol'(\partial X) \lambda^{d-1}+o(\lambda^{d-1}),
\label{11-9-16}
\end{equation}
where $\kappa(a)$ is given explicitly by
\begin{multline}
\kappa(a) = \frac{\omega_{d-1}}{(2\pi)^{d-1}} \biggl( -\frac{1}{2\pi} \int_{-1}^1 (1 - \eta^2)^{(d-1)/2} \frac{a}{a^2 + \eta^2} \, d\eta \\
- \frac{1}{4} + \uptheta(a) (1+a^2)^{(d-1)/2} \biggr) ;
\label{11-9-17}
\end{multline}
recall that $\uptheta(\cdot)$ is the Heaviside function,
$\omega_d$ is the volume of the unit ball in $\bR^d$, and $\Vol (X)$ and $\Vol'(\partial X)$ are $d$-dimensional volume of $X$ and $(d-1)$-dimensional volume of $\partial X$ respectively.

\item\label{thm-11-9-6-iii}
In the case $d=3$, we can evaluate this integral exactly and we find that
\begin{equation}
\kappa (a)=\frac{1}{4\pi}\Bigl(-\frac{1}{4}-\frac{1}{\pi}\arccot (a) (1+a^2)+(1+a^2)+ \frac{1}{\pi}a\Bigr)
\label{11-9-18}
\end{equation}
where $\arccot$ has range $(0,\pi)$.
\end{enumerate}
\end{theorem}

\begin{remark}\label{rem-11-9-7}
\begin{enumerate}[fullwidth, label=(\roman*)]
\item\label{rem-11-9-7-i}
Expression (\ref{11-9-18}) is simpler in terms of $\theta$. Defining $\tilde{\kappa}(\theta) = \kappa(a)$ where
$a = -\cot(\theta/2) = \cot(\pi - \theta/2)$, we have (still under the zero-measure assumption on periodic billiards)
\begin{gather}
\tilde{\N}(\lambda; \theta_1,\theta_2) = \bigl( \tilde{\kappa}(\theta_2)-\tilde\kappa(\theta_1)\bigr)\Vol'(\partial X) \lambda^{2}+o(\lambda^{2}),
\label{11-9-19}\\[2pt]
\tilde{\kappa}(\theta) = \frac{1}{4\pi} \Bigl( -\frac{1}{4} + \frac{1}{2\pi} \bigl( \frac{\theta - \sin \theta}{\sin^2(\theta/2)} \bigr) \Bigr).
\label{11-9-20}
\end{gather}

\item\label{rem-11-9-7-ii}
Despite different expressions for $a<0$ and $a>0$ one can observe that
$\kappa (a)$ is monotone increasing and continuous.

\item\label{rem-11-9-7-iii}
In particular, $\kappa (0)=\frac{1}{4} (2\pi)^{-d}\omega_{d-1}$ and
$\kappa (-\infty)=-\frac{1}{4} (2\pi)^{-d}\omega_{d-1}$ while $a=0$ and
$a = -\infty$ correspond to the Neumann and Dirichlet boundary conditions respectively (see Proposition~\ref{prop-11-9-4-12}).
\end{enumerate}
\end{remark}


\subsection{Calculations}
\label{sect-11-9-4}


In this section, we prove Theorem~\ref{thm-11-9-6}. Essentially, we have arrived at a our standard semiclassical spectral asymptotics problem.

\begin{proposition}\label{prop-11-9-8}
\begin{enumerate}[fullwidth, label=(\roman*)]
\item\label{prop-11-9-8-i}
Let $\N^-_h (a)$ be as in \textup{(\ref{11-9-13})}.
The following asymptotic holds as $h\to +0$:
\begin{equation}
\N^-_h (a) = (2\pi h)^{-d} \omega_d \Vol (X) + O(h^{1-d})
\label{11-9-21}
\end{equation}
\item\label{prop-11-9-8-ii}
Further, if the set of periodic billiards on $M$ has measure $0$ then as
$h\to +0$:
\begin{gather}
\N^-_h (a) =
(2\pi h)^{-d} \omega_d\Vol (X) + h^{1-d} \kappa(a)\Vol'(\partial X) + o(h^{1-d})
\label{11-9-22}
\end{gather}
with $\kappa(a)$ given by \textup{(\ref{11-9-17})}.
\end{enumerate}
\end{proposition}

\begin{proof}
One can check easily that the operator $P_{a,h}$ is microhyperbolic on the energy level  $0$ at each point $(x,\xi)\in T^*X$ in the direction $\xi$; further, the boundary value problem is microhyperbolic at each point
$(x'; \xi')\in T^*\partial X$ on the energy level  $0$ in the multidirection $(\xi', \xi_1^-,\xi_1^+)$ with $\xi_1=\xi_1^\pm $ roots of $\sum g^{jk}\xi_j\xi_k=0$. Finally, the boundary value problem is elliptic at each point of the elliptic zone ($\subset T^*\partial X$) if $a\le 0$, and either elliptic or microhyperbolic in the direction $\xi'$ at each point of the elliptic zone ($\subset T^*\partial X$) if $a> 0$
 Then Statements \ref{prop-11-9-8-i} and \ref{prop-11-9-8-ii} follow from Theorems \ref{thm-7-3-11} and \ref{thm-7-4-1}.

We now assume that the set of periodic billiards on $X$ has measure zero, and compute the second term in the spectral asymptotic explicitly. Similar calculations appear in  R.~Frank and L.~Geisinger~\cite{frank:gei:1}.

To do this, one can use method of freezing coefficients (see f.e. Section~\ref{sect-7-2}) which results in
\begin{equation}
h^{1-d} \kappa (a)=\int_{\bR^+} \bigl(e (0, x_1; 0, x_1;1) -
(2\pi h )^{-d}\omega_d \bigr)\, dx_1
\label{11-9-23}
\end{equation}
where $e(x', x_1; y', y_1;\tau )$ is the Schwartz kernel of the spectral projector $E(\tau)$ of the operator
$H_a=h^2 \Delta$ in half-space $\bR^{d-1}\times \bR^+\ni (x',x_1)$ with domain $\fD (H_a)= \{u \in \sH^2:\ (h\partial_{x_1} +a)u|_{x_1=0}=0\}$.


We obtain this spectral projector by integrating the spectral measure. This in turn is obtained via Stone's formula
\begin{equation}
d\uptheta (\sigma-P) = \frac{1}{2\pi i}
\Bigl( (P - (\sigma + i0))^{-1} - (P - (\sigma - i0)^{-1} \Bigr) \, d\sigma.
\label{11-9-24}
\end{equation}

Consider the resolvent for $P_{a,h}$, $(P_{a,h} - \sigma)^{-1}$, for
$\sigma \in \bC \setminus \bR$. Using the Fourier transform in the $x'$ variables, we can write the Schwartz kernel of this resolvent in the form
\begin{equation}
(2\pi h)^{1-d} \int e^{i(x'-y') \cdot \xi'}
(T_a + |\xi'|^2 - \sigma-1)^{-1}(x_1, y_1) \, d\xi'.
\label{11-9-25}
\end{equation}
Here $T_a$ is the one-dimensional operator $T_a=-h^2\partial ^2 +|\xi'|^2$ on $\sL^2(\bR_+)$ under the boundary condition $(h\partial +a)u|_{x_1=0}=0$. The spectral projector $\uptheta(\sigma-P_{a,h})$ is therefore given by
\begin{equation}
(2\pi h)^{1-d} \int_{-\infty}^1 \int e^{i(x'-y') \cdot \xi'} \,
\uptheta(\sigma - 1-|\xi'|^2-T_a)(x_1, y_1) \, d\xi' \, d\sigma.
\label{11-9-26}
\end{equation}

Thus, we need to find the spectral measure for $T_a$. Write
$\sigma - |\xi'|^2 -1= \eta^2$, where we take $\eta$ to be in the first quadrant of $\bC$ for $\Im \sigma > 0$, and in the fourth quadrant for $\Im \sigma < 0$.

\begin{lemma}\label{lemma-11-9-9}
\begin{enumerate}[label=(\roman*), wide, labelindent=0pt]
\item\label{lemma-11-9-9-i}
Suppose that $\Im \eta > 0$ and $\Re \eta \ge 0$. Then the resolvent kernel $\cK_{(T_a - \eta^2)^{-1}}$ takes the form
\begin{equation}
\cK_{(T_a - \eta^2)^{-1}}(x, y) = \left\{\begin{aligned}
\frac{i}{2h\eta} \Bigl( e^{i\eta(x-y)/h} + \frac{i\eta - a}{i\eta + a} e^{i\eta(x+y)/h} \Bigr) && x > y, \\[4pt]
\frac{i}{2h\eta} \Bigl( e^{i\eta(y-x)/h} + \frac{i\eta - a}{i\eta + a} e^{i\eta(x+y)/h} \Bigr) && x < y .
\end{aligned}\right.
\label{11-9-27}
\end{equation}
\item\label{lemma-11-9-9-ii}
If $\Im \eta < 0$ and $\Re \eta \ge 0$, then the resolvent kernel
$\cK_{(T_a - \eta^2)^{-1}}$ takes the form
\begin{multline}
\cK_{(T_a - \eta^2)^{-1}}(x, y) =\\
 \left\{\begin{aligned}
-\frac{i}{2h\eta} \Bigl( e^{i\eta(y-x)/h} + \frac{i\eta + a}{i\eta - a} e^{-i\eta(x+y)/h} \Bigr) && x > y, \\[4pt]
-\frac{i}{2h\eta} \Bigl( e^{i\eta(x-y)/h} + \frac{i\eta + a}{i\eta - a} e^{-i\eta(x+y)/h} \Bigr) && x < y .
\end{aligned}\right.
\label{11-9-28}
\end{multline}
\end{enumerate}
\end{lemma}

\begin{proof}
In the regions $x < y$ and $x > y$, the resolvent kernel must be a linear combination of $e^{i\eta x/h}$ and $e^{-i\eta x/h}$.
Moreover, for $\Im \eta > 0$, we can only have the $e^{+i\eta x/h}$ term, as $x \to \infty$, as the other would be exponentially increasing.
So we can write the kernel in the form
\begin{equation}
\left\{\begin{aligned}
& c_1 e^{+i\eta x/h}, &&x > y \\
&c_2 e^{+i\eta x/h} + c_3 e^{-i\eta x/h}, &&x < y.
\end{aligned}\right.
\label{11-9-29}
\end{equation}
We apply the boundary condition, and the two connection conditions at $x=y$, namely continuity, and a jump in the derivative of $-1/h$, in order to obtain the delta function $\updelta(x-y)$ after applying $T_a$. These three conditions determine the $c_i$ uniquely, and we find that, in the case $\Im \eta > 0$,
\begin{phantomequation}\label{11-9-30}\end{phantomequation}
\begin{align}
&c_1 =
\frac{i}{2h\eta}\bigl(e^{-i\eta y/h} +
\frac{i\eta-a}{i\eta + a}e^{+i\eta y/h}\bigr),
\tag*{$\textup{(\ref*{11-9-30})}_1$}\label{11-9-30-1}\\
&c_2 = \frac{i}{2h\eta} \frac{i\eta-a}{i\eta + a} e^{+i\eta y/h}, \qquad c_3 = \frac{i}{2h\eta} e^{+i\eta y/h},
\tag*{$\textup{(\ref*{11-9-30})}_{2,3}$}\label{11-9-30-2}
\end{align}
yielding \eqref{11-9-27}. A similar calculation yields \eqref{11-9-28}.
\end{proof}

We now apply \eqref{11-9-24} to find the Schwartz kernel of the spectral measure for $T_a$.

\begin{lemma}\label{lemma-11-9-10}
The spectral measure $d\uptheta (\tau-T_a)$ is given by the following.
\begin{enumerate}[label=(\roman*), fullwidth]
\item \label{lemma-11-9-10-i}
For $\tau \ge 0$, $\tau = \eta^2$
\begin{multline}
d\uptheta (\tau-T_a)=\\
\frac{1}{4\pi h \eta} \Bigl( e^{i\eta(x-y)/h} + e^{i\eta(y-x)/h} +
 \frac{i\eta - a}{i\eta + a} e^{i\eta(x+y)/h} + \frac{i\eta + a}{i\eta - a} e^{-i\eta(x+y)/h} \Bigr) \, 2\eta d\eta.
\label{11-9-31}
\end{multline}
\item\label{lemma-11-9-10-ii}
For $\tau < 0$, the spectral measure $dE(\tau)$ vanishes for $a \le 0$, while for $a > 0$
\begin{equation}
d\uptheta (\tau-T_a)=\frac{2a}{h} e^{-ax/h}e^{-ay/h} \updelta(\tau + a^2) d\tau.
\label{11-9-32}
\end{equation}
\end{enumerate}
\end{lemma}
\enlargethispage{\baselineskip}
\begin{proof}
This follows directly from Lemma~\ref{lemma-11-9-9} and Stone's formula (\ref{11-9-24}). The extra term for $a > 0$ arises from the pole in the denominator, $i\eta + a$ for $\Im \eta > 0$ and $i\eta - a$ for $\Im \eta < 0$ in the expressions (\ref{11-9-27}) and (\ref{11-9-28}), which only occurs for
$a >0$. For $\tau$ negative, we need to set $\eta = i \sqrt{-\tau} + 0$ in (\ref{11-9-27}) and $\eta = - i\sqrt{-\tau} + 0$ in (\ref{11-9-28}), and subtract. Then everything cancels except at the pole, where we obtain a delta function $-2\pi i\updelta(\sqrt{-\tau} - a)$, which arises from $(\sqrt{-\tau} + i0 + a)^{-1} - (\sqrt{-\tau} - i0 + a)^{-1}$. This term arises from the negative eigenvalue $-a^2$ which occurs for $a > 0$, corresponding to the eigenfunction $\sqrt{2a/h} \, e^{-ax/h}$.
\end{proof}

Plugging this into \eqref{11-9-26}, and making use of the fact that $d\sigma d\xi'= 2\eta d\eta d\xi'$, we find that the Schwartz kernel of
$\uptheta(- P_{a,h})$ is given by
\begin{multline}
(2\pi h)^{-d}\int_{0}^1\int\uptheta(1-|\xi'|^2-\eta^2) e^{i(x'-y')\cdot \xi'} \\
\times \Bigl( e^{i\eta(x_1-y_1)/h} + e^{i\eta(y_1-x_1)/h} +
\frac{i\eta - a}{i\eta + a} e^{i\eta(x_1+y_1)/h} +
\frac{i\eta + a}{i\eta - a} e^{-i\eta(x_1+y_1)/h} \Bigr) \, d\xi' d\eta
\label{11-9-33}
\end{multline}
for $a \le 0$ while for $a > 0$, it is given by the sum of \eqref{11-9-33} and
\begin{equation}
(2\pi h)^{1-d}\frac{2a}{h} e^{-ax_1/h} e^{-ay_1/h}
\int_{-\infty}^1 \int e^{i(x' - y') \cdot \xi'}
\updelta(\sigma - |\xi'|^2 + a^2) \, d\xi' d\sigma .
\label{11-9-34}
\end{equation}
We are actually interested in the value on the diagonal. Setting $x=y$, and performing the trivial $\xi'$ integral, we find that the Schwartz kernel of the spectral projector $\uptheta(-P_{a,h})(x,x)$ on the diagonal is given by
\begin{multline}
\frac{\omega_{d-1}}{ (2\pi h)^{d}} \int_{0}^1 (1 - \eta^2)^{(d-1)/2}
\biggl( 2 + \frac{i\eta - a}{i\eta + a} e^{2i\eta x_1/h} + \frac{i\eta + a}{i\eta - a} e^{-2i\eta x_1/h} \biggr) \, d\eta \\
+ \uptheta (a) \frac{(d-1) \omega_{d-1}}{ (2\pi h)^{d-1}} \frac{a}{h} e^{-2ax_1/h} \int_{-a^2}^1 (\sigma+a^2)^{(d-3)/2} \, d\sigma .
\label{11-9-35}
\end{multline}
Since
\begin{equation*}
\omega_{d-1}\int_0^1 2(1 - \eta^2)^{(d-1)/2} \, d\eta = \omega_d,
\end{equation*}
we see by comparing with \eqref{11-9-23} that this term disappears in the expression for $\kappa(a)$ and we have, after performing the $x_1$ integral as in (\ref{11-9-23})
\begin{multline}
h^{1-d} \kappa(a) = \frac{\omega_{d-1}}{ (2\pi h)^{d}}
\int_{0}^1 (1 - \eta^2)^{(d-1)/2} \\
\shoveright{\times \biggl(\frac{i\eta - a}{i\eta + a}
\Bigl( \frac{ih}{2} (\eta + i0)^{-1} \Bigr) \ -
\frac{i\eta + a}{i\eta - a}\Bigl( \frac{ih}{2} (\eta - i0)^{-1} \Bigr)
\biggr) \, d\eta }\\
+ \uptheta(a) \frac{(d-1) \omega_{d-1}}{2 (2\pi h)^{d-1}}
\int_{-a^2}^1 (\sigma+a^2)^{(d-3)/2} \, d\sigma .
\label{11-9-36}
\end{multline}
Simplifying a bit, and performing the $\sigma$ integral, we have
\begin{multline}
\kappa(a) = -\frac{i\omega_{d-1}}{2 (2\pi)^{d}}
\int_{-1}^1 (1 - \eta^2)^{(d-1)/2}\frac{(i\eta - a)^2}{a^2+\eta^2}
(\eta + i0)^{-1} \, d\eta \\
+ \uptheta(a) \frac{\omega_{d-1}}{ (2\pi)^{d-1}} (1+a^2)^{(d-1)/2} .
\label{11-9-37}
\end{multline}
We further simplify this expression by expanding
$(i\eta - a)^2 = a^2 - 2ia\eta - \eta^2$, and noting that the contribution of the $-\eta^2$ term is zero, as this gives an odd integrand in the $\eta$ integral. A similar statement can be made for the $a^2$ term, except that there is a contribution from the pole in this case. This leads to the expression
\begin{multline}
\kappa(a) =
\frac{\omega_{d-1}}{(2\pi)^{d-1}} \biggl( -\frac{1}{2\pi} \int_{-1}^1 (1 - \eta^2)^{(d-1)/2} \frac{a}{a^2 + \eta^2} \, d\eta \\
- \frac{1}{4} + \uptheta(a) (1+a^2)^{(d-1)/2} \biggr) .
\label{11-9-38}
\end{multline}
Although not immediately apparent, this formula is continuous at $a=0$. In fact, the function $a (a^2 + \eta^2)^{-1}$ has a distributional limit
$ \sgn(a) \pi \updelta(\eta)$ as $a$ tends to zero from above or below.
The change of sign as $a$ crosses $0$ means that the integral in (\ref{11-9-38}) has a jump of $-1$ as $a$ crosses zero from negative to positive. That exactly compensates the jump in the final term.

In odd dimensions, we can compute this integral exactly. In particular, in dimension $d=3$, we find that
\begin{equation}
\kappa(a) = \frac{\omega_2}{(2\pi)^2} \Bigl( -\frac{1}{4} + \frac{a}{\pi} + (1+a^2) \bigl(1 - \frac{\arccot a}{\pi} \bigr) \Bigr).
\label{11-9-39}
\end{equation}
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm-11-9-6}] This follows immediately from Proposition~\ref{prop-11-9-8} and Proposition~\ref{prop-11-9-2}.
\end{proof}

\begin{remark}\label{rem-11-9-11}
The second term of the expansion in Theorem 1.1 of R.~Frank and L.~Geisinger \cite{frank:gei:1} is obtained by computing
\begin{equation}
(2\pi h)^{1-d} \int_{-\infty}^1 (1-\sigma) \int e^{i(x'-y') \cdot \xi'} dE_{T_a}(\sigma - |\xi'|^2)(x_1, y_1) \, d\xi' \, d\sigma
\label{11-9-40}
\end{equation}
instead of (\ref{11-9-26}).
\end{remark}

\subsection{Relation to Dirichlet boundary condition}
\label{sect-11-9-5}

In this subsection we observe that the limit $a \to -\infty$ corresponds to the Dirichlet boundary condition. More precisely, we have

\begin{proposition}\label{prop-11-9-4-12}
Let $\N_h^-(-\infty)$ denote the limit
\begin{equation}
\N_h^-(-\infty) \coloneqq   \lim_{a \to -\infty} \N_h^-(a),
\label{11-9-41}
\end{equation}
where $\N_h^-(a)$ is given by \textup{(\ref{11-9-13})}. Then we have
\begin{multline}
\N_h^-(-\infty) = \N^-_{\D,h}\coloneqq  \\
\# \{ \lambda_{\D,j} \le h^{-1}:\ \lambda^2_{\D, j}
\text{\ \ is a Dirichlet eigenvalue of \ \ } \Delta \}.
\label{11-9-42}
\end{multline}
\end{proposition}


\begin{proof}
Because the quadratic form (\ref{11-9-11}) is monotone in $a$, the counting function $\N_h^-(a)$ is monotone in $a$. Hence the limit above exists.

Obviously $\N^-_{\D,h}\le \N^-_{h}(a)$ and therefore
$\N^-_{\D,h}\le \N^-_{h}(-\infty)$. Converse inequality
$\N^-_{\D,h}\ge \N^-_{h}(-\infty)$ easily follows from the compactness arguments. We leave easy details to the reader.
\end{proof}

%[Proof of Proposition~\ref{prop-11-9-4-12}]
% We use the min-max characterisation of eigenvalues.
%Let $\tilde{\N}_D(\lambda)$ denote the number of Dirichlet eigenvalues (counted with multiplicity) less than or equal to $\lambda = h^{-1}$. This is equal to the maximal dimension of a subspace of $\sH^1_0(X)$ on which the quadratic form $Q_D$, given by
%\begin{equation}
%Q_D(u, u) = h^2 \| \nabla u \|_2^2 - \| u \|_2^2
%\label{11-9--47}
%\end{equation}
%is negative semidefinite. On the other hand, $\tilde{\N}_h^-(a)$ is equal to the maximal dimension of a subspace of $\sH^1(X)$ on which the quadratic form $Q_a$ given by (\ref{11-9-11}) is (strictly) negative definite.
%
%We first show that $\tilde{\N}_D(h^{-1}) \le \tilde{\N}_h^-(-\infty)$.
%Let $V$ be the vector space spanned by Dirichlet eigenfunctions with eigenvalue $\le \lambda^2$. Clearly, the quadratic form $Q_a$ is negative semidefinite on $V$, and if $\lambda^2$ is not a Dirichlet eigenvalue, then it is negative definite, proving the assertion.
%
%In the case that $\lambda^2$ is a Dirichlet eigenvalue, we perturb $V$ to $V_\epsilon$, a vector space of $\sH^1(X)$ of the same dimension as $V$, so that, for for $\epsilon$ sufficiently small depending on $a$, $Q_a$ is negative definite on $V_\epsilon$. For simplicity we only do this in the case that the $\lambda^2$-eigenspace is one dimensional, leaving the general case to the reader. To do this, we choose an orthonormal basis of $V$ (with respect to the $\sL^2$ inner product) of Dirichlet eigenfunctions $v_1, \dots, v_k$ with eigenvalues $\lambda_1^2, \ldots, \lambda_k^2$, where $\lambda_k = \lambda$.
%Then we perturb only $v_k$, leaving the others fixed.
%We choose $w \in \sH^1_0(X) ^\perp$, the orthogonal complement of $\sH^1_0(X)$ in $\sH^1(X)$ (with respect to the inner product in $\sH^1(X)$), so that \begin{equation}
%Q_a(v_i, s) = 0, \qquad i < k \text{ \ and\ \ } Q_a(v_k, s) > 0.
%\label{11-9--48}
%\end{equation}
%We check that this is possible. Notice that $w \in H^1_0(M) ^\perp$ implies that $(\Delta +1)w = 0$ in $X$. Then as $v_i$ has zero boundary data, we have
%\begin{equation}
%(\lambda_i^2 + 1) ( v_i, w)_X = ( \Delta v_i, w )_X - ( v_i, \Delta w )_X
%= ( \partial_\nu v_i, w )_{\partial X} .
%\label{11-9--49}
%\end{equation}
%We choose $w$ so that $(\partial_\nu v_i, w)_{\partial X}$ vanishes for $i < k$ and is positive for $i=k$. This is possible: in fact, due to the unique solvability of the boundary value problem
%\begin{equation}
%(\Delta + 1)w = 0, \quad w |_{\partial X} = f \in \sH^{1/2}(X),
%\label{11-9--50}
%\end{equation}
%for $w \in \sH^1(M)$, we see that $w$ can have any boundary value in $\sH^{1/2}(\partial X)$ which is dense in $\sL^2(\partial X)$. Then using (\ref{11-9--49}) we see that $(\partial_\nu v_k, w )_{\partial X} > 0$ implies that $( v_k, w )_X >0$.
%
%We now define $V_\epsilon$ to be the span of $v_1, \dots, v_{k-1}$ and
%$v_k + \epsilon w$. Then we have
%\begin{equation}
%Q_a(v_i, v_k + \epsilon s) = 0, \ i < k
%\label{11-9--51}
%\end{equation}
%and
%\begin{align}
%Q_a(v_k+ \epsilon w,v_k + \epsilon w ) &=
%Q_a(v_k, v_k) + 2\epsilon Q_a(v_k, w) + \epsilon^2 Q_a(s, s) \label{eq-5-7}\\
%&= 2\epsilon Q_a(v_i, s_i) + \epsilon^2 Q_a(w_i, w_i) \notag\\
%&= - 2 \epsilon (h^2 + 1) (v_i, s_i)_M + O(\epsilon^2 a^2)\notag
%\end{align}
%which is strictly negative for $\epsilon a^2$ small enough. It follows that $Q_a$ is negative definite on $V_k$ when $\epsilon a^2$ is small enough. A similar construction can be made when $\lambda^2$ has multiplicity greater than $1$.
%
%We next show that $\tilde{\N}_D(h^{-1}) \ge \N_h^-(-\infty)$. We argue by contradiction: if not, then for any $a$, there is a vector space $W$ of dimension $\ge k+1$ on which $Q_a$ is negative definite. Then there is a nonzero vector $w \in W$ orthogonal (in the $H^1(M)$ inner product) to $V$. We can write $w = w' + s$ where $w' \in H^1_0(M)$ and $s \in H^1_0(M)^\perp$. Then $w'$ is a linear combination of Dirichlet eigenfunctions with eigenvalue $\ge \lambda'> \lambda$, where $\lambda'$ is the smallest eigenvalue larger than $\lambda$. We then have
%\begin{multline}
%0 > Q_a(w' + s, w' + s) = Q_a(w', w') + 2 Q_a(w', s) + Q_a(s, s) \\
%\ge (\lambda' - \lambda) \| w' \|_2^2 - 2(h^2 + 1) \| w' \|_2 \| s \|_{L^2(M)} - h a \| s \|_{L^2(\partial M)}^2 .
%\label{eq-5-8}
%\end{multline}
%However, some standard potential theory shows that $\| s \|_{L^2(M)}$ is bounded by a constant times $\| s\|_{L^2(\partial M)}$. To see this, extend $M$ to a larger manifold $\tilde M$ of the same dimension, and let $G(x,y)$ be the Schwartz kernel of the inverse of $(\Delta_{\tilde M} + 1)^{-1}$ on $L^2(\tilde M)$, with Dirichlet boundary conditions at $\partial \tilde M$. We can write $s$ as $\int_{\partial M} d_{\nu_y} G(x, y) h(y) \, dy$ where $(1/2 + D)h = s |_{\partial M}$ and $D$ is the double layer operator on $\partial M$ determined by $G$. Standard arguments show that $(1/2 + D)$ has a bounded inverse on $L^2(\partial M)$ and $d_{\nu_y} G(x, y)$ is a bounded integral operator from $L^2(\partial M)$ to $L^2(M)$.
%So we can write, for $a < 0$,
%\begin{multline*}
%0 > Q_a(w' + s, w' + s) \\
%\ge (\lambda' - \lambda) \| w' \|_2^2 - 2C(h^2 + 1) \| w' \|_2 \| s \|_{L^2( \partial M)} + h |a| \| s \|_{L^2(\partial M)^2}^2
%\end{multline*}
%and the RHS is clearly positive for $|a|$ large enough, giving us the desired contradiction.
%\end{proof}

\subsection{Discussion}
\label{sect-11-9-6}

\begin{remark}\label{rem-11-9-13}
\begin{enumerate}[fullwidth, label=(\roman*)]
\item\label{rem-11-9-13-i}
It looks disheartening that the remainder is just ``$o$'' in comparison with the principal part and only under geometric condition of the global nature but it is the nature of the beast. Consider $X$ a hemisphere; then for
$\lambda_n^2= n(n+d-1)$ with $n\in \bZ^+$ the operator $R(\lambda)$ has eigenvalue $0$ of multiplicity $\asymp n^{d-1}$ and therefore as $a_1=0$ or $a_2=0$ we do not have even an asymptotic but just an estimate.

\item\label{rem-11-9-13-ii}
We can explain this by pointing out that the problem we consider is truly $d$-dimensional, in contrast, for example, to the problem of distribution of negative eigenvalues of $H=\Delta$ with
\begin{equation}
\fD(H)=\{u\in \sH^2 (X)\colon \partial_\nu u|_{\partial X}+ a \Delta_b^{1/2} u|_{\partial X}=0\}
\label{11-9-43}
\end{equation}
with $\Delta_b$ positive Laplacian on $\partial X$ and $a> 1$ which is in fact $(d-1)$-dimensional.

\item\label{rem-11-9-13-iii}
On the other hand, calculations of Section~\ref{sect-11-9-4} imply that for $a\ne 0$ quantum periodicity will be broken and one can get remainder estimate $o(\lambda^{d-1})$ albeit with the oscillating principal part.
\end{enumerate}
\end{remark}


\begin{remark}\label{rem-11-9-14}
We can rephrase Theorem~\ref{thm-11-9-6} in terms of a limiting measure on the unit circle. For each $\lambda > 0$, let $\mu(h)$, $h = \lambda^{-1}$, denote the atomic measure determined by the spectrum of $C(\lambda)$:
\begin{equation}
\upmu(h) = (2\pi h)^{d-1} \sum_{e^{i\theta_j} \in \Spec C(h^{-1})} \updelta(\theta - \theta_j),
\label{11-9-44}
\end{equation}
where we include each eigenvalue according to its multiplicity as usual. Then Theorem~\ref{thm-11-9-6} can be expressed in the following way: the measures $\upmu(h)$ converge in the weak-$*$ topology as $h \to 0$ to the measure
\begin{equation}
\omega_{d-1} \Vol'(\partial X) \frac{d}{d\theta} \tilde \kappa(\theta) d\theta \quad \text{on \ \ } (0, 2\pi),\ \ \text{that is on \ } \bS^1 \setminus \{ 1 \}.
\label{11-9-45}
\end{equation}
In particular, this measure is absolutely continuous, and finite away from $e^{i\theta} = 1$ with an infinite accumulation of mass as
$\theta to 2\pi-0$. In this form, we can compare our result with results on the semiclassical spectral asymptotics of scattering matrices.

In K.~Datchev, J.~Gell-Redman, A.~Hassell and P.~Humphries~\cite{DGHH} and J.~Gell-Redman, A.~Hassell. and S.~Zelditch\cite{GHZ}, the scattering matrix $S_h(E)$ at energy $E$ for the Schr\"odinger operator $h^2 \Delta + V(x)$ on $\bR^d$ was studied in the semiclassical limit $h \to 0$. Assuming that $V$ is smooth and compactly supported, that $E$ is a nontrapping energy level, and that the set of periodic trajectories of the classical scattering transformation on $T^* S^{d-1}$ has measure zero, it was shown that the measure $\upmu(h)$ defined by (\ref{11-9-44}) converged weak-$*$ to a uniform measure on
$\bS^1 \setminus \{1 \}$, with an atom of infinite mass at the point $1$.

On the other hand, for polynomially decaying potentials, it was shown by A.~Sobolev and D.~Yafaev~\cite{sobolev:yafaev} in the case of central potentials and by J.~Gell-Redman and A.~Hassel more generally (work in progress) that there is a limiting measure which is nonuniform, and is qualitatively similar to the measure for $C(h^{-1})$ above in that it is finite away from $1$, with an infinite accumulation of mass at $1$ from one side.
\end{remark}


Since the proof of Theorem~\ref{thm-11-9-6} is based exclusively on equality (\ref{11-9-12}) and asymptotics for $\N_h(a_j)$ ($j=1,2$) it can be generalized to any situation when (\ref{11-9-12}) holds and we can establish those asymptotics. We leave this to the reader as

\begin{Problem}\label{Problem-11-9-15}
\begin{enumerate}[fullwidth, label=(\roman*)]
\item\label{Problem-11-9-15-i}
Under stronger non-periodicity assumptions to geodesic flow improve remainder estimate to $O(\lambda^{d-1}/\log \lambda )$ or even $O(\lambda^{d-1-\delta})$.


\item\label{Problem-11-9-15-ii}
Consider eigenvalues of operator $\rho (\lambda)$ with $\rho>0$ smooth on $\partial X$ and recover Statements~\ref{thm-11-9-6-i} and~\ref{thm-11-9-6-ii} of Theorem~\ref{thm-11-9-6} albeit with $\kappa(a) \Vol'(\partial X)$ replaced by
\begin{equation}
\int_{\partial X} \kappa (\rho (x')a)\,dS
\label{11-9-46}
\end{equation}
where $d\sigma$ is a natural measure on $\partial X$;
however without condition $\rho>0$ problem may be much more challenging; even self-adjointness is by no means guaranteed.

\item\label{Problem-11-9-15-iii}
Consider the same problem but with singularities which do not break (\ref{11-9-12}) and asymptotics for $\N_h(a_j)$ ($j=1,2$).

\item\label{Problem-11-9-15-iv}
Consider the same problem albeit when operator $R(\lambda)$ is defined only on $Y\subset \partial X$ while on $\partial X\setminus Y$ some fixed boundary condition (f.e. Dirichlet) is imposed. To recover $o(\lambda^{d-1})$ remainder estimate assume additionally that $\mes_{d-1} (\partial Y)=0$ where $\partial Y$ is a border of $Y$ as domain on $\partial X$ and we consider its $(d-1)$-dimensional measure.

\item\label{Problem-11-9-15-v}
Consider further generalizations: Schr\"odinger operators, second order matrix operators. We do not even need a compactness of $X$ as long as some basic assumptions are fulfilled.

\item\label{Problem-11-9-15-vi}
Consider higher order operators. F.e. one can consider operator arising from the variational problem
\begin{equation}
Q_s(u)=\|\nabla^m u\|_X^2 -
\sum_{0\le j\le m-1} \alpha_j s \|\partial_\nu ^j u\|_{\partial X}^2
\label{11-9-47}
\end{equation}
and denoting eigenvalues by $\lambda^{2m}$, plug
$\alpha_j=\bar{\alpha}_j\lambda^{m-j}$ with $s\in [a_1,a_2]$. Here
$-\infty \le \bar{\alpha}_j\le 0$ and $\bar{\alpha}_j=-\infty$ means that
$\partial_\nu^j u|_{\partial X}=0$.
\end{enumerate}
\end{Problem}


The following problem looks extremely challenging:

\begin{Problem}\label{Problem-11-9-16}
We know that the mollification with respect to $\lambda$ leads to the smaller remainder estimate.

Investigate if the mollification with respect to $a$ leads to the smaller remainder estimate.
\end{Problem}

\section*{Comments}

While some of the results in the simplest situations were established by different authors, all the results of Sections~\ref{sect-11-1}--\ref{sect-11-7} were proven as the corollaries of the general theorems of Chapter~\ref{sect-9} by the author during 1985--1986.

Results of Section~\ref{sect-11-8} are brand new and results of Section~\ref{sect-11-9} were obtained by A.~Hassel and the author~\cite{hassel:ivrii} in April 2014.

Operators of the form $P_{a, h}$ were considered by R.~Frank and L.~Geisinger \cite{frank:gei:1}. They showed that the trace of the negative part of $P_{a,h}$ has a two-term expansion as $h \to 0$ regardless of dynamical assumptions\footnote{\label{foot-11-63} The fact that Frank and Geisinger obtain a second term regardless of dynamical assumptions is simply due to the fact that they study $\Tr (f(P_{a,h}))$ with $f(\lambda) = -\lambda \uptheta(-\lambda)$, which is one order smoother than $f(\lambda) = \uptheta(-\lambda)$.}, and the second term in their expansion (the $\sL_d^{(2)}$ term in Theorem 1.1 of their paper~\cite{frank:gei:1}) is closely related to $\kappa(a)$--see Remark~\ref{rem-11-9-11}.



==> Ch11/cusp.tex <==
General mutidimensional cusps:

Let $\bR^{d'}\supset X'$ a cone with smooth $\partial X'$ (except $0$),
$\cU=\{x:\, \dist (x', \partial X')\le  Cf(x'), |x''|\le Cf(x')\}$, where $f$ is a function like before.

Assume that $X\setminus \cU= \{x:\, x'\in X', x''\in f(x')\Omega\}\setminus \cU$ and $X\cap  \cU$ is ``served'' by a scaling function $f(x')$.


Also generalize to allow $f$ decay to cusp ends.



